Confounder Adjustment in Multiple Hypothesis Testing

We consider large-scale studies in which thousands of significance tests are performed simultaneously. In some of these studies, the multiple testing procedure can be severely biased by latent confounding factors such as batch effects and unmeasured covariates that correlate with both primary variable(s) of interest (e.g. treatment variable, phenotype) and the outcome. Over the past decade, many statistical methods have been proposed to adjust for the confounders in hypothesis testing. We unify these methods in the same framework, generalize them to include multiple primary variables and multiple nuisance variables, and analyze their statistical properties. In particular, we provide theoretical guarantees for RUV-4 and LEAPP, which correspond to two different identification conditions in the framework: the first requires a set of "negative controls" that are known a priori to follow the null distribution; the second requires the true non-nulls to be sparse. Two different estimators which are based on RUV-4 and LEAPP are then applied to these two scenarios. We show that if the confounding factors are strong, the resulting estimators can be asymptotically as powerful as the oracle estimator which observes the latent confounding factors. For hypothesis testing, we show the asymptotic z-tests based on the estimators can control the type I error. Numerical experiments show that the false discovery rate is also controlled by the Benjamini-Hochberg procedure when the sample size is reasonably large.

==> _make <==
% JS is editing
\subsection{Simulations}
\label{sec:simulations}

\Cref{thm:asymptotics-nc,thm:consistency-rr,thm:asymptotics-rr,cor:type-I,thm:multiple-rr,thm:consistency-weak}
have provided theoretical guarantees in different senarios for the asymptotics setting when $n, p \to \infty$.
In this section, we use simulations to illustrate these results and consider finite sample properties of our estimators
and tests.

Data are generated from the model \eqref{eq:linear-model-y,eq:linear-model-z,eq:linear-model-x,eq:linear-model-e}. More specifically, $X_i$ are centered binary variables with $\frac{X_i + 1}{2} \overset{\mathrm{iid}}{\sim} \mathrm{Bernoulli}(1, 0.5)$. For generating the parameters, the noises variances have
$\sigma_i \overset{\mathrm{iid}}{\sim}\mathrm{InvGamma}(3, 2)$ thus $\mathbb{E}(\sigma_i^2) = \mathrm{Var}(\sigma_i^2) = 1$. $\|\bm{\alpha}\|_2^2 = 3$ thus the variance of $X_i$ explained by the latent factors is $75\%$, and we set each $\alpha_k = \frac{\|\bm{\alpha}\|_2}{\sqrt r}$ for $k = 1, 2, \cdots, r$. The treatment effect $\bm{\beta}$ has
independent components $\beta_i$ taking the values $3 \sqrt{1 + \|\bm{\alpha}\|_2^2}$ and $0$ with probability
$\pi = 0.1$ and $1 - \pi = 0.9$, respectively. We set the number of latent factors $r$ to be either $2$ or $10$.
For the latent factor matrix $\bm \Gamma$, 
$\bm\Gamma = \tilde{\bm\Gamma}\bm{D}$ where $\tilde{\bm\Gamma}$ is a $p \times r$ orthogonal matrix sampled uniformly
from the Stiefel manifold $V_r(\mathbb{R}^p)$ and $\bm(D) = \sqrt p\cdot \mathrm{diag}(d_1, \cdots, d_r)$ where 
$d_k = 3 - \frac{2(k-1)}{r - 1}$. Finally, we set $p = 5000$ and $n = 100$ or $500$ to mimic the data size in 
most genetic studies.


\subsection{Real data example}
\label{sec:gender-study}

In this section, we return to the two motivational examples in
\cref{sec:introduction}. Recall that without confounder adjustment,
the distribution of the regression $t$-statistics are clearly
underdispersed (\cref{fig:gender-naive-batch}), noncentered
(\cref{fig:alzheimers-naive}), skewed
(\cref{fig:gender-naive-batch,fig:alzheimers-naive}). These two examples are originally studied
in \citep{gagnon2013} using the negative control (NC) method and we
refer the reader to their paper for more empirical results.

In \cref{tab:gender,tab:alzheimers}, we present the results after
adjustment for the two datasets. The adjustment method here is the
maximum likelihood factor analysis described in \cref{sec:inference-gamma-sigma} and the
robust regression (RR) method with Tukey's bisquare loss described in
\cref{sec:unkn-zero-indic}. Since the true number of confounders is
unknown, we increase $r$ from $1$ to $25$ and study the empirical
performance. The empirical performance metrics are total number of
significant genes of p-value less than $0.01$ after the empirical calibration in
\cref{sec:hypothesis-testing} (second column), number of
the genes on X/Y chromosome that have p-value less than $0.01$ (third
column), and the number among the $100$ most significant genes that are on the X/Y chromosome (fourth column).
The summary statistics of regression t-statistics being reported
in \cref{tab:gender,tab:alzheimers} are the mean, median, standard
deviation (sd), median absolute deviation (mad), skewness, and
medcouple (a robustness measure of skewness). In general, the
statistics in \cref{eq:test-statistic} become more centered at $0$ and
less skewed as we include a few confounders in the model.

% latex table generated in R 3.1.2 by xtable 1.7-4 package
% Sun May 24 17:21:30 2015
\begin{table}[ht]
\centering
\caption{The first dataset in \cref{fig:gender-naive-batch}: $n = 84$,
$p = 12600$. The bolded row corresponds to the $r$ selected by BCV.}
\label{tab:gender}
\footnotesize
\begin{tabular}{$r|^r^r^r^r^r^r^r^r^r}
  \hline
r & \#sig. & X/Y & top 100 & mean & median & sd & mad & skewness & medcouple \\
  \hline
0 & 1369 & 107 & 11 & 0.11 & 0.043 & 0.36 & 0.237 & 2.99 & 0.2 \\
  1 & 335 & 80 & 16 & -0.34 & -0.36 & 1.03 & 1.01 & 0.74 & 0.033 \\
  2 & 218 & 74 & 20 & -0.079 & -0.086 & 1.14 & 1.12 & 0.612 & 0.011 \\
  3 & 272 & 80 & 28 & 0.0061 & 0.00086 & 1.12 & 1.07 & 0.818 & -0.0021 \\
  4 & 294 & 77 & 27 & 0.02 & 0.024 &  1.2 & 1.15 & 0.65 & -0.0099 \\
  5 & 380 & 84 & 29 & -0.0047 & -0.025 & 1.18 & 1.09 & 0.847 & 0.013 \\
  7 & 393 & 79 & 27 & -0.01 & -0.023 & 1.26 & 1.16 & 0.778 & -0.000074 \\
  10 & 411 & 79 & 30 & -0.0024 & -0.011 & 1.37 & 1.26 & 0.632 & -0.0038 \\
  15 & 443 & 86 & 29 & -0.00027 & -0.014 & 1.46 & 1.34 & 0.554 & 0.00026 \\
  20 & 425 & 80 & 29 & 0.0076 & -0.029 & 1.52 &  1.4 & 0.476 & 0.029 \\
\rowstyle{\bfseries}
  25 & 431 & 84 & 28 & 0.0069 & -0.027 & 1.65 & 1.51 & 0.422 & 0.024 \\
  30 & 449 & 77 & 30 & 0.0054 & -0.023 & 1.77 &  1.6 & 0.441 & 0.019 \\
  40 & 451 & 79 & 29 & 0.0091 & -0.0092 & 1.98 & 1.78 & 0.526 & 0.0075 \\
   \hline
\end{tabular}
\end{table}

% latex table generated in R 3.1.2 by xtable 1.7-4 package
% Sun May 24 17:20:06 2015
\begin{table}[ht]
\centering
\caption{The second dataset in \cref{fig:alzheimers-naive}: $n = 31$,
$p = 22283$. The bolded row corresponds to the $r$ selected by BCV.}
\label{tab:alzheimers}
\footnotesize
\begin{tabular}{$r|^r^r^r^r^r^r^r^r^r}
  \hline
r & \#sig. & X/Y & top 100 & mean & median & sd & mad & skewness & medcouple \\
  \hline
0 & 19059 & 783 & 15 & -1.8 & -1.8 & 0.599 & 0.513 & -3.46 & 0.082 \\
  1 & 753 & 115 & 20 & -0.44 & -0.44 & 1.08 & 0.995 & -1.55 & 0.0055 \\
  2 & 588 & 126 & 23 & -0.22 & -0.24 & 1.19 & 1.11 & -0.992 & 0.013 \\
  3 & 528 & 127 & 26 & -0.15 & -0.17 & 1.27 & 1.18 & -0.843 & 0.014 \\
  4 & 508 & 126 & 27 & -0.21 & -0.23 & 1.29 & 1.22 & -0.813 & 0.012 \\
  5 & 628 & 123 & 24 & -0.26 & -0.26 & 1.31 & 1.22 & -1.34 & -0.0074 \\
  7 & 578 & 117 & 24 & -0.28 & -0.28 & 1.46 & 1.37 & -0.888 & -0.0039 \\
  9 & 649 & 134 & 29 & -0.24 & -0.23 & 1.48 & 1.37 & -0.793 & -0.012
  \\
\rowstyle{\bfseries}

  11 & 702 & 141 & 31 & -0.16 & -0.16 & 1.52 & 1.37 & -0.599 & 0.003 \\
  13 & 722 & 138 & 28 & -0.15 & -0.16 & 1.66 & 1.49 & -0.875 & 0.0086 \\
  15 & 764 & 142 & 27 & -0.17 & -0.18 & 1.82 & 1.63 & -0.345 & 0.013 \\
  20 & 879 & 142 & 25 & -0.2 & -0.2 & 2.52 & 2.19 & -0.309 & -0.0026 \\
   \hline
\end{tabular}
\end{table}

A practical way to pick $r$ is the bi-cross-validation (BCV) method of
\citet{owen2015}, which uses randomly held-out submatrices to estimate
the mean squared error of reconstructing factor loading matrix. In \cref{fig:gender-output,fig:alzheimers-output},
we demonstrate the performance of BCV on these two datasets. The $r$
selected by BCV is respectively $25$ and $11$ (\cref{fig:gender-bcv,fig:alzheimers-bcv}), and they both result in presumed shape of z-statistics distribution
(\cref{fig:gender-t,fig:alzheimers-t}) and near optimal performance in
of selecting genes on the X/Y chromosome
(\cref{tab:gender,tab:alzheimers}). The fact that the empirical variance
of the z-statistics in both cases are slightly larger than $1$ is not
too surprising; see \cref{rmk:calibration} for some discussion.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/gender-bcv.pdf}
  \caption{Bi-cross-validation error selects $r=25$.}
  \label{fig:gender-bcv}
  \end{subfigure}
  \qquad
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/gender-output.pdf}
  \caption{Distribution of the statistics after
  confounder adjustment.}
  \label{fig:gender-t}
  \end{subfigure}
  \caption{The first dataset where the unadjusted t-statistics are
  shown in \cref{fig:gender-naive-batch}.}
  \label{fig:gender-output}
\end{figure}

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/alzheimers-bcv.pdf}
  \caption{Bi-cross-validation error selects $r=11$.}
  \label{fig:alzheimers-bcv}
  \end{subfigure}
  \qquad
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/alzheimers-output.pdf}
  \caption{Distribution of the statistics after
  confounder adjustment.}
  \label{fig:alzheimers-t}
  \end{subfigure}
  \caption{The second dataset where the unadjusted t-statistics are
  shown in \cref{fig:alzheimers-naive}.}
  \label{fig:alzheimers-output}
\end{figure}

Lastly we want to comment on the sample size $n$. Our entire
asymptotic analysis is based on $r$ fixed and $n,p \to \infty$. In the second
dataset $n$ is only $31$, so the adjustment result is not ideal. In
\cref{tab:alzheimers}, adding the first two confounders significantly
reduces the mean and skewness of the statistics, but the mean and
median of the statistics remain negative no matter how many factors
are used. This is likely due to the fact that $n$ is too small to
estimate the confounders accurately. However, the empirical
performance (e.g.\ number of X/Y genes in top $100$) suggests it
is still beneficial to adjust for the confounders.


==> app_lem_rr.tex <==
By using the representation of $\hat{\bm{\Gamma}}$ in
\eqref{eq:gamma-hat},
%and (C.4) in \citep{bai2012}.
%  \begin{equation*}
%    \label{eq:eq:sigma-hat}
%    \hat{\sigma}_j^2 = \frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
%    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}}),
%  \end{equation*}
we have
\[
\begin{split}
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) =& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
    \hat{\bm{\Gamma}}_j^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
/ \|\bm{X}\|_2 + \bm{\Gamma}_j^{(0)T} \bm{\alpha}^{(0)} - (\hat{\bm{\Gamma}}_j)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j\\
\end{split}
\]
where $\max_j|\delta_j| = o_p(1)$ and
$\max_j|\epsilon_j| = o_p(n^{-1/2})$ from
%\eqref{eq:avg-sigma-err}
%\Cref{lem:ml-baili}
\Cref{lem:gamma-ml}.
%and equation \eqref{eq:avg-gamma-err}.
Because
$\|\bm{\beta}\|_1 \sqrt{n} / p \to 0$ and $\psi'$ is bounded,
\[
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) = \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j + \bm{o}_p(n^{-1/2})
\]

Let $g_j$ be the expression inside $\psi$ in the last equation omitting $\epsilon_j$ and $\delta_j$. Conditionally on
$\tilde{\bm{Z}}_{-1}^{(0)}$, the variables $g_j, \mathrm{where}~ j=1,\dotsc,p$ are independent and
identically distributed with $\mathrm{E}(g_j) = 0$ and
$g_j = O_p (n^{-1/2}) $.
%Using the Cauchy-Schwartz inequality,
%$p^{-1}\sum_{j = 1}^p(\delta_jg_j)^2 = o_p(n^{-1})$.
Thus, using \Cref{assumption:psi-2nd-derivative}
and boundedness of $\hat \sigma_j$,
\[
\begin{split}
 & \Big\| \frac{1}{p} \sum_{j=1}^p \Big[\psi\Big(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\Big)
 - \psi(g_j)\Big]\hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 \\
\leq & D^2 \cdot \Big\| \frac{1}{p} \sum_{j=1}^p\big(|\epsilon_j| |\hat{\bm{\Gamma}}_j|+ |g_j|
|\delta_j\hat{\bm{\Gamma}}_j|\big) /\hat \sigma_j
%\big(|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}| + |\bm{\Gamma}_j^{(0)}|\big)/\hat \sigma_j
\Big\|_2  = o_p(n^{-1/2})
\end{split}
\]
%where the last approximation is got by using Cauchy-Schwartz inequality and \Cref{lem:ml-baili}.
%where $t_j$ are
%i.i.d. normal random variables by noticing $\tilde{\bm{Z}}_{-1}^{(0)}
%\bm{\alpha}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R} \bm{R}^T)^{-1}
%(\bm{\alpha} + \bm{u}/\|\bm{X}\|_2)$ and $\bm{R} \bm{R}^T \to \bm{I}_r$.
%Because for some $W'$ between $0$ and $W$ and
%$\psi(0) = 0$, $\psi(g_j) = \psi'(0) (n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}}))$ if $\beta_j =0$.


We can further use the facts that
$\psi(g_j)=\psi'(0) g_j +
o_p(n^{-1/2}) = O_p(n^{-1/2})$ and
%Cauchy-Schwartz inequality in a similar way and combine
$\psi(g_j) - \psi'(0)g_j$
are i.i.d., and combine \Cref{rmk:rotation} and \Cref{lem:gamma-ml} to get:
\[
\begin{split}
\left\|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right\|_2 &= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi(g_j)\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
%O_p(n^{-\frac{1}{2}}p^{-\frac{1}{2}}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi'(0)g_j\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
&=o_p(n^{-\frac{1}{2}})+ o_p(n^{-\frac{1}{2}})
= o_p(n^{-\frac{1}{2}})
\end{split}
\]


Similarly,
%$\psi$ is assumed to be bounded $|\psi(g_j)| \le C$ in
%\Cref{assumption:rho}. Therefore, by
because $\lim_{p \to \infty}
\frac{1}{p} \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ exists and is
positive definite (in \Cref{assumption:large-factor}),
we use \Cref{assumption:psi-2nd-derivative} and the uniform convergence
of $\hat {\bm \Sigma}$ and $\hat{\bm \Gamma}$ in \Cref{lem:gamma-ml} to get
\[
\begin{split}
  \left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1} &=
\Bigg[\frac{1}{p} \sum_{j=1}^p
  \psi'\left(g_j + \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right)
\hat{\bm{\Gamma}}_j \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
&= \Bigg[\frac{1}{p} \sum_{j = 1}^p
  \psi'\left(0\right)
  \bm{\Gamma}_j^{(0)} \bm{\Gamma}_j^{(0)T} / \sigma_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(\beta_j) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 \right]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(0) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \frac{1}{p} \sum_{\beta_j
%    \ne 0}
%  (\psi'(\beta_j) - \psi'(0)) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2  \right]^{-1} \\
&\overset{p}{\to} \Big[ \psi'(0) \frac{1}{p} \sum_{j=1}^p
  \bm{\Gamma}_j \bm{\Gamma}_j^T / \sigma_j^2 \Big]^{-1}
\end{split}
\]
%The last probability limit follows from $\hat{\bm{\Gamma}}
%\overset{p}{\to} \bm{\Gamma}$, $\hat{\bm{\sigma}}_j
%\overset{p}{\to} \sigma_j$ and $\psi'$, $\bm{\Gamma}$ and $\bm{\Sigma}$ are bounded.
This means that all the eigenvalues of
$\left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1}$ converge to finite constants.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> app_lem_weak.tex <==
Denote the SVD of $\bm \Gamma$ as $\bm{\Gamma} = \tilde{\bm \Gamma}\bm{D}$ 
where $\tilde{\bm\Gamma}^T\tilde{\bm\Gamma} = \bm{I}_r$
and $\tilde{\bm{\Gamma}} = \begin{pmatrix} \tilde{\bm{\Gamma}}_{\cdot
    1}& \tilde{\bm{\Gamma}}_{\cdot 2} & \cdots &
\tilde{\bm{\Gamma}}_{\cdot r} \end{pmatrix}$. 
Also, assume that the sample covariance matrix of
$\tilde{\bm{Y}}_{-1}$
has eigen decomposition $\bm{S} = \hat{\tilde{\bm{\Gamma}}}^T\hat{\bm{D}}^2\hat{\tilde{\bm{\Gamma}}}$
and $\hat {\bm{\Gamma}} = \hat{\tilde{\bm \Gamma}}\hat{\bm D}$ where 
$\hat{\bm{D}} = \mathrm{diag}(\hat d_1, \cdots, \hat d_{\hat r})$. 
Finally, expand $\tilde{\bm \Gamma}$ as 
$\tilde{\bm{\Gamma}}^* = \begin{pmatrix}\tilde{\bm\Gamma} &\tilde{\bm{\Gamma}}^C\end{pmatrix}$ so that
$\tilde{\bm{\Gamma}}^*$ is a $p \times p$ orthogonal matrix.
To prove \Cref{lem:weak-gamma}, we first prove the following lemma 
which characterize the eigenvalues and eigenvectors of PCA 
based on \citet{baik2006} and \citet{paul2007}.

\begin{lemma}\label{lem:app-weak}
  The esitmated eigenvalues satisfy 
  $\hat d_k^2 - d_k^2 = O_p(1)$ for $k = 1, 2, \cdots, \hat r$.
 For each $k = 1, 2, \cdots, \hat r$, the estimated eigenvectors 
 $\hat {\tilde {\bm \Gamma}}_{\cdot k}$ can be decomposed as 
 \begin{equation}\label{eq:pca-eigenvector}
\hat{\tilde{\bm{\Gamma}}}_{\cdot k} = \sum_{h = 1}^{r}\theta_{hk}\tilde{\bm{\Gamma}}_{\cdot h} +
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\tilde{\bm{\Gamma}}^C
\frac{\bm{z}_k}{\|\bm{z}_k\|_2},~k=1,2,\dotsc,\hat r,
\end{equation}
where  $\bm{\theta}_k = (\theta_{1k}, \cdots, \theta_{rk})$ 
   and $\bm{z}_k \sim \mathrm{N}(\bm{0}, \bm{I}_{p - r})$. 
 Also, $\|\bm{\theta}_k\|_2 \independent \bm{z}_k$. 
 Finally, for $k = 1, 2, \cdots, s$, then $1 - \|\bm{\theta}_k\|_2^2 = O_p(p^{-1})$.
 \end{lemma}

 \begin{proof}
   Notice that in our notation, for $i > 1$, the column covariance satisfies that 
   $\var(\tilde{\bm Y}_{i\cdot}) = \tilde{\bm\Gamma}\bm \Lambda \tilde{\bm\Gamma}^T$ 
   where $\bm\Lambda  = \diag(d_1^2 + 1, \cdots, d_r^2 + 1, 1, \cdots,1 )$.
   Thus, using \citet[Theorem 1.1 and Theorem 1.2]{baik2006},  if 
   $d_k^2 \geq \sqrt \gamma$, 
$$\hat d_k^2 - d_k^2 = \gamma + 1 - \frac{\gamma}{d_k^2} + o_p(1) = O_p(1)$$ 
On the other hand, for $d_k^2 \leq \sqrt \gamma$, 
we have $|\hat d_k^2 - d_k^2| \leq |\hat d_k^2| + |d_k^2| = O_p(1)$.

 To prove \eqref{eq:pca-eigenvector}, as $\tilde{\bm \Gamma}^\star$ form an orthogonal 
 basis of $\real^p$ and $\hat {\tilde {\bm \Gamma}}_{\cdot k}$ is a unit vector, 
 we can decompose it as $\hat {\tilde {\bm \Gamma}}_{\cdot k} = 
 \sum_{h = 1}^{r}\theta_{hk}\tilde{\bm{\Gamma}}_{\cdot h}
 + \sum_{h' = r+1}^{p}\theta_{h'k}\tilde{\bm{\Gamma}}^C_{\cdot h'}$ 
 where $\sum_{h = 1}^p\theta_{hk}^2 = 1$. Using \citet[Theorem 6]{paul2007}, we get that 
 $(\theta_{(r+1)k}, \cdots, \theta_{pk})/\sqrt{ 1 - \|\bm \theta_k\|^2_2}$ is distributed 
 uniformly on the unit sphere $\mathbb{S}^{p - r - 1}$ and is independent of 
 $\|\bm \theta_k\|_2$ (Though is \citet{paul2007} it's assumed that $\gamma < 1$, 
 Theorem $6$ is an non-asymptotic result which holds for any $n$ and $p$). Thus, 
\eqref{eq:pca-eigenvector} holds with $\bm{z}_k \sim \mathrm{N}(\bm{0}, \bm{I}_{p - r})$ 
and $\|\bm{\theta}_k\|_2 \independent \bm{z}_k$. 

Finally, we use \citet[Equation (18)]{paul2007} which holds for any $n$ and $p$:
$$ \frac{1}{\|\bm \theta_k\|_2^2} = 
\bm a_k^T\big[\bm I_{p - r} + \bm \Lambda_r^{1/2} \bm T_1^T
  (\hat d_k^2 \bm I - \bm {\Lambda}^\star)^{-1}
 \bm \Lambda^\star 
 (\hat d_k^2 \bm I_{p - r} - \bm {\Lambda}^\star)^{-1}
\bm T_1 \bm \Lambda_r^{1/2} \big]\bm a_k 
$$
where $\bm a_k = \bm \theta_k/\|\bm \theta_k\|_2$, 
$\bm \Lambda_r = \diag(d_1^2 + 1, \cdots, d_r^2 + 1)$. $\bm T_1$ is a 
$\min(p - r, n) \times r$ random 
matrix whose entries are i.i.d. $\mathrm{N}(0, 1/n)$ variables. 
$\bm \Lambda^\star$ are the 
eigenvalues of $\bm T_2^T \bm T_2$ where $\bm T_2$ is independent of $\bm T_1$ and is 
a $\min(p-r, n) \times \min(p-r, n)$ random matrix whose entries are i.i.d. 
$\mathrm{N}(0, 1)$. As a consequence of Marchenko-Pastur law, the largest eigenvalue of 
$\bm \Lambda^\star$ is $O(1)$. For $k = 1, 2, \cdots, s$, as $d_k^2 = O(p)$, we also have 
$\hat d_k^2 = O(p)$. Also, as 
$\bm T_1^T \bm T_1 = \bm I_r$, the largest eigenvalue of 
$\bm T_1^T
  (\hat d_k^2 \bm I - \bm {\Lambda}^\star)^{-1}
 \bm \Lambda^\star 
 (\hat d_k^2 \bm I_{p - r} - \bm {\Lambda}^\star)^{-1}
\bm T_1$ is in the order of $O(1/\hat d_k^4) = O(p^{-1})$. As $\bm a_k$ is a unit vector 
and the largest eigenvalue of $\bm \Lambda_r$ is $O(\sqrt p)$, we have that 
$$\frac{1}{\|\bm \theta_k\|_2^2} - 1 = O(p^{-1})$$
which indicates that $1 - \|\bm{\theta}_k\|_2^2 = O_p(p^{-1})$.
 \end{proof}

Now we continue to prove \Cref{lem:weak-gamma}. Rewrite \eqref{eq:pca-eigenvector} as 
%By \Cref{assumption:weak-factor}, we have $\tilde \Gamma_{jk} = \Gamma_{jk}/d_k = o(1)$
%for each $j$ and $k$. Combing with the fact that $\hat d_k = d_k + o(1)$, we have
\begin{equation*}
%\begin{split}
\hat{{{\Gamma}}}_{jk} - \Gamma_{jk} = \hat d_k\sum_{h = 1}^{r}\theta_{hk}\tilde{{\Gamma}}_{jh}
-\Gamma_{jk}+
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k
%&= d_k(\sum_{h = 1}^{r}\theta_{hk}\tilde{{\Gamma}}_{jh}
%-\tilde\Gamma_{jk})+
%(1 - \|\bm{\theta}_k\|_2^2)\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k + o_p(1).\\
%\end{split}
\end{equation*}
For the weak factors $k = s+1, \cdots, r$, using \Cref{assumption:weak-factor}, we have $\max_j|\Gamma_jk| = o(1)$. 
As $d_k = O(1)$, we also have $\max_j|\tilde \Gamma_jk| = o(1)$. Using \Cref{lem:app-weak}, also $\hat d_k = O_p(1)$.
As the components of $\bm z_k$ are i.i.d. Gaussian 
variables and each $\|\tilde {\bm \Gamma}_{j\cdot}^C\| \leq 1$, we 
have that $\max_j|\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k| \leq \max_j|z_{jk}| = O(\sqrt {\log n})$. Thus, 
it's easy to see that $\max_j|\hat \Gamma_{jk} - \Gamma_{jk}| = o_p(1)$.

For the strong factors $k = 1, 2, \cdots, s$, we further decompose as 
$$
\hat{\Gamma}_{jk} - \Gamma_{jk} = d_k(\sum_{h = 1}^{r}\theta_{hk}\tilde{\Gamma}_{jh}
-\tilde\Gamma_{jk}) +
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k 
+ (\hat d_k - d_k)\sum_{h = 1}^r \theta_{hk}\tilde{\Gamma}_{jh}
$$
Using \Cref{assumption:weak-factor}, we have $\max_j|\tilde \Gamma_jk|$

We will show that each term of the right hand side of the above equation is $o_p(1)$.
First, using the facts that $\|\bm{z}_k\|_2/\sqrt p = O_p(1)$, $\hat d_k - d_k = O_p(1)$,
$1 - \|\bm\theta_{k}\|_2^2 = o_p(1)$ if $d_k^2 \to \infty$ and $d_k^2/p = O(1)$, we get that
$\big(1 - \|\bm{\theta}_k\|_2^2\big)\frac{\hat d_k}{\|\bm{z}_k\|_2} =
o_p(1)$ whether or not
$d_k$ is finite. Also, by definition
each $\|\tilde{\bm{\Gamma}}_{\cdot i}^C\|_2 \leq 1$, thus
$\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k = O_p(1)$.
These results indicate that $(1 - \|\bm{\theta}_k\|_2^2)\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k = o_p(1)$.
Next, when $h \neq k$, using \Cref{assumption:weak-factor},
$d_k\tilde \Gamma_{jh} = \frac{d_k}{\sqrt p}\frac{\sqrt p}{d_h}\Gamma_{jh} = O(1)$. As $\theta_{hk} = o_p(1)$,
we get $d_k\sum_{h \neq k}\theta_{hk}\tilde{{\Gamma}}_{jh} = o_p(1)$. Finally,
$d_k(\theta_{kk}-1)\tilde \Gamma_{jk} = \frac{d_k}{\sqrt p}\frac{\sqrt p}{d_k}\Gamma_{jk}(\theta_{kk}-1) = o_p(1)$.
Combining all the above results, we get that $\hat{{{\Gamma}}}_{jk} - \Gamma_{jk} = o_p(1)$, thus \eqref{eq:pca}
holds.

%Now we prove \eqref{eq:avg-pca}.
%First, notice that using the Cauchy-Schwarz inequality,
%$\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\tilde \Gamma_{jk}\big| \le \big(\sum_{j = 1}^p\tilde{\Gamma}_{jk}^2\big)^{1/2} = 1$
%and similarly $\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\hat{\tilde{\Gamma}}_{jk}\big| \le  1$.
%For factor $k$ of strength $d_k^2 \to \infty$, as
%$\langle \tilde{\bm{\Gamma}}_{\cdot k}, \hat{\tilde{\bm{\Gamma}}}_{\cdot k}\rangle
%= \theta_{kk} \to 1$ and both of them are unit vectors,
% $\big\|\hat{\tilde{\bm{\Gamma}}}_{\cdot k} -
%{\tilde{\bm{\Gamma}}}_{\cdot k}\big\|_2 =
%o_p(1)$. Using the Cauchy-Schwarz inequality
%$\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\hat{\tilde \Gamma}_{jk} - \tilde \Gamma_{jk}\big|
%\le \big\|\hat{\tilde{\bm{\Gamma}}}_{\cdot k} -
%{\tilde{\bm{\Gamma}}}_{\cdot k} \big\|_2$, we get
%\[
%\frac{1}{p}\sum_{j=1}^p\left|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}\right|
%\leq \frac{1}{p}\sum_{j=1}^p\Big(|\hat{\tilde{{\Gamma}}}_{jk} - \tilde{{\Gamma}}_{jk}||\hat{{d}}_k|
%+ |\tilde{{\Gamma}}_{jk}||\hat{{d}}_k-{d}_k|\Big) = o_p(1)
%\]
%For factor $k$ whose $d_k^2=O(1)$, we directly get
%\[
%\frac{1}{p}\sum_{j=1}^p\left|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}\right|
%\leq \frac{1}{p}\sum_{j=1}^p\Big(|\hat{\tilde{{\Gamma}}}_{jk}| +| \tilde{{\Gamma}}_{jk}||\hat{{d}}_k|
%+ |\tilde{{\Gamma}}_{jk}||\hat{{d}}_k-{d}_k|\Big) = o_p(1)
%\]
%Thus, \eqref{eq:avg-pca} holds.
%Finally, as $\mathrm{corr}(\hat{\bm \Gamma}_{\cdot k_1}, \bm \Gamma_{\cdot k_2}) =
%\mathrm{corr}(\hat{\tilde{\bm \Gamma}}_{\cdot k_1}, \tilde{\bm \Gamma}_{\cdot k_2})$,
%\eqref{eq:angle-pca} is just a consequence of \eqref{eq:pca-eigenvector} and
%\citet[Theorems 4 and 5]{paul2007}.

%To avoid confusion, we use $\bm{\alpha}^*$ to represent the true $\bm{\alpha}$,
%and use $\bm{\alpha}$ to represent a variable in $\mathbb{R}^{r^{(0)}}$.
% Using \Cref{assumption:weak-factor,assumption:bound-alpha}, \Cref{lem:weak-gamma}
% and the fact that $\|\bm{X}\|_2/\sqrt n \to 1$,
% \Cref{thm:consistency-weak} will be a direct consequence of consistent
% $\hat{\bm{\alpha}}_{(S)}^{\mathrm{RR}}$, which is proved in the
% following lemma.



% \begin{proof}
%   Let $m_n = \min_{\bm{\alpha}_0 \in \Omega} \sum_{j=1}^p
%   \rho \Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Big)$. Using \Cref{assumption:rho}, we have $m_n \geq 0$. First, as $\rho$ has
%   bounded derivative, it is a Lipschitz function. Also as
%   $\|\bm{X}\|_2/\sqrt n \overset{a.s.}{\to} 1$ and $\|\bm{\beta}\|_1/p \to 0$,
%   \begin{equation*}
% \begin{split}
%   \sum_{j=1}^p
% \rho \Bigg( \frac{\tilde{Y}_{1j} /\|\bm{X}\|_2
% -\hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Bigg)
% &= \frac{1}{p} \sum_{j=1}^p \rho\Bigg(  \frac{ \beta_j + \bm{\Gamma}_j^T
%   \bm{\alpha} - \hat{\bm{\Gamma}}_j^T
% \bm{\alpha}_0}{\hat{\sigma}}\Bigg) + o_p(1) \\
% &= \frac{1}{p} \sum_{j=1}^p \rho\Bigg(  \frac{\bm{\Gamma}_j^T
%   \bm{\alpha} - \hat{\bm{\Gamma}}_j^T
% \bm{\alpha}_0}{\hat{\sigma}}\Bigg) + o_p(1)
% \end{split}
% \end{equation*}
% Then, notice that for $\bm{\alpha}_0 \in \Omega$
% \begin{equation*}
%   \begin{split}
%     & \bm{\Gamma}_j^T\bm{\alpha} - \hat{\bm{\Gamma}}_j^T\bm{\alpha}_0\\
%     =& \hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)})+
% (\bm{\Gamma}_j^{(S)} - \hat{\bm{\Gamma}}_j^{(S)})^T\bm{\alpha}_{(S)}
% + \bm{\Gamma}_j^{(W)T}\bm{\alpha}_{(W)} - \hat{\bm{\Gamma}}_j^{(W)T}\bm{\alpha}_{0(W)}\\
% =& \hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)}) + o_p(1)
% \end{split}
% \end{equation*}
% Using \Cref{lem:weak-gamma}, for $\bm{\alpha}_0 \in \Omega$,
% \[
%  \sum_{j=1}^p
% \rho \Bigg( \frac{\tilde{Y}_{1j} /\|\bm{X}\|_2
% -\hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Bigg)
% = \frac{1}{p}\sum_{j = 1}^p\rho
% \Bigg(\frac{\hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)})}
% {\hat \sigma}\Bigg)
%   + o_p(1)
% \]
% and the $o_p(1)$ term doesn't depend on $\bm{\alpha}_0$. Thus, $m_n = o_p(1)$, which
% indicates that
% \begin{equation} \label{eq:rho-op1}
%   \tilde\rho(\bm{\alpha}_{(S)} -
%   \hat{\bm{\alpha}}_{(S)}) = \frac{1}{p}\sum_{j = 1}^p\rho
%   \Bigg(\frac{\hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \hat{\bm{\alpha}}_{(S)})}
% {\hat \sigma}\Bigg)  = {o}_p(1)
% \end{equation}
% On the other hand, similar to \eqref{eq:consistency-key}, we show that for
% sufficiently small $\epsilon > 0$, there exists $\tau > 0$ such that
% \begin{equation} \label{eq:consistency-weak-key}
% \mathrm{P} \Big( \inf_{\|\bm{\alpha}_1\|_2 \ge \epsilon} \tilde \rho(\bm{\alpha}_1) > \tau \Big)
% \to 1.
% \end{equation}



% \end{proof}


==> app_thm_rr.tex <==
% JS is editing

Because $\hat{\bm{\alpha}}^{\mathrm{RR}}$ is consistent, we can
approximate the left hand side of \eqref{eq:Psi} by its second order
Taylor expansion (we abbreviate
$\bm{\Psi}_{p,\hat{\bm{\Gamma}}, \hat{\bm{\Sigma}}}$ to $\bm{\Psi}_p$
if it causes no confusion):
\[
\bm{0} = \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \nabla \bm{\Psi}_p(\bm{\alpha}^{(0)}) \cdot
(\hat{\bm{\alpha}}^{\mathrm{RR}} - \bm{\alpha}^{(0)}) + \bm{r}_p
\]
where $\bm{r}_p$ is the higher order term and
\Cref{assumption:psi-2nd-derivative} implies $\bm{r}_p =
\bm{o}_p(\|\hat{\bm{\alpha}}^{\mathrm{RR}} - \bm{\alpha}\|_2)$.
Therefore $\hat{\bm{\alpha}}^{\mathrm{RR}} = \bm{\alpha}^{(0)} - \left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm{o}_p(1) \right]^{-1}
\bm{\Psi}_p(\bm{\alpha}^{(0)})$ and
\begin{equation} \label{eq:beta-expand}
\begin{split}
\sqrt{n}(\hat{\bm{\beta}}^{\mathrm{RR}} - \bm{\beta}) =&
\frac{\sqrt{n}}{\|\bm{X}\|_2} \tilde{\bm{E}}^T_1
+ \sqrt{n} (\bm{\Gamma}^{(0)} -\hat{\bm{\Gamma}})
\hat{\bm{\alpha}}^{\mathrm{RR}} \\
&+ \hat{\bm{\Gamma}} \left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm{o}_p(1) \right]^{-1}
\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)})
\end{split}
\end{equation}

It's easy to show $(\sqrt{n}/\|\bm{X}\|_2) \tilde{\bm{E}}_{1, S}
+ \sqrt{n} (\bm{\Gamma}^{(0)}_S -\hat{\bm{\Gamma}}_S)
\hat{\bm{\alpha}}^{\mathrm{RR}} \overset{d}{\to} \mathrm{N}(\bm{0}, (1
+ \| \bm{\alpha}\|^2) \bm{\Sigma}_S)$ by
\Cref{lem:gamma-ml}. Therefore the proof of \Cref{thm:asymptotics-rr} is completed once we can show
the largest eigenvalue of $\left[ \nabla
\bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is $O_p(1)$
and $\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to}
\bm{0}$. We prove these two facts in the following lemma:

\begin{lemma} \label{lem:asymptotics-rr-bound}
  Under the assumptions and limits in \Cref{thm:asymptotics-rr}, the
  largest eigenvalue of the matrix $\left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is bounded in probability
  and $\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to} \bm{0}$.
\end{lemma}

\begin{proof}
By using the representation of $\hat{\bm{\Gamma}}$ in
\eqref{eq:gamma-hat},
%and (C.4) in \citep{bai2012}.
%  \begin{equation*}
%    \label{eq:eq:sigma-hat}
%    \hat{\sigma}_j^2 = \frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
%    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}}),
%  \end{equation*}
we have
\[
\begin{split}
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) =& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
    \hat{\bm{\Gamma}}_j^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
/ \|\bm{X}\|_2 + \bm{\Gamma}_j^{(0)T} \bm{\alpha}^{(0)} - (\hat{\bm{\Gamma}}_j)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j\\
\end{split}
\]
where $\max_j|\delta_j| = o_p(1)$ and
$\max_j|\epsilon_j| = o_p(n^{-1/2})$ from
%\eqref{eq:avg-sigma-err}
%\Cref{lem:ml-baili}
\Cref{lem:gamma-ml}.
%and equation \eqref{eq:avg-gamma-err}.
Because
$\|\bm{\beta}\|_1 \sqrt{n} / p \to 0$ and $\psi'$ is bounded,
\[
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) = \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j + \bm{o}_p(n^{-1/2})
\]

Let $g_j$ be the expression inside $\psi$ in the last equation omitting $\epsilon_j$ and $\delta_j$. Conditionally on
$\tilde{\bm{Z}}_{-1}^{(0)}$, the variables $g_j, \mathrm{where}~ j=1,\dotsc,p$ are independent and
identically distributed with $\mathrm{E}(g_j) = 0$ and
$g_j = O_p (n^{-1/2}) $.
%Using the Cauchy-Schwartz inequality,
%$p^{-1}\sum_{j = 1}^p(\delta_jg_j)^2 = o_p(n^{-1})$.
Thus, using \Cref{assumption:psi-2nd-derivative}
and boundedness of $\hat \sigma_j$,
\[
\begin{split}
 & \Big\| \frac{1}{p} \sum_{j=1}^p \Big[\psi\Big(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\Big)
 - \psi(g_j)\Big]\hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 \\
\leq & D^2 \cdot \Big\| \frac{1}{p} \sum_{j=1}^p\big(|\epsilon_j| |\hat{\bm{\Gamma}}_j|+ |g_j|
|\delta_j\hat{\bm{\Gamma}}_j|\big) /\hat \sigma_j
%\big(|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}| + |\bm{\Gamma}_j^{(0)}|\big)/\hat \sigma_j
\Big\|_2  = o_p(n^{-1/2})
\end{split}
\]
%where the last approximation is got by using Cauchy-Schwartz inequality and \Cref{lem:ml-baili}.
%where $t_j$ are
%i.i.d. normal random variables by noticing $\tilde{\bm{Z}}_{-1}^{(0)}
%\bm{\alpha}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R} \bm{R}^T)^{-1}
%(\bm{\alpha} + \bm{u}/\|\bm{X}\|_2)$ and $\bm{R} \bm{R}^T \to \bm{I}_r$.
%Because for some $W'$ between $0$ and $W$ and
%$\psi(0) = 0$, $\psi(g_j) = \psi'(0) (n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}}))$ if $\beta_j =0$.


We can further use the facts that
$\psi(g_j)=\psi'(0) g_j +
o_p(n^{-1/2}) = O_p(n^{-1/2})$ and
%Cauchy-Schwartz inequality in a similar way and combine
$\psi(g_j) - \psi'(0)g_j$
are i.i.d., and combine \Cref{rmk:rotation} and \Cref{lem:gamma-ml} to get:
\[
\begin{split}
\left\|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right\|_2 &= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi(g_j)\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
%O_p(n^{-\frac{1}{2}}p^{-\frac{1}{2}}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi'(0)g_j\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
&=o_p(n^{-\frac{1}{2}})+ o_p(n^{-\frac{1}{2}})
= o_p(n^{-\frac{1}{2}})
\end{split}
\]


Similarly,
%$\psi$ is assumed to be bounded $|\psi(g_j)| \le C$ in
%\Cref{assumption:rho}. Therefore, by
because $\lim_{p \to \infty}
\frac{1}{p} \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ exists and is
positive definite (in \Cref{assumption:large-factor}),
we use \Cref{assumption:psi-2nd-derivative} and the uniform convergence
of $\hat {\bm \Sigma}$ and $\hat{\bm \Gamma}$ in \Cref{lem:gamma-ml} to get
\[
\begin{split}
  \left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1} &=
\Bigg[\frac{1}{p} \sum_{j=1}^p
  \psi'\left(g_j + \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right)
\hat{\bm{\Gamma}}_j \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
&= \Bigg[\frac{1}{p} \sum_{j = 1}^p
  \psi'\left(0\right)
  \bm{\Gamma}_j^{(0)} \bm{\Gamma}_j^{(0)T} / \sigma_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(\beta_j) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 \right]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(0) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \frac{1}{p} \sum_{\beta_j
%    \ne 0}
%  (\psi'(\beta_j) - \psi'(0)) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2  \right]^{-1} \\
&\overset{p}{\to} \Big[ \psi'(0) \frac{1}{p} \sum_{j=1}^p
  \bm{\Gamma}_j \bm{\Gamma}_j^T / \sigma_j^2 \Big]^{-1}
\end{split}
\]
%The last probability limit follows from $\hat{\bm{\Gamma}}
%\overset{p}{\to} \bm{\Gamma}$, $\hat{\bm{\sigma}}_j
%\overset{p}{\to} \sigma_j$ and $\psi'$, $\bm{\Gamma}$ and $\bm{\Sigma}$ are bounded.
This means that all the eigenvalues of
$\left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1}$ converge to finite constants.
\end{proof}

% For \Cref{thm:consistency}, we first note that when $n,p \to \infty$
% and $\|\beta\|_0/p \to 0$,
% $\hat{\bm{\alpha}}^{\mathrm{RR}} \overset{p}{\to} \bm{\alpha}^{(0)}$
% is still true by the same argument in the proof of
% \Cref{thm:asymptotics-rr} and the fact that we can estimate the strong
% factors consistently. By using the same Taylor expansion in the proof
% of \Cref{thm:asymptotics-rr}, the consistency of
% $\hat{\bm{\beta}}^{\mathrm{RR}}$ is immediately proved by the
% following lemma:
% \begin{lemma}
%   Under the assumptions and limits in \Cref{thm:consistency}, the largest eigen value of $\left[ \nabla
%   \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is bounded in probability
% and $\bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to} 0$.
% \end{lemma}
% \begin{proof}
%   The statement of this lemma is almost the same as
%   \Cref{lem:asymptotics-rr-bound}, except we relax the sparsity
%   condition from $\|\bm{\beta}\|_0 \sqrt{n}/p \to 0$ to
%   $\|\bm{\beta}\|_0 /p \to 0$ and we are only able to prove
%   $\bm{\Psi}_p(\bm{\alpha}^{(0)}) = o_p(1)$ instead of
%   $o_p(1/\sqrt{n})$. By the same argument in
%   \Cref{lem:asymptotics-rr-bound}, $\left[ \nabla
%   \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1} = O_p(1)$ and
% \[
% \begin{split}
% \left|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right|
% &= \left| \frac{1}{p} \left( \sum_{\beta_j \ne 0} + \sum_{\beta_j = 0} \right) \psi\left(g_j
% + o_p(1)\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
% \right| \\
% &\le \frac{1}{p} D \|\bm{\beta}\|_0 + o_p(1) \\
% &= o_p(1)
% \end{split}
% \]
% Notice that here the denominator of $g_j$ may not converge to
% $\sigma_j$ any more because $\hat{\sigma}_j$ is not necessarily
% consistent for $\sigma_j$. However, in \Cref{assumption:bounded} we
% assume $\hat{\sigma}_j$ is bounded below and above, so inconsistency
% of $\hat{\sigma}_j$ doesn't change the conclusion that
% $\left|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right| = o_p(1)$.

% \end{proof}


==> app_thm_weak.tex <==
Now we prove the first claim in \Cref{thm:consistency-weak} that \ $\hat{{\alpha}}_{k}^{\mathrm{RR}} \overset{p}{\to}
    \alpha_{k}$, $k=1,\dotsc,s$. Let $S = \{1,2,\dotsc,s\}$. We follow the same strategy used in the proof of \Cref{thm:consistency-rr} in
    \Cref{app:consistency-rr} by showing that
\begin{equation} \label{eq:phi-op1-strong}
\varphi(\bm{\alpha}_S -
  \hat{\bm{\alpha}}_S) = \frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \sum_{k=1}^s \hat{\Gamma}_{jk} ({\alpha}_k -
  \hat{{\alpha}}_k)}{\hat{\sigma}}\right) = o_p(1)
\end{equation}
and
\begin{equation} \label{eq:consistency-key-strong}
  \mathrm{P} \left( \inf_{\|\tilde{\bm{\alpha}}\|_2 \ge \epsilon}
  {\varphi}(\tilde{\bm{\alpha}}) > \tau \right)
\to 1.
\end{equation}
Equation \eqref{eq:consistency-key-strong} can be proven using the same
argument in \Cref{app:consistency-rr}, so we omit it here. For
\eqref{eq:phi-op1-strong}, we again investigate for
$\|\tilde{\bm{\alpha}}\|_2 \le D'$
\begin{equation} \label{eq:lp-strong}
\begin{split}
l_p(\tilde{\bm{\alpha}}) &= \frac{1}{p}\sum_{j=1}^p
  \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
      \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}}\right) \\
&= \frac{1}{p}\sum_{j=1}^p
      \rho \left( \frac{\beta_j + \frac{\tilde{{E}}_{1j} + \bm \Gamma_j^T\tilde{\bm{W}}_1}{\|\bm{X}\|_2} +
\sum_{k=1}^r \left(\alpha_k
\Gamma_{j k}
-\tilde{\alpha}_k \hat{\Gamma}_{j k}\right)
}{\hat{\sigma}} \right)
\end{split}
\end{equation}
By \Cref{lem:weak-gamma} and boundedness of $\bm{\alpha}$ and
$\tilde{\bm{\alpha}}$ in \Cref{assumption:bound-alpha}, we have
$\sum_{k=s+1}^r \alpha_k
\Gamma_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{\Gamma}_{j k} = o_p(1)$ and
$\sum_{k=1}^s \Gamma_{jk} (\alpha_k - \tilde{\alpha}_k) = o_p(1)$. Because
$\rho$ has bounded derivative (\Cref{assumption:rho}),
$\|\bm{\beta}\|_1/p \to 0$, $\|\bm{X}\|_2 \to \infty$ and $\bm\Gamma$ is bounded,
we again have
$l_p(\tilde{\bm{\alpha}}) = \varphi(\bm{\alpha}_S -
\tilde{\bm{\alpha}}_S) + o_p(1)$ for any $\|\tilde{\bm{\alpha}}\|_2 \le
D'$ and the $o_p(1)$ term doesn't depend on
$\tilde{\bm{\alpha}}$. Therefore $\varphi(\bm{\alpha}_S -
  \hat{\bm{\alpha}}_S) = l_p(\hat{\bm{\alpha}}) + o_p(1) \le
  l_p(\bm{\alpha}) + o_p(1) = o_p(1)$.

To prove the second claim in \Cref{thm:consistency-weak}, notice that
\[
\hat{\beta}_j^{\mathrm{RR}} - {\beta}_j =
\frac{\tilde{{E}}_{1j} + \bm \Gamma_j^T\tilde{\bm{W}}_1}{\|\bm{X}\|_2} +
\sum_{k=1}^s \left(\alpha_k
{\Gamma}_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{{\Gamma}}_{j k}\right) +
\sum_{k=s+1}^r \left(\alpha_k
{\Gamma}_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{{\Gamma}}_{j k} \right)
\]
By the same argument as in the last paragraph,
$\hat{\beta}_j^{\mathrm{RR}} - {\beta}_j = \sum_{k=1}^s
\hat{\Gamma}_{jk} (\alpha_k - \hat{\alpha}_k) + o_p(1)$. Since
$\hat{\Gamma}_{jk} \overset{p}{\to} \Gamma_{jk}$ and $\hat{\alpha}_k
\overset{p}{\to} \alpha_k$ for $k = 1,\dotsc,s$, we conclude that
$\hat{\beta}_j^{\mathrm{RR}} \overset{p}{\to} \beta_j$.


==> app_weak_simu.tex <==
We decide the strength of the confounding factors in \Cref{sub:weak} based
on recent results in random matrix theory \citep{perry2009,
  donoho2013}. Their latent factor model is $ \bm Y = \sqrt n \bm {UDV}^T + \bm{E}$
where $\bm{U}^T\bm{U} = \bm{V}^T\bm{V} = \bm{I}_r$, $\bm{D}$ is a diagonal $r \times r$
matrix and $\bm{E} \sim \sigma^2 \mathrm{MN}(0, \bm{I}_n, \bm{I}_p)$. The goal is to recover the matrix $\sqrt n \bm{UDV}^T$ from
the observed matrix $\bm{Y}$ as accurately as possible.

A natural estimator of $\sqrt n \bm{UDV}^T$ is the truncated SVD of
$\bm Y$ using the first $k$ singular values/vectors, denoted by
$\bm{Y}(k)$. Let $r_0 = \arg \min_k \|\bm Y(k) - \sqrt n
\bm{UDV}^T\|_F$ be the optimal number of factors to include. \citet{donoho2013} show that
in the asymptotic setting of $n \to \infty$, $p \to \infty$, $d_j^2 \to
\mu_j~,j=1,\dotsc,p$
and $p/n \to \gamma > 0$, $r_0$ converges to $|\{ j: \mu_j > \mu^{\star}
\}|$ where the estimation threshold $\mu^{\star}$ is \citep{perry2009}
\begin{equation}
\label{eq:mu-star}
\mu^\star = \sigma^2 \left(\frac{1 + \gamma}{2} + \sqrt{\Big(\frac{1 +
      \gamma}{2}\Big)^2 + 3 \gamma}\right).
\end{equation}
Notice that the detection threshold in \Cref{sec:weak-factors}, $\mu =
\sigma^2\sqrt{\gamma}$, is less than $\mu^\star$. This implies that if
$\mu < \mu_j < \mu^\star$, the factor is detectable but too small to
be included in the truncated SVD to reduce the estimation error of
$\sqrt n \bm {UDV}^T$. \cite{donoho2013} propose an estimator $\hat r$
such that $\hat r \overset{a.s.}{\to} r_0$.

For our simulation experiment in \Cref{sub:weak}, as $\bm{Z}_{-1}^T\bm{Z}_{-1}/n \to \bm{I}_r$, though we assume
random factors, their results still hold. Since we set $\sigma^2 = 1$ and $p = 5000$,
the largest factor $d_1 = 3 \cdot \sqrt p = 212$.
When $n = 100$, $d_r = \sqrt{\mu_F} = 2.7$ and $\sqrt {\mu^\star} = 7.3$,
and we set $(d_2, \cdots, d_9) = (73.3, 64.5, 55.7, 46.8, 38.0, 29.2, 20.3, 11.5)$
for $r = 10$
which is an equal spaced decreasing sequence with $d_2 = 10\cdot \sqrt {\mu^\star}$.
When $n = 500$, $d_r = \sqrt{\mu} = 1.8$
and $\sqrt {\mu^\star} = 3.6$,
and correspondingly we set $(d_2, \cdots, d_9) =(36.4, 32.1, 27.8, 23.4, 19.1, 14.8, 10.4,  6.1)$
for $r = 10$.

Finally, we discuss the variance-bias tradeoff in our
simulation in \Cref{sub:weak}.
The oracle method has distribution
\[
\sqrt n (\hat \beta^{\mathrm{Oracle}}_j - \beta_j)\sim
\mathrm{N}(0, 1 + \|\bm \alpha\|_2^2).
\]
Next we consider the RR
method. In the case of $r=2$, we can rewrite \eqref{eq:y-tilde-1} as
\[
        \tilde{\bm{Y}}_1^T / \|\bm{X}\|_2 = \bm{\beta} + \bm{\Gamma}_{\cdot 1}(\alpha_1 + u_1/\|\bm{X}\|_2)
+ \bm{\Gamma}_{\cdot 2}(\alpha_2 + u_2/\|\bm{X}\|_2)
   + \tilde{\bm{E}}_{1}^T / \|\bm{X}\|_2
\]
where $u_i\sim \mathrm{N}(0, 1)$. In our simulation in
\Cref{sub:weak}, $r_0 = 1$ and RR only adjusts for one (the strongest) confounding
factor. As a consequence, $\check{e}_{j} = \Gamma_{j2}(\alpha_2 +
u_2/\|\bm{X}\|_2) + \tilde{E}_{1j}^T/\|\bm X\|_2 $ can be treated as
the new noise terms. Since $\Gamma_{j2}$ is generated by $\Gamma_{j2} = d_2\cdot\tilde{\Gamma}_{j2} = d_2 \cdot z_{j}/\|\bm{z}\|_2$ where
$\bm{z} = (z_1, \cdots, z_p)\sim \mathrm{N}(\bm 0, \bm I_p)$, when $n, p \to \infty$, 
$\mathbb{E}(\sqrt n \cdot \check{e}_j) = 0$,
$\mathrm{Var}(\sqrt n \cdot \check{e}_j) \to \alpha_2^2\cdot d_2^2\cdot n/p + 1$
and $\mathrm{Cov}(\sqrt n \cdot \check{e}_{j_1}, \sqrt n \cdot \check{e}_{j_2}) \to 0$
for $j_1 \neq j_2$.
Assuming that we asymptotically get the strong factor $\bm{\Gamma}_{\cdot 1}$ as
accurate as what the oracle gets,
then using \Cref{thm:consistency-weak} and similar to the calculation in \Cref{thm:asymptotics-rr},
we have
\[
\sqrt n (\hat \beta^{\mathrm{RR}}_j - \beta_j) \overset{d}{\to}
\mathrm{N}(0, 1 + \alpha_1^2 + \alpha_2^2\cdot d_2^2/\gamma).
\]
Thus, as long
as $d_2^2 < \gamma = p/n$, $\beta^{\mathrm{RR}}_j$ is more accurate
than $\beta^{\mathrm{Oracle}}_j$. The calibration method uses MAD to
estimate the variance inflation factor $(1 + \alpha_1^2 +
\alpha_2^2\cdot \gamma d_2^2)/(1 + \alpha_1^2)$ empirically. This is
why LEAPP and RR-MAD can control the type I error and FDR in \Cref{fig:p-5000-weak-methods}.

An interesting final observation is that $d_i^2 > \sigma^2 \gamma$ provides
a threshold of factor strength in the confounder
adjusting problem. When $\gamma$ is large, this is about the same as
the estimation threshold $\mu^{\star}$ \eqref{eq:mu-star} in the
low-rank matrix approximation problem.


==> asymp_eff.tex <==
Consider the oracle estimator of the primary effects $\bm{\beta}$ such that the confounding
variables $\bm{Z}$ were observed. In this
case, \eqref{eq:linear-model-y} becomes a linear model with random
predictors and the ordinary least squares estimator of
$\bm{\beta}$ and $\bm{\Gamma}$ have the minimum variance among all
linear estimators. The variance
of $(\hat{{\beta}}^{\mathrm{OLS}}_j,
\hat{\bm{\Gamma}}^{\mathrm{OLS}}_j)$ is $ \sigma_j^2
\mathrm{Var}(X_i, \bm{Z}_i)^{-1} / n$. Since
\[
\mathrm{Var}(X_i, \bm{Z}_i) =
\begin{pmatrix}
  1 & \bm{\alpha}^T \\
  \bm{\alpha} & \bm{I}_r + \bm{\alpha} \bm{\alpha}^T \\
\end{pmatrix},
\]
it is easy to show that $\mathrm{Var}(\hat{\beta}_j^{\mathrm{OLS}}) =
(1 + \|\bm{\alpha}\|_2^2) \sigma_j^2/n$. Also, for $j \ne k$,
$\mathrm{Cov}(\hat{\beta}_j^{\mathrm{OLS}},
\hat{\beta}_k^{\mathrm{OLS}}) = 0$ by conditioning on $\bm{X}$ and
$\bm{Z}$. In summary,
\[
\mathrm{Var}(\hat{\bm{\beta}}^{\mathrm{OLS}}) = \frac{1}{n} (1 + \| \bm{\alpha}
\|_2^2) \bm{\Sigma},
\]
which is the same asymptotic variance we derived in
\Cref{thm:asymptotics-nc,thm:asymptotics-rr}. Since the estimator
$\hat{\bm{\beta}}^{\mathrm{OLS}}$ require oracle knowledge of the
confounders $\bm{Z}$, we conclude that %our confounder adjusted estimators
$\hat{\bm{\beta}}^{\mathrm{NC}}$ and
$\hat{\bm{\beta}}^{\mathrm{RR}}$ are asymptotically efficient among
linear estimators under
the corresponding assumptions in \Cref{thm:asymptotics-nc,thm:asymptotics-rr}.

% \begin{remark} \label{rmk:alpha-intuition}
%  The variance $(1 + \| \bm{\alpha}\|_2^2) \bm{\Sigma} / n$ depends on
%  three quantities: $\| \bm{\alpha}\|_2^2$, the total covariance of
 % $\bm{Z}$ with $\bm{X}$; $\bm{\Sigma}$,
%  the intrinsic variance of $\bm{Y}$; and $n$, the number of
%  observations. 
As mentioned in \Cref{sec:linear-model-with},
  $\|\bm{\alpha}\|^2/(1 + \|\bm{\alpha}\|^2)$ is the proportion of
  variance of $\bm{X}$ that can be explained by the confounders. Our
  variance expression $(1 + \| \bm{\alpha}\|_2^2) \bm{\Sigma} / n$ of $\hat{\bm{\beta}}^{\mathrm{RR}}$ coincides with the intuition that the estimation of
  $\bm{\beta}$ should become harder as the confounders $\bm{Z}$ are more
  correlated with $\bm{X}$. % Since $\|
  % \bm{\alpha}\|_2^2$ can be much larger than $1$ in our model
  % \eqref{eq:linear-model-y}, ignoring the uncertainty of estimating
  % confounders in the asymptotic variance may also significantly bias the test $p$-values.
% \end{remark}


==> revision 2/_make <==
% JS is editing
\subsection{Simulations}
\label{sec:simulations}

\Cref{thm:asymptotics-nc,thm:consistency-rr,thm:asymptotics-rr,cor:type-I,thm:multiple-rr,thm:consistency-weak}
have provided theoretical guarantees in different senarios for the asymptotics setting when $n, p \to \infty$.
In this section, we use simulations to illustrate these results and consider finite sample properties of our estimators
and tests.

Data are generated from the model \eqref{eq:linear-model-y,eq:linear-model-z,eq:linear-model-x,eq:linear-model-e}. More specifically, $X_i$ are centered binary variables with $\frac{X_i + 1}{2} \overset{\mathrm{iid}}{\sim} \mathrm{Bernoulli}(1, 0.5)$. For generating the parameters, the noises variances have
$\sigma_i \overset{\mathrm{iid}}{\sim}\mathrm{InvGamma}(3, 2)$ thus $\mathbb{E}(\sigma_i^2) = \mathrm{Var}(\sigma_i^2) = 1$. $\|\bm{\alpha}\|_2^2 = 3$ thus the variance of $X_i$ explained by the latent factors is $75\%$, and we set each $\alpha_k = \frac{\|\bm{\alpha}\|_2}{\sqrt r}$ for $k = 1, 2, \cdots, r$. The treatment effect $\bm{\beta}$ has
independent components $\beta_i$ taking the values $3 \sqrt{1 + \|\bm{\alpha}\|_2^2}$ and $0$ with probability
$\pi = 0.1$ and $1 - \pi = 0.9$, respectively. We set the number of latent factors $r$ to be either $2$ or $10$.
For the latent factor matrix $\bm \Gamma$, 
$\bm\Gamma = \tilde{\bm\Gamma}\bm{D}$ where $\tilde{\bm\Gamma}$ is a $p \times r$ orthogonal matrix sampled uniformly
from the Stiefel manifold $V_r(\mathbb{R}^p)$ and $\bm(D) = \sqrt p\cdot \mathrm{diag}(d_1, \cdots, d_r)$ where 
$d_k = 3 - \frac{2(k-1)}{r - 1}$. Finally, we set $p = 5000$ and $n = 100$ or $500$ to mimic the data size in 
most genetic studies.


\subsection{Real data example}
\label{sec:gender-study}

In this section, we return to the two motivational examples in
\cref{sec:introduction}. Recall that without confounder adjustment,
the distribution of the regression $t$-statistics are clearly
underdispersed (\cref{fig:gender-naive-batch}), noncentered
(\cref{fig:alzheimers-naive}), skewed
(\cref{fig:gender-naive-batch,fig:alzheimers-naive}). These two examples are originally studied
in \citep{gagnon2013} using the negative control (NC) method and we
refer the reader to their paper for more empirical results.

In \cref{tab:gender,tab:alzheimers}, we present the results after
adjustment for the two datasets. The adjustment method here is the
maximum likelihood factor analysis described in \cref{sec:inference-gamma-sigma} and the
robust regression (RR) method with Tukey's bisquare loss described in
\cref{sec:unkn-zero-indic}. Since the true number of confounders is
unknown, we increase $r$ from $1$ to $25$ and study the empirical
performance. The empirical performance metrics are total number of
significant genes of p-value less than $0.01$ after the empirical calibration in
\cref{sec:hypothesis-testing} (second column), number of
the genes on X/Y chromosome that have p-value less than $0.01$ (third
column), and the number among the $100$ most significant genes that are on the X/Y chromosome (fourth column).
The summary statistics of regression t-statistics being reported
in \cref{tab:gender,tab:alzheimers} are the mean, median, standard
deviation (sd), median absolute deviation (mad), skewness, and
medcouple (a robustness measure of skewness). In general, the
statistics in \cref{eq:test-statistic} become more centered at $0$ and
less skewed as we include a few confounders in the model.

% latex table generated in R 3.1.2 by xtable 1.7-4 package
% Sun May 24 17:21:30 2015
\begin{table}[ht]
\centering
\caption{The first dataset in \cref{fig:gender-naive-batch}: $n = 84$,
$p = 12600$. The bolded row corresponds to the $r$ selected by BCV.}
\label{tab:gender}
\footnotesize
\begin{tabular}{$r|^r^r^r^r^r^r^r^r^r}
  \hline
r & \#sig. & X/Y & top 100 & mean & median & sd & mad & skewness & medcouple \\
  \hline
0 & 1369 & 107 & 11 & 0.11 & 0.043 & 0.36 & 0.237 & 2.99 & 0.2 \\
  1 & 335 & 80 & 16 & -0.34 & -0.36 & 1.03 & 1.01 & 0.74 & 0.033 \\
  2 & 218 & 74 & 20 & -0.079 & -0.086 & 1.14 & 1.12 & 0.612 & 0.011 \\
  3 & 272 & 80 & 28 & 0.0061 & 0.00086 & 1.12 & 1.07 & 0.818 & -0.0021 \\
  4 & 294 & 77 & 27 & 0.02 & 0.024 &  1.2 & 1.15 & 0.65 & -0.0099 \\
  5 & 380 & 84 & 29 & -0.0047 & -0.025 & 1.18 & 1.09 & 0.847 & 0.013 \\
  7 & 393 & 79 & 27 & -0.01 & -0.023 & 1.26 & 1.16 & 0.778 & -0.000074 \\
  10 & 411 & 79 & 30 & -0.0024 & -0.011 & 1.37 & 1.26 & 0.632 & -0.0038 \\
  15 & 443 & 86 & 29 & -0.00027 & -0.014 & 1.46 & 1.34 & 0.554 & 0.00026 \\
  20 & 425 & 80 & 29 & 0.0076 & -0.029 & 1.52 &  1.4 & 0.476 & 0.029 \\
\rowstyle{\bfseries}
  25 & 431 & 84 & 28 & 0.0069 & -0.027 & 1.65 & 1.51 & 0.422 & 0.024 \\
  30 & 449 & 77 & 30 & 0.0054 & -0.023 & 1.77 &  1.6 & 0.441 & 0.019 \\
  40 & 451 & 79 & 29 & 0.0091 & -0.0092 & 1.98 & 1.78 & 0.526 & 0.0075 \\
   \hline
\end{tabular}
\end{table}

% latex table generated in R 3.1.2 by xtable 1.7-4 package
% Sun May 24 17:20:06 2015
\begin{table}[ht]
\centering
\caption{The second dataset in \cref{fig:alzheimers-naive}: $n = 31$,
$p = 22283$. The bolded row corresponds to the $r$ selected by BCV.}
\label{tab:alzheimers}
\footnotesize
\begin{tabular}{$r|^r^r^r^r^r^r^r^r^r}
  \hline
r & \#sig. & X/Y & top 100 & mean & median & sd & mad & skewness & medcouple \\
  \hline
0 & 19059 & 783 & 15 & -1.8 & -1.8 & 0.599 & 0.513 & -3.46 & 0.082 \\
  1 & 753 & 115 & 20 & -0.44 & -0.44 & 1.08 & 0.995 & -1.55 & 0.0055 \\
  2 & 588 & 126 & 23 & -0.22 & -0.24 & 1.19 & 1.11 & -0.992 & 0.013 \\
  3 & 528 & 127 & 26 & -0.15 & -0.17 & 1.27 & 1.18 & -0.843 & 0.014 \\
  4 & 508 & 126 & 27 & -0.21 & -0.23 & 1.29 & 1.22 & -0.813 & 0.012 \\
  5 & 628 & 123 & 24 & -0.26 & -0.26 & 1.31 & 1.22 & -1.34 & -0.0074 \\
  7 & 578 & 117 & 24 & -0.28 & -0.28 & 1.46 & 1.37 & -0.888 & -0.0039 \\
  9 & 649 & 134 & 29 & -0.24 & -0.23 & 1.48 & 1.37 & -0.793 & -0.012
  \\
\rowstyle{\bfseries}

  11 & 702 & 141 & 31 & -0.16 & -0.16 & 1.52 & 1.37 & -0.599 & 0.003 \\
  13 & 722 & 138 & 28 & -0.15 & -0.16 & 1.66 & 1.49 & -0.875 & 0.0086 \\
  15 & 764 & 142 & 27 & -0.17 & -0.18 & 1.82 & 1.63 & -0.345 & 0.013 \\
  20 & 879 & 142 & 25 & -0.2 & -0.2 & 2.52 & 2.19 & -0.309 & -0.0026 \\
   \hline
\end{tabular}
\end{table}

A practical way to pick $r$ is the bi-cross-validation (BCV) method of
\citet{owen2015}, which uses randomly held-out submatrices to estimate
the mean squared error of reconstructing factor loading matrix. In \cref{fig:gender-output,fig:alzheimers-output},
we demonstrate the performance of BCV on these two datasets. The $r$
selected by BCV is respectively $25$ and $11$ (\cref{fig:gender-bcv,fig:alzheimers-bcv}), and they both result in presumed shape of z-statistics distribution
(\cref{fig:gender-t,fig:alzheimers-t}) and near optimal performance in
of selecting genes on the X/Y chromosome
(\cref{tab:gender,tab:alzheimers}). The fact that the empirical variance
of the z-statistics in both cases are slightly larger than $1$ is not
too surprising; see \cref{rmk:calibration} for some discussion.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/gender-bcv.pdf}
  \caption{Bi-cross-validation error selects $r=25$.}
  \label{fig:gender-bcv}
  \end{subfigure}
  \qquad
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/gender-output.pdf}
  \caption{Distribution of the statistics after
  confounder adjustment.}
  \label{fig:gender-t}
  \end{subfigure}
  \caption{The first dataset where the unadjusted t-statistics are
  shown in \cref{fig:gender-naive-batch}.}
  \label{fig:gender-output}
\end{figure}

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/alzheimers-bcv.pdf}
  \caption{Bi-cross-validation error selects $r=11$.}
  \label{fig:alzheimers-bcv}
  \end{subfigure}
  \qquad
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{../plots/alzheimers-output.pdf}
  \caption{Distribution of the statistics after
  confounder adjustment.}
  \label{fig:alzheimers-t}
  \end{subfigure}
  \caption{The second dataset where the unadjusted t-statistics are
  shown in \cref{fig:alzheimers-naive}.}
  \label{fig:alzheimers-output}
\end{figure}

Lastly we want to comment on the sample size $n$. Our entire
asymptotic analysis is based on $r$ fixed and $n,p \to \infty$. In the second
dataset $n$ is only $31$, so the adjustment result is not ideal. In
\cref{tab:alzheimers}, adding the first two confounders significantly
reduces the mean and skewness of the statistics, but the mean and
median of the statistics remain negative no matter how many factors
are used. This is likely due to the fact that $n$ is too small to
estimate the confounders accurately. However, the empirical
performance (e.g.\ number of X/Y genes in top $100$) suggests it
is still beneficial to adjust for the confounders.


==> revision 2/abstract.tex <==
We consider large-scale studies in which thousands of significance
tests are performed simultaneously. In some of these studies, the
multiple testing procedure can be severely biased by latent confounding factors such as batch
effects and unmeasured covariates that correlate with both primary
variable(s) of interest (e.g.\ treatment variable, phenotype) and the
outcome. Over the past decade, many statistical methods have been proposed
to adjust for the confounders in hypothesis testing.
We unify these methods in
the same framework, generalize them to include multiple primary variables and
multiple nuisance variables, and analyze their statistical properties. In
particular, we provide theoretical guarantees for RUV-4
\citep{gagnon2013} and LEAPP \citep{sun2012}, which correspond to two
different identification conditions in the framework:
the first requires a set of ``negative controls'' that are known
\textit{a priori} to follow the null distribution; the second requires
the true non-nulls to be sparse.
Two different estimators which are %slightly modified from
based on RUV-4 and
LEAPP are then applied to these two scenarios.
We show that if the confounding
factors are strong, the resulting estimators can be asymptotically as
powerful as the oracle estimator which observes the latent confounding
factors.
For hypothesis testing, we show the asymptotic $z$-tests based on the
estimators can control the type I error. Numerical experiments show
that the false discovery rate is also controlled by the
Benjamini-Hochberg procedure when the sample size is reasonably large.


==> revision 2/app_alpha_test.tex <==
First, we point out that when $\bm\alpha = \bm 0$, as $n, p \to \infty$ 
\begin{equation}\label{eq:asy-alpha-0}
\sqrt n \cdot \bm \alpha^{(0)} = \sqrt n \cdot \bm R^{-1} \tilde{\bm W}_1  \overset{d}{\to} \mathrm{N}(0, \bm I_r)
\end{equation}
where $\bm \alpha^{(0)}$, $\bm R$ and $\tilde{\bm W}_1$ are defined in \Cref{sec:inference-beta-alpha}. 
This is due to the fact that $\bm R \to \bm I_r$ (\Cref{rmk:rotation}) and 
$\sqrt n\tilde{\bm W}_1 \sim \mathrm{N}(\bm 0, \bm I_r)$, thus Slutsky's Theorem implies \eqref{eq:asy-alpha-0}.
Next, we show that 
\begin{equation}\label{eq:asy-hat-alpha}
\sqrt n \cdot({\hat {\bm \alpha} - \bm\alpha^{(0)}}) = \bm o_p(1)
\end{equation}

For the negative control scenario, using the expression of $\hat{\bm \alpha}^{\NC}$ in \eqref{eq:alpha-nc} and 
$\tilde{\bm Y}_{1, \calC}/\|\bm X\|_2$ in \eqref{eq:y-tilde-1-separate}, we get
\[
\begin{split}
\sqrt n (\hat{\bm \alpha} - \bm \alpha^{(0)}) 
=& \sqrt n(\hat{\bm \Gamma}_\calC \hat{\bm \Sigma}_\calC^{-1}\hat{\bm \Gamma}_\calC )^{-1}
\hat{\bm \Gamma}_\calC \hat{\bm \Sigma}_\calC^{-1}(\bm \Gamma_\calC^{(0)} - \hat{\bm \Gamma}_\calC) \bm \alpha^{(0)}\\
+& \frac{\sqrt n}{\|\bm X\|_2}(\hat{\bm \Gamma}_\calC \hat{\bm \Sigma}_\calC^{-1}\hat{\bm \Gamma}_\calC )^{-1}
\hat{\bm \Gamma}_\calC \hat{\bm \Sigma}_\calC^{-1}\tilde{\bm E}_{1\calC}^T.
\end{split}
\]
Using the facts we got in \eqref{eq:nc-facts} and $\bm \alpha^{(0)} = \bm o_p(1)$, we further get
\[
\sqrt n (\hat{\bm \alpha} - \bm \alpha^{(0)}) 
= (\bm \Gamma_\calC \bm \Sigma_\calC^{-1} \bm \Gamma_\calC)^{-1} \bm \Gamma_\calC \bm \Sigma_\calC^{-1}
\tilde{\bm E}_{1\calC}^T + \bm o_p(1).
\]
Under \Cref{assumption:nc-factor}, if $|\calC| \to \infty$, the maximum eigenvalue of 
$(\bm \Gamma_\calC \bm \Sigma_\calC^{-1} \bm \Gamma_\calC)^{-1}$ goes to $0$, thus \eqref{eq:asy-hat-alpha} holds 
for the negative control scenario.

For the sparsity scenario, in the proof of \Cref{thm:asymptotics-rr}, we have shown that 
\[
 \sqrt n(\hat{\bm \alpha}^\RR - \bm \alpha^{(0)}) = -\sqrt n \left[ \nabla 
 \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm o_p(1) \right]^{-1} 
 \bm{\Psi}_p(\bm \alpha^{(0)})
\]
Thus, because of \Cref{lem:asymptotics-rr-bound}, \eqref{eq:asy-hat-alpha} also holds for the sparsity scenario.

Finally, combining \eqref{eq:asy-alpha-0} and \eqref{eq:asy-hat-alpha}, \Cref{thm:alpha-test} holds.



==> revision 2/app_consistency.tex <==
As in the proof of \Cref{thm:asymptotics-nc}, we prove the
conclusions in this theorem for any fixed $\tilde{\bm{W}}_1$ and fixed
sequences $\{\bm{X}^{(n)}\}_{n=1}^{\infty}$ and
$\{\bm{R}^{(n,p)}\}_{n=1,p=1}^{\infty}$ such that
$\|\bm{X}^{(n)}\|_2/\sqrt{n} \to 1$ and $\bm{R}^{(n,p)} \to \bm{I}_r$ as $n,p \to \infty$. For brevity we
will write $\bm{X}$ and $\bm{R}$ instead of $\bm{X}^{(n)}$ and $\bm{R}^{(n,p)}$ for the rest of this proof.
%Also we treat $\bm{\Gamma}^{(0)}$ as bounded by $D$ as discussed in
%\Cref{rmk:rotation}.
We abbreviate $\hat{\bm{\alpha}}^{\mathrm{RR}}$
as $\hat{\bm{\alpha}}$ in this proof. To avoid confusion, we
use $\bm \alpha$ for the true value of the parameter and
$\tilde{\bm \alpha}$ to represent a vector in $\mathbb{R}^r$.

  Because $\bm{\alpha}^{(0)} \to \bm{\alpha}$, we prove
  this theorem by showing that for any $\epsilon > 0$,
  $\mathrm{P}(\|\hat{\bm{\alpha}} -
  \bm{\alpha}^{(0)}\|_0 \ge \epsilon) \to 0$. We break down our proof
  to two key results: First, we show $\hat{\bm{\alpha}}$ and
  $\bm{\alpha}^{(0)}$ are close in the following sense
\begin{equation} \label{eq:phi-op1}
\varphi(\bm{\alpha}^{(0)} -
  \hat{\bm{\alpha}}) = \frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \hat{\bm{\Gamma}}_j^T (\bm{\alpha}^{(0)} -
  \hat{\bm{\alpha}})}{\hat{\sigma}_j}\right) = o_p(1),
\end{equation}
and second, we show that for sufficiently small
  $\epsilon > 0$, there exists $\tau > 0$ such that as $n, p \to \infty$
\begin{equation} \label{eq:consistency-key}
  \mathrm{P} \left( \inf_{\|\tilde{\bm{\alpha}}\|_2 \ge \epsilon}
  {\varphi}(\tilde{\bm{\alpha}}) > \tau \right)
\to 1.
\end{equation}

Based on these two results and the observation that
\[
\{ \|\bm{\alpha}^{(0)} - \hat{\bm{\alpha}}\|_2 < \epsilon \} \supseteq
\left\{ {\varphi}(\bm{\alpha}^{(0)} - \hat{\bm{\alpha}}) < \tau \right\} \bigcap
\left\{ \inf_{\|\tilde{\bm{\alpha}}\|_2 \ge \epsilon} {\varphi}(\tilde{\bm{\alpha}}) > \tau \right\},
\]
we conclude that $\mathrm{P}(\|\hat{\bm{\alpha}} -  \bm{\alpha}^{(0)}\|_2 \ge \epsilon) \to 0$.

Let's start with \eqref{eq:phi-op1}. Denote
$l_p(\tilde{\bm{\alpha}}) = p^{-1}\sum_{j=1}^p
  \rho \left( {\tilde{Y}_{1j} / \|\bm{X}\|_2 -
  \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}/{\hat{\sigma}_j}\right)$. By
  \eqref{eq:alpha-rr}, we have $\hat{\bm{\alpha}}^{\mathrm{RR}} = \arg
  \min l_p(\tilde{\bm{\alpha}})$, so $l_p(\hat{\bm{\alpha}}) \le
  l_p(\bm{\alpha}^{(0)})$. We examine the difference between
  $l_p(\tilde{\bm{\alpha}})$ and $\varphi(\bm{\alpha}^{(0)} - \tilde{\bm{\alpha}})$ for any
  $\tilde{\bm{\alpha}}$, starting from
\begin{equation*}
\begin{split}
l_p(\tilde{\bm{\alpha}}) & = \frac{1}{p}\sum_{j=1}^p
  \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
      \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right) \\
& = \frac{1}{p} \sum_{j=1}^p \rho\left(  \frac{ \beta_j + (\bm{\Gamma}^{(0)}_j)^T
  \bm{\alpha}^{(0)} + \tilde{E}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T
    \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right).\\
\end{split}
\end{equation*}
Because $\rho$ has bounded derivative, $|\rho(x) - \rho(y)| \le D |x -
y|$ for any $x,y \in \mathbb{R}$. In the statement of
\Cref{thm:consistency-rr} we assume $\|\bm{\beta}\|_1/p \to 0$. This
together with $\|\bm{X}\|_2 \to 0$ implies that
\begin{equation*}
  l_p(\tilde{\bm{\alpha}}) = \frac{1}{p} \sum_{j=1}^p \rho\left(  \frac{ (\bm{\Gamma}^{(0)}_j)^T
  \bm{\alpha}^{(0)} - \hat{\bm{\Gamma}}_j^T
    \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right) + o_p(1).
\end{equation*}
Next,
\[
\left|\frac{ (\bm{\Gamma}^{(0)}_j)^T
  \bm{\alpha}^{(0)}  - \hat{\bm{\Gamma}}_j^T
    {\tilde{\bm{\alpha}}}}{\hat{\sigma}_j} - \frac{
  \hat{\bm{\Gamma}}_j (\bm{\alpha}^{(0)} -
  {\tilde{\bm{\alpha}}})}{\hat{\sigma}_j}\right|
=  \left|
  \frac{(\bm{\Gamma}^{(0)}_j - \hat{\bm{\Gamma}}_j)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}
\right| \overset{p}{\to} \bm{0}.
\]
Therefore, by the same argument as before,
\begin{equation}
  \label{eq:consistency-proof-1}
  l_p(\tilde{\bm{\alpha}}) = \frac{1}{p} \sum_{j=1}^p \rho\left( \frac{
  \hat{\bm{\Gamma}}_j (\bm{\alpha}^{(0)} -
  {\tilde{\bm{\alpha}}})}{\hat{\sigma}_j} \right) + o_p(1) =
\varphi(\bm{\alpha}^{(0)} - \tilde{\bm{\alpha}}) + o_p(1).
\end{equation}
Also, $\varphi(\bm{0}) = 0$ because $\rho(0)
= 0$. Therefore $l_p(\hat{\bm{\alpha}}) \le l_p(\bm{\alpha}^{(0)}) =
o_p(1)$. Notice that the $o_p(1)$ term in
\eqref{eq:consistency-proof-1} does not depend on $\hat{\bm{\alpha}}$,
hence $\varphi(\bm{\alpha}^{(0)} - \hat{\bm{\alpha}}) =
l_p(\hat{\bm{\alpha}}) + o_p(1) = o_p(1)$.

Next we prove \eqref{eq:consistency-key}. Since $\rho(x)$ is 
non-decreasing when $x \geq 0$,
\[
\inf_{\|\tilde{\bm{\alpha}}\|_2 \ge \epsilon} \frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right) \ge
\inf_{\|\tilde{\bm{\alpha}}\|_2 = \epsilon}
\frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right).
\]
If $p/n^k \to 0$ for some $k > 0$, then using \Cref{lem:gamma-ml}, there exists 
some constant $D^\star$ that $\Prob(\max_j\|\hat {\bm \Gamma}_j\|_2 \leq D^\star) \to 1$.
Thus when $\max_j\|\hat {\bm \Gamma}_j\|_2 \leq D^\star$ holds,
there is sufficiently small $\epsilon > 0$, the $\tilde{\bm{\alpha}}$ on the right hand
side is within the neighborhood where $\rho$ is strongly convex in
\Cref{assumption:rho}, so for some $\kappa > 0$
\[
\inf_{\|\tilde{\bm{\alpha}}\|_2 = \epsilon}
\frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right) \ge
\inf_{\|\tilde{\bm{\alpha}}\|_2 = \epsilon} \kappa \cdot
\frac{1}{p} \sum_{j=1}^p \left(\frac{
  \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}_j}\right)^2 = \kappa\epsilon^2 \cdot
\lambda_{\mathrm{min}}\left( \hat{\bm{\Gamma}}^T
  \hat{\bm{\Sigma}}^{-1} \hat{\bm{\Gamma}} \right).
\]
By the uniform consistency of $\hat{\bm{\Gamma}}$ and $\hat{\bm{\Sigma}}$ using \Cref{lem:gamma-ml}, we
conclude \eqref{eq:consistency-key} is true for $\tau = \kappa\epsilon^2
\lambda_{\mathrm{min}}(\bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}) /
2$, where $\lambda_{\mathrm{min}}(\bm{\Gamma}^T \bm{\Sigma}^{-1}
\bm{\Gamma}) > 0$ by \Cref{assumption:large-factor}.


==> revision 2/app_copd_add_table.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[h]%{\textwidth}
\centering
\footnotesize
\begin{tabular}{|$r|^r^r^r^r^r^r|^r^r^r^r|}
  \hline
r & mean & median & sd & mad & skewness & medc. & \#sig. & X/Y & top 100 & p-value \\
  \hline
0 & 0.077 & 0.14 & 1.25 & 1.04 & -0.949 & -0.064 & 605 & 97 & 58 &  NA\\
  1 & 0.19 & 0.21 & 1.37 &  1.2 & -0.556 & -0.02 & 458 & 90 & 72 & 0.013 \\
  2 & 0.15 & 0.19 & 1.41 & 1.23 & -0.464 & -0.027 & 457 & 91 & 74 & 0.039 \\
  3 & 0.015 & 0.055 & 1.38 & 1.18 & -0.442 & -0.035 & 509 & 97 & 75 & 0.00096 \\
  4 & 0.045 & 0.065 & 1.27 & 1.03 & -0.661 & -0.018 & 608 & 101 & 78 & 5.2e-07 \\
  5 & 0.044 & 0.067 &  1.3 & 1.06 & -0.573 & -0.019 & 612 & 100 & 76 & 1.8e-06 \\
  7 & 0.071 & 0.088 & 1.34 & 1.11 & -0.527 & -0.0097 & 572 & 99 & 76 & 2.7e-06 \\
  10 & 0.024 & 0.057 & 1.39 & 1.15 & -0.539 & -0.025 & 658 & 100 & 75 & 5.3e-07 \\
  15 & 0.097 & 0.12 & 1.48 & 1.23 & -0.619 & -0.018 & 659 & 102 & 76 & 2.4e-08 \\
  20 & 0.051 & 0.072 & 1.48 & 1.24 & -0.628 & -0.015 & 625 & 102 & 76 & 6.5e-11 \\
  30 & 0.021 & 0.038 & 1.58 & 1.28 & -0.709 & -0.01 & 748 & 109 & 81 & 5.6e-13 \\
  \rowstyle{\bfseries}
  33 & 0.032 & 0.052 & 1.63 & 1.33 & -0.669 & -0.013 & 751 & 109 & 79 & 2.7e-12 \\
  40 & 0.027 & 0.052 & 1.75 & 1.44 & -0.544 & -0.017 & 846 & 111 & 78 & 6.3e-11 \\
  50 & 0.034 & 0.054 & 1.93 & 1.59 & -0.389 & -0.0088 & 954 & 117 & 76 & 1.3e-09 \\
   \hline
\end{tabular}
\caption{\small Supplementary Dataset ($n = 143$, $p = 54675$). This
  is  same as dataset 1 except the primary variable is gender instead
  of COPD severity.}
  \label{table:supp_copd}
\end{table}


==> revision 2/app_lem_ml.tex <==
% JS is editing



Here we prove uniform convergence of the estimated factors and noise
%%% changed noises to noise variances
variances based on the results of \citet{bai2012},
which are needed to prove
\Cref{thm:asymptotics-nc,thm:consistency-rr,thm:asymptotics-rr,cor:type-I}. In
the proof of the following lemma, we intensively
use some of the technical results in \citet{bai2012} and also modify
internal parts of their proof. Before reading the proof of
%%% interval -> internal
\Cref{lem:gamma-ml}, we recommend that the reader first
read the original proof in \citet{bai2012,bai2012supplement}. To help the readers to follow,
the variables $N$, $T$, $\Lambda$ (or $\Lambda^\star$) and $f$ (or $f^\star$)
in \citet{bai2012}
correspond to $p$, $n$, $\bm \Gamma^{(0)}$ and
$\tilde{\bm Z}^{(0)}$ in our notation. %Also, we want to remind that in \Cref{rmk:rotation}
%we have explained that though $\bm \Gamma^{(0)}$ is not uniformly bounded, the results in
%\citet{bai2012} will still hold.

\begin{lemma} \label{lem:gamma-ml}
  Under \Cref{assumption:error,assumption:bounded,assumption:large-factor},
%\begin{equation} \label{eq:sigma-consistent}
%|\hat{\sigma}_j^2 - \sigma_j^2| = O_p(n^{-\frac{1}{2}}),~j=1,\dotsc,p
%\end{equation}
%\begin{equation}\label{eq:gamma-err}
%|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}
%-\frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}|
% = \bm{o}_p(n^{-\frac{1}{2}}),~j=1,\cdots,p,
%\end{equation}
%\begin{equation}\label{eq:avg4-sigma-gamma-err}
%\frac{1}{p}\sum_{j=1}^p(\hat{\sigma}_j^2 - \sigma_j^2)^4 =
%O_p(n^{-1}),\quad
%\frac{1}{p} \sum_{j=1}^p\|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}\|_2^4
%= o_p(n^{-1}).
%\frac{1}{p} \sum_{j=1}^p \left|\frac{1}{\hat{\sigma}_j} -
 %   \frac{1}{\sigma_j}\right| \overset{p}{\to} 0
%\end{equation}
%\begin{equation}\label{eq:avg-gamma-err}
%\frac{1}{p} \sum_{j=1}^p\big\|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}
%-\frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\big\|_2^2
% = {o}_p(n^{-1}).
%\end{equation}
for any fixed index set
 $S$ with finite cardinality,
\begin{equation}\label{eq:gamma-asym}
\sqrt{n} (\hat{\bm{\Gamma}}_S - \bm{\Gamma}_S^{(0)}) \overset{d}{\to}
\mathrm{MN}(0, \bm{\Sigma}_S, \bm{I}_r)
\end{equation}
where $\bm{\Sigma}_S$ is the noise covariance matrix of the variables in $S$.
Further, if there exists $k > 0$ such that $p/n^{k} \to 0$ when $p \to \infty$, then
\begin{equation}\label{eq:max-sigma-err}
\max_{1 \le j \le p}|\hat{\sigma_j^2} - \sigma_j^2| =
O_p(\sqrt{\log p / n}),~
\max_{1 \le j \le p}|\hat{\bm \Gamma}_j - \bm\Gamma_j^{(0)}| = \bm O_p(\sqrt{\log p / n}), ~\mathrm{and}
\end{equation}
%\begin{equation}\label{eq:max-gamma}
%\max_{j = 1, 2,\cdots,p}|\hat{\bm \Gamma}_j| = \bm O_p(1), ~\mathrm{and}
%\end{equation}
%\begin{equation}\label{eq:avg-gamma-err}
%\frac{1}{p}\sum_{j=1}^p
%|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)} - \frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}
%|= \bm{o}_p(n^{-\frac{1}{2}})
%\end{equation}
\begin{equation}\label{eq:max-gamma-err}
\max_{j = 1, 2,\cdots,p} \Big|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}
-\frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\Big|
 = \bm{o}_p(n^{-\frac{1}{2}}).
\end{equation}
\end{lemma}

  \begin{remark} \label{rmk:rotation}
If we directly apply the results in \citet{bai2012} to prove \Cref{lem:ml-baili}, we
need uniform boundedness of $\bm{\Gamma}^{(0)}$ which is not always true. However, it is easy to show $\bm{R} \overset{a.s.}{\to}
\bm{I}_r$ by applying \citet[Lemma A.1]{bai2012}. Also, as $\bm{R}\bm{R}^T$ is the sample
%%% here $\Gamma\in\real^{r\times p}$ is of growing dimension.  We need
%%% some kind of uniform bound on it. It looks like Assumption 2 does it.
covariance matrix, the maximum entry of
$|\bm{R} - \bm{I}|$ is ${O}_p(n^{-1/2})$,
thus the maximum entry of
$|\bm{\Gamma}^{(0)} - \bm{\Gamma}| = |\bm{\Gamma}(\bm R - \bm I)|$ is also ${O}_p(n^{-1/2})$. As a
consequence, although $\bm{\Gamma}^{(0)}$ is not always uniformly bounded, all the results in
\citet{bai2012} still hold as we stated in \Cref{lem:ml-baili} and \Cref{lem:gamma-ml}.
%Finally, the variation of
%$\bm{\Gamma}^{(0)}$ is nonnegligible when considering the asymptotic
%distribution of $\sqrt{n} (\hat{\bm{\Gamma}}_j -
%\bm{\Gamma}_j)$. However, this variation is
%unimportant for estimating $\bm{\beta}$, as we only need a good estimator of the column space of $\bm{\Gamma}$.
\end{remark}


\begin{proof}

Our factor model corresponds to the IC3 identification condition in
\citet{bai2012}. Equation \eqref{eq:gamma-asym}
is an immediate consequence of \citet[Theorem 5.2]{bai2012}, except here we additionally consider the asymptotic
  covariance of $\sqrt{n} (\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)})$
  and $\sqrt{n} (\hat{\bm{\Gamma}}_k - \bm{\Gamma}_k^{(0)})$.
  %Equation
  %\eqref{eq:gamma-err} and the
  The asymptotic distribution of $\sqrt{n} (\hat{\bm{\Gamma}}_S -
  \bm{\Gamma}^{(0)}_S)$ immediately follows from equation (F.1) in
  \citet{bai2012supplement}:
\begin{equation} \label{eq:gamma-hat}
\sqrt{n-1} (\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}) =
\frac{1}{\sqrt{n-1}} \sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij} + \bm{o}_p(1).
\end{equation}
%Using \citet[Theorem 5.2]{bai2012} and boundedness of $\sigma_j$ and $\hat \sigma_j$, we can get
%the first equation of \eqref{eq:avg4-sigma-gamma-err}. The second equation
%of \eqref{eq:avg4-sigma-gamma-err} is proved in the last two lines of
%\citet[Supplement page 13]{bai2012}.

Now we prove \eqref{eq:max-sigma-err}.
Let $\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)} = \bm{b}_{1j} + \bm{b}_{2j} +\cdots + \bm{b}_{10,j}$
where
$\bm{b}_{kj}$ represents the $k$th term in the right hand side of
equation (A.14) in \citet{bai2012}.
Also, let  $\hat \sigma_j^2 - \sigma_j^2 = a_{1j} + a_{2j} +\cdots + a_{10,j}$ where
$a_{kj}$ represents the $k$th term in the right hand side of equation (B.9) in \citet{bai2012supplement}.
To bound each $\bm b_j$ and $a_j$ term, we extensively use Lemma C.1 of \citet{bai2012supplement}.
First, we give a clearer approximation to replace $(a)$ and $(c)$ in Lemma C.1 of \citet{bai2012supplement}:
\begin{equation}\label{eq:baiC1a}
\|\hat{\bm{H}}
\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
(\hat{\bm{\Gamma}} - \bm{\Gamma}^{(0)})\|_F = O_p(n^{-1}) +O_p(n^{-1/2}p^{-1/2})
\end{equation}
and
\begin{equation}\label{eq:baiC1e}
\frac{1}{n-1}\big\|\hat{\bm{H}}
\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
\tilde{\bm{E}}_{-1}^T\tilde{\bm{Z}}^{(0)}\big\|_F = O_p(n^{-1/2}p^{-1/2}) + O_p(n^{-1})
\end{equation}
where $\hat{\bm{H}} = (\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}\hat{\bm{\Gamma}})^{-1}$
and $\|\cdot\|_F$ is the Frobenius norm.
To show \eqref{eq:baiC1e}, one just needs to apply
$\hat {\bm H}_p = p\hat{\bm H} = \bm O_p(1)$ \citep[Corollary A.1]{bai2012},
%%% I can't find that Corollary in Bai and Li (2012)
\Cref{rmk:rotation} and $(n-1)^{-1}(\tilde {\bm Z}^{(0)}_{-1})^T\tilde {\bm Z}^{(0)}_{-1} = \bm I_r$
to simplify Lemma C.1(e) of \citet{bai2012supplement}. To prove \eqref{eq:baiC1a}, notice that under our conditions
(or the IC3 condition of \citet{bai2012}), the left hand side of (A.13) in
\citet{bai2012} is actually $\bm 0$ as the terms $\hat M_{ff}$ and $M_{ff}^\star$ in their notation are exactly $\bm I_r$.
Also, $\hat{\bm H}\hat{\bm \Gamma}^{(0)T}\hat {\bm \Sigma}^{-1}
 {\bm \Gamma}= \bm I_r + \bm o_p(1)$ from \citet[Corollary A.1]{bai2012}.
 Thus, \eqref{eq:baiC1a} holds by applying Lemma C.1 of \citet{bai2012supplement}.
 As a consequence, by applying \citet[Lemma C.1]{bai2012supplement}, \eqref{eq:baiC1a} and \eqref{eq:baiC1e},
 we now have $\max_j|\bm b_{kj}| = \bm o_p(n^{-1/2})$ for $k \neq 8, 10$ and
$\max_j|a_{kj}| = o_p(n^{-1/2})$ for $k \neq 1, 2, 8, 9, 10$. Using independence of the noise,
it's also easy to see that $\max_j|\bm b_{8j}| = O_p(\sqrt{\log p / n})$ and
$\max_j|a_{kj}| = O_p(\sqrt{\log p / n})$ for $k = 1, 10$.

Next, we show the following facts under the condition that $p/n^k \to 0$ when $p \to \infty$ for some $k > 0$.
Let
$(e_{ti})_{(n-1)\times p} = \tilde{\bm E}\bm{\Sigma}^{-1/2}$ denote a
random matrix whose entries are then i.i.d.\
$\mathrm{N}(0,1)$ variables. Then for each
$s = 1, 2, \cdots, r$,
\begin{equation}\label{eq:noise-fact}
  \max_{j = 1,2, \cdots, p}\frac{1}{(n-1)p}
  \Big|\sum_{i = 1}^p\Gamma_{is}\sum_{t = 1}^{n-1}
  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big| = o_p(n^{-1/2}),~\mathrm{and}
\end{equation}
%\begin{equation}\label{eq:noise-fact1}
%  \frac{1}{(n-1)^2p^2}\sum_{j = 1}^p
%  \sum_{i = 1}^p\Big(\sum_{t = 1}^{n-1}
%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big)^2 = O_p(n^{-1})
%\end{equation}
%If $n = \Omega(\log p\log\log p)$, then also
\begin{equation}\label{eq:noise-fact2}
  \max_{j = 1,2, \cdots, p}\frac{1}{(n-1)^2p}
  \sum_{i = 1}^p\Big(\sum_{t = 1}^{n-1}
  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big)^2 = o_p(n^{-1/2}).
\end{equation}
To prove \eqref{eq:noise-fact},
we only need to show
$\max_j\frac{1}{(n-1)p}
  \big|\sum_{i \neq j}\sum_{t = 1}^{n-1}
  \Gamma_{is}e_{ti}e_{tj}\big| = o_p(n^{-1/2})
$ as the remaining term is $o_p(n^{-1/2})$ because of the
independence. This approximation is proven by
the union bound and  boundedness of $\bm{\Gamma}$:
%and the fact that
%$\frac{1}{p}\|\bm{\Gamma}_{\cdot s}\|_2^2$ is bounded away from $0$ for large enough $p$:
for $\forall \epsilon > 0$
\begin{equation*}
\begin{split}
 &      \lim_{n,p\to \infty}\mathrm{P}\Big(\sqrt n\max_{j = 1,2,\cdots, p}\frac{1}{(n-1)p}
  \big|\sum_{i \neq j}\sum_{t = 1}^{n-1}
  \Gamma_{is}e_{ti}e_{tj}\big| > \epsilon\Big) \\
   \leq & \lim_{n,p\to \infty}2p \cdot \mathrm{P}\Big(\frac{\sqrt n D}{(n-1)p}
  \sum_{i \neq 1}\sum_{t = 1}^{n-1}e_{ti}e_{t1} > \epsilon\Big)\\
  = & \lim_{n,p\to \infty}2p \cdot \mathrm{P}\Bigg(\frac{\sqrt n}{n-1}\sum_{t = 1}^{n-1}e_{t1}
  \big(\frac{1}{\sqrt {p-1}}\sum_{i \neq 1}e_{ti}\big) >
  \frac{\epsilon}{D}\frac{p}{\sqrt{p-1}}\Bigg)\\
  \leq& \lim_{n,p\to \infty}2p \cdot \mathrm{E}\Bigg[\Big(\frac{\sqrt n}{n-1}\sum_{t = 1}^{n-1}e_{t1}
  \big(\frac{1}{\sqrt {p-1}}\sum_{i \neq 1}e_{ti}\big)\Big)^4\Bigg]/
  \Big(\frac{\epsilon}{D}\frac{p}{\sqrt{p-1}}\Big)^4 = 0
%  = & \lim_{p\to\infty}2p\Big(1 - \Phi\big(\epsilon_1 \frac{p}{\sqrt{p-1}}\big)\Big) = 0\\
\end{split}
\end{equation*}
%where $\epsilon_1$ are some positive constants.
%The last equation holds as for Gaussian distribution,
%$1 - \Phi(x) \leq \frac{\exp(-x^2/2)}{x\sqrt {2\pi}}$.
To see why the last equality holds,
$(p - 1)^{-1/2}\sum_{i \neq 1}e_{ti}\sim \mathrm{N}(0, 1)$
is independent from $e_{t1}$, thus the fourth moment of $(n-1)^{-1/2}\sum_{t = 1}^{n-1}e_{t1}
  \big((p-1)^{-1/2}\sum_{i \neq 1}e_{ti}\big)$ is bounded
  which enables us to use the Markov inequality.
% To prove \eqref{eq:noise-fact1}, one only need to notice the simple fact
% that  $\frac{1}{(n-1)^2}\big(\sum_{t = 1}^{n-1}
%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\big)$ has the same mean (say $\mu_0$) and
%  the same standard deviation (say $\sigma_0$), both of order $O_p(n^{-1})$, for each $i\neq j$.
%  Then the average of the $p^2 - p$ terms also has mean $\mu_0$ and standard deviation bounded
%  by $\sigma_0$, both of order $O_p(n^{-1})$.
To prove \eqref{eq:noise-fact2}, we start with the same union bound as for \eqref{eq:noise-fact},
\[
\begin{split}
   & \lim_{n,p\to \infty}\mathrm{P}\Big(\max_{j = 1,2,\cdots, p}\frac{1}{(n-1)^2p}
   \sum_{i \neq j}\big(\sum_{t = 1}^{n-1}e_{ti}e_{tj}\big)^2  >
   \epsilon\Big) \\
   \le & \lim_{n,p\to \infty} p \cdot \mathrm{P}\Big(\frac{1}{(n-1)^2p}
   \sum_{i=2}^p\big(\sum_{t = 1}^{n-1}e_{ti}e_{t1}\big)^2  >
   \epsilon\Big) \\
 %  = & \lim_{n,p\to \infty} p \cdot \mathrm{P}\Bigg(\frac{1}{p(n-1)}
%   \sum_{i=2}^p \Big(\frac{\bm{e}_{\cdot i}^T \bm{e}_{\cdot 1}}{\sqrt{n-1}} \Big)^2  >
%   \epsilon\Bigg) \\
   \le & \lim_{n,p\to \infty} 2p^2 \cdot \mathrm{P}\Big(\frac{1}{n-1}
   \sum_{t = 1}^{n-1}e_{t2}e_{t1}  >
   \sqrt\epsilon\Big)\\
   \le & \lim_{n,p\to \infty} 2p^2 \cdot
   \mathrm{E}\Big[\Big(\frac{1}{n-1}\sum_{t=1}^{n-1}e_{t2}e_{t1}\Big)^{4k}\Big]/\epsilon^{2k}\\
   \le & \lim_{n,p\to \infty} 2C/\epsilon^{2k}\cdot\big(p^2/n^{2k}\big) = 0\\
\end{split}
\]
where $C$ is some positive constant.
The second last inequality is due to Markov inequality and last inequality holds
as $e_{t_2}e_{t1}, t= 1, 2,\cdots n-1$ are independent and have finite moments of any order.
%holds as by checking the moment generating function,
%for any $t$, the variable $e_{t2}e_{t1}$ is a sub-exponential, thus we can
%use the Bernstein inequality to bound the tail probability.
The last limit holds when we assume $p/n^k \to 0$.

Equation \eqref{eq:noise-fact} directly implies that
\begin{equation*}
\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}{\bm{\Gamma}}_j
\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
= \bm{o}_p(n^{-1/2})
\end{equation*}
as $\hat{\bm H} = \bm O_p(p^{-1})$. Using \eqref{eq:noise-fact2} and
$p^{-1}\sum_j\|\hat{\bm \Gamma}_j - \bm\Gamma^{(0)}_j\|_2^2 = O_p(n^{-1})$ from \Cref{lem:ml-baili}, we get by
using the Cauchy-Schwartz inequality:
\begin{equation*}
\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}(\hat {\bm{\Gamma}}_j - \bm\Gamma_j^{(0)})
\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
= \bm{o}_p(n^{-1})
\end{equation*}
Similarly, combining with \Cref{rmk:rotation}, we get
\begin{equation*}
\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}({\bm{\Gamma}}_j^{(0)} - \bm\Gamma_j)
\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
= \bm{o}_p(n^{-1})
\end{equation*}
By writing $\hat{\bm{\Gamma}}_j = \bm{\Gamma}_j + \bm{\Gamma}_j^{(0)} - \bm{\Gamma}_j
+ \hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}$ and using boundedness of
both $\hat \sigma_j$ and $\sigma_j$,
\begin{equation}\label{eqn:B4-a}
 \max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
\sum_{i=1}^p\frac{1}{\hat\sigma_i^2}
\hat{\bm{\Gamma}}_j
\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
= \bm{o}_p(n^{-1/2})
\end{equation}
which indicates that $\max_j|a_{9j}| = o_p(n^{-1/2})$.

To bound the remaining terms, we use the fact that $\max_{j = 1, \cdots, p}|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$.
To see this, first notice that because of boundedness of $\hat \sigma_j$ and $\sigma_j$ and the fact that
 $\hat{\bm{H}} = \bm{O}_p(p^{-1})$, we have
 $\max_{j}|\bm{b}_{10,j}| = \bm O_p(p^{-1}\max_j{|\hat{\bm{\Gamma}}_j|})$. Combining the previous results, we have
$\max_{j}|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}|
 = \bm{O}_p(\sqrt{\log p / n}) +  \bm o_p(\max_j{|\hat{\bm{\Gamma}}_j|})$ which indicates
 that $\max_j|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$. Thus,
 $\max_j|a_{8j}| = o_p(\max_j|\hat\sigma_j^2 - \sigma_j^2|)$ is negligible
 and $\max_{j}|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}|
 = \bm{O}_p(\sqrt{\log p / n}) +  \bm o_p(\max_j|\hat \sigma_j^2 -
 \sigma_j^2|)$. The latter conclusion also indicates that $\max_j
 |a_{2j}| = \bm{O}_p(\sqrt{\log p / n}) +  \bm o_p(\max_j|\hat \sigma_j^2 -
 \sigma_j^2|)$. As a
 consequence, the second claim in \eqref{eq:max-sigma-err} holds.

Finally, To prove \eqref{eq:max-gamma-err},
we actually have already shown that
$\max_j|\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}-\bm{b}_{8j}| = \bm{o}_p(n^{-1/2})$.
Then,
\begin{equation*}
  \begin{split}
    &\max_{j = 1, 2, \cdots, p}\Big|\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)} -
  \frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\Big|\\
  \leq & \max_{j = 1, 2, \cdots, p}\Big|\hat {\bm{\Gamma}}_j -
  \bm{\Gamma}_j^{(0)} - \bm{b}_{8j}\Big| + \max_{j = 1, 2, \cdots, p}\Big|\bm{b}_{8j} -
  \frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\Big|\\
  \leq & \bm{o}_p(n^{-1/2}) + \|\hat{\bm{H}}
\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
(\hat{\bm{\Gamma}} - \bm{\Gamma}^{(0)})\|_F
\max_{j = 1, 2, \cdots, p}
\Big|\frac{1}{n-1}\sum_{i = 2}^n\tilde{\bm{Z}}_{i}^{(0)}\tilde
E_{ij}\Big| \\
=&
\bm{o}_p(n^{-1/2})
\end{split}
\end{equation*}
Thus, \eqref{eq:max-gamma-err} holds.

%%that
%%the term $\hat M_{ff}$ and $M_{ff}^\star$ in their notation is exactly $\bm I_r$ as we are in their IC3 condition.
%%We will show that the average of
%%the square $L_2$ norm of all the terms except $\bm b_{8j}$ has order
%%$o_p(n^{-1})$ and bound the difference between
%%$\bm b_{8j} = (n-1)^{-1}\hat {\bm H}\hat{\bm \Gamma}\hat{\bm \Sigma}^{-1}\bm{\Gamma}^{(0)}
%%\sum_{i = 2}^n\tilde{\bm Z}_i^{(0)}\tilde E_{ij}$ and
%%$(n-1)^{-1}\sum_{i = 2}^n \tilde {\bm{Z}}_i^{(0)}\tilde E_{ij}$.
%%
%%Directly applying Lemma C.1 of \citet{bai2012}, we get $p^{-1}\sum_{j=1}^p\|\bm{b}_{kj}\|_2^2 = o_p(n^{-1})$
%% for $k = 5, 6, 9$.
%% As $\hat {\bm H}_p = p\hat{\bm H} = \bm O_p(1)$ \citep[Corollary A.1]{bai2012}, the factor matrix $\bm \Gamma$
%% is bounded and $(n-1)^{-1}(\tilde {\bm Z}^{(0)}_{-1})^T\tilde {\bm Z}^{(0)}_{-1} = \bm I_r$,
%%we actually have
%%$(n-1)^{-1}\big\|\hat{\bm{H}}
%%\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
%%\tilde{\bm{E}}_{-1}^T\tilde{\bm{Z}}^{(0)}\big\|_F = O_p(n^{-1/2}p^{-1/2}) + O_p(n^{-1})
%% $ extended from  \citet[Lemma C.1(e)]{bai2012}, where $\|\cdot\|_F$ is the Frobenius norm. Thus,
%% $p^{-1}\sum_{j=1}^p\|\bm{b}_{kj}\|_2^2 = o_p(n^{-1})$
%% for $k = 3, 4, 7$ (as $\hat{\bm H}\hat{\bm \Gamma}^{(0)T}\hat {\bm \Sigma}^{-1}
%% {\bm \Gamma}= \bm I_r + \bm o_p(1)$ from \citet[Corollary A.1]{bai2012}).
%% Also, as we have mentioned, the left hand side of (A.13) in
%%\citet{bai2012} is actually $\bm 0$. By applying Lemma C.1 of \citet{bai2012} to (A.13)
%%in \citet{bai2012}, we get $\|\hat{\bm{H}}
%%\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
%%(\hat{\bm{\Gamma}} - \bm{\Gamma}^{(0)})\|_F = O_p(n^{-1}) +O_p(n^{-1/2}p^{-1/2})$.
%%Thus, $p^{-1}\sum_{j=1}^p\|\bm{b}_{kj}\|_2^2 = o_p(n^{-1})$
%% for $k = 1, 2$.
%% For the $10$th term, applying the
%% Cauchy-Schwartz inequality to $\sum_j\|\hat{\bm \Gamma}_j(\hat \sigma_j^2 - \sigma_j^2)/\hat \sigma_j^2\|_2$
%% and using Theorem 5.1 of \citet{bai2012}, we get
%%$p^{-1}\sum_{j=1}^p\|\bm{b}_{10,j}\|_2^2 = o_p(n^{-1})$. Finally,
%%$p^{-1}\sum_{j=1}^p\|\bm{b}_{8j} -
%%\frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\|_2^2
%%= o_p(n^{-1})$
%%because of the independency among $\tilde{E}_{ij}$. In conclusion, our
%%equation \eqref{eq:avg-gamma-err} holds.




%%Finally, we prove \eqref{eq:max-sigma-err}
%%and \eqref{eq:max-gamma-err} under the condition that $n \ge c \log
%%p\log\log p$ for some $c > 0$.
%%We first show the following facts. Let
%%$(e_{ti})_{(n-1)\times p} = \tilde{\bm E}\bm{\Sigma}^{-1/2}$ denote a
%%random matrix whose entries are then i.i.d.\
%%$\mathrm{N}(0,1)$ variables. Then for each
%%$s = 1, 2, \cdots, r$,
%%\begin{equation}\label{eq:noise-fact}
%%  \max_{j = 1,2, \cdots, p}\frac{1}{(n-1)p}
%%  \Big|\sum_{i = 1}^p\Gamma_{is}\sum_{t = 1}^{n-1}
%%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big| = o_p(n^{-1/2}),~\mathrm{and}
%%\end{equation}
%%%\begin{equation}\label{eq:noise-fact1}
%%%  \frac{1}{(n-1)^2p^2}\sum_{j = 1}^p
%%%  \sum_{i = 1}^p\Big(\sum_{t = 1}^{n-1}
%%%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big)^2 = O_p(n^{-1})
%%%\end{equation}
%%%If $n = \Omega(\log p\log\log p)$, then also
%%\begin{equation}\label{eq:noise-fact2}
%%  \max_{j = 1,2, \cdots, p}\frac{1}{(n-1)^2p}
%%  \sum_{i = 1}^p\Big(\sum_{t = 1}^{n-1}
%%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\Big)^2 = o_p(n^{-1/2}).
%%\end{equation}
%%To prove \eqref{eq:noise-fact},
%%we only need to show
%%$\max_j\frac{1}{(n-1)p}
%%  \big|\sum_{i \neq j}\sum_{t = 1}^{n-1}
%%  \Gamma_{is}e_{ti}e_{tj}\big| = o_p(n^{-1/2})
%%$ as the remaining term is $o_p(n^{-1/2})$ because of the
%%independence. This approximation is proven by
%%the union bound and  boundedness of $\bm{\Gamma}$:
%%%and the fact that
%%%$\frac{1}{p}\|\bm{\Gamma}_{\cdot s}\|_2^2$ is bounded away from $0$ for large enough $p$:
%%for $\forall \epsilon > 0$
%%\begin{equation*}
%%\begin{split}
%% &      \lim_{n,p\to \infty}\mathrm{P}\Big(\sqrt n\max_{j = 1,2,\cdots, p}\frac{1}{(n-1)p}
%%  \big|\sum_{i \neq j}\sum_{t = 1}^{n-1}
%%  \Gamma_{is}e_{ti}e_{tj}\big| > \epsilon\Big) \\
%%   \leq & \lim_{n,p\to \infty}2p \cdot \mathrm{P}\Big(\frac{\sqrt n D}{(n-1)p}
%%  \sum_{i \neq 1}\sum_{t = 1}^{n-1}e_{ti}e_{t1} > \epsilon\Big)\\
%%  = & \lim_{n,p\to \infty}2p \cdot \mathrm{P}\Bigg(\frac{\sqrt n}{n-1}\sum_{t = 1}^{n-1}e_{t1}
%%  \big(\frac{1}{\sqrt {p-1}}\sum_{i \neq 1}e_{ti}\big) >
%%  \frac{\epsilon}{D}\frac{p}{\sqrt{p-1}}\Bigg)\\
%%  \leq& \lim_{n,p\to \infty}2p \cdot \mathrm{E}\Bigg[\Big(\frac{\sqrt n}{n-1}\sum_{t = 1}^{n-1}e_{t1}
%%  \big(\frac{1}{\sqrt {p-1}}\sum_{i \neq 1}e_{ti}\big)\Big)^4\Bigg]/
%%  \Big(\frac{\epsilon}{D}\frac{p}{\sqrt{p-1}}\Big)^4 = 0
%%%  = & \lim_{p\to\infty}2p\Big(1 - \Phi\big(\epsilon_1 \frac{p}{\sqrt{p-1}}\big)\Big) = 0\\
%%\end{split}
%%\end{equation*}
%%%where $\epsilon_1$ are some positive constants.
%%%The last equation holds as for Gaussian distribution,
%%%$1 - \Phi(x) \leq \frac{\exp(-x^2/2)}{x\sqrt {2\pi}}$.
%%To see why the last equality holds,
%%$(p - 1)^{-1/2}\sum_{i \neq 1}e_{ti}\sim \mathrm{N}(0, 1)$
%%is independent from $e_{t1}$, thus the fourth moment of $(n-1)^{-1/2}\sum_{t = 1}^{n-1}e_{t1}
%%  \big((p-1)^{-1/2}\sum_{i \neq 1}e_{ti}\big)$ is bounded
%%  which enables us to use the Markov inequality.
%%% To prove \eqref{eq:noise-fact1}, one only need to notice the simple fact
%%% that  $\frac{1}{(n-1)^2}\big(\sum_{t = 1}^{n-1}
%%%  [e_{ti}e_{tj} - \mathrm{E}(e_{ti}e_{tj})]\big)$ has the same mean (say $\mu_0$) and
%%%  the same standard deviation (say $\sigma_0$), both of order $O_p(n^{-1})$, for each $i\neq j$.
%%%  Then the average of the $p^2 - p$ terms also has mean $\mu_0$ and standard deviation bounded
%%%  by $\sigma_0$, both of order $O_p(n^{-1})$.
%%To prove \eqref{eq:noise-fact2}, we start with the same union bound as for \eqref{eq:noise-fact},
%%\[
%%\begin{split}
%%   & \lim_{n,p\to \infty}\mathrm{P}\Big(\max_{j = 1,2,\cdots, p}\frac{1}{(n-1)^2p}
%%   \sum_{i \neq j}\big(\sum_{t = 1}^{n-1}e_{ti}e_{tj}\big)^2  >
%%   \epsilon\Big) \\
%%   \le & \lim_{n,p\to \infty} p \cdot \mathrm{P}\Big(\frac{1}{(n-1)^2p}
%%   \sum_{i=2}^p\big(\sum_{t = 1}^{n-1}e_{ti}e_{t1}\big)^2  >
%%   \epsilon\Big) \\
%% %  = & \lim_{n,p\to \infty} p \cdot \mathrm{P}\Bigg(\frac{1}{p(n-1)}
%%%   \sum_{i=2}^p \Big(\frac{\bm{e}_{\cdot i}^T \bm{e}_{\cdot 1}}{\sqrt{n-1}} \Big)^2  >
%%%   \epsilon\Bigg) \\
%%   \le & \lim_{n,p\to \infty} 2p^2 \cdot \mathrm{P}\Big(\frac{1}{n-1}
%%   \sum_{t = 1}^{n-1}e_{t2}e_{t1}  >
%%   \sqrt\epsilon\Big)\\
%%   \le & \lim_{n,p\to \infty} 2p^2 \exp(-n\epsilon_2) = 0\\
%%\end{split}
%%\]
%%where $\epsilon_2$ is some positive constant.
%%The last inequality holds as by checking the moment generating function,
%%for any $t$, the variable $e_{t2}e_{t1}$ is a sub-exponential, thus we can
%%use the Bernstein inequality to bound the tail probability. The last limit holds
%%when we assume $n \ge c \log p\log\log p$.
%For any fixed $\bm{e}_{\cdot 1}$, $\bm{e}_{\cdot i}^T
%\bm{e}_{\cdot 1} / \sqrt{n-1}$ is normally distributed with mean $0$ and variance
%$\|\bm{e}_{\cdot 1}\|^2 / (n-1)$. bycentral limit theorem,
%\[
%\frac{1}{\sqrt{2(p-1)}} \left[ \frac{n-1}{\|\bm{e}_{\cdot 1}\|^2} \sum_{i=2}^p \Big(\frac{\bm{e}_{\cdot i}^T
%\bm{e}_{\cdot 1}}{\sqrt{n-1}} \Big)^2 - (p-1) \right] \overset{d}{\to} \mathrm{N}(0,1)
%\]
%By using the concentration of $\|\bm{e}_{\cdot 1}\|^2 / (n-1)$, one
%can easily verify \eqref{eq:noise-fact2}.
% a similar trick. First, as $n/{(\log p)^2} >0$ when
%n, p \to \infty$, we only need to show that
% $$  \max_j\frac{1}{(n-1)p(\log p)^2}
% \sum_{i \neq j}\big(\sum_{t = 1}^{n-1}e_{ti}e_{tj}\big)^2 = o_p(1)$$
%  Using CLT again, we have
% that $\forall \epsilon > 0$
% \begin{equation*}
% \begin{split}
%   &  \lim_{n,p\to \infty}\mathrm{P}\Big(\max_{j = 1,2,\cdots, p}\frac{1}{(n-1)p(\log p)^2}
%   \sum_{i \neq j}\big(\sum_{t = 1}^{n-1}e_{ti}e_{tj}\big)^2  > \epsilon\Big) \\
%   \leq & \lim_{n,p\to \infty}p\mathrm{P}\Big(\frac{1}{(n-1)p(\log p)^2}
%   \sum_{i \neq 1}\big(\sum_{t = 1}^{n-1}e_{ti}e_{t1}\big)^2> \epsilon\Big)\\
%   \leq & \lim_{n,p\to \infty}p^2
%   \mathrm{P}\Big(\frac{1}{n-1}\big(\sum_{t = 1}^{n-1}e_{t2}e_{t1}\big)^2>
%   \epsilon (\log p)^2\Big)\\
%   = & \lim_{n,p\to \infty}2p^2\mathrm{P}
%   \Big(\frac{1}{\sqrt{n-1}}\sum_{t = 1}^{n-1}e_{t2}e_{t1}>
%   \sqrt{\epsilon}\log p\Big)\\
%   = & \lim_{p\to\infty}2p^2\Big[1 - \Phi\big(\epsilon_2 \log
%   p\big)\Big] \\
%   \leq & \lim_{p\to\infty}2p^2
%   \frac{\exp(-\epsilon_2^2(\log p)^2/2)}{\log p \sqrt{2\pi}} \\
%   = & \lim_{p\to\infty}2p^2
%   \frac{p^{-\epsilon_2^2\log p/2}}{\log p \sqrt{2\pi}} =  0 \\
% \end{split}
% \end{equation*}
% wher $\epsilon_2$ is some positive constant.
%%Equation \eqref{eq:noise-fact} directly implies that
%%\begin{equation*}
%%\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
%%\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}{\bm{\Gamma}}_j
%%\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
%%\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
%%= \bm{o}_p(n^{-1/2})
%%\end{equation*}
%%as $\hat{\bm H} = \bm O(p^{-1})$. Using \eqref{eq:noise-fact2} and
%%$p^{-1}\sum_j\|\hat{\bm \Gamma}_j - \bm\Gamma^{(0)}_j\|_2^2 = O_p(n^{-1})$ from \Cref{lem:ml-baili}, we get by
%%using Cauchy-Schwartz inequality:
%%\begin{equation*}
%%\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
%%\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}(\hat {\bm{\Gamma}}_j - \bm\Gamma_j^{(0)})
%%\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
%%\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
%%= \bm{o}_p(n^{-1})
%%\end{equation*}
%%Similarly, combining with \Cref{rmk:rotation}, we get
%%\begin{equation*}
%%\max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
%%\sum_{i=1}^p\frac{1}{\sigma_i\sigma_j}({\bm{\Gamma}}_j^{(0)} - \bm\Gamma_j)
%%\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
%%\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
%%= \bm{o}_p(n^{-1})
%%\end{equation*}
%%By writing $\hat{\bm{\Gamma}}_j = \bm{\Gamma}_j + \bm{\Gamma}_j^{(0)} - \bm{\Gamma}_j
%%+ \hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}$ and using boundedness of
%%both $\hat \sigma_j$ and $\sigma_j$,
%%%\begin{equation}\label{eqn:B4-a-avg}
%%% \frac{1}{p}\sum_{j=1}^p\Big|\hat{\bm{H}}\big(
%%%\sum_{i=1}^p\frac{1}{\hat\sigma_i^2}
%%%\hat{\bm{\Gamma}}_j
%%%\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
%%%\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
%%%= \bm{o}_p(n^{-1/2})
%%%\end{equation}
%%%If $n = \Omega(\log p\log\log p)$, then also
%%\begin{equation}\label{eqn:B4-a}
%% \max_{j = 1, \cdots, p}\Big|\hat{\bm{H}}\big(
%%\sum_{i=1}^p\frac{1}{\hat\sigma_i^2}
%%\hat{\bm{\Gamma}}_j
%%\frac{1}{n-1}\sum_{t = 2}^n[\tilde E_{ti}\tilde E_{tj} -
%%\mathrm{E}(\tilde E_{ti}\tilde E_{tj})]\big)\Big|
%%= \bm{o}_p(n^{-1/2})
%%\end{equation}
%where $\hat{\bm{H}} = (\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}\hat{\bm{\Gamma}})^{-1}$.

%Next, we prove \eqref{eq:avg-sigma-err}.
%Let $\hat \sigma_j^2 - \sigma_j^2 = a_{1j} + a_{2j} +\cdots + a_{10,j}$ where
%$a_{kj}$ represents the $k$th term in the right hand side of \citep[(B.9)]{bai2012}.
%Notice that for \citep[lem. C.1. (e)]{bai2012}, under their IC3 condition, we actually have
%$\big\|\hat{\bm{H}}
%\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}\frac{1}{n-1}
%\tilde{\bm{E}}_{-1}^T\tilde{\bm{Z}}^{(0)}\big\|_F = O_p(n^{-1/2}p^{-1/2}) + O_p(n^{-1})
% $. Then, using \citep[Lem. C.1]{bai2012}, \Cref{rmk:rotation},
%boundedness of $\bm{\Gamma}$ and \eqref{eqn:B4-a-avg}, we have
% $\max_j|a_{kj}| = o_p(n^{-1/2})$ thus $\frac{1}{p}\sum_{j=1}^p|a_{kj}| = o_p(n^{-1/2})$
% for $k \neq 1, 2, 8, 10$. Using independency and \citep[lem. C.1. (a)]{bai2012}, we get
% $\frac{1}{p}\sum_{j=1}^p|a_{kj}| = o_p(n^{-1/2})$ for $k = 1, 10$. Using
% \citep[thm. 5.1.]{bai2012} and Cauchy-Schwartz inequality, we get
%$\frac{1}{p}\sum_{j=1}^p|a_{kj}| = o_p(n^{-1/2})$ for $k = 2, 8$.
%Thus, the first equation in \eqref{eq:avg-sigma-err} holds; the second
%equation of \eqref{eq:avg-sigma-err} is just an immediate corrolary.

%Then we prove \eqref{eq:avg-gamma-err}.
%let $\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)} = \bm{b}_{1j} + \bm{b}_{2j} +\cdots + \bm{b}_{10,j}$
%where
%$\bm{b}_{kj}$ represents the $k$th term in the right hand side of \citep[(A.14)]{bai2012}.
%Notice that under the IC3 condition of \citep{bai2012}, the left hand side of
%\citep[(A.13)]{bai2012} is $0$,
%by applying \citep[lem.C.1.]{bai2012}, we get
%$\|\hat{\bm{H}}
%\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
%(\hat{\bm{\Gamma}} - \bm{\Gamma}^{(0)})\|_F = O_p(n^{-1}) +O_p(n^{-1/2}p^{-1/2})$
%where  $\|\cdot\|_F$ is the Frobenius norm.
%Thus, using \citep[thm.5.1 and lem.C.1.]{bai2012}, \Cref{rmk:rotation},
%boundedness of $\bm{\Gamma}$ and \eqref{eqn:B4-a-avg},
%we get $\max_j|\bm{b}_{kj}| = \bm{o}_p(n^{-1/2})$ thus
%$\frac{1}{p}\sum_{j=1}^p|\bm{b}_{kj}| = \bm{o}_p(n^{-1/2})$
% for $k \neq 8, 10$. Again, using
% \citep[thm. 5.1.]{bai2012} and Cauchy-Schwartz inequality, we get
%$\frac{1}{p}\sum_{j=1}^p|\bm{b}_{10,j}| = \bm{o}_p(n^{-1/2})$. As
%$\frac{1}{p}\sum_{j=1}^p|\bm{b}_{8j} -
%\frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}| = \bm{o}_p(n^{-1/2})$,
%\eqref{eq:avg-gamma-err} holds.

%Finally, we prove \eqref{eq:max-sigma-err} and \eqref{eq:max-gamma-err} with the
%additional assumption that $n = \Omega(\log p\log\log p)$.
%%Next, we prove \eqref{eq:max-sigma-err}.
%%First, $\max_{j = 1, \cdots, p}|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$. To see this,
%%using \eqref{eqn:B4-a} and \citet[Lemma C.1]{bai2012}, we have already got
%% $\max_{j}|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j|
%% = \bm{o}_p(n^{-1/2}) + \max_{j}|\bm{b}_{8j}| + \max_{j}|\bm{b}_{10,j}|$.
%% Also, because of the independence of the noise, it's easy to see that $\max_{j}|\bm{b}_{8j}| = o_p(1)$. In addition,
%% because of boundedness of $\hat \sigma_j$ and $\sigma_j$ and the fact that
%% $\hat{\bm{H}} = \bm{O}_p(p^{-1})$, we get
%% $\max_{j}|\bm{b}_{10,j}| = o_p(\max_j{|\hat{\bm{\Gamma}}_j|})$.
%% %As $\bm{b}_{10,j} = \frac{\hat\sigma_j - \sigma_j^2}{\hat\sigma_j^2}\hat{\bm{H}}\hat{\bm{\Gamma}}_j$, $\hat{\bm{H}} = \bm{O}_p(p^{-1})$ \citep[Corollary A.1. (b)]{bai2012} and
%% Thus, equation $\max_{j = 1, \cdots, p}|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$ holds.
%%Then, to prove \eqref{eq:max-sigma-err},
%%let $\hat \sigma_j^2 - \sigma_j^2 = a_{1j} + a_{2j} +\cdots + a_{10,j}$ where
%%$a_{kj}$ represents the $k$th term in the right hand side of equation (B.9) in \citet{bai2012}.
%%Notice that using Lemma C.1 of \citet{bai2012} and \eqref{eqn:B4-a} we have already got
%%$\max_j|a_{kj}| = o_p(n^{-1/2})$ for $k \neq 1, 2, 8, 10$.
%%For the tenth term, as
%% $\max_j|(n-1)^{-1}\sum_{i = 2}^n\tilde{\bm{Z}}_{i}^{(0)}\tilde E_{ij}| = \bm{o}_p(1)$,
%% we get $\max_j|a_{10,j}| = o_p(n^{-1/2})$.
%%For the eighth term,  $\max_j|a_{8j}| = o_p(\max_j|\hat\sigma_j^2 - \sigma_j^2|)$
%%by using $\max_j|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$.
%%Because of boundedness of $\sigma_j$ and independence of $\tilde{E}_{tj}$, we get
%%$\max_j|a_{1j}| = o_p(1)$.
%%Finally, using $\max_j|\hat{\bm{\Gamma}}_j| = \bm{O}_p(1)$, we get
%%$\max_j|a_{2j}| = o_p(\max_j|\hat\sigma_j^2 - \sigma_j^2|) + o_p(1)$.
%%Thus, \eqref{eq:max-sigma-err} holds.
%%To prove \eqref{eq:max-gamma-err},
%%using \eqref{eq:max-sigma-err},
%%we actually have already shown that
%%$\max_j|\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}-\bm{b}_{8j}| = \bm{o}_p(n^{-1/2})$.
%%Then,
%%\begin{equation*}
%%  \begin{split}
%%    &\max_{j = 1, 2, \cdots, p}\Big|\hat {\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)} -
%%  \frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\Big|\\
%%  \leq & \max_{j = 1, 2, \cdots, p}\Big|\hat {\bm{\Gamma}}_j -
%%  \bm{\Gamma}_j^{(0)} - \bm{b}_{8j}\Big| + \max_{j = 1, 2, \cdots, p}\Big|\bm{b}_{8j} -
%%  \frac{1}{n-1}\sum_{i=2}^n \tilde{\bm{Z}}_i^{(0)} \tilde{E}_{ij}\Big|\\
%%  \leq & \bm{o}_p(n^{-1/2}) + \|\hat{\bm{H}}
%%\hat{\bm{\Gamma}}^T\hat{\bm{\Sigma}}^{-1}
%%(\hat{\bm{\Gamma}} - \bm{\Gamma}^{(0)})\|_F
%%\max_{j = 1, 2, \cdots, p}
%%\Big|\frac{1}{n-1}\sum_{i = 2}^n\tilde{\bm{Z}}_{i}^{(0)}\tilde E_{ij}\Big| =
%%\bm{o}_p(n^{-1/2})
%%\end{split}
%%\end{equation*}
%%Thus, \eqref{eq:max-gamma-err} holds.
\end{proof}


==> revision 2/app_lem_multiple.tex <==

First, note that by the strong law of large numbers
$\frac{1}{n}
\begin{pmatrix}
  \bm{X}_0 & \bm{X}_1 \\
\end{pmatrix}^T
\begin{pmatrix}
  \bm{X}_0 & \bm{X}_1 \\
\end{pmatrix}
\overset{a.s.}{\to} \bm{\Sigma}_{\bm{X}}$. Using the
QR decomposition of
$
\begin{pmatrix}
  \bm{X}_0 & \bm{X}_1 \\
\end{pmatrix} = \bm{Q} \bm{U}
$ and writing $\bm{U} =
\begin{pmatrix}
  \bm{V} \\
  \bm{0} \\
\end{pmatrix}
$ and $\bm{V} =
\begin{pmatrix}
  \bm{U}_{00} & \bm{U}_{01} \\
  \bm{0} & \bm{U}_{11} \\
\end{pmatrix}
$,
it's clear that $\frac{1}{n} \bm{V}^T \bm{V}
\overset{a.s.}{\rightarrow} \bm{\Sigma}_{\bm{X}}$.
Since $\bm{\Sigma}_{\bm{X}}$ is nonsingular, both
$\bm{U}_{00}$ and $\bm{U}_{11}$ are full rank
square matrices with probability $1$. Thus using the block matrix inversion formula, we have
$\bm{V}^{-1} =
\begin{pmatrix}
  \star & \star \\
    \bm{0} & \bm{U}_{11}^{- 1}
\end{pmatrix}$ where $\star$ represents some $d_0 \times d_0$ or $d_0
\times d_1$ matrix.
Therefore the right bottom block of $n \bm{V}^{-1} \bm{V}^{-T}$
is $n \bm{U}_{11}^{-1} \bm{U}_{11}^{-T}$ and converges to
$\bm{\Omega}_{11}$ almost surely.


==> revision 2/app_lem_rr.tex <==
By using the representation of $\hat{\bm{\Gamma}}$ in
\eqref{eq:gamma-hat},
%and (C.4) in \citep{bai2012}.
%  \begin{equation*}
%    \label{eq:eq:sigma-hat}
%    \hat{\sigma}_j^2 = \frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
%    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}}),
%  \end{equation*}
we have
\[
\begin{split}
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) =& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
    \hat{\bm{\Gamma}}_j^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
/ \|\bm{X}\|_2 + \bm{\Gamma}_j^{(0)T} \bm{\alpha}^{(0)} - (\hat{\bm{\Gamma}}_j)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j\\
\end{split}
\]
where $\max_j|\delta_j| = o_p(1)$ and
$\max_j|\epsilon_j| = o_p(n^{-1/2})$ from
%\eqref{eq:avg-sigma-err}
%\Cref{lem:ml-baili}
\Cref{lem:gamma-ml}.
%and equation \eqref{eq:avg-gamma-err}.
Because
$\|\bm{\beta}\|_1 \sqrt{n} / p \to 0$ and $\psi'$ is bounded,
\[
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) = \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j + \bm{o}_p(n^{-1/2})
\]

Let $g_j$ be the expression inside $\psi$ in the last equation omitting $\epsilon_j$ and $\delta_j$. Conditionally on
$\tilde{\bm{Z}}_{-1}^{(0)}$, the variables $g_j, \mathrm{where}~ j=1,\dotsc,p$ are independent and
identically distributed with $\mathrm{E}(g_j) = 0$ and
$g_j = O_p (n^{-1/2}) $.
%Using the Cauchy-Schwartz inequality,
%$p^{-1}\sum_{j = 1}^p(\delta_jg_j)^2 = o_p(n^{-1})$.
Thus, using \Cref{assumption:psi-2nd-derivative}
and boundedness of $\hat \sigma_j$,
\[
\begin{split}
 & \Big\| \frac{1}{p} \sum_{j=1}^p \Big[\psi\Big(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\Big)
 - \psi(g_j)\Big]\hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 \\
\leq & D^2 \cdot \Big\| \frac{1}{p} \sum_{j=1}^p\big(|\epsilon_j| |\hat{\bm{\Gamma}}_j|+ |g_j|
|\delta_j\hat{\bm{\Gamma}}_j|\big) /\hat \sigma_j
%\big(|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}| + |\bm{\Gamma}_j^{(0)}|\big)/\hat \sigma_j
\Big\|_2  = o_p(n^{-1/2})
\end{split}
\]
%where the last approximation is got by using Cauchy-Schwartz inequality and \Cref{lem:ml-baili}.
%where $t_j$ are
%i.i.d. normal random variables by noticing $\tilde{\bm{Z}}_{-1}^{(0)}
%\bm{\alpha}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R} \bm{R}^T)^{-1}
%(\bm{\alpha} + \bm{u}/\|\bm{X}\|_2)$ and $\bm{R} \bm{R}^T \to \bm{I}_r$.
%Because for some $W'$ between $0$ and $W$ and
%$\psi(0) = 0$, $\psi(g_j) = \psi'(0) (n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}}))$ if $\beta_j =0$.


We can further use the facts that
$\psi(g_j)=\psi'(0) g_j +
o_p(n^{-1/2}) = O_p(n^{-1/2})$ and
%Cauchy-Schwartz inequality in a similar way and combine
$\psi(g_j) - \psi'(0)g_j$
are i.i.d., and combine \Cref{rmk:rotation} and \Cref{lem:gamma-ml} to get:
\[
\begin{split}
\left\|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right\|_2 &= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi(g_j)\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
%O_p(n^{-\frac{1}{2}}p^{-\frac{1}{2}}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi'(0)g_j\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
&=o_p(n^{-\frac{1}{2}})+ o_p(n^{-\frac{1}{2}})
= o_p(n^{-\frac{1}{2}})
\end{split}
\]


Similarly,
%$\psi$ is assumed to be bounded $|\psi(g_j)| \le C$ in
%\Cref{assumption:rho}. Therefore, by
because $\lim_{p \to \infty}
\frac{1}{p} \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ exists and is
positive definite (in \Cref{assumption:large-factor}),
we use \Cref{assumption:psi-2nd-derivative} and the uniform convergence
of $\hat {\bm \Sigma}$ and $\hat{\bm \Gamma}$ in \Cref{lem:gamma-ml} to get
\[
\begin{split}
  \left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1} &=
\Bigg[\frac{1}{p} \sum_{j=1}^p
  \psi'\left(g_j + \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right)
\hat{\bm{\Gamma}}_j \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
&= \Bigg[\frac{1}{p} \sum_{j = 1}^p
  \psi'\left(0\right)
  \bm{\Gamma}_j^{(0)} \bm{\Gamma}_j^{(0)T} / \sigma_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(\beta_j) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 \right]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(0) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \frac{1}{p} \sum_{\beta_j
%    \ne 0}
%  (\psi'(\beta_j) - \psi'(0)) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2  \right]^{-1} \\
&\overset{p}{\to} \Big[ \psi'(0) \frac{1}{p} \sum_{j=1}^p
  \bm{\Gamma}_j \bm{\Gamma}_j^T / \sigma_j^2 \Big]^{-1}
\end{split}
\]
%The last probability limit follows from $\hat{\bm{\Gamma}}
%\overset{p}{\to} \bm{\Gamma}$, $\hat{\bm{\sigma}}_j
%\overset{p}{\to} \sigma_j$ and $\psi'$, $\bm{\Gamma}$ and $\bm{\Sigma}$ are bounded.
This means that all the eigenvalues of
$\left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1}$ converge to finite constants.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> revision 2/app_lem_weak.tex <==
Denote the SVD of $\bm \Gamma$ as $\bm{\Gamma} = \tilde{\bm \Gamma}\bm{D}$ 
where $\tilde{\bm\Gamma}^T\tilde{\bm\Gamma} = \bm{I}_r$
and $\tilde{\bm{\Gamma}} = \begin{pmatrix} \tilde{\bm{\Gamma}}_{\cdot
    1}& \tilde{\bm{\Gamma}}_{\cdot 2} & \cdots &
\tilde{\bm{\Gamma}}_{\cdot r} \end{pmatrix}$. 
Also, assume that the sample covariance matrix of
$\tilde{\bm{Y}}_{-1}$
has eigen decomposition $\bm{S} = \hat{\tilde{\bm{\Gamma}}}^T\hat{\bm{D}}^2\hat{\tilde{\bm{\Gamma}}}$
and $\hat {\bm{\Gamma}} = \hat{\tilde{\bm \Gamma}}\hat{\bm D}$ where 
$\hat{\bm{D}} = \mathrm{diag}(\hat d_1, \cdots, \hat d_{\hat r})$. 
Finally, expand $\tilde{\bm \Gamma}$ as 
$\tilde{\bm{\Gamma}}^* = \begin{pmatrix}\tilde{\bm\Gamma} &\tilde{\bm{\Gamma}}^C\end{pmatrix}$ so that
$\tilde{\bm{\Gamma}}^*$ is a $p \times p$ orthogonal matrix.
To prove \Cref{lem:weak-gamma}, we first prove the following lemma 
which characterize the eigenvalues and eigenvectors of PCA 
based on \citet{baik2006} and \citet{paul2007}.

\begin{lemma}\label{lem:app-weak}
  The esitmated eigenvalues satisfy 
  $\hat d_k^2 - d_k^2 = O_p(1)$ for $k = 1, 2, \cdots, \hat r$.
 For each $k = 1, 2, \cdots, \hat r$, the estimated eigenvectors 
 $\hat {\tilde {\bm \Gamma}}_{\cdot k}$ can be decomposed as 
 \begin{equation}\label{eq:pca-eigenvector}
\hat{\tilde{\bm{\Gamma}}}_{\cdot k} = \sum_{h = 1}^{r}\theta_{hk}\tilde{\bm{\Gamma}}_{\cdot h} +
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\tilde{\bm{\Gamma}}^C
\frac{\bm{z}_k}{\|\bm{z}_k\|_2},~k=1,2,\dotsc,\hat r,
\end{equation}
where  $\bm{\theta}_k = (\theta_{1k}, \cdots, \theta_{rk})$ 
   and $\bm{z}_k \sim \mathrm{N}(\bm{0}, \bm{I}_{p - r})$. 
 Also, $\|\bm{\theta}_k\|_2 \independent \bm{z}_k$. 
 Finally, for $k = 1, 2, \cdots, s$, then $1 - \|\bm{\theta}_k\|_2^2 = O_p(p^{-1})$.
 \end{lemma}

 \begin{proof}
   Notice that in our notation, for $i > 1$, the column covariance satisfies that 
   $\var(\tilde{\bm Y}_{i\cdot}) = \tilde{\bm\Gamma}\bm \Lambda \tilde{\bm\Gamma}^T$ 
   where $\bm\Lambda  = \diag(d_1^2 + 1, \cdots, d_r^2 + 1, 1, \cdots,1 )$.
   Thus, using \citet[Theorem 1.1 and Theorem 1.2]{baik2006},  if 
   $d_k^2 \geq \sqrt \gamma$, 
$$\hat d_k^2 - d_k^2 = \gamma + 1 - \frac{\gamma}{d_k^2} + o_p(1) = O_p(1)$$ 
On the other hand, for $d_k^2 \leq \sqrt \gamma$, 
we have $|\hat d_k^2 - d_k^2| \leq |\hat d_k^2| + |d_k^2| = O_p(1)$.

 To prove \eqref{eq:pca-eigenvector}, as $\tilde{\bm \Gamma}^\star$ form an orthogonal 
 basis of $\real^p$ and $\hat {\tilde {\bm \Gamma}}_{\cdot k}$ is a unit vector, 
 we can decompose it as $\hat {\tilde {\bm \Gamma}}_{\cdot k} = 
 \sum_{h = 1}^{r}\theta_{hk}\tilde{\bm{\Gamma}}_{\cdot h}
 + \sum_{h' = r+1}^{p}\theta_{h'k}\tilde{\bm{\Gamma}}^C_{\cdot h'}$ 
 where $\sum_{h = 1}^p\theta_{hk}^2 = 1$. Using \citet[Theorem 6]{paul2007}, we get that 
 $(\theta_{(r+1)k}, \cdots, \theta_{pk})/\sqrt{ 1 - \|\bm \theta_k\|^2_2}$ is distributed 
 uniformly on the unit sphere $\mathbb{S}^{p - r - 1}$ and is independent of 
 $\|\bm \theta_k\|_2$ (Though is \citet{paul2007} it's assumed that $\gamma < 1$, 
 Theorem $6$ is an non-asymptotic result which holds for any $n$ and $p$). Thus, 
\eqref{eq:pca-eigenvector} holds with $\bm{z}_k \sim \mathrm{N}(\bm{0}, \bm{I}_{p - r})$ 
and $\|\bm{\theta}_k\|_2 \independent \bm{z}_k$. 

Finally, we use \citet[Equation (18)]{paul2007} which holds for any $n$ and $p$:
$$ \frac{1}{\|\bm \theta_k\|_2^2} = 
\bm a_k^T\big[\bm I_{p - r} + \bm \Lambda_r^{1/2} \bm T_1^T
  (\hat d_k^2 \bm I - \bm {\Lambda}^\star)^{-1}
 \bm \Lambda^\star 
 (\hat d_k^2 \bm I_{p - r} - \bm {\Lambda}^\star)^{-1}
\bm T_1 \bm \Lambda_r^{1/2} \big]\bm a_k 
$$
where $\bm a_k = \bm \theta_k/\|\bm \theta_k\|_2$, 
$\bm \Lambda_r = \diag(d_1^2 + 1, \cdots, d_r^2 + 1)$. $\bm T_1$ is a 
$\min(p - r, n) \times r$ random 
matrix whose entries are i.i.d. $\mathrm{N}(0, 1/n)$ variables. 
$\bm \Lambda^\star$ are the 
eigenvalues of $\bm T_2^T \bm T_2$ where $\bm T_2$ is independent of $\bm T_1$ and is 
a $\min(p-r, n) \times \min(p-r, n)$ random matrix whose entries are i.i.d. 
$\mathrm{N}(0, 1)$. As a consequence of Marchenko-Pastur law, the largest eigenvalue of 
$\bm \Lambda^\star$ is $O(1)$. For $k = 1, 2, \cdots, s$, as $d_k^2 = O(p)$, we also have 
$\hat d_k^2 = O(p)$. Also, as 
$\bm T_1^T \bm T_1 = \bm I_r$, the largest eigenvalue of 
$\bm T_1^T
  (\hat d_k^2 \bm I - \bm {\Lambda}^\star)^{-1}
 \bm \Lambda^\star 
 (\hat d_k^2 \bm I_{p - r} - \bm {\Lambda}^\star)^{-1}
\bm T_1$ is in the order of $O(1/\hat d_k^4) = O(p^{-1})$. As $\bm a_k$ is a unit vector 
and the largest eigenvalue of $\bm \Lambda_r$ is $O(\sqrt p)$, we have that 
$$\frac{1}{\|\bm \theta_k\|_2^2} - 1 = O(p^{-1})$$
which indicates that $1 - \|\bm{\theta}_k\|_2^2 = O_p(p^{-1})$.
 \end{proof}

Now we continue to prove \Cref{lem:weak-gamma}. Rewrite \eqref{eq:pca-eigenvector} as 
%By \Cref{assumption:weak-factor}, we have $\tilde \Gamma_{jk} = \Gamma_{jk}/d_k = o(1)$
%for each $j$ and $k$. Combing with the fact that $\hat d_k = d_k + o(1)$, we have
\begin{equation*}
%\begin{split}
\hat{{{\Gamma}}}_{jk} - \Gamma_{jk} = \hat d_k\sum_{h = 1}^{r}\theta_{hk}\tilde{{\Gamma}}_{jh}
-\Gamma_{jk}+
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k
%&= d_k(\sum_{h = 1}^{r}\theta_{hk}\tilde{{\Gamma}}_{jh}
%-\tilde\Gamma_{jk})+
%(1 - \|\bm{\theta}_k\|_2^2)\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k + o_p(1).\\
%\end{split}
\end{equation*}
For the weak factors $k = s+1, \cdots, r$, using \Cref{assumption:weak-factor}, we have $\max_j|\Gamma_jk| = o(1)$. 
As $d_k = O(1)$, we also have $\max_j|\tilde \Gamma_jk| = o(1)$. Using \Cref{lem:app-weak}, also $\hat d_k = O_p(1)$.
As the components of $\bm z_k$ are i.i.d. Gaussian 
variables and each $\|\tilde {\bm \Gamma}_{j\cdot}^C\| \leq 1$, we 
have that $\max_j|\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k| \leq \max_j|z_{jk}| = O(\sqrt {\log n})$. Thus, 
it's easy to see that $\max_j|\hat \Gamma_{jk} - \Gamma_{jk}| = o_p(1)$.

For the strong factors $k = 1, 2, \cdots, s$, we further decompose as 
$$
\hat{\Gamma}_{jk} - \Gamma_{jk} = d_k(\sum_{h = 1}^{r}\theta_{hk}\tilde{\Gamma}_{jh}
-\tilde\Gamma_{jk}) +
\sqrt{1 - \|\bm{\theta}_k\|_2^2}\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k 
+ (\hat d_k - d_k)\sum_{h = 1}^r \theta_{hk}\tilde{\Gamma}_{jh}
$$
Using \Cref{assumption:weak-factor}, we have $\max_j|\tilde \Gamma_jk|$

We will show that each term of the right hand side of the above equation is $o_p(1)$.
First, using the facts that $\|\bm{z}_k\|_2/\sqrt p = O_p(1)$, $\hat d_k - d_k = O_p(1)$,
$1 - \|\bm\theta_{k}\|_2^2 = o_p(1)$ if $d_k^2 \to \infty$ and $d_k^2/p = O(1)$, we get that
$\big(1 - \|\bm{\theta}_k\|_2^2\big)\frac{\hat d_k}{\|\bm{z}_k\|_2} =
o_p(1)$ whether or not
$d_k$ is finite. Also, by definition
each $\|\tilde{\bm{\Gamma}}_{\cdot i}^C\|_2 \leq 1$, thus
$\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k = O_p(1)$.
These results indicate that $(1 - \|\bm{\theta}_k\|_2^2)\frac{\hat d_k}{\|\bm{z}_k\|_2}\tilde{\bm{\Gamma}}_{j\cdot}^C\cdot\bm{z}_k = o_p(1)$.
Next, when $h \neq k$, using \Cref{assumption:weak-factor},
$d_k\tilde \Gamma_{jh} = \frac{d_k}{\sqrt p}\frac{\sqrt p}{d_h}\Gamma_{jh} = O(1)$. As $\theta_{hk} = o_p(1)$,
we get $d_k\sum_{h \neq k}\theta_{hk}\tilde{{\Gamma}}_{jh} = o_p(1)$. Finally,
$d_k(\theta_{kk}-1)\tilde \Gamma_{jk} = \frac{d_k}{\sqrt p}\frac{\sqrt p}{d_k}\Gamma_{jk}(\theta_{kk}-1) = o_p(1)$.
Combining all the above results, we get that $\hat{{{\Gamma}}}_{jk} - \Gamma_{jk} = o_p(1)$, thus \eqref{eq:pca}
holds.

%Now we prove \eqref{eq:avg-pca}.
%First, notice that using the Cauchy-Schwarz inequality,
%$\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\tilde \Gamma_{jk}\big| \le \big(\sum_{j = 1}^p\tilde{\Gamma}_{jk}^2\big)^{1/2} = 1$
%and similarly $\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\hat{\tilde{\Gamma}}_{jk}\big| \le  1$.
%For factor $k$ of strength $d_k^2 \to \infty$, as
%$\langle \tilde{\bm{\Gamma}}_{\cdot k}, \hat{\tilde{\bm{\Gamma}}}_{\cdot k}\rangle
%= \theta_{kk} \to 1$ and both of them are unit vectors,
% $\big\|\hat{\tilde{\bm{\Gamma}}}_{\cdot k} -
%{\tilde{\bm{\Gamma}}}_{\cdot k}\big\|_2 =
%o_p(1)$. Using the Cauchy-Schwarz inequality
%$\frac{1}{\sqrt p}\sum_{j = 1}^p\big|\hat{\tilde \Gamma}_{jk} - \tilde \Gamma_{jk}\big|
%\le \big\|\hat{\tilde{\bm{\Gamma}}}_{\cdot k} -
%{\tilde{\bm{\Gamma}}}_{\cdot k} \big\|_2$, we get
%\[
%\frac{1}{p}\sum_{j=1}^p\left|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}\right|
%\leq \frac{1}{p}\sum_{j=1}^p\Big(|\hat{\tilde{{\Gamma}}}_{jk} - \tilde{{\Gamma}}_{jk}||\hat{{d}}_k|
%+ |\tilde{{\Gamma}}_{jk}||\hat{{d}}_k-{d}_k|\Big) = o_p(1)
%\]
%For factor $k$ whose $d_k^2=O(1)$, we directly get
%\[
%\frac{1}{p}\sum_{j=1}^p\left|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}\right|
%\leq \frac{1}{p}\sum_{j=1}^p\Big(|\hat{\tilde{{\Gamma}}}_{jk}| +| \tilde{{\Gamma}}_{jk}||\hat{{d}}_k|
%+ |\tilde{{\Gamma}}_{jk}||\hat{{d}}_k-{d}_k|\Big) = o_p(1)
%\]
%Thus, \eqref{eq:avg-pca} holds.
%Finally, as $\mathrm{corr}(\hat{\bm \Gamma}_{\cdot k_1}, \bm \Gamma_{\cdot k_2}) =
%\mathrm{corr}(\hat{\tilde{\bm \Gamma}}_{\cdot k_1}, \tilde{\bm \Gamma}_{\cdot k_2})$,
%\eqref{eq:angle-pca} is just a consequence of \eqref{eq:pca-eigenvector} and
%\citet[Theorems 4 and 5]{paul2007}.

%To avoid confusion, we use $\bm{\alpha}^*$ to represent the true $\bm{\alpha}$,
%and use $\bm{\alpha}$ to represent a variable in $\mathbb{R}^{r^{(0)}}$.
% Using \Cref{assumption:weak-factor,assumption:bound-alpha}, \Cref{lem:weak-gamma}
% and the fact that $\|\bm{X}\|_2/\sqrt n \to 1$,
% \Cref{thm:consistency-weak} will be a direct consequence of consistent
% $\hat{\bm{\alpha}}_{(S)}^{\mathrm{RR}}$, which is proved in the
% following lemma.



% \begin{proof}
%   Let $m_n = \min_{\bm{\alpha}_0 \in \Omega} \sum_{j=1}^p
%   \rho \Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Big)$. Using \Cref{assumption:rho}, we have $m_n \geq 0$. First, as $\rho$ has
%   bounded derivative, it is a Lipschitz function. Also as
%   $\|\bm{X}\|_2/\sqrt n \overset{a.s.}{\to} 1$ and $\|\bm{\beta}\|_1/p \to 0$,
%   \begin{equation*}
% \begin{split}
%   \sum_{j=1}^p
% \rho \Bigg( \frac{\tilde{Y}_{1j} /\|\bm{X}\|_2
% -\hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Bigg)
% &= \frac{1}{p} \sum_{j=1}^p \rho\Bigg(  \frac{ \beta_j + \bm{\Gamma}_j^T
%   \bm{\alpha} - \hat{\bm{\Gamma}}_j^T
% \bm{\alpha}_0}{\hat{\sigma}}\Bigg) + o_p(1) \\
% &= \frac{1}{p} \sum_{j=1}^p \rho\Bigg(  \frac{\bm{\Gamma}_j^T
%   \bm{\alpha} - \hat{\bm{\Gamma}}_j^T
% \bm{\alpha}_0}{\hat{\sigma}}\Bigg) + o_p(1)
% \end{split}
% \end{equation*}
% Then, notice that for $\bm{\alpha}_0 \in \Omega$
% \begin{equation*}
%   \begin{split}
%     & \bm{\Gamma}_j^T\bm{\alpha} - \hat{\bm{\Gamma}}_j^T\bm{\alpha}_0\\
%     =& \hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)})+
% (\bm{\Gamma}_j^{(S)} - \hat{\bm{\Gamma}}_j^{(S)})^T\bm{\alpha}_{(S)}
% + \bm{\Gamma}_j^{(W)T}\bm{\alpha}_{(W)} - \hat{\bm{\Gamma}}_j^{(W)T}\bm{\alpha}_{0(W)}\\
% =& \hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)}) + o_p(1)
% \end{split}
% \end{equation*}
% Using \Cref{lem:weak-gamma}, for $\bm{\alpha}_0 \in \Omega$,
% \[
%  \sum_{j=1}^p
% \rho \Bigg( \frac{\tilde{Y}_{1j} /\|\bm{X}\|_2
% -\hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\Bigg)
% = \frac{1}{p}\sum_{j = 1}^p\rho
% \Bigg(\frac{\hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \bm{\alpha}_{0(S)})}
% {\hat \sigma}\Bigg)
%   + o_p(1)
% \]
% and the $o_p(1)$ term doesn't depend on $\bm{\alpha}_0$. Thus, $m_n = o_p(1)$, which
% indicates that
% \begin{equation} \label{eq:rho-op1}
%   \tilde\rho(\bm{\alpha}_{(S)} -
%   \hat{\bm{\alpha}}_{(S)}) = \frac{1}{p}\sum_{j = 1}^p\rho
%   \Bigg(\frac{\hat{\bm{\Gamma}}_j^{(S)T}(\bm{\alpha}_{(S)} - \hat{\bm{\alpha}}_{(S)})}
% {\hat \sigma}\Bigg)  = {o}_p(1)
% \end{equation}
% On the other hand, similar to \eqref{eq:consistency-key}, we show that for
% sufficiently small $\epsilon > 0$, there exists $\tau > 0$ such that
% \begin{equation} \label{eq:consistency-weak-key}
% \mathrm{P} \Big( \inf_{\|\bm{\alpha}_1\|_2 \ge \epsilon} \tilde \rho(\bm{\alpha}_1) > \tau \Big)
% \to 1.
% \end{equation}



% \end{proof}


==> revision 2/app_simu_figs.tex <==
\begin{figure}[hp]
  \centering
   \includegraphics[width = \textwidth]{plots/sim_strong05.pdf}
  \caption{Compare the performance of nine different approaches when the variance of
    $\bm{X}$ explained by the confounding factors is $5\%$.   The error bars are one
  standard deviation over $100$ repeated simulations. The
  three dashed horizontal lines from bottom to top are the nominal significance level, FDR level,
 oracle power and the precision of the smallest $100$ p-values, respectively.}
  \label{fig:p-5000-methods05}
\end{figure}

\begin{figure}[hp]
  \centering
   \includegraphics[width = \textwidth]{plots/sim_strong00.pdf}
  \caption{Compare the performance of nine different approaches when latent factors are
   unconfounding.   The error bars are one
  standard deviation over $100$ repeated simulations. The
  three dashed horizontal lines from bottom to top are the nominal significance level, FDR level,
 oracle power and the precision of the smallest $100$ p-values, respectively.}
  \label{fig:p-5000-methods05}
\end{figure}


==> revision 2/app_test.tex <==
We begin with a lemma regarding the test statistics.

\begin{lemma}
\label{lem:test-statistic-uniform}
The test statistics \eqref{eq:test-statistic} can be written as $t_j =
z_j + v_j$ for $j\in\mathcal{N}_p$, where $z_{j}, j\in\mathcal{N}_p$ are independent standard normal variables
and $v_j, j\in\mathcal{N}_p$ satisfy $\max_{1 \le j \le p} |v_j| =
o_p(1)$.
\end{lemma}
\begin{proof}
  We first prove this lemma for the RR estimator
  $\hat{\beta}^{\mathrm{RR}}$ and the corresponding test
  statistics. Let
\[
z_j = \frac{\tilde{E}_{1j} +\frac{1}{\sqrt{n-1}}\sum_{i=2}^n
  \tilde{E}_{ij} (\tilde{\bm{Z}}_i^{(0)})^T \bm{\alpha}}{\sigma_j \sqrt{1 +
    \|\bm{\alpha}\|^2}}.
\]
It is easy to verify that $z_j$ i.i.d.\ $\sim \mathrm{N}(0,1),~j=1,\dotsc,p$.
By using the expression of
  $\hat{\bm{\beta}}^{\mathrm{RR}}$ in \eqref{eq:beta-expand}, we can show
  for $j \in \mathcal{N}$ (so $\beta_j = 0$), that
\[
\begin{split}
&\max_{j \in \mathcal{N}_p}\left|\|\bm{X}\|_2 \hat{\beta}_j - \sigma_j \sqrt{1 +
    \|\bm{\alpha}\|^2} z_j\right| \\
=&\max_{j \in \mathcal{N}_p}\left|\|\bm{X}\|_2 \hat{\beta}_j - \left[\tilde{E}_{1j} +\frac{1}{\sqrt{n-1}}\sum_{i=2}^n
  \tilde{E}_{ij} (\tilde{\bm{Z}}_i^{(0)})^T \bm{\alpha}\right]\right| \\
=& \max_{j \in \mathcal{N}_p} \left|
\|\bm{X}\|_2 (\bm{\Gamma}_j^{(0)} - \hat{\bm{\Gamma}}_j)^T
\hat{\bm{\alpha}} - \frac{1}{\sqrt{n-1}}\sum_{i=2}^n
  \tilde{E}_{ij} (\tilde{\bm{Z}}_i^{(0)})^T \bm{\alpha} + r_j \right| \\
=& o_p(1),
\end{split}
\]
where $r_j =  \hat{\bm{\Gamma}}_j^T \left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm{o}_p(1) \right]^{-1}
\|\bm{X}\|_2 \bm{\Psi}_p(\bm{\alpha}^{(0)})$. The last step is due to
the uniform convergence of $\hat{\bm{\Gamma}}_j$ in
\eqref{eq:max-gamma-err} and \Cref{lem:asymptotics-rr-bound} to
uniformly control $r_j$. Now we can show, by using the uniform
convergence rate of $\hat{\sigma}^2$, that
\[
\begin{split}
\max_{j \in \mathcal{N}_p} |v_j|  =& \max_{j \in \mathcal{N}_p} \left|\frac{\|\bm{X}\|_2\hat{\beta}_j}{\hat{\sigma}_j \sqrt{1 +
    \|\hat{\bm{\alpha}}\|^2}} - z_j\right| \\
 =& \max_{j \in \mathcal{N}_p} \frac{\left|\|\bm{X}\|_2\hat{\beta}_j - \hat{\sigma}_j \sqrt{1 +
    \|\hat{\bm{\alpha}}\|^2 } z_j \right|}{\hat{\sigma}_j \sqrt{1 +
    \|\hat{\bm{\alpha}}\|^2}} \\
=& O_p\left(\max_{j \in \mathcal{N}_p}\left|\|\bm{X}\|_2\hat{\beta}_j - \hat{\sigma}_j \sqrt{1 +
    \|\hat{\bm{\alpha}}\|^2 } z_j \right|\right) \\
\le& O_p\left(\max_{j \in \mathcal{N}_p}\left|\|\bm{X}\|_2 \hat{\beta}_j - \sigma_j \sqrt{1 +
    \|\bm{\alpha}\|^2} z_j \right| \right) \\ &+ O_p\left(\max_{j \in
  \mathcal{N}_p}\left| \hat{\sigma}_j \sqrt{1 +
    \|\hat{\bm{\alpha}}\|^2} z_j - \sigma_j \sqrt{1 +
    \|\bm{\alpha}\|^2} z_j   \right| \right) \\
=&o_p(1).
\end{split}
\]
For the negative control estimator, the same argument holds
by noticing the $\bm{o}_p(1)$ term in
\eqref{eq:beta-nc-asymptotics-intermediate} is also uniform over $j$ (similar to $r_j$).
\end{proof}

To prove the first conclusion in \Cref{cor:type-I}, we
show the left hand side of \eqref{eq:type-I} has expectation
converging to $\alpha$ and variance converging to zero. For the expectation, for
  any $\epsilon > 0$,
\[
\begin{split}
\frac{1}{|\mathcal{N}_p|} \sum_{j \in \mathcal{N}_p} \mathrm{P}(|t_j| >
z_{\alpha/2})
&\le \frac{1}{|\mathcal{N}_p|} \sum_{j \in \mathcal{N}_p}
\mathrm{P}(|z_j| > z_{\alpha/2} - \epsilon) + \mathrm{P}(|v_j| >
\epsilon) \\
& = 2 (1 - \mathrm{\Phi}(z_{\alpha/2} - \epsilon)) +
\frac{1}{|\mathcal{N}_p|} \sum_{j \in \mathcal{N}_p} \mathrm{P}(|v_j| >
\epsilon) \\
& \le 2 (1 - \mathrm{\Phi}(z_{\alpha/2} - \epsilon)) +
\mathrm{P}(\max_{1 \le j \le p} |v_j| > \epsilon) \\
& \to 2 (1 - \mathrm{\Phi}(z_{\alpha/2} - \epsilon)).
\end{split}
\]
Similarly, one can prove $\lim_{n,p \to \infty}\frac{1}{|\mathcal{N}_p|} \sum_{j \in
  \mathcal{N}_p} \mathrm{P}(|t_j| > z_{\alpha/2}) \ge 2
(1 - \mathrm{\Phi}(z_{\alpha/2} + \epsilon))$ for any $\epsilon > 0$. Thus
the expectation converges to $\alpha$ when $n,p \to \infty$.

For the variance, we compute the second moment of the left hand side
of \eqref{eq:type-I}: for any $\epsilon > 0$,
\[
\begin{split}
&\frac{1}{|\mathcal{N}_p|^2} \sum_{j,k \in \mathcal{N}_p} \mathrm{P}(|t_j| >
z_{\alpha/2}, |t_k| > z_{\alpha / 2}) \\
=& \frac{1}{|\mathcal{N}_p|^2} \sum_{j \in \mathcal{N}_p} \mathrm{P}(|t_j| >
z_{\alpha/2}) + \frac{1}{|\mathcal{N}_p|^2} \sum_{j,k \in
  \mathcal{N}_p, j \ne k} \mathrm{P}(|t_j| > z_{\alpha/2}, |t_k| > z_{\alpha / 2}) \\
\le& \frac{1}{|\mathcal{N}_p|} \left[2 (1 - \mathrm{\Phi}(z_{\alpha/2} - \epsilon)) +
\mathrm{P}(\max_{1 \le j \le p} |v_j| > \epsilon) \right] \\
&+ \frac{1}{|\mathcal{N}_p|^2} \sum_{j,k \in
  \mathcal{N}_p, j \ne k} \mathrm{P}(|z_j| > z_{\alpha/2} -
\epsilon,|z_k| > z_{\alpha/2} - \epsilon) \\
&+ \mathrm{P}(|v_j| >
\epsilon) + \mathrm{P}(|v_k| > \epsilon) \\
= & \frac{1}{|\mathcal{N}_p|^2} \sum_{j,k \in
  \mathcal{N}_p, j \ne k} \mathrm{P}(|z_j| > z_{\alpha/2} -
\epsilon,|z_k| > z_{\alpha/2} - \epsilon) + o(1) \\
= & \frac{|\mathcal{N}_p|-1}{|\mathcal{N}_p|} [2 (1 - \mathrm{\Phi}(z_{\alpha/2}
- \epsilon))]^2 + o(1) \\
\to & 4[1 - \mathrm{\Phi}(z_{\alpha/2}
- \epsilon)]^2
\end{split}
\]
Similarly we can prove the lower bound of the second moment. In
conclusion, the second moment converges to $\alpha^2$, hence the
variance of \eqref{eq:type-I} converges to $0$.

To prove the second conclusion in \Cref{cor:type-I}, we begin with
\[
\begin{split}
&\mathrm{P}\Big(\sum_{j \in \mathcal{N}_p} I(|t_j| > \mathrm{\Phi}^{-1}(1 - \alpha/(2p))) \ge
  1\Big) \\
=& \mathrm{P}\Big(\max_{j \in \mathcal{N}_p} |t_j|
  >\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) \Big) \\
=& \mathrm{P}\Big(\max_{j \in \mathcal{N}_p} |z_j + v_j|
  >\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) \Big) \\
\le & \mathrm{P}\Big(\max_{j \in \mathcal{N}_p} |z_j|
  >\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) - \max_{j \in \mathcal{N}_p}
  |v_j| \Big) \\
\le & \mathrm{P}\Big(\max_{1 \le j \le p} |z_j|
  >\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) - \max_{j \in \mathcal{N}_p}
  |v_j| \Big) \\
\end{split}
\]
The conclusion \eqref{eq:fwer} then follows from $\mathrm{P}\Big(\max_{1 \le j \le p} |z_j|
  >\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) \Big) \le \alpha$ (the validity
  of Bonferroni for i.i.d.\ normals), the fact that
  $\mathrm{\Phi}^{-1}(1 - \alpha/(2p)) \to \infty$ as $p \to \infty$,
  and the result in \Cref{lem:test-statistic-uniform} that $\max_{j
    \in \mathcal{N}_p} |v_j| = o_p(1)$.

==> revision 2/app_thm_multiple.tex <==
First, for the known zero indices scenario,
$\hat{\bm{\Alpha}}_1^{\mathrm{NC}}$ has the following formula, which is similar to
\eqref{eq:alpha-nc}:
\begin{equation}\label{eq:alpha-nc-ext}
\hat{\bm{\Alpha}}_1^{\mathrm{NC}} = (\hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_{\mathcal{C}}^{-1}
  \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_{\mathcal{C}}^{-1}
  \tilde{\bm{Y}}_{1,\mathcal{C}}^T \bm{U}_{11}^{-T}
\end{equation}
which implies a similar formula as \eqref{eq:beta-nc-asymptotics-intermediate}:
\begin{equation}
\label{eq:beta-nc-asymptotics-intermediate-ext}
\begin{split}
\sqrt{n} (\hat{\bm{\Beta}}^{\mathrm{NC}}_{1,S} -
\bm{\Beta}_{1,S}) =& \sqrt n\tilde{\bm{E}}_{1,S}^T\bm{U}_{11}^{-T}  -
\sqrt n\cdot\bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T  \bm{\Sigma}_\mathcal{C}^{-1}
\bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1} \tilde{\bm{E}}_{1,C}^T\bm{U}_{11}^{-T} \\
  +& \sqrt{n} \cdot (\bm{\Gamma}_{S}^{(0)}  -
\hat{\bm{\Gamma}}_{S} ) {\bm{\Alpha}}_1^{(0)} \\
  +& \sqrt{n} \cdot \bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T
  \bm{\Sigma}_\mathcal{C}^{-1}  \bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
  (\hat{\bm{\Gamma}}_{\mathcal{C}}  -  \bm{\Gamma}_{\mathcal{C}}^{(0)})
  {\bm{\Alpha}}_1^{(0)} + \bm{o}_p(1),
\end{split}
\end{equation}
where ${\bm{\Alpha}}_1^{(0)} = \bm{R}^{-1}(\bm{A}_1 + \bm{\mathrm{U}}\bm{U}_{11}^{-T})$.
Following
the proof of \Cref{thm:asymptotics-nc} by using \Cref{lem:part-asym}, we get
\eqref{eq:nc-asym-ext}.

For the unknown zero indices scenario, \Cref{lem:part-asym} guarantees the consistency of
each column of $\hat{\bm{\Alpha}}_1^{\mathrm{RR}}$ by using \Cref{thm:consistency-rr}.
Then the Taylor expansion used in the proof of \Cref{thm:asymptotics-rr}
still works at each column of $\bm{\Alpha}_1^{(0)}$. Similar to \eqref{eq:beta-expand},
we get
\begin{equation} \label{eq:beta-expand-ext}
\begin{split}
\sqrt{n}(\hat{\bm{\Beta}}_1^{\mathrm{RR}} - \bm{\Beta}_1) =&
  \sqrt{n} \tilde{\bm{E}}_1^T\bm{U}_{11}^{-T}
+ \sqrt{n} (\bm{\Gamma}^{(0)} -\hat{\bm{\Gamma}})
\hat{\bm{\Alpha}}_1^{\mathrm{RR}} \\
&+ \hat{\bm{\Gamma}}
\begin{pmatrix}\bm{g}_1 & \bm{g}_2 & \cdots & \bm{g}_{d_1}\end{pmatrix}
\end{split}
\end{equation}
where $ \bm{g}_i = \left[ \nabla
\bm{\Psi}_p(\bm{\Alpha}_{1, i}^{(0)}) \right]^{-1}
(\sqrt{n} \bm{\Psi}_p\big(\bm{\Alpha}_{1, i}^{(0)}) + \bm{o}_p(1)\big)$.
Following the proof of \Cref{thm:asymptotics-rr}, we get each $\bm{g}_i = \bm{o}_p(1)$.
Thus
$$
\sqrt{n}(\hat{\bm{\Beta}}_1^{\mathrm{RR}} - \bm{\Beta}_1) =
  \sqrt{n} \tilde{\bm{E}}_1^T\bm{U}_{11}^{-T}
+ \sqrt{n} \cdot(\bm{\Gamma}^{(0)} -\hat{\bm{\Gamma}})
\hat{\bm{\Alpha}}_1^{\mathrm{RR}} + \bm{o}_p(1)
$$
and \eqref{eq:rr-asym-ext} holds.

%Using \Cref{lem:part-asym}, the proof is
%essentially the same as the proof for \Cref{thm:asymptotics-rr} by
%writing everything in the matrix form and substituting $\|\bm{X}\|_2$ by
%$\bm{U}_{11}$.


==> revision 2/app_thm_nc.tex <==
First, note that by the strong law of large numbers $n^{-1/2}\|\bm{X}\|_2 =
\sqrt{n^{-1}\sum_{i=1}^n X_i^2} \overset{a.s.}{\to} 1$, and $$\bm{R}
\bm{R}^T = (n-1)^{-1} \tilde{\bm{Z}}_{-1}^T \tilde{\bm{Z}}_{-1} \overset{a.s.}{\to}
\bm{I}_r.$$ Indeed one can show that $\bm{R} \overset{a.s.}{\to} \bm{I}_r$
by applying \citet[Lemma A.1]{bai2012}. We proceed to prove our theorem by
showing the conclusion holds for any fixed $\bm{u}$ and fixed
sequences $\{\bm{X}^{(n)}\}_{n=1}^{\infty}$ and
$\{\bm{R}^{(n,p)}\}_{n=1,p=1}^{\infty}$ such that
$\|\bm{X}^{(n)}\|_2/\sqrt{n} \to 1$ and $\bm{R}^{(n,p)}
\to \bm{I}_r$ as $n,p \to \infty$. For brevity we
will write $\bm{X}$ and $\bm{R}$
instead of $\bm{X}^{(n)}$ and $\bm{R}^{(n,p)}$ for the rest of this proof.

Plugging \eqref{eq:y-tilde-1-separate} in the estimator
\eqref{eq:alpha-nc} and \eqref{eq:beta-nc}, we obtain
%   \[
% \begin{split}
%   \hat{\bm{\beta}}^{\mathrm{NC}}_{-C} =& \tilde{\bm{Y}}_{1,-C}^T / \| \bm{X} \|_2 -
%   \hat{\bm{\Gamma}}_{-C}  (\hat{\bm{\Gamma}}_{C}^T \hat{\bm{\Sigma}}^{-1}
%   \hat{\bm{\Gamma}}_{C})^{-1} \hat{\bm{\Gamma}}_{C}^T \hat{\bm{\Sigma}}^{-1}
%   \tilde{\bm{Y}}_{1,C}^T / \| \bm{X} \|_2 \\
%   =& \bm{\beta}_{-C} + \bm{\Gamma}_{-C}^{(0)} \bm{\alpha}^{(0)} +
%   \tilde{\bm{E}}^T_{1,-C} / \|\bm{X}\|_2 \\ &- \hat{\bm{\Gamma}}_{-C}
%   (\hat{\bm{\Gamma}}_{C}^T \hat{\bm{\Sigma}}^{-1}
%   \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}^{-1}
%   (\bm{\Gamma}_{\mathcal{C}}^{(0)} \bm{\alpha}^{(0)} + \tilde{\bm{E}}^T_{1,C} / \|\bm{X}\|_2).
% \end{split}
% \]
% Therefore
\[
\begin{split}
\sqrt{n} (\hat{\bm{\beta}}^{\mathrm{NC}}_{-\mathcal{C}} -
\bm{\beta}_{-\mathcal{C}}) =& \frac{\sqrt{n}}{\|\bm{X}\|_2}
(\tilde{\bm{E}}^T_{1,-\mathcal{C}} - \hat{\bm{\Gamma}}_{-\mathcal{C}}
(\hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1}
  \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1} \tilde{\bm{E}}^T_{1,\mathcal{C}}) \\
  +& \sqrt{n} \cdot (\bm{\Gamma}_{-\mathcal{C}}^{(0)}  -
  \hat{\bm{\Gamma}}_{-\mathcal{C}} ) \bm{\alpha}^{(0)} \\
  +& \sqrt{n} \cdot \hat{\bm{\Gamma}}_{-\mathcal{C}} (\hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1}
  \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}^T
  \hat{\bm{\Sigma}}_\mathcal{C}^{-1} (\hat{\bm{\Gamma}}_{\mathcal{C}}  -  \bm{\Gamma}_{\mathcal{C}}^{(0)}) \bm{\alpha}^{(0)}.
\end{split}
\]
As $n,p \to \infty$,
$\sqrt{n}/\|\bm{X}\|_2 \overset{a.s.}{\to} 1$.
Also, as $p/n^k \to 0$ for some $k > 0$, using
\Cref{lem:gamma-ml} and \Cref{rmk:rotation}, both $\hat{\bm \Sigma}$ and $\hat{\bm \Gamma}$ has
entrywise uniform convergence in probability to $\bm \Sigma$ and $\bm \Gamma$.
Using
\Cref{assumption:nc-factor}, we get
\begin{equation}
\begin{split} \label{eq:nc-facts}
\Big(\frac{1}{|\mathcal{C}|}\hat{\bm{\Gamma}}_{
  \mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}\Big)^{-1}=&
 \Big(\frac{1}{|\mathcal{C}|}\bm{\Gamma}_{
  \mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}\bm{\Gamma}_{\mathcal{C}}\Big)^{-1} + \bm o_p(1)\\
\frac{1}{|\mathcal{C}|}\hat{\bm{\Gamma}}_{\mathcal{C}}^T
  \hat{\bm{\Sigma}}_\mathcal{C}^{-1}\tilde{\bm{E}}^T_{1,\mathcal{C}} =&
 \frac{1}{|\mathcal{C}|}\bm{\Gamma}_{\mathcal{C}}^T
  \bm{\Sigma}_\mathcal{C}^{-1}\tilde{\bm{E}}^T_{1,\mathcal{C}} + \bm o_p(1)\\
\frac{1}{|\mathcal{C}|}\hat{\bm{\Gamma}}_{\mathcal{C}}^T
  \hat{\bm{\Sigma}}_\mathcal{C}^{-1}\big(\sqrt n(\hat{\bm{\Gamma}}_{\mathcal{C}} - \bm{\Gamma}_{\mathcal{C}}^{(0)})\big)
  = &
 \frac{1}{|\mathcal{C}|}\bm{\Gamma}_{\mathcal{C}}^T
  \bm{\Sigma}_\mathcal{C}^{-1}\big(\sqrt n(\hat{\bm{\Gamma}}_{\mathcal{C}} - \bm{\Gamma}_{\mathcal{C}}^{(0)})\big)
  + \bm o_p(1)
  \end{split}
\end{equation}
%\[
%\begin{split}
%\hat{\bm{\Gamma}}_{S} (\hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1}
%  \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1} \hat{\bm{\Gamma}}_{\mathcal{C}}^T
%  \hat{\bm{\Sigma}}_\mathcal{C}^{-1}
%  &=\hat{\bm{\Gamma}}_{S} \Big(\frac{1}{|\mathcal{C}|}\hat{\bm{\Gamma}}_{
%  \mathcal{C}}^T \hat{\bm{\Sigma}}_\mathcal{C}^{-1}
%  \hat{\bm{\Gamma}}_{\mathcal{C}}\Big)^{-1} \frac{1}{|\mathcal{C}|}\hat{\bm{\Gamma}}_{\mathcal{C}}^T
%  \hat{\bm{\Sigma}}_\mathcal{C}^{-1}\\
%  &=
%\bm{\Gamma}_{S}^{(0)} [(\bm{\Gamma}_{\mathcal{C}}^{(0)})^T \bm{\Sigma}_\mathcal{C}^{-1}
%  \bm{\Gamma}_{\mathcal{C}}^{(0)}]^{-1} (\bm{\Gamma}_{\mathcal{C}}^{(0)})^T
%  \bm{\Sigma}_\mathcal{C}^{-1} + \bm{o}_p(1)\\ &=
%  \bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
%  \bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
%  + \bm{o}_p(1).
%\end{split}.
%\]
which implies
\begin{equation}
\label{eq:beta-nc-asymptotics-intermediate}
\begin{split}
\sqrt{n} (\hat{\bm{\beta}}^{\mathrm{NC}}_{S} -
\bm{\beta}_{S}) =& \tilde{\bm{E}}^T_{1,S}  -
\bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T  \bm{\Sigma}_\mathcal{C}^{-1}
\bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1} \tilde{\bm{E}}^T_{1,\mathcal{C}} \\
  +& \sqrt{n} \cdot (\bm{\Gamma}_{S}^{(0)}  -
  \hat{\bm{\Gamma}}_{S} ) \bm{\alpha}^{(0)} \\
  +& \sqrt{n} \cdot \bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T
  \bm{\Sigma}_\mathcal{C}^{-1}  \bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
  (\hat{\bm{\Gamma}}_{\mathcal{C}}  -  \bm{\Gamma}_{\mathcal{C}}^{(0)}) \bm{\alpha}^{(0)} + \bm{o}_p(1).
\end{split}
\end{equation}
Note that $\tilde{\bm{E}}_1 \independent \hat{\bm{\Gamma}}$, $\tilde{\bm{E}}_{1,\mathcal{C}}
\independent \tilde{\bm{E}}_{1,S}$, and $\sqrt{n} (\hat{\bm{\Gamma}}_S -
\bm{\Gamma}^{(0)}_S) \overset{d}{\to} \mathrm{N}(0, \bm{\Sigma}_S \otimes
\bm{I}_r)$, the four main terms on the right hand side of
\eqref{eq:beta-nc-asymptotics-intermediate} are (asymptotically)
uncorrelated, so we only need to work out their individual
variances. Since $\tilde{\bm{E}}_1^T \sim \mathrm{N}(\bm{0}, \bm{\Sigma})$,
we have $\tilde{\bm{E}}^T_{1,S} \sim \mathrm{N}(\bm{0}, \bm{\Sigma}_{S})$ and
$\bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T  \bm{\Sigma}_\mathcal{C}^{-1} \bm{\Gamma}_{\mathcal{C}})^{-1}
\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1} \tilde{\bm{E}}^T_{1,C} \sim \mathrm{N}(\bm{0}, \bm{\Delta}_S)$.
Similarly, $\sqrt{n} \cdot (\bm{\Gamma}_{S}^{(0)}  -
  \hat{\bm{\Gamma}}_{S} ) \bm{\alpha}^{(0)} \overset{d}{\to}
  \mathrm{N}(\bm{0}, \|\bm{\alpha}\|^2 \bm{\Sigma}_{S})$, and
  $$\sqrt{n} \cdot \bm{\Gamma}_{S} (\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
  \bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
  (\hat{\bm{\Gamma}}_{\mathcal{C}}  -  \bm{\Gamma}_{\mathcal{C}}^{(0)}) \bm{\alpha}^{(0)}
  \overset{d}{\to} \mathrm{N}(\bm{0}, \|\bm{\alpha}\|^2 \bm{\Delta}_S).$$


==> revision 2/app_thm_rr <==
In
fact, by using the representation of $\hat{\bm{\Gamma}}$ in
\eqref{eq:gamma-hat} and (C.4) in \citep{bai2012}.
  \begin{equation*}
    \label{eq:eq:sigma-hat}
    \hat{\sigma}_j^2 = \frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}}),
  \end{equation*}
we have
\[
\begin{split}
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) =& \frac{1}{p} \sum_{j=1}^p \psi\left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
    \hat{\bm{\Gamma}}_j^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\right)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\left( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 + \bm{\Gamma}_j^T \bm{\alpha}^{(0)} - (\hat{\bm{\Gamma}}_j^0)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\right)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\left( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 + \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + o_p(n^{-\frac{1}{2}})
    }{\sqrt{\frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}})}}\right)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\end{split}
\]
Let $W_j$ be the expression inside $\psi$ in the last equation without
the two $o_p(n^{-\frac{1}{2}})$ terms. Condition on
$\tilde{\bm{Z}}_{-1}^0$, $W_j$ and $W_k$ are independent if $j \ne
k$ and $W_j \overset{d}{=} W_k$ if $\beta_j = \beta_k = 0$. It is not hard to show the denominator of $W_j$ converges in
probability to $\sigma_j$, while the numerator of $W_j$ is $\beta_j +
n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}})$ where $t_j$ are
i.i.d. normal random variables by noticing $\tilde{\bm{Z}}_{-1}^{(0)}
\bm{\alpha}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R} \bm{R}^T)^{-1}
(\bm{\alpha} + \bm{u}/\|\bm{X}\|_2)$ and $\bm{R} \bm{R}^T \to \bm{I}_r$. Because $\psi(W) = \psi(0) + \psi'(0) W +
\frac{1}{2} \psi''(0) W'^2$ for some $W'$ between $0$ and $W$ and
$\psi(0) = 0$, $\psi(W_j) = \psi'(0) (n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}}))$ if $\beta_j =
0$. Also $\psi$ is assumed to be bounded $|\psi(W_j)| \le C$ in
\cref{assumption:rho}. Therefore, by using $\lim_{p \to \infty}
\frac{1}{p} \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ exists and is
positive definite (in \cref{assumption:large-factor})
\[
\begin{split}
\left|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right| &= \left| \frac{1}{p} \sum_{j=1}^p \psi\left(W_j
+ o_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\right| \\
&= \left| \frac{1}{p} \left( \sum_{\beta_j \ne 0} + \sum_{\beta_j = 0} \right) \psi\left(W_j
+ o_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\right| \\
&\le \frac{1}{p} C \|\bm{\beta}\|_0 + O_p(n^{-\frac{1}{2}}
p^{-\frac{1}{2}}) \\
&= o_p(n^{-\frac{1}{2}})
\end{split}
\]

Similarly,
\[
\begin{split}
  \left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1} &=
\left[\frac{1}{p} \sum_{j=1}^p
  \psi'\left(W_j + o_p(n^{-\frac{1}{2}})\right)
\hat{\bm{\Gamma}}_j \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2
\right]^{-1} \\
&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(\beta_j) +
    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 \right]^{-1} \\
&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(0) +
    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \frac{1}{p} \sum_{\beta_j
    \ne 0}
  (\psi'(\beta_j) - \psi'(0)) \hat{\bm{\Gamma}}_j
  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2  \right]^{-1} \\
&\overset{p}{\to} \left[ \psi'(0) \frac{1}{p} \sum_{j=1}^p
  \bm{\Gamma}_j \bm{\Gamma}_j^T / \sigma_j^2 \right]^{-1}
\end{split}
\]
The last probability limit follows from $\hat{\bm{\Gamma}}
\overset{p}{\to} \bm{\Gamma}$, $\hat{\bm{\sigma}}_j
\overset{p}{\to} \sigma_j$ and $\psi'$, $\bm{\Gamma}$ and $\bm{\Sigma}$ are bounded. This means all the eigenvalues of
$\left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1}$ are converging to some constants.


==> revision 2/app_thm_rr.tex <==
% JS is editing

Because $\hat{\bm{\alpha}}^{\mathrm{RR}}$ is consistent, we can
approximate the left hand side of \eqref{eq:Psi} by its second order
Taylor expansion (we abbreviate
$\bm{\Psi}_{p,\hat{\bm{\Gamma}}, \hat{\bm{\Sigma}}}$ to $\bm{\Psi}_p$
if it causes no confusion):
\[
\bm{0} = \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \nabla \bm{\Psi}_p(\bm{\alpha}^{(0)}) \cdot
(\hat{\bm{\alpha}}^{\mathrm{RR}} - \bm{\alpha}^{(0)}) + \bm{r}_p
\]
where $\bm{r}_p$ is the higher order term and
\Cref{assumption:psi-2nd-derivative} implies $\bm{r}_p =
\bm{o}_p(\|\hat{\bm{\alpha}}^{\mathrm{RR}} - \bm{\alpha}\|_2)$.
Therefore $\hat{\bm{\alpha}}^{\mathrm{RR}} = \bm{\alpha}^{(0)} - \left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm{o}_p(1) \right]^{-1}
\bm{\Psi}_p(\bm{\alpha}^{(0)})$ and
\begin{equation} \label{eq:beta-expand}
\begin{split}
\sqrt{n}(\hat{\bm{\beta}}^{\mathrm{RR}} - \bm{\beta}) =&
\frac{\sqrt{n}}{\|\bm{X}\|_2} \tilde{\bm{E}}^T_1
+ \sqrt{n} (\bm{\Gamma}^{(0)} -\hat{\bm{\Gamma}})
\hat{\bm{\alpha}}^{\mathrm{RR}} \\
&+ \hat{\bm{\Gamma}} \left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) + \bm{o}_p(1) \right]^{-1}
\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)})
\end{split}
\end{equation}

It's easy to show $(\sqrt{n}/\|\bm{X}\|_2) \tilde{\bm{E}}_{1, S}
+ \sqrt{n} (\bm{\Gamma}^{(0)}_S -\hat{\bm{\Gamma}}_S)
\hat{\bm{\alpha}}^{\mathrm{RR}} \overset{d}{\to} \mathrm{N}(\bm{0}, (1
+ \| \bm{\alpha}\|^2) \bm{\Sigma}_S)$ by
\Cref{lem:gamma-ml}. Therefore the proof of \Cref{thm:asymptotics-rr} is completed once we can show
the largest eigenvalue of $\left[ \nabla
\bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is $O_p(1)$
and $\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to}
\bm{0}$. We prove these two facts in the following lemma:

\begin{lemma} \label{lem:asymptotics-rr-bound}
  Under the assumptions and limits in \Cref{thm:asymptotics-rr}, the
  largest eigenvalue of the matrix $\left[ \nabla
  \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is bounded in probability
  and $\sqrt{n} \bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to} \bm{0}$.
\end{lemma}

\begin{proof}
By using the representation of $\hat{\bm{\Gamma}}$ in
\eqref{eq:gamma-hat},
%and (C.4) in \citep{bai2012}.
%  \begin{equation*}
%    \label{eq:eq:sigma-hat}
%    \hat{\sigma}_j^2 = \frac{1}{n-1} \tilde{\bm{E}}_{-1,j}^T
%    \tilde{\bm{E}}_{-1,j} + o_p(n^{-\frac{1}{2}}),
%  \end{equation*}
we have
\[
\begin{split}
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) =& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
    \hat{\bm{\Gamma}}_j^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
/ \|\bm{X}\|_2 + \bm{\Gamma}_j^{(0)T} \bm{\alpha}^{(0)} - (\hat{\bm{\Gamma}}_j)^T
    \bm{\alpha}^{(0)}}{\hat{\sigma}_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j \\
=& \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\beta_j + \tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j\\
\end{split}
\]
where $\max_j|\delta_j| = o_p(1)$ and
$\max_j|\epsilon_j| = o_p(n^{-1/2})$ from
%\eqref{eq:avg-sigma-err}
%\Cref{lem:ml-baili}
\Cref{lem:gamma-ml}.
%and equation \eqref{eq:avg-gamma-err}.
Because
$\|\bm{\beta}\|_1 \sqrt{n} / p \to 0$ and $\psi'$ is bounded,
\[
\bm{\Psi}_{p}(\bm{\alpha}^{(0)}) = \frac{1}{p} \sum_{j=1}^p \psi\Big( \frac{\tilde{E}_{1j}
    / \|\bm{X}\|_2 - \frac{1}{n-1} \tilde{\bm{E}}_{-1,j} \tilde{\bm{Z}}_{-1}^{(0)} \bm{\alpha}^{(0)} + \epsilon_j}
    {\sigma_j + \delta_j}\Big)
\hat{\bm{\Gamma}}_j / \hat{\sigma}_j + \bm{o}_p(n^{-1/2})
\]

Let $g_j$ be the expression inside $\psi$ in the last equation omitting $\epsilon_j$ and $\delta_j$. Conditionally on
$\tilde{\bm{Z}}_{-1}^{(0)}$, the variables $g_j, \mathrm{where}~ j=1,\dotsc,p$ are independent and
identically distributed with $\mathrm{E}(g_j) = 0$ and
$g_j = O_p (n^{-1/2}) $.
%Using the Cauchy-Schwartz inequality,
%$p^{-1}\sum_{j = 1}^p(\delta_jg_j)^2 = o_p(n^{-1})$.
Thus, using \Cref{assumption:psi-2nd-derivative}
and boundedness of $\hat \sigma_j$,
\[
\begin{split}
 & \Big\| \frac{1}{p} \sum_{j=1}^p \Big[\psi\Big(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\Big)
 - \psi(g_j)\Big]\hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 \\
\leq & D^2 \cdot \Big\| \frac{1}{p} \sum_{j=1}^p\big(|\epsilon_j| |\hat{\bm{\Gamma}}_j|+ |g_j|
|\delta_j\hat{\bm{\Gamma}}_j|\big) /\hat \sigma_j
%\big(|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}| + |\bm{\Gamma}_j^{(0)}|\big)/\hat \sigma_j
\Big\|_2  = o_p(n^{-1/2})
\end{split}
\]
%where the last approximation is got by using Cauchy-Schwartz inequality and \Cref{lem:ml-baili}.
%where $t_j$ are
%i.i.d. normal random variables by noticing $\tilde{\bm{Z}}_{-1}^{(0)}
%\bm{\alpha}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R} \bm{R}^T)^{-1}
%(\bm{\alpha} + \bm{u}/\|\bm{X}\|_2)$ and $\bm{R} \bm{R}^T \to \bm{I}_r$.
%Because for some $W'$ between $0$ and $W$ and
%$\psi(0) = 0$, $\psi(g_j) = \psi'(0) (n^{-\frac{1}{2}} t_j + o_p(n^{-\frac{1}{2}}))$ if $\beta_j =0$.


We can further use the facts that
$\psi(g_j)=\psi'(0) g_j +
o_p(n^{-1/2}) = O_p(n^{-1/2})$ and
%Cauchy-Schwartz inequality in a similar way and combine
$\psi(g_j) - \psi'(0)g_j$
are i.i.d., and combine \Cref{rmk:rotation} and \Cref{lem:gamma-ml} to get:
\[
\begin{split}
\left\|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right\|_2 &= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
+ \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\| \frac{1}{p} \sum_{j=1}^p \psi\left(g_j
\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
\Big\|_2 + o_p(n^{-1/2}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi(g_j)\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
%O_p(n^{-\frac{1}{2}}p^{-\frac{1}{2}}) \\
&= \Big\|\frac{1}{p}\sum_{j = 1}^p\psi'(0)g_j\frac{\bm{\Gamma}^{(0)}_j}{\sigma_j}\Big\|_2
+ o_p(n^{-1/2})\\
&=o_p(n^{-\frac{1}{2}})+ o_p(n^{-\frac{1}{2}})
= o_p(n^{-\frac{1}{2}})
\end{split}
\]


Similarly,
%$\psi$ is assumed to be bounded $|\psi(g_j)| \le C$ in
%\Cref{assumption:rho}. Therefore, by
because $\lim_{p \to \infty}
\frac{1}{p} \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ exists and is
positive definite (in \Cref{assumption:large-factor}),
we use \Cref{assumption:psi-2nd-derivative} and the uniform convergence
of $\hat {\bm \Sigma}$ and $\hat{\bm \Gamma}$ in \Cref{lem:gamma-ml} to get
\[
\begin{split}
  \left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1} &=
\Bigg[\frac{1}{p} \sum_{j=1}^p
  \psi'\left(g_j + \frac{\epsilon_j-\delta_jg_j}{\hat\sigma_j}\right)
\hat{\bm{\Gamma}}_j \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
&= \Bigg[\frac{1}{p} \sum_{j = 1}^p
  \psi'\left(0\right)
  \bm{\Gamma}_j^{(0)} \bm{\Gamma}_j^{(0)T} / \sigma_j^2 + \bm{o}_p(1)
\Bigg]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(\beta_j) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 \right]^{-1} \\
%&= \left[ \frac{1}{p} \sum_{j=1}^p \left(\psi'(0) +
%    O_p(n^{-\frac{1}{2}})\right) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2 + \frac{1}{p} \sum_{\beta_j
%    \ne 0}
%  (\psi'(\beta_j) - \psi'(0)) \hat{\bm{\Gamma}}_j
%  \hat{\bm{\Gamma}}_j^T / \hat{\sigma}_j^2  \right]^{-1} \\
&\overset{p}{\to} \Big[ \psi'(0) \frac{1}{p} \sum_{j=1}^p
  \bm{\Gamma}_j \bm{\Gamma}_j^T / \sigma_j^2 \Big]^{-1}
\end{split}
\]
%The last probability limit follows from $\hat{\bm{\Gamma}}
%\overset{p}{\to} \bm{\Gamma}$, $\hat{\bm{\sigma}}_j
%\overset{p}{\to} \sigma_j$ and $\psi'$, $\bm{\Gamma}$ and $\bm{\Sigma}$ are bounded.
This means that all the eigenvalues of
$\left[\nabla \bm{\Psi}_p(\bm{\alpha}^{(0)})\right]^{-1}$ converge to finite constants.
\end{proof}

% For \Cref{thm:consistency}, we first note that when $n,p \to \infty$
% and $\|\beta\|_0/p \to 0$,
% $\hat{\bm{\alpha}}^{\mathrm{RR}} \overset{p}{\to} \bm{\alpha}^{(0)}$
% is still true by the same argument in the proof of
% \Cref{thm:asymptotics-rr} and the fact that we can estimate the strong
% factors consistently. By using the same Taylor expansion in the proof
% of \Cref{thm:asymptotics-rr}, the consistency of
% $\hat{\bm{\beta}}^{\mathrm{RR}}$ is immediately proved by the
% following lemma:
% \begin{lemma}
%   Under the assumptions and limits in \Cref{thm:consistency}, the largest eigen value of $\left[ \nabla
%   \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1}$ is bounded in probability
% and $\bm{\Psi}_p(\bm{\alpha}^{(0)}) \overset{p}{\to} 0$.
% \end{lemma}
% \begin{proof}
%   The statement of this lemma is almost the same as
%   \Cref{lem:asymptotics-rr-bound}, except we relax the sparsity
%   condition from $\|\bm{\beta}\|_0 \sqrt{n}/p \to 0$ to
%   $\|\bm{\beta}\|_0 /p \to 0$ and we are only able to prove
%   $\bm{\Psi}_p(\bm{\alpha}^{(0)}) = o_p(1)$ instead of
%   $o_p(1/\sqrt{n})$. By the same argument in
%   \Cref{lem:asymptotics-rr-bound}, $\left[ \nabla
%   \bm{\Psi}_p(\bm{\alpha}^{(0)}) \right]^{-1} = O_p(1)$ and
% \[
% \begin{split}
% \left|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right|
% &= \left| \frac{1}{p} \left( \sum_{\beta_j \ne 0} + \sum_{\beta_j = 0} \right) \psi\left(g_j
% + o_p(1)\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j
% \right| \\
% &\le \frac{1}{p} D \|\bm{\beta}\|_0 + o_p(1) \\
% &= o_p(1)
% \end{split}
% \]
% Notice that here the denominator of $g_j$ may not converge to
% $\sigma_j$ any more because $\hat{\sigma}_j$ is not necessarily
% consistent for $\sigma_j$. However, in \Cref{assumption:bounded} we
% assume $\hat{\sigma}_j$ is bounded below and above, so inconsistency
% of $\hat{\sigma}_j$ doesn't change the conclusion that
% $\left|\bm{\Psi}_{p}(\bm{\alpha}^{(0)})\right| = o_p(1)$.

% \end{proof}


==> revision 2/app_thm_weak.tex <==
Now we prove the first claim in \Cref{thm:consistency-weak} that \ $\hat{{\alpha}}_{k}^{\mathrm{RR}} \overset{p}{\to}
    \alpha_{k}$, $k=1,\dotsc,s$. Let $S = \{1,2,\dotsc,s\}$. We follow the same strategy used in the proof of \Cref{thm:consistency-rr} in
    \Cref{app:consistency-rr} by showing that
\begin{equation} \label{eq:phi-op1-strong}
\varphi(\bm{\alpha}_S -
  \hat{\bm{\alpha}}_S) = \frac{1}{p} \sum_{j=1}^p \rho\left(\frac{
  \sum_{k=1}^s \hat{\Gamma}_{jk} ({\alpha}_k -
  \hat{{\alpha}}_k)}{\hat{\sigma}}\right) = o_p(1)
\end{equation}
and
\begin{equation} \label{eq:consistency-key-strong}
  \mathrm{P} \left( \inf_{\|\tilde{\bm{\alpha}}\|_2 \ge \epsilon}
  {\varphi}(\tilde{\bm{\alpha}}) > \tau \right)
\to 1.
\end{equation}
Equation \eqref{eq:consistency-key-strong} can be proven using the same
argument in \Cref{app:consistency-rr}, so we omit it here. For
\eqref{eq:phi-op1-strong}, we again investigate for
$\|\tilde{\bm{\alpha}}\|_2 \le D'$
\begin{equation} \label{eq:lp-strong}
\begin{split}
l_p(\tilde{\bm{\alpha}}) &= \frac{1}{p}\sum_{j=1}^p
  \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
      \hat{\bm{\Gamma}}_j^T \tilde{\bm{\alpha}}}{\hat{\sigma}}\right) \\
&= \frac{1}{p}\sum_{j=1}^p
      \rho \left( \frac{\beta_j + \frac{\tilde{{E}}_{1j} + \bm \Gamma_j^T\tilde{\bm{W}}_1}{\|\bm{X}\|_2} +
\sum_{k=1}^r \left(\alpha_k
\Gamma_{j k}
-\tilde{\alpha}_k \hat{\Gamma}_{j k}\right)
}{\hat{\sigma}} \right)
\end{split}
\end{equation}
By \Cref{lem:weak-gamma} and boundedness of $\bm{\alpha}$ and
$\tilde{\bm{\alpha}}$ in \Cref{assumption:bound-alpha}, we have
$\sum_{k=s+1}^r \alpha_k
\Gamma_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{\Gamma}_{j k} = o_p(1)$ and
$\sum_{k=1}^s \Gamma_{jk} (\alpha_k - \tilde{\alpha}_k) = o_p(1)$. Because
$\rho$ has bounded derivative (\Cref{assumption:rho}),
$\|\bm{\beta}\|_1/p \to 0$, $\|\bm{X}\|_2 \to \infty$ and $\bm\Gamma$ is bounded,
we again have
$l_p(\tilde{\bm{\alpha}}) = \varphi(\bm{\alpha}_S -
\tilde{\bm{\alpha}}_S) + o_p(1)$ for any $\|\tilde{\bm{\alpha}}\|_2 \le
D'$ and the $o_p(1)$ term doesn't depend on
$\tilde{\bm{\alpha}}$. Therefore $\varphi(\bm{\alpha}_S -
  \hat{\bm{\alpha}}_S) = l_p(\hat{\bm{\alpha}}) + o_p(1) \le
  l_p(\bm{\alpha}) + o_p(1) = o_p(1)$.

To prove the second claim in \Cref{thm:consistency-weak}, notice that
\[
\hat{\beta}_j^{\mathrm{RR}} - {\beta}_j =
\frac{\tilde{{E}}_{1j} + \bm \Gamma_j^T\tilde{\bm{W}}_1}{\|\bm{X}\|_2} +
\sum_{k=1}^s \left(\alpha_k
{\Gamma}_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{{\Gamma}}_{j k}\right) +
\sum_{k=s+1}^r \left(\alpha_k
{\Gamma}_{j k}
-\hat{\alpha}^{\mathrm{RR}}_k \hat{{\Gamma}}_{j k} \right)
\]
By the same argument as in the last paragraph,
$\hat{\beta}_j^{\mathrm{RR}} - {\beta}_j = \sum_{k=1}^s
\hat{\Gamma}_{jk} (\alpha_k - \hat{\alpha}_k) + o_p(1)$. Since
$\hat{\Gamma}_{jk} \overset{p}{\to} \Gamma_{jk}$ and $\hat{\alpha}_k
\overset{p}{\to} \alpha_k$ for $k = 1,\dotsc,s$, we conclude that
$\hat{\beta}_j^{\mathrm{RR}} \overset{p}{\to} \beta_j$.


==> revision 2/app_weak_simu.tex <==
We decide the strength of the confounding factors in \Cref{sub:weak} based
on recent results in random matrix theory \citep{perry2009,
  donoho2013}. Their latent factor model is $ \bm Y = \sqrt n \bm {UDV}^T + \bm{E}$
where $\bm{U}^T\bm{U} = \bm{V}^T\bm{V} = \bm{I}_r$, $\bm{D}$ is a diagonal $r \times r$
matrix and $\bm{E} \sim \sigma^2 \mathrm{MN}(0, \bm{I}_n, \bm{I}_p)$. The goal is to recover the matrix $\sqrt n \bm{UDV}^T$ from
the observed matrix $\bm{Y}$ as accurately as possible.

A natural estimator of $\sqrt n \bm{UDV}^T$ is the truncated SVD of
$\bm Y$ using the first $k$ singular values/vectors, denoted by
$\bm{Y}(k)$. Let $r_0 = \arg \min_k \|\bm Y(k) - \sqrt n
\bm{UDV}^T\|_F$ be the optimal number of factors to include. \citet{donoho2013} show that
in the asymptotic setting of $n \to \infty$, $p \to \infty$, $d_j^2 \to
\mu_j~,j=1,\dotsc,p$
and $p/n \to \gamma > 0$, $r_0$ converges to $|\{ j: \mu_j > \mu^{\star}
\}|$ where the estimation threshold $\mu^{\star}$ is \citep{perry2009}
\begin{equation}
\label{eq:mu-star}
\mu^\star = \sigma^2 \left(\frac{1 + \gamma}{2} + \sqrt{\Big(\frac{1 +
      \gamma}{2}\Big)^2 + 3 \gamma}\right).
\end{equation}
Notice that the detection threshold in \Cref{sec:weak-factors}, $\mu =
\sigma^2\sqrt{\gamma}$, is less than $\mu^\star$. This implies that if
$\mu < \mu_j < \mu^\star$, the factor is detectable but too small to
be included in the truncated SVD to reduce the estimation error of
$\sqrt n \bm {UDV}^T$. \cite{donoho2013} propose an estimator $\hat r$
such that $\hat r \overset{a.s.}{\to} r_0$.

For our simulation experiment in \Cref{sub:weak}, as $\bm{Z}_{-1}^T\bm{Z}_{-1}/n \to \bm{I}_r$, though we assume
random factors, their results still hold. Since we set $\sigma^2 = 1$ and $p = 5000$,
the largest factor $d_1 = 3 \cdot \sqrt p = 212$.
When $n = 100$, $d_r = \sqrt{\mu_F} = 2.7$ and $\sqrt {\mu^\star} = 7.3$,
and we set $(d_2, \cdots, d_9) = (73.3, 64.5, 55.7, 46.8, 38.0, 29.2, 20.3, 11.5)$
for $r = 10$
which is an equal spaced decreasing sequence with $d_2 = 10\cdot \sqrt {\mu^\star}$.
When $n = 500$, $d_r = \sqrt{\mu} = 1.8$
and $\sqrt {\mu^\star} = 3.6$,
and correspondingly we set $(d_2, \cdots, d_9) =(36.4, 32.1, 27.8, 23.4, 19.1, 14.8, 10.4,  6.1)$
for $r = 10$.

Finally, we discuss the variance-bias tradeoff in our
simulation in \Cref{sub:weak}.
The oracle method has distribution
\[
\sqrt n (\hat \beta^{\mathrm{Oracle}}_j - \beta_j)\sim
\mathrm{N}(0, 1 + \|\bm \alpha\|_2^2).
\]
Next we consider the RR
method. In the case of $r=2$, we can rewrite \eqref{eq:y-tilde-1} as
\[
        \tilde{\bm{Y}}_1^T / \|\bm{X}\|_2 = \bm{\beta} + \bm{\Gamma}_{\cdot 1}(\alpha_1 + u_1/\|\bm{X}\|_2)
+ \bm{\Gamma}_{\cdot 2}(\alpha_2 + u_2/\|\bm{X}\|_2)
   + \tilde{\bm{E}}_{1}^T / \|\bm{X}\|_2
\]
where $u_i\sim \mathrm{N}(0, 1)$. In our simulation in
\Cref{sub:weak}, $r_0 = 1$ and RR only adjusts for one (the strongest) confounding
factor. As a consequence, $\check{e}_{j} = \Gamma_{j2}(\alpha_2 +
u_2/\|\bm{X}\|_2) + \tilde{E}_{1j}^T/\|\bm X\|_2 $ can be treated as
the new noise terms. Since $\Gamma_{j2}$ is generated by $\Gamma_{j2} = d_2\cdot\tilde{\Gamma}_{j2} = d_2 \cdot z_{j}/\|\bm{z}\|_2$ where
$\bm{z} = (z_1, \cdots, z_p)\sim \mathrm{N}(\bm 0, \bm I_p)$, when $n, p \to \infty$, 
$\mathbb{E}(\sqrt n \cdot \check{e}_j) = 0$,
$\mathrm{Var}(\sqrt n \cdot \check{e}_j) \to \alpha_2^2\cdot d_2^2\cdot n/p + 1$
and $\mathrm{Cov}(\sqrt n \cdot \check{e}_{j_1}, \sqrt n \cdot \check{e}_{j_2}) \to 0$
for $j_1 \neq j_2$.
Assuming that we asymptotically get the strong factor $\bm{\Gamma}_{\cdot 1}$ as
accurate as what the oracle gets,
then using \Cref{thm:consistency-weak} and similar to the calculation in \Cref{thm:asymptotics-rr},
we have
\[
\sqrt n (\hat \beta^{\mathrm{RR}}_j - \beta_j) \overset{d}{\to}
\mathrm{N}(0, 1 + \alpha_1^2 + \alpha_2^2\cdot d_2^2/\gamma).
\]
Thus, as long
as $d_2^2 < \gamma = p/n$, $\beta^{\mathrm{RR}}_j$ is more accurate
than $\beta^{\mathrm{Oracle}}_j$. The calibration method uses MAD to
estimate the variance inflation factor $(1 + \alpha_1^2 +
\alpha_2^2\cdot \gamma d_2^2)/(1 + \alpha_1^2)$ empirically. This is
why LEAPP and RR-MAD can control the type I error and FDR in \Cref{fig:p-5000-weak-methods}.

An interesting final observation is that $d_i^2 > \sigma^2 \gamma$ provides
a threshold of factor strength in the confounder
adjusting problem. When $\gamma$ is large, this is about the same as
the estimation threshold $\mu^{\star}$ \eqref{eq:mu-star} in the
low-rank matrix approximation problem.


==> revision 2/asymp_eff.tex <==
Consider the oracle estimator of the primary effects $\bm{\beta}$ such that the confounding
variables $\bm{Z}$ were observed. In this
case, \eqref{eq:linear-model-y} becomes a linear model with random
predictors and the ordinary least squares estimator of
$\bm{\beta}$ and $\bm{\Gamma}$ have the minimum variance among all
linear estimators. The variance
of $(\hat{{\beta}}^{\mathrm{OLS}}_j,
\hat{\bm{\Gamma}}^{\mathrm{OLS}}_j)$ is $ \sigma_j^2
\mathrm{Var}(X_i, \bm{Z}_i)^{-1} / n$. Since
\[
\mathrm{Var}(X_i, \bm{Z}_i) =
\begin{pmatrix}
  1 & \bm{\alpha}^T \\
  \bm{\alpha} & \bm{I}_r + \bm{\alpha} \bm{\alpha}^T \\
\end{pmatrix},
\]
it is easy to show that $\mathrm{Var}(\hat{\beta}_j^{\mathrm{OLS}}) =
(1 + \|\bm{\alpha}\|_2^2) \sigma_j^2/n$. Also, for $j \ne k$,
$\mathrm{Cov}(\hat{\beta}_j^{\mathrm{OLS}},
\hat{\beta}_k^{\mathrm{OLS}}) = 0$ by conditioning on $\bm{X}$ and
$\bm{Z}$. In summary,
\[
\mathrm{Var}(\hat{\bm{\beta}}^{\mathrm{OLS}}) = \frac{1}{n} (1 + \| \bm{\alpha}
\|_2^2) \bm{\Sigma},
\]
which is the same asymptotic variance we derived in
\Cref{thm:asymptotics-nc,thm:asymptotics-rr}. Since the estimator
$\hat{\bm{\beta}}^{\mathrm{OLS}}$ require oracle knowledge of the
confounders $\bm{Z}$, we conclude that %our confounder adjusted estimators
$\hat{\bm{\beta}}^{\mathrm{NC}}$ and
$\hat{\bm{\beta}}^{\mathrm{RR}}$ are asymptotically efficient among
linear estimators under
the corresponding assumptions in \Cref{thm:asymptotics-nc,thm:asymptotics-rr}.

% \begin{remark} \label{rmk:alpha-intuition}
%  The variance $(1 + \| \bm{\alpha}\|_2^2) \bm{\Sigma} / n$ depends on
%  three quantities: $\| \bm{\alpha}\|_2^2$, the total covariance of
 % $\bm{Z}$ with $\bm{X}$; $\bm{\Sigma}$,
%  the intrinsic variance of $\bm{Y}$; and $n$, the number of
%  observations. 
As mentioned in \Cref{sec:linear-model-with},
  $\|\bm{\alpha}\|^2/(1 + \|\bm{\alpha}\|^2)$ is the proportion of
  variance of $\bm{X}$ that can be explained by the confounders. Our
  variance expression $(1 + \| \bm{\alpha}\|_2^2) \bm{\Sigma} / n$ of $\hat{\bm{\beta}}^{\mathrm{RR}}$ coincides with the intuition that the estimation of
  $\bm{\beta}$ should become harder as the confounders $\bm{Z}$ are more
  correlated with $\bm{X}$. % Since $\|
  % \bm{\alpha}\|_2^2$ can be much larger than $1$ in our model
  % \eqref{eq:linear-model-y}, ignoring the uncertainty of estimating
  % confounders in the asymptotic variance may also significantly bias the test $p$-values.
% \end{remark}


==> revision 2/discussions.tex <==
\subsection{Confounding vs.\ unconfounding}
\label{sec:latent-but-unconf}

The issue of multiple testing dependence arises because $\bm{Z}$ in
the true model \eqref{eq:previous-model} is unobserved.
%From
%there, the data are confounded or unconfounded depending on whether
%$\bm Z$ and $\bm X$ are dependent or not.
%Though we only consider
%confounded problem in this paper, it should not be surprising to the
%reader that
%%%% actually we do both because our alpha could be zero
We have focused on the case where $\bm{Z}$ is confounded with
the primary variable.
Some similar results were obtained earlier
for the unconfounded case, corresponding to $\bm{\alpha}=0$ in our notation.
For example, \citet{lan2014} used a factor model to improve the
efficiency of significance tests of the regression intercepts.
\citet{jin2012comment,li2014rate} developed more powerful procedures for testing
$\bm{\beta}$ while still controlling FDR under unconfounded dependence.

In another related work, \citet{fan2012} imposed a factor structure
on the unconfounded test statistics, whereas this paper and the articles discussed later in
\Cref{sec:comp-with-exist} assume a factor structure on the raw data.
\citet{fan2012} used an approximate factor model to accurately estimate the false
discovery proportion. Their correction procedure also includes a
step of robust regression. Nevertheless, it is often difficult to interpret the factor
structure of the test statistics. In comparison, the latent variables
$\bm{Z}$ in our model \eqref{eq:linear-model}, whether confounding or
not, can be interpreted as batch effects, laboratory conditions, or
other systematic bias. Such problems are widely observed in genetics
studies (see e.g.\ the review article \citep{leek2010}).

As a final remark, some of the models and methods developed in
the context of unconfounded hypothesis testing may be useful for
confounded problems as well. For example,
the relationship between $\bm{Z}$ and $\bm{X}$  needs not be linear
as in~\eqref{eq:linear-model-z-sec1}. In certain applications, it may be
more appropriate to use a time-series model \citep{sun2009} or
a mixture model \citep{efron2010}.

\subsection{Marginal effects vs.\ direct effects}
\label{sec:marginal-effects-vs}

In \Cref{sec:introduction}, we switched our interest from
the marginal effects $\bm{\tau}$ in \eqref{eq:marginal-effect} to the
direct effects $\bm{\beta}$. We believe that they are usually more
scientifically meaningful and interpretable than the marginal effects.
For instance, if the treated (control) samples are analyzed by machine
A (machine B), and the machine A outputs
higher values than B, we certainly do not
want to include the effects of this machine to machine variation on the outcome
measurements.

When model
\eqref{eq:linear-model} is interpreted as a ``structural
equations model'' \citep{bollen1989}, $\bm \beta$ is indeed the causal effect of
$\bm{X}$ on $\bm{Y}$ \citep{pearl2009}. In this paper we do not make
such structural assumptions about the data generating
process. Instead, we use \eqref{eq:linear-model} to describe the screening
procedure commonly applied in high throughput data analysis. The model
\eqref{eq:linear-model} also describes how we think the marginal
effects can be confounded and hence different from the more meaningful direct effects
$\bm{\beta}$. Additionally, the asymptotic setting in this paper is quite
different from that in the traditional structural equations model.

% The regression \cref{eq:marginal-effect} and the asymptotics $n,p \to
% \infty$ suggest the rows (observations) and columns (responses) in
% $\bm{Y}$ are in some sense transposable. % This property becomes even
% clearer if we wish to include some response-specific features
% (typically a $p \times q$ matrix) in the model, resulting in a
% bilinear regression \citep{gabriel1978least}.

% In the related work by \citet{fan2012},
% In a comment of the article by \citet{fan2012}, \citet{wasserman2012}
% also discusses about the marginal effects: ``The
% coefficients of a marginal regression are difficult to interpret \ldots
% You can have a huge regression effect and a zero marginal
% effect. Conversely, you can have a tiny regression effect
% and a huge marginal effect.''

% Because
% of the difficulty of interpreting marginal effects, in practice we rarely
% trust the assumption that they are sparse. The lack of sparsity, as a
% result, raises the question that whether FDR is even the meaningful error metric to control.

%%%% we discussed also that gene 1 might affect genes 2, 3, 4 and together
%%%% affect Y.  In this case we might want \tau.  Perhaps we should say this.

%  estimated marginal effects between $\bm X$ and $\bm Y$
% which have known covariance dependence
% conditional on the data by
% considering a particular approximate factor model,
% where the factors are assumed unconfounded.
% They then used robust regression to estimate $\bm \beta$
% and compute test statistics
% which is similar to our second step.
% %propose a procedure that estimates the false discovery proportion
% %under arbitrary covariance dependence by considering a particular
% %approximate factor model as in
% %\Cref{sec:inference-when-sigma}. However, the approximate factor model in
% %\citet{fan2012} is only used to estimate the false discovery
% %proportion.
% %For the unconfounding problem, \citet{fan2012}
% %propose a procedure that estimates the false discovery proportion
% %under arbitrary covariance dependence by considering a particular
% %approximate factor model as in
% %\Cref{sec:inference-when-sigma}. However, the approximate factor model in
% %\citet{fan2012} is only used to estimate the false discovery
% %proportion.
% %Their test statistic is indeed very similar to our
% %standardized z-scores in \eqref{eq:test-statistic}.
% They also have a similar result as our \Cref{thm:asymptotics-rr} that the variance of
% $\hat{\bm{\beta}}$ under $\bm \alpha = \bm 0$  is approximately $\bm{\Sigma}/n$,
% which reaches the oracle efficiency asymptotically.
% %In our framework, if all the factors are strong and unconfounding and $\bm{\Sigma}$ is
% %diagonal, \Cref{thm:asymptotics-rr} implies that the variance of
% %$\hat{\bm{\beta}}$ is approximately $\bm{\Sigma}/n$. This is more
% %efficient than the naive regression estimator which has variance
% %$\left(\bm{\Gamma} \bm{\Gamma}^T + \bm{\Sigma}\right)/n$, also noted
% %by \citet{lan2014}.

% Apart from these similarites, the fact that the latent
% factors are correlated with the primary variable ($\bm{\alpha} \ne
% \bm{0}$) makes the problem essentially different and much more difficult. In
% the unconfounded problem, the naive linear regression
% without factor adjustment %(or two sample t-test)
%  already has provided individually valid tests. The main difficulty
% is to construct more efficient test statistics and decorrelate
% them. In the confounded problem, however, the main challenge is to
% debias the test statistics by an additional step of estimating $\bm{\alpha}$.

\subsection{Comparison with existing confounder adjustment methods}
\label{sec:comp-with-exist}

We discuss in more detail how previous methods of confounder
%%% changed `the existing' to `previous' because we might have missed some others
adjustment, namely SVA \citep{leek2007,leek2008},
RUV-4 \citep{gagnon2013,gagnon2012}
and
LEAPP \citep{sun2012}, fit in the framework \cref{eq:linear-model}. See
\citet{perry2013degrees} for an alternative approach of bilinear
regression with latent factors that is also motivated by
high-throughput data analysis.

\subsubsection{SVA}
\label{sec:sva}

There are two versions of SVA: the reduced subset SVA (subset-SVA) of
\citet{leek2007} and the iteratively reweighted SVA (IRW-SVA) of
\citet{leek2008}. Both of them can be interpreted as the two-step
statistical procedure in the framework \cref{eq:linear-model}. In the first step, SVA
estimates the confounding factors by applying PCA to the residual matrix
$({\bm{I}}-{\bm{H}}_{{\bm{X}}}) {\bm{Y}}$ where
${\bm{H}}_{{\bm{X}}}
={\bm{X}} ({\bm{X}}^T
{\bm{X}})^{- 1} {\bm{X}}^T$ is the
projection matrix of ${\bm{X}}$.
In contrast, we
%follow the approach in LEAPP that
applied factor analysis to the rotated residual matrix
$(\bm{Q}^T{\bm{Y}})_{- 1}$, where $\bm{Q}$ comes from
the QR decomposition of $\bm X$ in \Cref{sec:extens-mult-regr}.
To see why these two approaches lead to the same estimate
of $\bm{\Gamma}$, we introduce the block form of $\bm Q = \begin{pmatrix} \bm Q_1 & \bm Q_2\end{pmatrix}$ where
$\bm Q_1 \in \mathbb{R}^{n \times d}$ and $\bm Q_2 \in \mathbb{R}^{n
  \times (n-d)}$. It is easy to show that $(\bm{Q}^T{\bm{Y}})_{- 1} = \bm
Q_2^T \bm Y$ and $({\bm{I}}-{\bm{H}}_{{\bm{X}}}) {\bm{Y}} = \bm Q_2 \bm Q_2^T \bm Y$.
Thus our rotated matrix $(\bm{Q}^T{\bm{Y}})_{- 1}$ decorrelates the
residual matrix by left-multiplying by $\bm{Q}_2$ (because $\bm Q_2^T\bm
Q_2 = \bm I_{n - d}$).
Because $(\bm Q_2^T \bm Y)^T\bm Q_2^T \bm Y = (\bm Q_2 \bm
Q_2^T \bm Y)^T\bm Q_2 \bm
Q_2^T \bm Y$,
%In fact,
$(\bm Q^T\bm Y)_{-1}$ and $(\bm I - \bm H_{\bm X})\bm Y$
%$\bm
%Q_2^T \bm Y$ and $\bm Q_2 \bm
%Q_2^T \bm Y$
have the same sample covariance matrix, they will yield the same
factor loading estimate under PCA and also under MLE.
%%% trying to make clear that the two matrix multiplies give the same
%%% answer as each other under PCA and they give the same answer as each
%%% other under MLE but the PCA answers can differ from the MLE answers.
%right singular vectors, so the PCA
%estimates of the factor loadings are exactly the same.
The main advantage
of using the rotated matrix is theoretical: the rotated residual matrices
have independent rows.  % which greatly facilitates the theoretical analysis.
%\marginpar{I reworded this paragraph heavily. Please have another look.}
%the $n$ rows of
%$({\bm{I}}-{\bm{H}}_{{\bm{X}}}) {\bm{Y}}$ are not independent and indeed
%the matrix has rank $n-1$. In comparison, the $n-1$ rows of $({\bm{O}}{\bm{Y}})_{- 1}$ are
%independent
% , which makes it easier for us to apply methods other than PCA (for example, the maximum likelihood method we used)
%  and study the theoretical properties.
 %In practice, when $n$ is fairly large, these two approaches yield almost the same results.

% Though these
% two approaches are very similar, we think that using
% $({\bm{O}}{\bm{Y}})_{- 1}$ will give
% better estimates of the latent factors, as the residual matrix
% $({\bm{I}}-{\bm{H}}_{{\bm{X}}})
% {\bm{Y}}$ is not of full rank. Actually, conditional on
% ${\bm{X}}$ and ${\bm{Z}}$,
% $({\bm{O}}{\bm{Y}})_{- 1} \sim
% \mathrm{N} (({\bm{O}}{\bm{Z}})_{- 1}
% {\bm{\Gamma}}^T, {\bm{I}}_{n - 1}
% \otimes {\bm{\Sigma}})$ has independent error terms, while
% $({\bm{I}_n}-{\bm{H}}_{{\bm{X}}})
% {\bm{Y}} \sim \mathrm{N}
% (({\bm{I}_n}-{\bm{H}}_{{\bm{X}}})
% {\bm{Z}}{\bm{\Gamma}}^T,
% ({\bm{I}_n}-{\bm{H}}_{{\bm{X}}})
% \otimes {\bm{\Sigma}})$ is suffering from dependent errors
% across samples.

% Recall that the second step is to estimate ${\bm{\beta}}$ based on the
% confounding factors estimated in the first step.
Because SVA doesn't assume an
explicit relationship between the primary variable $\bm{X}$ and the
confounders $\bm{Z}$, it cannot use the regression \cref{eq:y-tilde-1}
to estimate $\bm{\alpha}$ (not even defined) and $\bm{\beta}$. Instead, the two SVA algorithms try to reconstruct the
surrogate variables, which are essentially the confounders
$\bm{Z}$ in our framework. Assuming the true primary effect
$\bm{\beta}$ is sparse, the subset-SVA algorithm finds the outcome
variables $\bm{Y}$ that have the smallest marginal correlation with $\bm{X}$
and uses their principal scores as $\bm{Z}$. Then, it computes the p-values
by F-tests comparing the linear regression models with and without $\bm{Z}$. This procedure can
easily fail because a small marginal correlation does not imply no real effect of $\bm X$
due to the confounding factors. For example, most of
the marginal effects in the gender study in
\Cref{fig:gender-naive} are very small, but after confounding
adjustment we find some are indeed significant (see \Cref{sec:gender-study}).

The IRW-SVA algorithm modifies subset-SVA by iteratively choosing the subset.% rather than in one step.
At each step, IRW-SVA gives a weight to each outcome
variable based on how likely $\beta_j = 0$ the current estimate of
surrogate variables. The weights are then used in
a weighted PCA algorithm
to update the estimated surrogate variables. IRW-SVA may be
related to our robust regression estimator in
\Cref{sec:unkn-zero-indic} in the sense that an M-estimator is
commonly solved by Iteratively Reweighted Least Squares (IRLS) and the
weights also represents how likely the data point is an outlier.
However, unlike IRLS, the iteratively reweighted PCA algorithm is not even guaranteed to converge.
%%% if we use Tukey's then we have also got convergence issues.
Some previous articles \citep{gagnon2013,sun2012} and our
experiments in \Cref{sec:simulations} and Supplement
\citep{wang2015supplement} show that SVA is outperformed by the
NC and RR estimators in most confounded examples. % When confounding is a minor
% issue, SVA may perform slightly better.


\subsubsection{RUV}\label{sec:ruv}

%The RUV algorithm is similar to SVA in that it also applies factor
%analysis to the residual matrix and attempts to reconstruct the
%confounders $\bm{Z}$. The main difference is
%RUV introduces the
%concept of negative controls to correct for confounding, which
%motivates our first identifiability condition and the corresponding
%negative control estimator in
%\Cref{sec:known-zero-indices}.
\citet{gagnon2013} derived the RUV-4
estimator of $\bm \beta$ via a sequence of heuristic calculations.
In \Cref{sec:known-zero-indices}, we derived an analytically more tractable
estimator $\hat{\bm \beta}^{\mathrm{NC}}$ which is actually the same as RUV-4,
%it is indeed
%the same as our NC estimator \cref{eq:alpha-nc,eq:beta-nc}
 with the
only difference being that we use MLE instead of PCA to estimate the factors and GLS instead of OLS in
\cref{eq:alpha-nc}. To see why $\hat{\bm\beta}^{\mathrm{NC}}$ is essentially the same as
$\hat{\bm\beta}^{\mathrm{RUV-4}}$,
in the first step of RUV-4 it uses the residual matrix to estimate
$\bm \Gamma$ and $\bm Z$, which yields the same estimate as using
the rotated matrix (\Cref{sec:sva}). In the second step,
RUV-4 estimates $\bm \beta$ via a regression of $\bm{Y}$ on
$\bm X$ and $\hat{\bm Z} = \bm Q\begin{pmatrix}\tilde{\bm Z}_{-1}^T&
  \hat{\bm \alpha}^T\end{pmatrix}^T$. This is equivalent to using
ordinary least squares (OLS) to estimate $\bm{\alpha}$ in \eqref{eq:y-tilde-1-separate}.
% Because of the difficulty of theretical analysis
% without explicit assumptions of $\bm{Z}$, \citet{gagnon2013} are not
% able to derive the asymptotic variance in
% \cref{thm:asymptotic-nc}. Instead,
Based on more heuristic
calculations, the authors claim that the RUV-4 estimator has approximately
the oracle variance. We rigorously prove
this statement in \Cref{thm:asymptotics-nc} when the number of negative
controls is large and give a finite sample correction when the negative
controls are few. In \Cref{sec:simulations} we show this correction is
very useful to control the type I error and FDR in simulations.

% To overcome
% identifiability, RUV uses negative controls, which are exactly the known zero
% indices in \cref{sec:known-zero-indices}. Our estimate
% $\hat{{\bm{\beta}}}^{\mathrm{NC}}$ is very similar to the
% $\hat{{\bm{\beta}}}$ in RUV-4, but we have found
% out that for any fixed and finite index set $S$, there is an inflated error term
% ${\bm{A}_S}={\bm{\Gamma}}_{S}
% ({\bm{\Gamma}}_C^T {\bm{\Sigma}}_C^{- 1}
% {\bm{\Gamma}}_C)^{- 1} {\bm{\Gamma}}_{S}$ than the usual least square estimates
% when $\bm{Z}$ is observed
% that should be considered when calculating p-values, due to the inaccuracy
% in using negtive controls to estimate the confounded part of the latent
% factors. RUV-4 didn't consider $\bm{A}_S$, and the consequence is that if the size of negtive controls is not large
% enough, omitting the inflated variance may result in over estimating the
% significance of genes, so the true FDR could be higher than the
% nominal FDR.

% For IRW-SVA, it implicitly assumes sparsity of ${\bm{\beta}}$
% as what we did in \cref{sec:unkn-zero-indic}, and tries to iteratively reweight each variable (gene) $j$
% based how likely $\beta_j = 0$ given the current estimates. Their
% procedure might be treated as an IRLS (Iteratively Reweighted Least Square)
% scheme for robust PCA, though there is no guarantee of convergence for their
% iteration. On the other hand, we used M-estimator of robust regression to
% estimate the confounded part of the latent factors, which is easier to analyze
% and has clear theoretical guarantees. Finally, for LEAPP, they used
% $\Theta$-IPOD for outlier detection, which is a non-convex problem. We
% simplifies this by assuming no leverage points in
% ${\bm{\Gamma}}$ and then is able to use a more general
% class of M-estimator. In general, our approach is derived from LEAPP, thus can
%  be also considered as its theoretical justification.

\subsubsection{LEAPP}
\label{sec:leapp}

%As mentioned
%earlier, the %Householder transformation
%rotation we use to decouple the
%estimation of $\bm{\Gamma}$ and $\bm{\beta}$ originates from
%LEAPP.
We follow the two-step procedure and robust regression framework in
LEAPP \citep{sun2012} in this paper, thus
the test statistics $t_j^{\mathrm{RR}}$ are very similar to the test statistics in LEAPP.
%and
%The framework of our paper and the RR estimator in \Cref{sec:unkn-zero-indic}
%also come from the LEAPP algorithm%is very similar to our RR estimator in.
The difference is that LEAPP uses the
$\Theta$-IPOD algorithm of \citet{she2011} for outlier detection,
which is robust against outliers at leverage points but is not easy
to analyze.  Indeed \citet{sun2012} replaced it by the Dantzig selector
in its theoretical appendix.
The classical M-estimator, although not robust to leverage
points \citep{yohai1987high}, allows us to study the theoretical properties more easily. In practice,
LEAPP and RR estimator usually produce very similar results; see
\Cref{sec:simulations} for a numerical comparison.


\subsection{Inference when \texorpdfstring{$\bm \Sigma$}{TEXT} is nondiagonal}
\label{sec:inference-when-sigma}

Our analysis is based on the assumption that the noise covariance matrix
$\bm\Sigma$ is diagonal,
%In this section we go back to the setting of strong factors in
%\Cref{sec:model} and discuss how to relax the assumption that $\bm{\Sigma}$ is
%diagonal.
though in many applications, the researcher might suspect that the
outcome variables $\bm{Y}$ in model \cref{eq:linear-model} are still
correlated after conditioning on the latent factors.
%%%  I think that any correlation pattern can be represented via latent variables
%%% but that some of those patterns might require infinitely many latents
%%% Also those latents may include both confounded and unconfounded
%%% ones so I changed `confounding factors' to `latent factors'
Typical examples include gene regulatory networks \citep{de2004} and
cross-sectional panel data \citep{pesaran2004}, where the
variable dependence sometimes cannot be fully explained by the
latent factors or may simply require too many of them.
% In such cases, the researcher can still use
% the method we described in \Cref{sec:stat-infer} (or some slight
% modification) to adjust for the confounding factors, but she may also
% want to assess the robustness of this procedure.
%Here we briefly discuss
\citet{bai2012approximate} extend the theoretical results in
\citet{bai2012} to approximate factor models allowing for weakly correlated noise.
Approximate factor models have also been discussed in \citet{fan2013}.


==> revision 2/experiments.tex <==
% JS is editing

\subsection{Simulations}
\label{sec:simulations}

We have provided theoretical guarantees of confounder adjusting
methods in various settings and the asymptotic regime of $n, p \to \infty$ (e.g.\
\Cref{thm:asymptotics-nc,thm:consistency-rr,thm:asymptotics-rr,cor:type-I,thm:multiple-rr}).
Now we use numerical simulations to verify these results and further
study the finite sample properties of our estimators and tests statistics.

The simulation data are generated from the single primary variable model
\eqref{eq:linear-model}. More
specifically, $X_i$ is a centered binary variable
$
(X_i + 1)/2
\overset{\mathrm{i.i.d.}}{\sim} \mathrm{Bernoulli}(0.5),
$
and $\bm{Y}_i$, $\bm{Z}_i$ are generated according to
\cref{eq:linear-model}.

For the parameters in the
model, the noise variances are generated by
%%% changed sigma to sigma^2
$\sigma_j^2 \overset{\mathrm{i.i.d.}}{\sim}\mathrm{InvGamma}(3, 2),~j=1,\dotsc,p$, and so
$\mathbb{E}(\sigma_j^2) = \mathrm{Var}(\sigma_j^2) = 1$. We set each
$\alpha_k = \|\bm{\alpha}\|_2/\sqrt r$ equally for $k = 1, 2, \cdots,
r$ where $\|\bm{\alpha}\|_2^2$ is set to $1$, so the variance of $X_i$
explained by the confounding factors is $R^2 = 50\%$. (Additional
results for $R^2 = 5\%$ and $0$ are in the Supplement.)
The primary effect $\bm{\beta}$ has
independent components $\beta_i$ taking the values $3 \sqrt{1 + \|\bm{\alpha}\|_2^2}$ and $0$ with probability
$\pi = 0.05$ and $1 - \pi = 0.95$, respectively, so the nonzero
effects are sparse and have effect size $3$. This implies that the oracle estimator has
power approximately $\mathrm{P}(\mathrm{N}(3,1) > z_{0.025}) =
0.85$ to detect the signals at a significance level of $0.05$. We set the number of latent
factors $r$ to be either $2$ or $10$. For the latent factor loading matrix $\bm \Gamma$, we take
$\bm\Gamma = \tilde{\bm\Gamma}\bm{D}$ where $\tilde{\bm\Gamma}$ is a
$p \times r$ orthogonal matrix sampled uniformly from the Stiefel
manifold $V_r(\mathbb{R}^p)$, the set of all $p \times r$ orthogonal
matrix. Based on \Cref{assumption:large-factor}, we set the latent factor strength $\bm{D} =
\sqrt p\cdot \mathrm{diag}(d_1, \cdots, d_r)$ where $d_k = 3 -
2(k-1)/(r - 1)$ thus $d_1$ to $d_r$ are distributed evenly inside the interval $[3, 1]$.
As the number of factors $r$ can be easily estimated for this strong factor setting
(more discussions can be found in \citet{owen2015}),
we assume that the number $r$ of factors is known to all of the algorithms in this simulation.


%%% we could say why this is reasonable by citing the proper Bai paper

% We consider two settings of the factor
% strength $\bm{D}$: in the first setting (\Cref{sub:strong}), all the
% latent factors are strong enough to satisfy
% \Cref{assumption:large-factor}; in the second setting
% (\Cref{sub:weak}), there is only one strong factor followed by many
% weak factors.
We set $p = 5000$, $n = 100$ or $500$ to mimic the data size of many
genetic studies. For the negative control scenario, we choose
$|\mathcal C|= 30$ negative controls at random from the zero positions of
$\bm \beta$.
We expect that negative control methods would perform better with a larger value of
$|\mathcal{C}|$ and worse with a smaller value.
The choice $|\mathcal{C}|=30$ is around the size of the spike-in controls in
many microarray experiments \citep{gagnon2012}.
For the loss function in
our sparsity scenario, we use Tukey's bisquare which is optimized via IRLS
with an ordinary least-square fit as the starting values of the coefficients.
Finally, each of the four combinations of $n$ and $r$ is randomly repeated $100$ times.

We compare the performance of nine
different approaches. There are two baseline methods:
the ``naive'' method estimates $\bm\beta$ by a
linear regression of $\bm{Y}$ on just the observed primary variable
$\bm{X}$ and calculates p-values using the classical t-tests, while the
``oracle'' method regresses $\bm{Y}$ on both $\bm{X}$ and the
confounding variables $\bm{Z}$ as described in \Cref{sec:linear-model-with}.
%%% now listing them chronologically
There are three methods in the RUV-4/negative controls family:
the RUV-4 method \citep{gagnon2013},
our ``NC'' method which computes test statistics using
$\hat{\bm\beta}^{\mathrm{NC}}$ and its variance estimate $(1 + \|\hat{\bm{\alpha}}\|_2^2)(\hat{\bm{\Sigma}}+\hat{\bm{\Delta}})$,  and our ``NC-ASY'' method
which uses the same $\hat{\bm \beta}^{\mathrm{NC}}$ but estimates its variance by
$(1 + \|\hat{\bm{\alpha}}\|_2^2)\hat{\bm{\Sigma}}$.
%%% does RUV-4 also do this variance estimation?.  IE is it more like NC or NC-ASY?
We compare four methods in the SVA/LEAPP/sparsity family:
these are ``IRW-SVA'' \citep{leek2008},  ``LEAPP'' \citep{sun2012},
the ``LEAPP(RR)'' method which is our RR estimator using M-estimation at the robustness stage and
computes the test-statistics using \eqref{eq:test-statistic}, and
 the ``LEAPP(RR-MAD)'' method which uses the median absolute deviation (MAD) of
the test statistics in \eqref{eq:test-statistic} to calibrate them.
(see \Cref{sec:hypothesis-testing})% with the customary scaling to match
% the standard deviation for a Gaussian distribution to estimate the standard deviation of $\hat{\bm \beta}^\mathrm{RR}$

To measure the performance of these methods, we report the type I
error (\Cref{cor:type-I}), power, false discovery proportion (FDP)
and precision of hypotheses with the smallest $100$ p-values
in the $100$ simulations. For both the type I error and power, we set
the significance level to be $0.05$. For FDP, we use
Benjamini-Hochberg procedure with FDR controlled at $0.2$. These
metrics are plotted in \Cref{fig:p-5000-methods} under different
settings of $n$ and $r$.
 % In \Cref{fig:p-5000-methods}, we show the average of these measurements over $B = 100$ repeated experiments for each
% of the four $n$ and $r$ combinations. We also provides one standard deviation error bars for these measurements.

% \subsubsection{Strong confounding factors}
% \label{sub:strong}

\begin{figure}[hp]
  \centering
   \includegraphics[width = \textwidth]{plots/sim_strong50.pdf}
  \caption{\small Compare the performance of nine different approaches (from
  left to right): naive regression ignoring the confounders (Naive),
  IRW-SVA, negative control with finite sample
  correction (NC) in \cref{eq:nc-var-delta}, negative control with asymptotic oracle variance (NC-ASY) in
  \cref{eq:nc-var-oracle},  RUV-4,  robust regression (LEAPP(RR)),
  robust regression with calibration (LEAPP(RR-MAD)),
   LEAPP, oracle regression which observes the confounders (Oracle).
   The error bars are one
  standard deviation over $100$ repeated simulations. The
  three dashed horizontal lines from bottom to top are the nominal significance level, FDR level and oracle power, respectively.}
  \label{fig:p-5000-methods}
\end{figure}


%\begin{figure}[hp]
%  \centering
%  \begin{subfigure}[b]{0.45\textwidth}
%  \includegraphics[width = \textwidth]{plots/n_100_r_2_p_5000_sparsity_005.pdf}
%  \caption{$n = 100$ and $r = 2$}
%  \label{fig:100-2-methods}
%  \end{subfigure}
%  \qquad
%  \begin{subfigure}[b]{0.45\textwidth}
%  \includegraphics[width = \textwidth]{plots/n_100_r_10_p_5000_sparsity_005.pdf}
%  \caption{$n = 100$ and $r = 10$}
%  \label{fig:100-10-methods}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.45\textwidth}
%  \includegraphics[width = \textwidth]{plots/n_500_r_2_p_5000_sparsity_005.pdf}
%  \caption{$n = 500$ and $r = 2$}
%  \label{fig:500-2-methods}
%  \end{subfigure}
%  \qquad
%  \begin{subfigure}[b]{0.45\textwidth}
%  \includegraphics[width = \textwidth]{plots/n_500_r_10_p_5000_sparsity_005.pdf}
%  \caption{$n = 500$ and $r = 10$}
%  \label{fig:500-10-methods}
%  \end{subfigure}
%  \caption{Compare the performance of nine different approaches. The error bars for type I error and Fdp are one
%  standard deviation error bars over $100$ repeated simulations. The three dotted lines are for a reference of
%  the nominated significance level, controled FDR level and the power that the oracle method achieves respectively.}
%  \label{fig:p-5000-methods}
%\end{figure}

First, from \Cref{fig:p-5000-methods}, we see that the oracle method has exactly the same type I error
and FDP as specified, while the naive method and SVA fail drastically.
SVA performs performs better than the naive method in terms of the precision of the smallest $100$
p-values, but is still much worse than other methods.
Next, for the
negative control scenario, as we only have $|\mathcal{C}| = 30$ negative controls, ignoring the inflated variance term
$\bm{\Delta}_S$ in \Cref{thm:asymptotics-nc} will lead to
overdispersed test statistics, and that's why
the type I error and FDP of both NC-ASY and RUV-4 are much larger than the
nominal level. %As we have discussed in \Cref{sec:ruv}, the estimator
%RUV-4 is quite similar to our NC-ASY, and
%also fails to control for type I error and FDP.
%neither does RUV-4
%consider the variance inflation when $|\mathcal{C}|$ is small.
By contrast, the NC method correctly controls type I error and FDP
by considering the variance inflation, %when $|\mathcal{C}|$ is small,
though as expected it loses some power compared with the oracle.
%as only the negative controls are used when estimating $\bm{\alpha}$.
For the sparsity scenario, the ``LEAPP(RR)'' method performs as the
asymptotic theory predicted when $n = 500$,
while when $n = 100$ the p-values seem a bit too small.
%the MAD empirical calibration of variance is needed when $n$ drops to $100$.
This is not surprising because the
asymptotic oracle variance in \Cref{thm:asymptotics-rr} can be
optimistic when the sample size is not sufficiently large, as we discussed in \Cref{rmk:calibration}.
On the other hand, the methods which use empirical calibration
for the variance of test statistics, namely the original LEAPP and ``LEAPP(RR-MAD)'',  control
both FDP and type I error for data of small sample size in our simulations.
%Also, as this calibration
%technique is also used in LEAPP, LEAPP performs very similar to ``RR-MAD''.
The price for the finite sample calibration is that it tends to be slightly
conservative, resulting in a loss of power to some extent.

In conclusion, the simulation results
are consistent with our theoretical guarantees when $p$ is as large as $5000$
and $n$ is as large as $500$. When $n$ is small, the variance of the test statistics will
be larger than the asymptotic variance for the sparsity scenario and we can use empirical calibrations (such as MAD)
to adjust for the difference.


% \subsubsection{Weak confounding factors}
% \label{sub:weak}
% %In the second simulation experiment,
% We then consider how weaker factors can
% affect the validity of the test statistics. This is studied
% theoretically in \Cref{sec:weak-factors}.

% Instead of generating noise with unequal variances from an
% inverse-Gamma distribution, we follow the assumption in
% \Cref{sec:weak-factors} and set $\sigma_i^2 \equiv 1$. Also, PCA
% is used to estimate the latent factors.
% %is equivalent to maximum likelihood in this case.
% For the factor strength $\bm D$, we include one strong factor $d_1 = 3 \sqrt p$ and one undetectable factor
% $d_r^2 = \sqrt{p/n}$. When $r = 10$, we generate
% the additional $8$ factors $d_2$ to $d_9$
% as weaker factors that are above the detection
% threshold of PCA. The estimated number of factors will be $\hat{r} =
% 1$ when $r = 2$ and $\hat{r} = 9$ when $r = 10$ (see \Cref{app:weak-simu} for more details). Other parameters are generated the same as before. The simulation results are shown in \Cref{fig:p-5000-weak-methods}.

% \begin{figure}[hp]
%   \centering
%    \includegraphics[width = \textwidth]{plots/sim_weak.pdf}
%   \caption{Compare the performance of the nine different approaches
%     in presense of weaker factors. The
%   three dashed horizontal lines from below to above are the nominated significance level, FDR level and oracle power, respectively.}
%   \label{fig:p-5000-weak-methods}
% \end{figure}

% %\Cref{fig:p-5000-weak-methods} shows the performance of the nine
% %different approaches in the second simulation experiment.
% From \Cref{fig:p-5000-weak-methods}, the most
% important conclusion is that several methods, namely RUV-4, NC-ASY, NC and
% RR, fail to control the type I error and FDR in presence of weak factors,
% in contrast to the strong factor only setting in
% \Cref{sub:strong}. This is due to the asymptotic distributions given
% by \Cref{thm:asymptotics-nc,thm:asymptotics-rr} being no longer correct
% in presence of weak factors, as discussed in
% \Cref{sec:weak-factors}. In this particular experiment, LEAPP and
% RR-MAD, which include an empirical calibration step of the test
% statistics, are able to control the type I error and FDR.

% Surprisingly, all the methods in \Cref{fig:p-5000-weak-methods} have power
% higher than the oracle when $r = 2$, which contradicts the
% intuition that the oracle should always be the best (LEAPP and RR-MAD
% have about the same type I error and FDR as the oracle). This
% paradox can be easily explained by the classical ``bias-variance
% tradeoff''. Although the oracle knows $\bm Z$,
% there is still uncertainty remaining in estimating $\bm \Gamma$ which
% in turns increases the variance of $\hat{\bm \beta}$ by a constant
% factor $1 + \|\bm \alpha\|_2^2$, which doesn't depend on
% $\bm\Gamma$. On the other hand, %for factor analysis
% in our simulation
% setting when $r = 2$, there is always one
% strong factor that can be estimated very accurately by PCA and one
% undetectable factor that is neglected. Neglecting the undetectable
% factor is equivalent to forcing the
% estimate of $\alpha_2$ to $0$, which decreases the variance inflation
% factor of $\hat{\bm \beta}$ from $1 +  \alpha_1^2 + \alpha_2^2$ to  $1
% + \alpha_1^2$ while increasing the bias of $\hat{\bm \beta}$ from
% $\bm{0}$ to $\alpha_2 \bm{\Gamma}_{\cdot 2}$. Each entry of the weak
% factor $\bm{\Gamma}_{\cdot 2}$ is quite small, therefore the increase
% of bias is much smaller than the decrease of variance. %when the
% %neglected factor(s) are small.
% A more detailed argument of this tradeoff can be found in \Cref{app:weak-simu}.

% Lastly we want to point out $\tilde{\bm\Gamma}$ in this simulation is
% generated uniformly from Stiefold manifold, which makes the bias term $\alpha_2
% \bm{\Gamma}_{\cdot 2}$ behave like increased variance of $\hat{\bm
%   \beta}$. This is the reason why the empirically calibrated methods
% such as RR-MAD and LEAPP can control the type I error and FDR in the case of $r=2$. However in general,
% when the weak factors loadings are arbitrary, there is no guarantee that the empirical
% calibration method can still debias the confounder adjustment methods
% including NC and RR.
% % in the noise term whose
% % magnitude is proportional to the strengh of the neglected factor.
% % Thus, when the neglected factor
% % is small enough, we would then rather ignore it than using it, let alone
% % estimating it when factors are in fact unknown.
% % A detailed calculation
% % in \Cref{app:weak-simu} shows that a factor should
% % at least have strength $d_i^2 > \frac{p}{n}$
% % to be included in our simulation setting.


\subsection{Real data examples}
\label{sec:gender-study}

In this section, we return to the three motivating real data examples in
\Cref{sec:introduction}. The main goal here is to demonstrate a practical
procedure for confounder adjustment and show that our asymptotic results
are reasonably accurate in real data. In an open-source R package \texttt{cate}
(available on CRAN), we also provide the necessary tools to carry
out the procedure.

\subsubsection{The datasets}
\label{sec:datasets}

First we briefly describe the three datasets. The first dataset
\citep{singh2011} is tries to identify candidate genes associated with
the extent of emphysema and can be downloaded from the GEO database
(Series GSE22148). We preprocessed the data using the standard
Robust Multi-array Average (RMA) approach \citep{irizarry2003}. The primary variable of interest is
the severity (moderate or severe) of the Chronic Obstructive Pulmonary Disease (COPD). The dataset also
include age, gender, batch and date of the $143$ sampled patients which are served as nuisance covariates.
%but we
%find that adding these covariate to the linear regression does little
%to change to the t-statistics of interest.

The second and third datasets are taken from \citet{gagnon2013} where they used them to
compare RUV methods with other methods
such as SVA and LEAPP. The original scientific studies are
\citet{vawter2004} and \citet{blalock2004}, respectively.
The primary variable of interest is gender in both datasets, though
the original objective in \citet{blalock2004} is to identify genes
associated with Alzheimer's disease. \citet{gagnon2013} switch the
primary variable to gender in order to have a gold standard: the
%%% the term 'gold standard' is historical referring to at time when the US
%%% dollar was redeemable for gold.  The standard came and went several
%%% times in the 20th century.
differentially expressed genes should mostly come from or relate to
the X or Y chromosome. We follow their suggestion and use this
standard to study the performance of our RR estimator. In addition, as the first COPD dataset
also contains gender information of the samples, we apply this suggestion and
use gender as the primary variable for the COPD data as a supplementary dataset.

Finally, we want to mention that the second dataset has repeated samples from the same
individuals while the individual information is lost. We
suspect that the individual information are then strong latent factors
%(and of course confounded with gender)
which caused the atypical
concentration of the histograms in \Cref{fig:gender-naive} and \Cref{fig:gender-batch}.
%We will show later that the historgram can be corrected after confounder adjustment.
This suggests necessity of a latent factor model for this dataset.

\subsubsection{Confounder adjustment}
\label{sec:conf-adjustm}

Recall that without the confounder adjustment,
the distribution of the regression $t$-statistics in these datasets
can be skewed, noncentered, underdispersed, or overdispersed as shown
in \Cref{fig:confounding-problem}. The adjustment method used here is the
maximum likelihood factor analysis described in
\Cref{sec:inference-gamma-sigma} followed by the robust regression
(RR) method with Tukey's bisquare loss described in
\Cref{sec:unkn-zero-indic}. Since the true number of confounders is unknown, we increase
$r$ from $1$ to $n/2$ and study the empirical performance. We report the results without
empirical calibration for illustrative purposes, though in practice we suggest using
calibration for better control of type I errors and FDP.

% latex table generated in R 3.2.1 by xtable 1.7-4 package
% Sat Dec 26 01:33:26 2015
\setlength{\tabcolsep}{3pt}
\begin{table}[hp]
\centering
\begin{subtable}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{|$r|^r^r^r^r^r^r|^r^r|}
  \hline
r & mean & median & sd & mad & skewness & medc. & \#sig. & p-value \\
  \hline
0 & -0.16 & 0.024 & 2.65 & 2.57 & -0.104 & -0.091 & 164 &  NA\\
  1 & -0.45 & -0.39 & 2.85 & 2.52 & -0.25 & 0.00074 & 1162 & 0.0057 \\
  2 & 0.012 & -0.039 & 1.35 & 1.33 & 0.139 & 0.042 & 542 & $<$1e-10 \\
  3 & 0.014 & -0.05 & 1.43 & 1.41 & 0.169 & 0.048 & 552 & $<$1e-10 \\
  % 4 & 0.013 & -0.065 & 1.48 & 1.44 & 0.207 & 0.057 & 621 & $<$1e-10 \\
  5 & -0.029 & -0.11 & 1.52 & 1.48 & 0.236 & 0.057 & 647 & $<$1e-10 \\
  7 & -0.1 & -0.14 & 1.42 & 1.35 & 0.109 & 0.027 & 837 & $<$1e-10 \\
  10 & -0.06 & -0.085 & 1.13 & 1.12 & 0.103 & 0.022 & 506 & $<$1e-10 \\
  % 15 & -0.11 & -0.11 & 1.13 & 1.13 & 0.0375 & 0.0035 & 464 & $<$1e-10 \\
  20 & -0.083 & -0.095 &  1.2 & 1.19 & 0.0604 & 0.0095 & 479 & $<$1e-10 \\
  % 30 & -0.1 & -0.11 & 1.29 & 1.27 & 0.0599 & 0.0088 & 567 & $<$1e-10 \\
  \rowstyle{\bfseries}
  33 & -0.099 & -0.11 & 1.33 &  1.3 & 0.0727 & 0.0056 & 579 & $<$1e-10 \\
  40 & -0.1 & -0.12 & 1.43 &  1.4 & 0.0775 & 0.0072 & 585 & $<$1e-10 \\
  50 & -0.16 & -0.17 & 1.58 & 1.53 & 0.0528 & 0.0032 & 678 & $<$1e-10 \\
   \hline
\end{tabular}
\caption{\small Dataset 1 ($n = 143$, $p = 54675$). Primary variable:
  severity of COPD.}
\label{tab:COPD}
\end{subtable}


\begin{subtable}[t]{\textwidth}
\centering
\footnotesize

\begin{tabular}{|$r|^r^r^r^r^r^r|^r^r^r^r|}
  \hline
r & mean & median & sd & mad & skewness & medc. & \#sig. & X/Y & top 100 & p-value \\
  \hline
0 & 0.11 & 0.043 & 0.36 & 0.237 & 2.99 & 0.2 & 1036 & 58 & 11 &  NA\\
  1 & -0.44 & -0.47 & 1.06 & 1.04 & 0.688 & 0.035 & 108 & 20 & 20 & 0.74 \\
  2 & -0.14 & -0.15 & 1.15 & 1.13 & 0.601 & 0.015 & 113 & 21 & 21 & 0.31 \\
  3 & 0.013 & 0.012 & 1.13 & 1.08 & 0.795 & -0.01 & 168 & 34 & 28 & 0.03 \\
  % 4 & 0.022 & 0.023 & 1.21 & 1.16 & 0.631 & -0.0048 & 176 & 30 & 27 & 0.042 \\
  5 & 0.044 & 0.019 & 1.18 & 1.08 & 0.878 & 0.017 & 238 & 32 & 27 & 0.0083 \\
  7 & 0.03 & 0.012 & 1.26 & 1.15 & 0.784 & 0.0062 & 269 & 35 & 25 & 0.006 \\
  10 & 0.023 & 0.00066 & 1.36 & 1.24 & 0.661 & 0.011 & 270 & 38 & 27 & 0.019 \\
  15 & 0.049 & 0.022 & 1.46 & 1.31 & 0.584 & 0.012 & 296 & 36 & 29 & 0.00082 \\
  20 & 0.029 & -0.0009 & 1.53 & 1.36 & 0.502 & 0.019 & 314 & 36 & 28 & 7.2e-07
  \\
  \rowstyle{\bfseries}
  25 & 0.048 & 0.012 & 1.68 & 1.48 & 0.452 & 0.026 & 354 & 37 & 27 & 1.1e-06 \\
  30 & 0.026 & 0.012 & 1.82 & 1.61 & 0.436 & 0.0068 & 337 & 40 & 27 & 8.7e-08 \\
  40 & 0.061 & 0.046 & 2.07 & 1.79 & 0.642 & 0.0028 & 363 & 41 & 27 & 7.7e-10 \\
   \hline
\end{tabular}
%
%\begin{tabular}{|$r|^r^r^r^r^r^r|^r^r^r|}
%  \hline
%r & mean & median & sd & mad & skewness & medcouple & \#sig. & X/Y & top 100 \\
%  \hline
%0 & 0.11 & 0.043 & 0.36 & 0.237 & 2.99 & 0.2 & 1036 & 58 & 11 \\
%  1 & -0.34 & -0.36 & 1.03 & 1.01 & 0.74 & 0.033 & 117 & 21 & 20 \\
%  2 & -0.079 & -0.086 & 1.14 & 1.12 & 0.612 & 0.011 & 113 & 21 & 21 \\
%  3 & 0.0061 & 0.00086 & 1.12 & 1.07 & 0.818 & -0.0021 & 164 & 33 & 28 \\
%  4 & 0.02 & 0.024 &  1.2 & 1.15 & 0.65 & -0.0099 & 176 & 29 & 27 \\
%  5 & -0.0047 & -0.025 & 1.18 & 1.09 & 0.847 & 0.013 & 242 & 33 & 28 \\
%  7 & -0.01 & -0.023 & 1.26 & 1.16 & 0.778 & -0.000074 & 259 & 35 & 27 \\
%  10 & -0.0024 & -0.011 & 1.37 & 1.26 & 0.632 & -0.0038 & 251 & 35 & 30 \\
%  15 & -0.00027 & -0.014 & 1.46 & 1.34 & 0.554 & 0.00026 & 269 & 36 & 29 \\
%  20 & 0.0076 & -0.029 & 1.52 &  1.4 & 0.476 & 0.029 & 263 & 37 & 29
%  \\
%\rowstyle{\bfseries}
%  25 & 0.0069 & -0.027 & 1.65 & 1.51 & 0.422 & 0.024 & 274 & 39 & 28 \\
%  30 & 0.0054 & -0.023 & 1.77 &  1.6 & 0.441 & 0.019 & 299 & 40 & 30 \\
%  40 & 0.0091 & -0.0092 & 1.98 & 1.78 & 0.526 & 0.0075 & 295 & 40 & 29 \\
%   \hline
%\end{tabular}
\caption{\small Dataset 2 ($n = 84$, $p = 12600$). Primary variable: gender.}
\label{tab:gender}
\end{subtable}

\begin{subtable}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{|$r|^r^r^r^r^r^r|^r^r^r^r|}
  \hline
r & mean & median & sd & mad & skewness & medc. & \#sig. & X/Y & top 100 & p-value \\
  \hline
0 & -1.8 & -1.8 & 0.599 & 0.513 & -3.46 & 0.082 & 418 & 39 & 20 &  NA\\
  1 & -0.55 & -0.56 & 1.09 & 1.01 & -1.53 & 0.01 & 261 & 29 & 23 & 0.00024 \\
  2 & -0.2 & -0.22 &  1.2 & 1.11 & -0.99 & 0.014 & 320 & 38 & 22 & 0.00014 \\
  3 & -0.096 & -0.12 & 1.27 & 1.18 & -0.844 & 0.017 & 311 & 42 & 25 & 0.00014 \\
  % 4 & -0.16 & -0.17 &  1.3 & 1.23 & -0.8 & 0.0095 & 275 & 37 & 27 & 3.4e-05 \\
  5 & -0.33 & -0.32 & 1.31 & 1.22 & -1.29 & -0.011 & 305 & 35 & 23 & 2.1e-07 \\
  7 & -0.37 & -0.36 & 1.46 & 1.36 & -0.855 & -0.0099 & 300 & 38 & 23 & 4.0e-07 \\
  % 9 & -0.27 & -0.25 & 1.48 & 1.38 & -0.791 & -0.019 & 337 & 41 & 28 & 7.0e-08 \\
  \rowstyle{\bfseries}
  11 & -0.13 & -0.12 & 1.51 & 1.36 & -0.601 & -0.0051 & 432 & 48 & 31 & 1.8e-09 \\
  % 13 & -0.099 & -0.1 & 1.66 & 1.49 & -0.886 & 0.006 & 448 & 49 & 28 & 1.3e-08 \\
  15 & -0.12 & -0.13 & 1.83 & 1.62 & -0.341 & 0.013 & 492 & 54 & 25 & 2.3e-08 \\
  20 & -0.13 & -0.14 & 2.61 & 2.23 & -0.327 & 0.0045 & 613 & 50 & 26 & 4.0e-06 \\
   \hline
\end{tabular}
\caption{\small Dataset 3 ($n = 31$, $p = 22283$). Primary variable: gender.}
\label{tab:alzheimers}
\end{subtable}
\caption{\small Summary of the adjusted z-statistics. The first group is
  summary statistics of the z-statistics before the empirical
  calibration. The second group is some performance metrics after the
  empirical calibration, including total number of significant genes
  of p-value less than $0.01$ in
  \Cref{rmk:calibration} (\#sig.), number of the genes on X/Y
  chromosome that have p-value less than $0.01$ (X/Y), the number
  among the $100$ most significant genes that are on the X/Y
chromosome (top 100) and the p-value of the confounding test in \Cref{sec:test-confound}.
The bold row corresponds to the $r$ selected by BCV (\Cref{fig:output}).}
\label{tab:output}
\end{table}


\begin{figure}[hp]
  \centering
  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/COPD-bcv.pdf}
  \caption{\small Dataset 1: BCV selects $r=33$.}
  \label{fig:COPD-bcv}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/COPD-output.pdf}
  \caption{\small Dataset 1: histogram. }
  \label{fig:COPD-t}
  \end{subfigure} \\

  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/gender-bcv.pdf}
  \caption{\small Dataset 2: BCV selects $r=25$.}
  \label{fig:gender-bcv}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/gender-output.pdf}
  \caption{\small Dataset 2: histogram. }
  \label{fig:gender-t}
  \end{subfigure} \\

  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/alzheimers-bcv.pdf}
  \caption{\small Dataset 3: BCV selects $r=11$.}
  \label{fig:alzheimers-bcv}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.42\textwidth}
  \includegraphics[width = \textwidth]{plots/alzheimers-output.pdf}
  \caption{\small Dataset 3: histogram.}
  \label{fig:alzheimers-t}
  \end{subfigure}

  \caption{\small Histograms of z-statistics after confounder adjustment (without calibration)
    using the number of confounders $r$ selected by
    bi-cross-validation.}
  \label{fig:output}

\end{figure}

In \Cref{tab:output} and \Cref{fig:output}, we present the results after
confounder adjustment for the three datasets. % The results of using gender as the primary
% variable for COPD data as a supplementary dataset is in \Cref{app:copd_add_table}.
We report
two groups of summary statistics in \Cref{tab:output}: the first group is several
summary statistics of all the z-statistics computed using
\cref{eq:test-statistic}, %without the empirical calibration,
including the mean, median, standard
deviation, median absolute deviation (scaled for consistency
of normal distribution), skewness, and
the medcouple.
The medcouple \citep{brys2004}) is a robust measure of skewness.
After subtracting the median observation some positive and some
negative values remain.  For any pair of values $x_1\ge 0$ and $x_2\le0$
with $x_1+|x_2|>0$ one can compute $(x_1-|x_2|)/(x_1 +|x_2|)$. The medcouple is the median
of all those ratios.
The second group of statistics has performance metrics to
evaluate the effectiveness of the confounder adjustment. See
the caption of \Cref{tab:output} for more detail.

In all three datasets, the z-statistics become more centered at $0$ and
less skewed as we include a few confounders in the model.
Though the standard deviation (SD) suggests overdispersed variance,
the overdispersion will go away if
we add MAD calibration as SD and MAD have similar values. The
similarity between SD and MAD values also indicates that
the majority of statistics after confounder adjustment are
approximately normally distributed.
Note that %the moment based skewness
%sometimes rises because a small
%fraction of the z-statistics are very large.
the medcouple values shrink towards zero after adjustment,
suggesting that skewness then only arises from small fraction of the genes,
which is in accordance with our assumptions that the primary effects should be sparse.
%but the
%standard deviation or MAD are usually greater than 1. This
%indicates the majority of statistics after confounder adjustment are
%approximately normally distributed with overdispersed variance. This
%observation is in accordance with our theoretical results; see
%\Cref{rmk:calibration} for some discussion on the overdispersed
%variance.

In practice, some latent factors may be too weak to meet
\Cref{assumption:large-factor} (i.e.\ $d_j \ll \sqrt{p}$) , making it
difficult to choose an appropriate $r$.
A practical way to pick the number of confounders $r$
with presence of heteroscedastic noise we investigate here is the
bi-cross-validation (BCV) method of \citet{owen2015}, which uses randomly held-out submatrices to estimate
the mean squared error of reconstructing factor loading matrix. It is
shown in \citet{owen2015} that BCV outperforms many existing methods
in recovering the latent signal matrix and the number of factors $r$, especially in high-dimensional datasets ($n, p\to \infty$).
In \Cref{fig:output},
we demonstrate the performance of BCV on these three datasets. The $r$
selected by BCV is respectively $33$, $25$ and $11$
(\Cref{fig:COPD-bcv,fig:gender-bcv,fig:alzheimers-bcv}), and they all
result in the presumed shape of z-statistics distribution
(\Cref{fig:COPD-t,fig:gender-t,fig:alzheimers-t}). For the second and
the third datasets where we have a gold standard, the $r$ selected
by BCV has near optimal performance in selecting genes on the X/Y chromosome
(columns 3 and 4 in \Cref{tab:gender,tab:alzheimers}).
%For the first dataset, the number of factors chosen by BCV seems to be too large to be trustable, and one can instead use
Another method we applied is proposed by
\citet{onatski2010determining} based on the empirical distribution of
eigenvalues. This method estimates $r$ as $2$, $9$ and $3$ respectively for the three datasets.
% See the survey article by \citet{owen2015} for a comprehensive comparison of these methods.
% In \Cref{tab:gender}, we demonstrate the performance of the LEAPP(RR) method.
% Because LEAPP and LEAPP(RR-MAD) rank the genes in the same order as RR they
% have the same values as RR for the X/Y and top 100 criteria to which the
% gold standard applies. These criteria are not very sensitive to the number of
% latent factors included in the gender data models.
Table 3 of \citet{gagnon2013} has the ``top 100'' values for RUV-4 on the second and third dataset.
%%% lets make sure this is right.  I am not sure whether our datasets 2 and 3
%%% exactly the same as their preprocessed and not preprocessed data.
%%% Also Terry and others are sure to make the comparison if we don't do it.
They reported 26 for LEAPP, 28 for RUV-4, and 27 for SVA in the second dataset,
and 27 for LEAPP, 31 for RUV-4, and 26 for SVA in the third dataset.
Notice that the precision of the top $100$ significant genes is relatively stable when $r$
is above certain number. %Indeed, the confounder adjustment methods (NC
%and RR) studied in this paper are relatively robust to overestimating
%$r$.
% Intuitively, this is because that the overestimated factors have very small singular values
% thus having negligible influence in estimating $\bm \beta$.
Intuitively, the factor analysis is applied to
the residuals of $\bm{Y}$ on $\bm{X}$ and the overestimated factors
also have very small eigenvalues, thus they usually do not change
$\hat{\bm{\beta}}$ a lot. See also
\citet{gagnon2013} for more discussion on the robustness of the
negative control estimator to overestimating $r$.
% The influnce of $r$ in estimating $\sigma_i$ and the validity of p-values dependents on how
% \Cref{assumption:large-factor} is satisfied on the real dataset, and is beyond the scope of
% this paper.

Lastly we want to point out that both the small sample size of the datasets
and presence of weak factors can result in overdispersed variance of the test statistics.
The BCV plots indicate presence of many weak factors in the first two datasets.
In the third
dataset, the sample size $n$ is only $31$, so the adjustment result is
not ideal. Nevertheless, the empirical
performance (e.g.\ number of X/Y genes in top $100$) suggests it
is still beneficial to adjust for the confounders.


%Lastly we want to comment on the sample size $n$. Our entire
%asymptotic analysis is based on $r$ fixed and $n,p \to \infty$. In the third
%dataset, the sample size $n$ is only $31$, so the adjustment result is not ideal. In
%\Cref{tab:alzheimers}, adding the first two confounders significantly
%reduces the mean and skewness of the statistics, but the mean and
%median of the statistics remain negative no matter how many factors
%are used. A possible explanation is that the sample size $n$ is too small to
%estimate the confounders accurately.


==> revision 2/infer_beta.tex <==
% is editing

The estimation of $\bm{\alpha}$ and $\bm{\beta}$ is based on the
first row of the rotated outcome $\tilde{\bm{Y}}_1$ in \eqref{eq:Y-tilde-1}, which can be
rewritten as
\begin{equation} \label{eq:y-tilde-1}
  \tilde{\bm{Y}}_1^T / \|\bm{X}\|_2 = \bm{\beta} + \bm{\Gamma}
  (\bm{\alpha} + \tilde{\bm{W}}_1 / \|\bm{X}\|_2) + \tilde{\bm{E}}_{1}^T / \|\bm{X}\|_2
\end{equation}
where $\tilde{\bm{W}}_1 \sim \mathrm{N}(0, \bm{I}_p)$ is from
\cref{eq:Z-tilde} and $\tilde{\bm{W}}_1$ is independent of $\tilde{\bm{E}}_1 \sim
\mathrm{N}(0, \bm{\Sigma})$. Note that $\tilde{\bm
  Y}_{1}/\|\bm{X}\|_2$ is proportional to the sample covariance
between $\bm Y$ and $\bm X$.
All the methods described in this section
first try to find a good estimator $\hat{\bm{\alpha}}$.
% of$\bm{\alpha}$
They then use $\hat{\bm{\beta}} = \tilde{\bm{Y}}_1^T/\|\bm{X}\|_2 -
\hat{\bm{\Gamma}} \hat{\bm{\alpha}}$ to estimate $\bm{\beta}$.
%As
%mentioned earlier, the estimators of $\bm{\alpha}$ are different under the two identifiability conditions.

To reduce variance, we choose to estimate \eqref{eq:y-tilde-1} conditional on $\tilde{\bm{W}}_1$.
% Notice that we don't need to separate estimating of $\bm{\alpha}$ from
%the random term $\tilde{\bm{W}}_1/\|\bm{X}\|_2$ in \eqref{eq:y-tilde-1}.
 Also, to use the results in \Cref{lem:ml-baili}, we replace $\bm{\Gamma}$ by $\bm{\Gamma}^{(0)}$.
% as mentioned earlier in \Cref{rmk:rotation}, $\hat{\bm{\Gamma}}$ is
%actually closer to $\bm{\Gamma} \bm{R}$ than $\bm{\Gamma}$.
%To deal with this issue,
Then, we can rewrite \eqref{eq:y-tilde-1} as
\begin{equation} \label{eq:y-tilde-1-0}
  \tilde{\bm{Y}}_1^T / \|\bm{X}\|_2 = \bm{\beta} + \bm{\Gamma}^{(0)}
  \bm{\alpha}^{(0)} + \tilde{\bm{E}}_1^T / \|\bm{X}\|_2
\end{equation}
where $\bm{\Gamma}^{(0)} = \bm{\Gamma} \bm{R}$ and $\bm{\alpha}^{(0)} =
\bm{R}^{-1} (\bm{\alpha} + \tilde{\bm{W}}_1 / \|\bm{X}\|_2)$. Notice that the random $\bm{R}$
%is random, it
only depends on $\tilde{\bm{Y}}_{-1}$ and
thus is independent of $\tilde{\bm{Y}}_1$.
%For the other random quantity $u$,
In the proof of the results in this section, we first consider the estimation
of $\bm{\beta}$ for fixed $\tilde{\bm{W}}_1$, $\bm{R}$ and $\bm{X}$,
% and hence $\bm{\alpha}^{(0)}$,
and then show the asymptotic distribution of $\hat{\bm{\beta}}$
indeed does not depend on $\tilde{\bm{W}}_1$, $\bm{R}$ or $\bm{X}$, and thus also holds unconditionally.

\subsubsection{Negative control scenario}
\label{sec:known-zero-indices}

If we know a set $\mathcal{C}$ such that $\bm{\beta}_{\mathcal{C}} = 0$
(so $\bm{\Theta} \subset \bm{\Theta}_1$), then $\tilde{\bm{Y}}_1$ can be correspondingly separated into two parts:
\begin{equation} \label{eq:y-tilde-1-separate}
  \begin{split}
  \tilde{\bm{Y}}_{1,\mathcal{C}}^T / \|\bm{X}\|_2 &=
  \bm{\Gamma}_{\mathcal{C}}^{(0)} \bm{\alpha}^{(0)} +
  \tilde{\bm{E}}_{1,\mathcal{C}}^T / \|\bm{X}\|_2, \quad\text{and}\\
  \tilde{\bm{Y}}_{1,-\mathcal{C}}^T / \|\bm{X}\|_2 &= \bm{\beta}_{-\mathcal{C}} +
  \bm{\Gamma}_{-\mathcal{C}}^{(0)} \bm{\alpha}^{(0)} + \tilde{\bm{E}}_{1,-\mathcal{C}}^T / \|\bm{X}\|_2.
  \end{split}
\end{equation}
This estimator matches the RUV-4 estimator of \cite{gagnon2013}
except that it uses quasi-maximum likelihood estimates of $\bm{\Sigma}$
and $\bm{\Gamma}$ instead of using PCA, and generalized linear squares
instead of ordinary linear squares regression. The details are in Section~\ref{sec:ruv}.
%%% we should describe the matchup right here so that Terry Speed
%%% and Gagnon-Bartsch see right away that we are honoring their contribution

The number of negative controls $|\mathcal{C}|$ may grow as $p \to \infty$.
We impose an additional assumption on the latent factors of the negative controls.

\begin{assumption}\label{assumption:nc-factor}
 % The limit
 $\lim_{p \to \infty}|\mathcal{C}|^{-1}
 \bm{\Gamma}^T_\mathcal{C}\bm{\Sigma}_{\mathcal{C}}^{-1}\bm{\Gamma}_\mathcal{C}$
 exists and is positive definite.
\end{assumption}

We consider the following negative control (NC) estimator where $\bm{\alpha}^{(0)}$ is estimated by generalized least squares:
\begin{align}
  &\hat{\bm{\alpha}}^{\mathrm{NC}} = (\hat{\bm{\Gamma}}_{\mathcal{C}}^T
  \hat{\bm{\Sigma}}_{\mathcal{C}}^{-1}
  \hat{\bm{\Gamma}}_{\mathcal{C}})^{-1}
  \hat{\bm{\Gamma}}_{\mathcal{C}}^T \hat{\bm{\Sigma}}_{\mathcal{C}}^{-1}
  \tilde{\bm{Y}}_{1,\mathcal{C}}^T / \| \bm{X} \|_2,~\mathrm{and} \label{eq:alpha-nc} \\
  &\hat{\bm{\beta}}^{\mathrm{NC}} = \tilde{\bm{Y}}_{1,-\mathcal{C}}^T / \| \bm{X} \|_2 -
  \hat{\bm{\Gamma}}_{-\mathcal{C}}
  \hat{\bm{\alpha}}^{\mathrm{NC}}. \label{eq:beta-nc}
\end{align}

Our goal is to show consistency and asymptotic variance of $\hat{\bm{\beta}}^{\mathrm{NC}}_{-\mathcal{C}}$.
Let $\bm \Sigma_\mathcal{C}$ represents the noise covariance matrix of the variables in $\mathcal{C}$. % and $\Sigma_{-\mathcal{C}}$ represent
 % the noise covariance matrix of the variables in $-\mathcal{C}$, then
 We then have

% \begin{remark}
% We name the estimator NC because of its similarity to the two-stage
% least squares in instrumental variable regression. The first least
% squares is implicit in our derivation through the rotation in
% \eqref{eq:Y-tilde}. The second least squares is the least squares on
% the negative controls in \eqref{eq:alpha-nc}. Indeed
% \citep{gagnon2013} derived exactly the same estimator
% $\hat{\bm{\beta}}^{\textrm{2SULS}}$ through a series of heuristic
% calculations and they name the estimator RUV-4. We refer the reader to
% \Cref{sec:discussions} for more discussions on RUV-4 and its
% relationship to instrumental variable regression.
% \end{remark}

\begin{theorem} \label{thm:asymptotics-nc}
  Under
  \Cref{assumption:error,assumption:bounded,assumption:large-factor,assumption:nc-factor},
  if $n,p \to \infty$ and $p/n^k \to 0$ for some
  $k > 0$, then for any fixed index set $\mathcal{S}$
with finite cardinality and
 $\mathcal{S} \cap \mathcal{C} = \emptyset$, we have
\begin{equation} \label{eq:nc-var-delta}
\sqrt{n} (\hat{\bm{\beta}}^{\mathrm{NC}}_{\mathcal{S}} - \bm{\beta}_{\mathcal{S}}) \overset{d}{\to}
\mathrm{N}(\bm{0}, (1 + \|\bm{\alpha}\|_2^2) (\bm{\Sigma}_{\mathcal{S}} + \bm{\Delta}_{\mathcal{S}}))
\end{equation}
where $\bm{\Delta}_{\mathcal{S}} = \bm{\Gamma}_{\mathcal{S}} (\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
  \bm{\Gamma}_{\mathcal{C}})^{-1} \bm{\Gamma}_{\mathcal{S}}^T$.

If in addition, $|\mathcal{C}| \to \infty$, the minimum eigenvalue
of $\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
\bm{\Gamma}_{\mathcal{C}} \to \infty$ by \Cref{assumption:nc-factor}, then
the maximum entry of $\bm{\Delta}_{\mathcal{S}}$ goes to $0$. Therefore in this case
\begin{equation} \label{eq:nc-var-oracle}
\sqrt{n} (\hat{\bm{\beta}}^{\mathrm{NC}}_{\mathcal{S}} - \bm{\beta}_{\mathcal{S}}) \overset{d}{\to}
\mathrm{N}(\bm{0}, (1 + \|\bm{\alpha}\|_2^2) \bm{\Sigma}_{\mathcal{S}}).
\end{equation}
\end{theorem}

The asymptotic variance in \eqref{eq:nc-var-oracle} is the same as the
variance of the oracle least squares in \eqref{eq:var-beta-oracle}.
Comparable oracle efficiency statements can be found in the econometrics literature
% for the negative control case
%%% it looked like we are saying that econometricians also used negative controls
%%% I think if they did, Speed and Gagnon-Bartsch would have said so.
\citep{bai2006,wang2015}.
This is also the variance
used implicitly in RUV-4 as it treats the estimated
$\bm Z$ as given when deriving test statistics for $\bm \beta$.
%Our estimator $\hat{ \bm \beta}^{\mathrm{NC}}$ is an equally well
%performing alternative to RUV-4, despite that we derive a variance
%inflation term $\bm\Delta_S$ for finite $|\mathcal{C}|$.
%%% I think that this sentence is confusing.  It says that NC
%%% performs as well as RUV-4 despite the variance inflation term.
%%% But that variance is really there, in both estimators.  If I understand
%%% correctly the RUV-4 estimator has that variance, but their methhods
%%% fail to account for it.
When the number
of negative controls is not too large, say $|\mathcal{C}| = 30$, the
correction term $\bm{\Delta}_S$ is nontrivial and gives more accurate
estimate of the variance of $\hat{\bm{\beta}}^{\mathrm{NC}}$. See \Cref{sec:simulations} for more simulation results.

% \begin{remark}
%   Note that
%   we assume $\lim_{p \to \infty}\frac{1}{p} \bm{\Gamma}^T
%   \bm{\Sigma}^{-1} \bm{\Gamma} \succ 0$ in
%   \Cref{assumption:large-factor} to control the error of factor
%   analysis. Therefore, the condition that the minimum eigenvalue of $\bm{\Gamma}_{\mathcal{C}}^T \bm{\Sigma}_\mathcal{C}^{-1}
%   \bm{\Gamma}_{\mathcal{C}} \to \infty$ in theorem \cref{thm:asymptotics-nc} is fairly weak
%   when $|\mathcal{C}| \to \infty$.
%   For example, if $|\mathcal{C}| \to \infty$
%   and the rows of $\bm{\Gamma}$ are i.i.d. random vectors or bounded below, it is easy
%   to verify that condition is satisfied.  % Intuitively
%   % the asymptotic variance derived in \cref{thm:asymptotics-nc}
%   % depends on the number of negative controls and
%   % $\|\bm{\alpha}\|_2^2$, the total correlation
%   % of the latent factors with treatment variable $\bm{X}$. We refer
%   % the readers to \Cref{sec:asympt-effic} (in particualr
%   % \Cref{rmk:alpha-intuition}) for a further discussion.
% \end{remark}


\subsubsection{Sparsity scenario}
\label{sec:unkn-zero-indic}

When the zero indices in $\bm{\beta}$ are unknown but sparse (so $\bm{\Theta}
\subseteq \bm{\Theta}_2$),
the estimation of
$\bm{\alpha}$ and $\bm{\beta}$ from $ \tilde{\bm{Y}}_1^T / \|\bm{X}\|_2 = \bm{\beta} + \bm{\Gamma}^{(0)} \bm{\alpha}^{(0)} + \tilde{\bm{E}}_1^T / \|\bm{X}\|_2$
can be cast as a robust regression by viewing $\tilde{\bm{Y}}_1^T$ as observations and $\bm{\Gamma}^{(0)}$ as design
matrix. The nonzero entries in $\bm{\beta}$ correspond to
outliers in this linear regression. % When $n,p \to \infty$ and
% $\|\bm{\beta}\|_0$ is relatively small, robust regression techniques
% allow us to estimate $\bm{\beta}$ efficiently.

The problem here has two nontrivial differences compared to
classical robust regression. First, we expect some entries of
$\bm{\beta}$ to be nonzero, and our goal is to
%study how many nonzeros
%are allowed to still guarantee consistency
make inference on the outliers; second, we don't observe
the design matrix $\bm{\Gamma}^{(0)}$ but only have its estimator
$\hat{\bm{\Gamma}}$. In fact, if $\bm{\beta} = \bm{0}$ and
$\bm{\Gamma}^{(0)}$ is observed, the ordinary least squares
estimator of $\bm{\alpha}^{(0)}$ is unbiased and has variance of order
$1/(np)$, because the noise in \cref{eq:y-tilde-1} has variance $1/n$
and there are $p$ observations. Our main conclusion is
that $\bm{\alpha}^{(0)}$ can still be estimated very accurately given
the two technical difficulties.

Given a robust loss function $\rho$, we consider the following estimator:
\begin{align}
  \label{eq:alpha-rr}
  &\hat{\bm{\alpha}}^{\mathrm{RR}} = \arg \min \sum_{j=1}^p
  \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T \bm{\alpha}}{\hat{\sigma}_j}\right), ~\text{and}\\
  \label{eq:beta-rr}
  &\hat{\bm{\beta}}^{\mathrm{RR}} = \tilde{\bm{Y}}_1 / \|\bm{X}\|_2 - \hat{\bm{\Gamma}} \hat{\bm{\alpha}}^{\mathrm{RR}}.
\end{align}
For a broad class of loss functions $\rho$, estimating $\bm{\alpha}$ by \cref{eq:alpha-rr} is equivalent to
\begin{equation} \label{eq:sparse-penalty}
(\hat{\bm{\alpha}}^{\mathrm{RR}}, \tilde{\bm{\beta}}) = \arg
\min_{\bm{\alpha}, \bm{\beta}} ~ \sum_{j=1}^p \frac{1}{\hat{\sigma}_j^2} (\tilde{Y}_{1j}/\|\bm X\|_2 -
\beta_j - \hat{\bm{\Gamma}}_j^T \bm{\alpha})^2 + P_{{\lambda}}(\bm{\beta}),
\end{equation}
where $P_{{\lambda}}(\bm{\beta})$ is a penalty to promote sparsity
of $\bm{\beta}$  \citep{she2011}.
%%% This next sentence breaks the flow in our 'same alpha different beta' story.
%%% If it is really important, then we can find a way to put it back in.
%For example, if $\hat{\sigma}_j \equiv \sigma$,
%the Huber loss $\rho$ corresponds to the lasso penalty $P_{\lambda}(\bm{\beta})
%= \lambda \|\bm{\beta}\|_1$.
However $\hat{\bm{\beta}}^{\mathrm{RR}}$ is not identical to
$\tilde{{\bm{\beta}}}$, which is a sparse vector that does not have an asymptotic normal
distribution. The LEAPP algorithm \citep{sun2012} uses the
form~\eqref{eq:sparse-penalty}. Replacing it by the robust regression \cref{eq:alpha-rr,eq:beta-rr} allows us to derive significance tests of $H_{0j}:\beta_j = 0$.
%For this reason, we estimate $\bm{\beta}$
%by \cref{eq:beta-rr} instead of using~\eqref {eq:sparse-penalty}
%, though $\tilde{{\bm{\beta}}}$ may have smaller
%mean squared error %compared to $\hat{\bm{\beta}}^{\mathrm{RR}}$
% due to its shrinkage-type estimation.

% Our goal is to show $\hat{\bm{\beta}}^{\mathrm{RR}}$ is consistent for
% $\bm{\beta}$ and
% calculate its asymptotic variance.
%For analytic tractability we replace the $\Theta$-IPOD robust regression
%used in LEAPP by a smooth M-estimator
%In our numerical work, we use Tukey's $\rho$ corresponding to Tukey's
%biweight $\psi$ function.
We assume a smooth loss $\rho$
for the theoretical analysis:
\begin{assumption} \label{assumption:rho}
The penalty $\rho:\real\to[0,\infty)$
with $\rho(0) = 0$.  The function $\rho(x)$ is non-increasing when $x \leq 0$ and is
  non-decreasing when $x > 0$. The derivative
  $\psi = \rho'$ exists and $|\psi|\le D$ for some $D<\infty$.
Furthermore, $\rho$ is strongly convex in a neighborhood of $0$.
\end{assumption}

A sufficient condition for the local strong convexity is that $\psi' > 0$
exists in a neighborhood of $0$.
The next theorem establishes the consistency of $\hat{\bm{\beta}}^{\mathrm{RR}}$.

% To prove the consistency of $\hat{\bm{\alpha}}^{\mathrm{RR}}$ we
% assume
% \begin{assumption} \label{assumption:uniqueness}
%   $\bm{\alpha}$ is the unique solution to
% \end{assumption}

% \begin{assumption} \label{assumption:strong-convexity}
%   For any $\epsilon > 0$ and $p > p_{\epsilon}$,
% \[
% \inf_{\|\bm{\alpha}\|_2 \ge \epsilon} \left\|
% \frac{1}{p} \sum_{j=1}^p \psi\left(\frac{\bm{\Gamma}_j^T
%     \bm{\alpha}}{\sigma_j}\right) \frac{\bm{\Gamma}_j}{\sigma_j}
% \right\|_2 > 0.
% \]
% \end{assumption}

\begin{theorem} \label{thm:consistency-rr}
    Under \Cref{assumption:error,assumption:bounded,assumption:large-factor,assumption:rho% assumption:uniqueness,
      % assumption:strong-convexity,
      % assumption:psi-2nd-derivative
    },
    if $n,p \to \infty$, $p/n^k \to 0$ for some
  $k > 0$ and $\|\bm{\beta}\|_1/p \to 0$, then $\hat{\bm{\alpha}}^{\mathrm{RR}}
  \overset{p}{\to} \bm{\alpha}$. As a consequence, for any $j$,
  $\hat{{\beta}}_j^{\mathrm{RR}} \overset{p}{\to} {\beta}_j$.
\end{theorem}
% \begin{proof}
%   See \cref{app:consistency-rr}.
% \end{proof}

% For possible relaxations of this classical assumption, we refer the
% reader to \citep[sec. 5.3]{vandervaart2000}.

To derive the asymptotic distribution, we consider the estimating equation corresponding to \eqref{eq:alpha-rr}. By taking the derivative of \eqref{eq:alpha-rr},
$\hat{\bm{\alpha}}^{\mathrm{RR}}$ satisfies
\begin{equation} \label{eq:Psi}
\bm{\Psi}_{p,\hat{\bm{\Gamma}},\hat{\bm{\Sigma}}}(\hat{\bm{\alpha}}^{\mathrm{RR}})
= \frac{1}{p} \sum_{j=1}^p \psi\left( \frac{\tilde{Y}_{1j} /
    \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T
    \hat{\bm{\alpha}}^{\mathrm{RR}}}{\hat{\sigma}_j}\right) \hat{\bm{\Gamma}}_j / \hat{\sigma}_j = \bm{0}.
\end{equation}

The next assumption is used to control the higher order term in a Taylor expansion of $\bm{\Psi}$.
\begin{assumption} \label{assumption:psi-2nd-derivative}
The first two derivatives of $\psi$ exist and both $|\psi'(x)|\le D$ and $|\psi''(x)|\le D$
hold at all $x$ for some $D<\infty$.
 % $\psi'(x)$ is bounded by
 % $D$ for any $x$, $\psi''(x)$ is bounded by $D$ for $x$ in a neighborhood of $0$.
\end{assumption}

Examples of loss functions $\rho$ that satisfy
\Cref{assumption:rho,assumption:psi-2nd-derivative} include smoothed
Huber loss and Tukey's bisquare.

The next theorem gives the asymptotic distribution of
$\hat{\bm{\beta}}^{\mathrm{RR}}$ when the nonzero entries of
$\bm{\beta}$ are sparse enough. The asymptotic variance of
$\hat{\bm{\beta}}^{\mathrm{RR}}$ is, again, the oracle variance in \eqref{eq:var-beta-oracle}.

\begin{theorem} \label{thm:asymptotics-rr}
  Under \Cref{assumption:error,assumption:bounded,assumption:large-factor,assumption:rho%, assumption:uniqueness
    ,assumption:psi-2nd-derivative}, if $n,p \to \infty$, with $p/n^k \to 0$ for some
  $k > 0$ and $\|
  \bm{\beta} \|_1 \sqrt{n}/p \to 0$, then
\[
\sqrt{n} (\hat{\bm{\beta}}_\mathcal{S}^{\mathrm{RR}} - \bm{\beta}_\mathcal{S}) \overset{d}{\to}
\mathrm{N}(\bm{0}, (1 + \|\bm{\alpha}\|_2^2) \bm{\Sigma}_\mathcal{S})
\]
for any fixed index set $S$ with finite cardinality.
\end{theorem}
% \begin{remark}
If $n/p \to 0$,  then a sufficient condition for $\| \bm{\beta} \|_1
\sqrt{n}/p \to 0$ in \Cref{thm:asymptotics-rr} is $\|\bm{\beta} \|_1 = O(\sqrt{p})$.
If instead $n/p \to c \in (0,\infty)$, then $\|\bm{\beta} \|_1 = o(\sqrt{p})$ suffices.
% The identification condition in \Cref{sec:model} only required about half
% of the $\beta_j$ to be zero.
% The $\sqrt{n}$-consistency of $\hat{\bm{\beta}}$
% that we get in \Cref{thm:asymptotics-rr} requires
% more than just that level of sparsity.

%we need the true
%$\bm{\beta}$ to be far more sparse than what is needed for
%identification in \Cref{sec:model}.
%%% is this really extra sparsity?  The L_1 norm could be small for a dense beta.

% We refer the readers to
% \cref{sec:asympt-effic} (in particualr \cref{rmk:alpha-intuition}) for
% a discussion of the asymptotic variance derived in \cref{thm:asymptotics-rr}.
% \end{remark}

% \begin{proof}
% We begin with showing $\hat{\bm{\alpha}}^{\mathrm{RR}}$ is
% consistent for $\bm{\alpha}^{(0)}$ when $n,p \to \infty$. Let
% $\bm{\alpha}'$ be the solution to
% $\bm{\Psi}_{p,\bm{\Gamma}^{(0)},{\bm{\Sigma}}}(\bm{\alpha}) =
% \bm{0}$. Under the assumptions listed in the theorem,
% \citet[thm. 10.16]{maronna2006} ensures that $\bm{\alpha}'
% \overset{p}{\to} \bm{\alpha}^{(0)}$ when $p \to \infty$ if
% $\bm{\beta}=\bm{0}$.
% If $\bm{\beta} \ne \bm{0}$ but $\|\bm{\beta}\|_0
% \sqrt{n}/p \to 0$, the outlier terms $\frac{1}{p} \sum_{\beta_j \ne
%   0} \psi\left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 -
%     \bm{\Gamma}_j^{(0)T}
%     \hat{\bm{\alpha}}^{\mathrm{RR}}}{{\sigma}_j}\right)
% \bm{\Gamma}_j^{(0)} / {\sigma}_j
% \le D^3 \|\bm{\beta}\|_0 / p \to 0$
% have negligible contribution to $\bm{\alpha}'$, so $\bm{\alpha}'
% \overset{p}{\to} \bm{\alpha}^{(0)}$ still holds.
% Using \eqref{eq:avg-sigma-err} and \eqref{eq:avg-gamma-err}, and the boundness of $\bm{\Gamma}^{(0)}$,
% $\sigma_j$ and $\hat \sigma_j$, we have that
% \begin{equation}\label{eq:avg-other-err}
% \frac{1}{p}\sum_{j=1}^p|\hat\sigma_j - \sigma_j| = o_p(1),
% ~\frac{1}{p}\sum_{j = 1}^p\Big|\frac{\hat{\bm{\Gamma_j}}}{\hat\sigma_j} - \frac{\bm{\Gamma}_j^{(0)}}{\sigma_j}\Big| = \bm{o}_p(1)
% \end{equation}
% Note that also $\|\bm{X}\|_2/\sqrt{n} \to 1$,
% we can then do Taylor expansion for $\psi$
% and use \cref{assumption:rho}
%   to obtain
%   \begin{equation}
%     \label{eq:two-psi-difference}
% \bm{\Psi}_{p,\hat{\bm{\Gamma}},{\hat{\bm{\Sigma}}}}(\bm{\alpha}) =
%   \bm{\Psi}_{p,\bm{\Gamma}^{(0)},{\bm{\Sigma}}}(\bm{\alpha}) +
%   \bm{o}_p(1), \forall \bm{\alpha}
%   \end{equation}
% % By continuous
% % mapping theorem $\hat{\bm{\alpha}}^{\mathrm{RR}} \overset{p}{\to}
% % \bm{\alpha}^{(0)}$.
% Consider a given $\epsilon > 0$ and the correponding $\delta$ in \cref{assumption:strong-convexity}. By using
% \eqref{eq:two-psi-difference} at $\bm{\alpha} = \bm{\alpha}^{(0)}$, $\bm{\alpha}' \overset{p}{\to}
% \bm{\alpha}^{(0)}$ and the fact that $\bm{\Psi}$ has bounded
% derivative, we have
% $\mathrm{P}(|\bm{\Psi}_{p,\hat{\bm{\Gamma}},\hat{\bm{\Sigma}}}(\bm{\alpha}')| <
% \delta) \to 1$. This together with
% \cref{assumption:strong-convexity} imply $\mathrm{P}(\|\bm{\alpha}' -
% \hat{\bm{\alpha}}\|_2 \le \epsilon) \to 1$. Because $\bm{\alpha}'
% \overset{p}{\to} \bm{\alpha}^{(0)}$, we conclude that
% $\hat{\bm{\alpha}} \overset{p}{\to} \bm{\alpha}^{(0)}$ as well.


% \end{proof}

% As a corollary, since the $\bm{\beta}$ estimators are asymptotically
% independent, the usual FDR-control approaches to multiple hypothesis
% is asymptotically valid after adjusting for the confounding variables:
% \begin{corollary} \label{cor:fdr}
%   Under the assumptions in \cref{thm:asymptotics-nc,thm:asymptotics-rr}, the Benjamini-Hochberg procedure applied
%   to the asymptotic Z-tests based on
%   $\hat{\bm{\beta}}^{\mathrm{NC}}_{-C}$ or
%   $\hat{\bm{\beta}}^{\mathrm{RR}}$ controls the false discovery rate asymptotically.
% \end{corollary}


==> revision 2/infer_gamma.tex <==
% In this step, we are interested in using $\tilde{\bm{Y}}_{-1}$ to estimate
% $\bm{\Gamma}$ and $\bm{\Sigma}$ as $n,p
% \to \infty$.
The most popular approaches for factor analysis are principal
component analysis (PCA) and maximum likelihood (ML). \citet{bai2002} derived a class of estimators of
$r$ by principal component analysis using various information
criteria. The estimators are consistent under
\Cref{assumption:large-factor} in this section and some additional
technical assumptions in \citet{bai2002}. Due to this reason, we assume the number of confounding factors $r$ is known
in %our theoretical analysis.
this section. See \citet[Section 3]{owen2015} for a comprehensive
literature review of choosing $r$ in practice.

We are most interested in the asymptotic behavior of factor analysis when both
$n,p \to \infty$. In this case, PCA cannot consistently estimate the
noise variance $\bm{\Sigma}$ \citep{bai2012}. For theoretical analysis, we
use the quasi maximum likelihood estimate in \citet{bai2012} to get $
\hat{\bm{\Gamma}}$ and $\hat{\bm{\Sigma}}$. This estimator is called
``quasi''-MLE because it treats the factors $\tilde{
  \bm{Z}}_{-1}$ as fixed quantities. Since the confounders $\bm{Z}$ in
our model \cref{eq:linear-model} are random variables, we introduce a
rotation matrix $\bm{R} \in \mathbb{R}^{r \times r}$ and let
$\tilde{\bm{Z}}_{-1}^{(0)} = \tilde{\bm{Z}}_{-1} (\bm{R}^{-1})^T$,
$\bm{\Gamma}^{(0)} = \bm{\Gamma} \bm{R}$ be the target factors and
factor loadings that are studied in \citet{bai2012}.

To make $\tilde{\bm{Z}}_{-1}^{(0)}$ and $\bm{\Gamma}^{(0)}$ identifiable, \citet{bai2012} consider five
different identification conditions. However, the parameter of
interest in model \cref{eq:linear-model} is $\bm{\beta}$ instead of
$\bm{\Gamma}$ or $\bm{\Gamma}^{(0)}$. As we have discussed in
\Cref{sec:identification-beta}, we only need the
column space of $\bm{\Gamma}$ to estimate $\bm{\beta}$, which gives us
some flexibility of choosing the identification condition. In our
theoretical analysis we use the third condition (IC3) in
\citet{bai2012},  which imposes the constraints that $(n-1)^{-1} (\tilde{\bm{Z}}_{-1}^{(0)})^T \tilde{\bm{Z}}_{-1}^{(0)} =
\bm{I}_r$ and $p^{-1} \tilde{\bm{\Gamma}}^{(0)T} \bm{\Sigma}^{-1}
\bm{\Gamma}^{(0)}$ is diagonal. Therefore, the
rotation matrix $\bm{R}$ satisfies $\bm{R}
\bm{R}^T = (n-1)^{-1} \tilde{\bm{Z}}_{-1}^T \tilde{\bm{Z}}_{-1}$.

The quasi-log-likelihood being maximized in \citet{bai2012} is
\begin{align}\label{eq:qmle}
  - \frac{1}{2p} \log \mathrm{det}\left(\bm{\Gamma}^{(0)} (\bm{\Gamma}^{(0)})^T + \bm{\Sigma}\right) - \frac{1}{2p}
  \mathrm{tr}\left\{\bm{S} \left[\bm{\Gamma}^{(0)} (\bm{\Gamma}^{(0)})^T + \bm{\Sigma}\right]^{-1}\right\}
\end{align}
where $\bm{S}$ is the sample covariance matrix of $\tilde{\bm{Y}}_{-1}$.
%Let $\bm{R} \in \mathbb{R}^{r \times r}$ be the
%rotation matrix such that
%$\tilde{\bm{Z}}_{-1}^{(0)} = \tilde{\bm{Z}}_{-1} \bm{R}^{-T}$ and
%$\bm{\Gamma}^{(0)} = \bm{\Gamma} \bm{R}$.
%Notice that $\bm{R}$ is a
%random matrix that only depend on $\tilde{\bm{Y}}_{-1}$ and $\bm{R}
%\bm{R}^T = \frac{1}{n-1} \tilde{\bm{Z}}_{-1}^T \tilde{\bm{Z}}_{-1}$.

The theoretical results in this section rely heavily on
recent findings in \citet{bai2012}. They use these three assumptions.

\begin{assumption} \label{assumption:error}
  The noise matrix $\bm{E}$ follows the matrix normal distribution $\bm{E} \sim \mathrm{MN}(\bm{0}, \bm{I}_n,
  \bm{\Sigma})$ and $\bm{\Sigma}$ is a diagonal matrix.
  %$\mathrm{E}[e_{ij}^4] \le D^4$ for all $i$ and $j$, for some $D < \infty$.
\end{assumption}

\begin{assumption} \label{assumption:bounded}
  There exists a positive constant $D$ such that $\|\bm{\Gamma}_{j}\|_2
  \le D$, $D^{-2} \le \sigma_j^2 \le D^2$ for all $j$, and the estimated
  variances $\hat{\sigma}_j^2 \in [D^{-2}, D^2]$ for all $j$.
\end{assumption}

\begin{assumption} \label{assumption:large-factor}
  The limits $\lim_{p \to \infty} p^{-1} \bm{\Gamma}^T
  \bm{\Sigma}^{-1} \bm{\Gamma}$ and $\lim_{p \to \infty} \sum_{j=1}^p
  \sigma_j^{-4} (\bm{\Gamma}_j \otimes \bm{\Gamma}_{j})
  (\bm{\Gamma}_j^T \otimes \bm{\Gamma}_{j}^T)$ exist and are positive
  definite matrices.
\end{assumption}

%\begin{remark}
%  The uniform boundedness of $\hat{\sigma}_j$ in \Cref{assumption:bounded} is very important for
%  the theoretical analysis in \citet{bai2012}. However, it is possible
%  that some estimated variance $\hat{\sigma}_j$ is negative for a
%  dataset. The original assumption in \citet{bai2012} is ``the
%  variances $\sigma_j^2$ are estimated in the compact set $[D^{-2},
%  D^2]$''. This is algorithmically feasible, but the first order
%  optimality condition that \citet{bai2012} use to prove the
%  theoretical results does not consider the case
%  that some $\hat{\sigma}_j^2$ is on the boundary of this interval.
%\end{remark}

% \citet{bai2012} prove the consistency and asymptotic normality of
% $\hat{\bm{\Gamma}}$ and $\hat{\bm{\Sigma}}$:
\begin{lemma}[\citet{bai2012}]\label{lem:ml-baili}
  Under
  \Cref{assumption:error,assumption:bounded,assumption:large-factor},
the maximizer $(\hat{\bm{\Gamma}},\hat{\bm{\Sigma}})$
of the quasi-log-likelihood~\eqref{eq:qmle} satisfies
\[
\sqrt n(\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}) \overset{d}{\to}
  \mathrm{N}(\bm{0}, \sigma_j^2 \bm{I}_r),
\quad\text{and}\quad\sqrt n(\hat\sigma^2_j -
  \sigma^2_j)  \overset{d}{\to} \mathrm{N}(0, 2\sigma_j^4).
\]
%\[
%\frac{1}{p}\sum_{j=1}^p\frac{1}{\hat{\sigma}_j^2}
%  \|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j^{(0)}\|_2^2 = O_p(n^{-1}),~
%  \frac{1}{p}\sum_{j=1}^p(\hat\sigma_j^2 - \sigma_j^2)^2 =
%  O_p(n^{-1}).
%\]
\end{lemma}
%%% I changed the second part to be about \sigma^2 not \sigma.
%%% I think that's right, but correct it if its wrong.
In \Cref{app:lem-ml}, we prove some strengthened
technical results of \Cref{lem:ml-baili} that are used in the proof of
subsequent theorems.

\begin{remark}
  Assumption~\ref{assumption:bounded} is Assumption D
from \cite{bai2012}.  It requires that the diagonal elements of the
quasi-MLE $\hat\Sigma$ be uniformly bounded away from zero and infinity.
We would prefer boundedness to be a consequence of some assumptions
on the distribution of the data,
but at present we are unaware of any other results like
Lemma~\ref{lem:ml-baili}
which do not use this assumption. In practice, the
quasi-likelihood problem \eqref{eq:qmle} is commonly solved by the
Expectation-Maximization (EM) algorithm. Similar to
\citet{bai2012,bai2014theory}, we do not find it necessary
to impose an upper or lower bound for the parameters in the EM
algorithm in the numerical experiments.

\end{remark}


==> revision 2/intro.tex <==
%  holds the lock!

Multiple hypothesis testing has become
an important statistical problem for many scientific fields, where
tens of thousands of tests are typically performed simultaneously.
Traditionally the tests are assumed to be
independent of each other, so the
false discovery rate (FDR) can be easily controlled by e.g.,
the Benjamini-Hochberg procedure \citep{benjamini1995}. Recent years have witnessed an extensive investigation of
multiple hypothesis testing under dependence, ranging from
permutation tests \citep{korn2004,tusher2001},
% permutation tests for unknown dependence structure
positive dependence
\citep{benjamini2001}, weak dependence \citep{clarke2009,storey2004}, accuracy calculation under
dependence \citep{efron2007,owen2005}
 to mixture models \citep{efron2010,sun2009} and latent factor models \citep{fan2012,fan2013,lan2014}. Many of these works provide theoretical guarantees for
FDR control under the assumption that
%All these works assume
the individual test statistics are valid and may even be
correlated.
%so the type I error is controlled but neither FWER nor FDR is
%without their adjustment.

In this paper, we investigate a more challenging setting.
The test statistics may be correlated with each other due to
latent factors and those latent factors may also be correlated
with the variable of interest.
As a result, the test statistics are not only correlated but are also confounded.
We use the phrase ``confounding'' to emphasize
that these latent factors can significantly bias the individual
p-values, therefore this problem is fundamentally different from the
literature in the previous paragraph and poses an immediate threat to
the reproducibility of the discoveries. Many confounder adjustment
methods have already been proposed for multiple testing over the last
decade \citep{gagnon2013,leek2008,price2006,sun2012}. Our goal is to
unify these methods in the same framework and study their statistical properties.
%because the type I error is not immediately controlled.

\vspace{3mm}

\textit{The confounding problem.~~} We start with three real data examples to illustrate the confounding problem. The first microarray data (\Cref{fig:COPD-naive}) is used by \citet{singh2011} to identify candidate genes
associated with a chronic lung disease called emphysema. The second (\Cref{fig:gender-naive,fig:gender-batch}) and
third (\Cref{fig:alzheimers-batch}) data are used by \citet{gagnon2013} to
study the performance of various confounder adjustment methods. For each dataset, we plot the histogram of
t-statistics of a simple linear model that regresses the gene
expression on the variable of interest (disease status for the first
and gender for the second and third datasets). These statistics are
commonly used in genome-wide association studies (GWAS) to find
potentially interesting genes. See
\Cref{sec:datasets} for more detail of these datasets.

The histograms of t-statistics in \Cref{fig:confounding-problem}
clearly depart from the approximate theoretical null distribution
$\mathrm{N}(0,1)$. The bulk of the test statistics can be skewed
(\Cref{fig:COPD-naive,fig:gender-naive}), overdispersed
(\Cref{fig:COPD-naive}), underdispersed
(\Cref{fig:gender-naive,fig:gender-batch}), or noncentered
(\Cref{fig:alzheimers-batch}). In these cases, neither the theoretical null
$\mathrm{N}(0,1)$, nor even the empirical null as shown in the histograms, look
appropriate for measuring significance.
%%% Brad Efron uses the empirical null that way.
%We also note that Dataset 2 has some known batch and microarray platform
%variables. When these are added to the regression, the resulting
%t-statistics in \Cref{fig:gender-batch} are less underdispersed
%compared to \Cref{fig:gender-naive}. However, it is still far from the theoretical null.
%This is what we would expect if the
%problem had been caused by latent confounders.
\Citet{schwartzman2010comment} proved that
a largely overdispersed histogram like \Cref{fig:COPD-naive} cannot be explained by correlation alone,
and is possibly due to the presence of confounding factors.
For a sneak preview of the
confounder adjustment, the reader can find the histograms after our confounder
adjustment in \Cref{fig:output} at the end of this paper.
The p-values of our test of confounding
(\Cref{sec:test-confound}) in \Cref{tab:output} indicate that all the three datasets
suffer from confounding latent factors.



Other common sources of confounding in gene expression profiling include
systematic ancestry differences \citep{price2006}, environmental changes
\citep{fare2003,gasch2000} and surgical manipulation
\citep{lin2006}. See \citet{lazar2013} for a survey.
In many studies, especially for observational clinical research and human expression data,
the latent factors, either genetic or technical, are confounded with primary variables
of interest due to the observational nature of the studies and heterogeneity of samples
\citep{ransohoff2005,rhodes2005}.
Similar
confounding problems also occur in other high-dimensional datasets
such as brain imaging \citep{schwartzman2008} and metabonomics \citep{craig2006}.


\begin{figure}[hp]
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{plots/COPD-batch.pdf}
  \caption{\small Dataset 1.}
  \label{fig:COPD-naive}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.45\textwidth}
 \includegraphics[width = \textwidth]{plots/gender-naive.pdf}
  \caption{\small Dataset 2.}
  \label{fig:gender-naive}
  \end{subfigure}
  \\
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{plots/alzheimers-batch.pdf}
  \caption{\small Dataset 3.}
  \label{fig:alzheimers-batch}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width = \textwidth]{plots/gender-batch.pdf}
  \caption{\small Dataset 2 (batch correction).}
  \label{fig:gender-batch}
  \end{subfigure}
  \caption{ \small
  Dataset 1 is the COPD dataset \citep{singh2011}. Dataset 2 and 3 are from
  \citet{gagnon2013}.
  Histograms of regression t-statistics in three microarray studies show clear departure from the
    theoretical null distribution $\mathrm{N}(0,1)$. The mean and
    standard deviation of the normal approximation are obtained from
    the median and median absolute deviation of the statistics. See
    \Cref{sec:gender-study} for the empirical distributions after confounder
    adjustment.}
  \label{fig:confounding-problem}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width = \textwidth]{plots/alzheimers-batch.pdf}
%   \caption{A different microarray study in
%     \citet{gagnon2013}. The unadjusted regression
%     t-statistics are clearly not centered at $0$.}
%   \label{fig:alzheimers-naive}
% \end{figure}


\vspace{3mm}

\textit{Previous methods.~~} As early as \citet{alter2000},
principal component analysis has been suggested to estimate the confounding
factors. This approach can work reasonably well if the confounders
clearly stand out. For example, in population
genetics, \citet{price2006} proposed a procedure called EIGENSTRAT that
removes the largest few principal
components from their SNP genotype data, claiming they closely resemble the ancestry
difference. In gene expression data, however, it is often unrealistic to
assume they always represent the confounding factors. The largest
principal component may also correlate with the
primary effects of interest. Therefore, directly removing them can result in loss of statistical power.



More recently, an emerging literature considers the confounding problem
in similar statistical settings and a variety of methods have been
proposed for confounder adjustment
\citep{friguet2009,gagnon2013,gagnon2012,leek2007,leek2008,sun2012}. %However, though
These statistical methods are shown to
%are a great improvement over
%the naive EIGENSTRAT procedure in many simulated and real data sets,
work better than the EIGENSTRAT procedure for gene expression data. However,
little is known about their theoretical properties. Indeed, the
authors did not focus on model identifiability and rely on impressive heuristic calculations
to derive their estimators.
%, which can greatly undermine the
%applicability of these methods in real scientific studies.
In this paper, we address the identifiability problem, rederive the
estimators in \citep{gagnon2013,sun2012} in a more principled way and provide
theoretical guarantees for them.
%%% I took out 'closely related'.  It is not specific enough.


Before describing the modeling framework, we want to clarify our
terminology. The confounding factors or confounders considered in the
present paper are referred to by different names in the literature, such as
``surrogate variables'' \citep{leek2007}, ``latent factors'' \citep{friguet2009}, ``batch effects''
\citep{leek2010}, ``unwanted variation'' \citep{gagnon2012} and
``latent effects'' \citep{sun2012}. We believe they are all describing
the same phenomenon: that there exist some unobserved variables that
correlate with both the primary variable(s) of interest and the outcome
variables (e.g.\ gene expression). This problem is generally known
as confounding \citep{fisher1935,kish1959}. A famous example is Simpson's paradox.
The term  ``confounding'' has multiple
meanings in the literature.
We use the meaning from \cite{greenland1999}:
``a mixing of effects of extraneous factors (called confounders) with the effect of
interest''.
%%% I don't think we need to identify Greenland et al as providing the dominant
%%% meaning.  Also I'm not sure that it is dominant.  We just need to clarify
%%% the meaning we choose.

\vspace{3mm}

\textit{Statistical model of confounding.~~} Most of the confounder
adjustment methods mentioned above are built around the following model
\begin{equation} \label{eq:previous-model}
\bm{Y} = \bm{X} \bm{\beta}^T + \bm{Z} \bm{\Gamma}^T + \bm{E}
\end{equation}
Here $\bm{Y}$ is a $n \times p$ observed matrix (e.g.\ gene expression); $\bm{X}$ is an $n \times 1$ observed primary variable of
interest (e.g.\ treatment-control, phenotype, health trait); $\bm{Z}$
is an $n \times r$ latent confounding factor matrix; $\bm{E}$ is
often assumed to be a Gaussian noise matrix. The $p \times 1$ vector
$\bm{\beta}$ contains the primary effects we want to estimate.

Model \eqref{eq:previous-model} is very general for multiple
testing dependence. \citet[Proposition 1]{leek2008} suggest that
multiple hypothesis tests based on linear regression can always be
represented by \eqref{eq:previous-model} using sufficiently many
factors. However, equation \eqref{eq:previous-model} itself is not
enough to model confounded tests.  To
elucidate the concept of confounding, we need to characterize the
relationship between the latent variables $\bm{Z}$ and the primary
variable $\bm{X}$. To be more specific, we assume the
regression of $\bm{Z}$ on $\bm{X}$ also follows a linear relationship
\begin{equation} \label{eq:linear-model-z-sec1}
\bm{Z} = \bm{X} \bm{\alpha}^T + \bm{W},
\end{equation}
where $\bm{W}$ is a $n \times r$ random noise matrix
independent of $\bm{X}$ and $\bm{E}$ and the $r \times 1$ vector
$\bm{\alpha}$ characterizes the extent of confounding in this
data. By plugging \eqref{eq:linear-model-z-sec1} in
\eqref{eq:previous-model}, the linear regression of $\bm{Y}$ on
$\bm{X}$ gives an unbiased estimate of the marginal effects
\begin{equation} \label{eq:marginal-effect}
\bm{\tau} = \bm{\beta} + \bm{\Gamma} \bm{\alpha}
\end{equation}
When $\bm{\alpha} \ne \bm{0}$, $\bm{\tau}$ is not the same as
$\bm{\beta}$ by \eqref{eq:marginal-effect}. In this case, the data
$(\bm{X},\bm{Y})$ are confounded by $\bm{Z}$. Since the
confounding factors $\bm{Z}$ are data artifacts in this model, the
statistical inference of $\bm{\beta}$ is much more interesting
than that of $\bm{\tau}$. See \Cref{sec:marginal-effects-vs} for more
discussion on the marginal and the direct effects.

% \vspace{3mm}

% \textit{Two-step procedure.~~}
Following LEAPP \citep{sun2012}, we use
a QR decomposition to decouple the estimation of  $\bm{\Gamma}$ from $\bm{\beta}$.
%Consequently, the inference procedure naturally split into two steps:
The inference procedure splits into the following two steps:

\begin{description}
\item[Step 1] By regressing out $\bm{X}$ in \cref{eq:previous-model},
  $\bm{\Gamma}$ is the loading matrix in a factor analysis model and can be efficiently estimated by maximum likelihood.
\item[Step 2] Equation \eqref{eq:marginal-effect} can be viewed as a
  linear regression of the marginal effects $\bm{\tau}$ on the factor
  loadings $\bm{\Gamma}$. To estimate $\bm{\alpha}$ and $\bm{\beta}$,
  we replace $\bm{\tau}$ by its observed value and $\bm{\Gamma}$ by
  its estimate in Step 1.
\end{description}

As mentioned before,
other existing confounder adjustment methods including SVA
\citep{leek2008} and RUV-4 \citep{gagnon2013} can be unified in this two-step statistical procedure.
See \Cref{sec:comp-with-exist} for a detailed discussion of these methods.

\vspace{3mm}

\textit{Contributions.~~} Our first contribution in \Cref{sec:model}
is to establish identifiability for the confounded multiple testing
model. In the first step of estimating
factor loadings $\bm{\Gamma}$, identifiability is well studied in
classical multivariate statistics. However, the second step of
estimating the effects $\bm{\beta}$ is not identifiable
  without additional constraints. We consider two different sufficient
  conditions for global identifiability. The
  first condition assumes the researcher has a ``negative control''
  variable set for which there should be no direct effect. This
  negative control set often serves as a quality control precaution in microarray studies \citep{gagnon2012}, but they can also be used to adjust for the confounding factors. The second identification condition assumes at
  least half of the true effects are zero, i.e., the true alternative
  hypotheses are sparse. These two identification conditions
  correspond to the approaches of RUV-4 \citep{gagnon2013} and LEAPP \citep{sun2012}, respectively.

Our second contribution in \Cref{sec:stat-infer} is to derive valid and efficient statistical methods under these identification
conditions in the second step. In order to estimate the effects, it is essential to estimate the coefficients $\bm{\alpha}$
relating  the primary variable to the confounders. Under the two
different identification conditions, we study two
different regression methods which are analytically tractable and
equally well performing alternatives to RUV-4 and LEAPP. For the
negative control (NC) scenario, $\hat{\bm{\alpha}}^{\mathrm{NC}}$ and
$\hat{\bm{\beta}}^{\mathrm{NC}}$ are obtained
by generalized least squares using the negative
controls. For the sparsity scenario, $\hat{\bm{\alpha}}^{\mathrm{RR}}$ and
$\hat{\bm{\beta}}^{\mathrm{RR}}$ are obtained by using a simpler
and more analytically tractable robust regression (RR) than the one used in LEAPP.

When the factors are strong (as large as the noise magnitude),
for both scenarios we find that the
resulting estimators of $\bm{\beta}$ are asymptotically as efficient
as the oracle estimator which is allowed to observe the confounding
factors.  It is surprising that no essential loss of efficiency is incurred
by searching for the confounding variables.
%%%  I changed it from adjusting to searching.  The oracle is also adjusting (but not searching).
Our asymptotic  analysis relies on some recent theoretical results for factor analysis due to \citet{bai2012}. The
asymptotic regime we consider has both $n$, the number of
observations, and $p$, the number of outcome variables (e.g.\ genes),
going to infinity. The most important condition that we require for asymptotic
efficiency in
the negative control scenario is that the number of negative controls increases to infinity;
in the sparsity scenario, we need the $L_1$ norm of the effects to satisfy $\|\bm{\beta}\|_1 \sqrt{n} / p \to
0$. The fact that $p \gg n$ in many multiple hypothesis
testing problems plays an important role in these asymptotics.

Next in \Cref{sec:stat-infer}, we show that the asymptotic $z$-statistics based
on the efficient estimators of $\bm{\beta}$ can control the type I
error. This is not a trivial corollary from the asymptotic
distribution of the test statistics because the size of $\bm{\beta}$ is growing and the
$z$-statistics are weakly correlated. Proving FDR control is more
technically demanding and is beyond the scope of this paper. Instead,
we use numerical simulations to study the empirical performance
(including FDR) of our tests. We also give a significance test of
confounding (null hypothesis $\bm{\alpha} = \bm{0}$) in
\Cref{sec:stat-infer}. This test can help the experimenter to
determine if there is any hidden confounder in the design or the
experiment process.

In \Cref{sec:extens-mult-regr}, we generalize the
confounder adjustment model to include multiple primary variables and multiple nuisance covariates.
We show the statistical methods and theory for the single
primary variable regression problem \cref{eq:previous-model} can be
smoothly extended to the multiple regression problem.

% Our final contribution in \Cref{sec:weak-factors} is to study the
% robustness of the methods when some confounders are not sufficiently
% strong. We show that our estimate of $\bm{\beta}$ is still consistent by
% using random matrix theory for the principal component analysis
% (PCA). The asymptotic $z$-tests cannot be used in this case any more,
% but our estimator of $\bm{\beta}$ can still provide an accurate ranking of all the effects.

\vspace{3mm}

\textit{Outline.~~} \Cref{sec:model} introduces the model and
describes the two identification
conditions. \Cref{sec:stat-infer} studies the statistical inference.
\Cref{sec:extens-mult-regr} extends our framework to a
linear model with multiple primary variables and multiple known controlling
covariates. % \Cref{sec:weak-factors} studies the validity of our method
% when some confounding factors are weak.
\Cref{sec:discussions}
discusses our theoretical analysis in the context of previous literature, including
the existing procedures for debiasing the confounders and existing
theoretical results of multiple hypothesis testing under dependence
(but no confounding). \Cref{sec:numerical-experiments} studies the
empirical behavior of our estimators in simulations and real data
examples. Technical proofs of the results are provided in Supplement
\citep{wang2015supplement}.

To help the reader follow this paper and compare our methods and theory
with existing approaches, \Cref{tab:literature} summarizes some
related publications with more detailed discussion in
\Cref{sec:discussions}.

\setlength{\tabcolsep}{3pt}
\begin{table}[t]
  \footnotesize
  \begin{center}
  \begin{tabular}{c|c|c|}
    \cline{2-3}
    & \multicolumn{2}{c|}{Noise conditional on latent
      factors} \\ \cline{2-3}
    & Independent % & Weakly correlated
    & Correlated \\ \cline{1-3}
    \multicolumn{1}{|c|}{\begin{tabular}[x]{@{}c@{}} Positive or weak \\ dependence\end{tabular}} &
    \multicolumn{2}{c|}{
    \begin{tabular}[x]{@{}c@{}}\citet{benjamini2001}\\\citet{storey2004}
    \\ \citet{clarke2009}\end{tabular} }
      \\ \cline{1-3}
    \multicolumn{1}{|c|}{\begin{tabular}[x]{@{}c@{}} Unconfounding \\
        factors \end{tabular}} &
    \multicolumn{1}{c|}{\begin{tabular}[x]{@{}c@{}}         \citet*{friguet2009} \\
        %\citet{sun2009} \\\citet{efron2010} \\
    \citet{desai2012cross} \\ \end{tabular}} &
    \multicolumn{1}{c|}{ \begin{tabular}[x]{@{}c@{}}\citet*{fan2012}\\\citet{lan2014}\\\textit{Discussed in \Cref{sec:latent-but-unconf,sec:marginal-effects-vs}}\end{tabular}
    } \\
    \cline{1-3}
    \multicolumn{1}{|c|}{\begin{tabular}[x]{@{}c@{}}Confounding \\
    factors \\ \end{tabular}}
    & \begin{tabular}[x]{@{}c@{}} \citet{leek2007,leek2008}\\
    \citet{gagnon2012} \\ % \citet*{gagnon2013} \\
    \citet*{sun2012} \\ \textit{Studied in
      \Cref{sec:model,sec:stat-infer,sec:extens-mult-regr}} \\ \textit{Discussed in \Cref{sec:comp-with-exist}}\end{tabular}
    & \begin{tabular}[x]{@{}c@{}} \textit{Discussed in
      \Cref{sec:inference-when-sigma}} \\ \textit{(future research)} \\ \end{tabular} \\ \cline{1-3}
  \end{tabular}
  \end{center}
  \vspace{0.5em}
  \caption{\small Selected literature in multiple hypothesis testing under
    dependence.\\ The categorization is partially subjective as
some authors do not use exactly the same terminology.}
  \label{tab:literature}
\end{table}

\vspace{3mm}
\textit{Notation.~~} Throughout the article, we use bold upper-case
letters for matrices and lower-case letters for vectors. We use
Latin letters for random variables and Greek letters for model
parameters. Subscripts of matrices are used to indicate row(s)
whenever possible. For example, if $\mathcal{C}$ is a set of indices,
then $\bm{\Gamma}_{\mathcal{C}}$ is the corresponding rows of $\bm{\Gamma}$. The $L_0$ norm of a vector is defined as the number
of nonzero entries: $\|\bm{\beta}\|_0
= |\{ 1 \le j \le p: \beta_j \ne 0 \}|$. A random matrix $\bm{E} \in \mathbb{R}^{n \times
  p}$ is said to follow a \textit{matrix normal} distribution with mean $\bm{M}\in \mathbb{R}^{n \times p}$, row covariance
$\bm{U} \in \mathbb{R}^{n \times n}$ and
column covariance $\bm{V} \in \mathbb{R}^{p \times p}$, abbreviated as
$\bm{E} \sim \mathrm{MN}(\bm{M}, \bm{U}, \bm{V})$, if the
vectorization of $\bm{E}$ by column follows the multivariate normal distribution $\mathrm{vec}(\bm{E}) \sim
\mathrm{N}(\mathrm{vec}(\bm{M}), \bm{V} \otimes \bm{U})$. When $\bm{U}
= \bm{I}_n$, this means the rows of $\bm{E}$ are i.i.d.\
$\mathrm{N}(0, \bm{V})$. We use the
usual notation in asymptotic statistics that a random variable is
${O}_p(1)$ if it is bounded in probability, and
${o}_p(1)$ if it converges to $0$ in
probability. Bold symbols ${\bm{O}}_p(1)$ or
${\bm{o}}_p(1)$ mean each entry of the vector is ${O}_p(1)$ or ${o}_p(1)$.


==> revision 2/model.tex <==
% qz is editing
\subsection{Linear model with confounders}
\label{sec:linear-model-with}

We consider a single primary variable of interest in this
section. It is common to add intercepts and known confounder effects
(such as lab and batch effects) in the regression model. This extension to
multiple linear regression does not change the main theoretical
results in this paper and is discussed in
\Cref{sec:extens-mult-regr}.

For simplicity, all the variables in this section are assumed to have mean $0$ marginally. Our
model is built on equation \eqref{eq:previous-model} that is already widely
used in the existing literature and we rewrite it here:
\refstepcounter{equation}\label{eq:linear-model}
\begin{equation}
  \tag{\theequation a}\label{eq:linear-model-y}
   {\bm{Y}}_{n \times p} = {\bm{X}}_{n \times 1} \,
   {\bm{\beta}}_{p \times 1}^T + \bm{Z}_{n \times r} \,
   \bm{\Gamma}_{p \times r}^T +
   \bm{E}_{n \times p}.
\end{equation}
As mentioned earlier, it is also crucial to model the dependence
of the confounders $\bm{Z}$ and the primary variable $\bm{X}$. We
assume a linear relationship as in \cref{eq:linear-model-z-sec1}
\begin{equation} \tag{\theequation b} \label{eq:linear-model-z}
\bm{Z} = \bm{X} \bm{\alpha}^T + \bm{W},
\end{equation}
and in addition some distributional assumptions on $\bm{X}$, $\bm{W}$ and the noise matrix $\bm{E}$
\begin{align}
  \tag{\theequation c} \label{eq:distribution-x}
  &X_i \overset{\mathrm{i.i.d.}}{\sim} \mathrm{mean}~0,~
  \mathrm{variance}~1,~i=1,\dotsc,n, \\
 \tag{\theequation d} \label{eq:distribution-w}
&\bm{W} \sim
\mathrm{MN}(\bm{0}, \bm{I}_n, \bm{I}_r),~\bm{W} \independent \bm{X}, \\
  \tag{\theequation e} \label{eq:distribution-e}
  &\bm{E} \sim \mathrm{MN}(\bm{0},
  \bm{I}_n, \bm{\Sigma}),~\bm{E} \independent (\bm{X},\bm{Z}).
\end{align}

The parameters in the model \cref{eq:linear-model} are $\bm{\beta} \in
\mathbb{R}^{p \times 1}$ the primary effects we are most interested in,
$\bm{\Gamma} \in \mathbb{R}^{p \times r}$ the influence of confounding
factors on the outcomes, $\bm{\alpha} \in
\mathbb{R}^{r \times 1}$ the association of the primary variable with
the confounding factors, and $\bm{\Sigma} \in
\mathbb{R}^{p \times p}$ the noise covariance
matrix. We assume $\bm{\Sigma}$ is diagonal $\bm{\Sigma}
= \mathrm{diag}(\sigma_1^2,\dotsc,\sigma_p^2)$, so the noise
for different outcome variables is independent. We discuss possible
ways to relax this independence assumption in \Cref{sec:inference-when-sigma}.

In \eqref{eq:distribution-x}, $X_i$ is not required to be
Gaussian or even continuous. For example, a binary or categorical
variable after normalization also meets this assumption. As mentioned
in \Cref{sec:introduction}, the parameter vector $\bm{\alpha}$
measures how severely the data are confounded. For a more
intuitive interpretation, consider an oracle procedure of estimating
$\bm{\beta}$ when the confounders $\bm{Z}$ in
\cref{eq:linear-model-y} are observed. The best linear unbiased estimator in this
case is the ordinary least squares $(\hat{{\beta}}^{\mathrm{OLS}}_j,
\hat{\bm{\Gamma}}^{\mathrm{OLS}}_j)$, whose variance is $ \sigma_j^2
\mathrm{Var}(X_i, \bm{Z}_i)^{-1} / n$. Using \cref{eq:linear-model-z,eq:distribution-w},
% Since
% \[
% \mathrm{Var}(X_i, \bm{Z}_i) =
% \begin{pmatrix}
%   1 & \bm{\alpha}^T \\
%   \bm{\alpha} & \bm{I}_r + \bm{\alpha} \bm{\alpha}^T \\
% \end{pmatrix},
% \]
it is easy to show that $\mathrm{Var}(\hat{\beta}_j^{\mathrm{OLS}}) =
(1 + \|\bm{\alpha}\|_2^2) \sigma_j^2/n$ and
$\mathrm{Cov}(\hat{\beta}_j^{\mathrm{OLS}}, \hat{\beta}_k^{\mathrm{OLS}}) = 0$ for $j \ne k$. In summary,
\begin{equation} \label{eq:var-beta-oracle}
\mathrm{Var}(\hat{\bm{\beta}}^{\mathrm{OLS}}) = \frac{1}{n} (1 + \| \bm{\alpha}
\|_2^2) \bm{\Sigma}.
\end{equation}
Notice that in the unconfounded linear model in which $\bm{Z} =
\bm{0}$, the variance of the OLS estimator of $\bm{\beta}$ is
$\bm{\Sigma}/n$. Therefore, $1 + \|\bm \alpha\|_2^2$ represents the
relative loss of efficiency when we add observed variables $\bm{Z}$ to the
regression which are correlated with $\bm{X}$. In
\Cref{sec:inference-beta-alpha}, we show that the oracle efficiency
\eqref{eq:var-beta-oracle} can be asymptotically achieved even when
$\bm{Z}$ is unobserved.

% notice that marginally $\mathrm{var}(\bm{Z}_i) = \bm{I}_r +
% \bm{\alpha}\bm{\alpha}^T$. After some easy algebra, one can show that
% the fraction of variance of $X_i$ that can be explained by
% the confounders $\bm{Z}_i$ is
% \[
% \max_{\bm{\rho}}\mathrm{corr}(\bm{\rho}^T\bm{Z}_i, X_i) = \max_{\bm{\rho}}
% \frac{\bm{\rho}^T\bm{\alpha}}{\sqrt{\bm{\rho}^T(\bm{I}_r + \bm{\alpha}\bm{\alpha}^T)
% \bm{\rho}}} = \frac{\|\bm{\alpha}\|_2^2}{1 +\|\bm{\alpha}\|_2^2}.
% \]
% This quantity is directly related to the
% efficiency of estimating $\bm{\beta}$ under model \cref{eq:linear-model}.
% \marginpar{Introclass correlation?}
%correlation $\bm{\rho} =
%\mathrm{cor}(\bm{Z}_i,X_i)$ through $\rho_k = \alpha_k / \sqrt{1 + \alpha_k^2},~k=1,\dotsc,r$.

%\qz{Only the joint distribution of $\bm{X}$ and $\bm{Z}$ matters.}

Let $\bm{\theta} =
(\bm{\alpha}, \bm{\beta}, \bm{\Gamma}, \bm{\Sigma})$ be all the
parameters and $\bm{\Theta}$ be the parameter space. Without any
constraint, the model \cref{eq:linear-model} is unidentifiable. In
\Cref{sec:identification-gamma,sec:identification-beta} we show how to restrict $\bm{\Theta}$ to ensure identifiability.

% Also, when $\bm{\alpha}\neq \bm{0}$,
% the latent factors are confounded with the primary variable and
% the naive
% linear regression estimator applied to $\bm{Y} = \bm{X} \bm{\beta}^T +
% \bm{E}$ can be greatly biased if the data actually follow
% \eqref{eq:linear-model-y}. The main goal of this paper is to correct such
% bias by adjusting for the confounders.

\subsection{Rotation}
\label{sec:rotation}

%First, following \citet{sun2012}, we introduce
Following \citet{sun2012}, we introduce
a transformation of the data to make the
identification issues clearer. Consider the Householder rotation matrix $\bm{Q}^{T} \in
\mathbb{R}^{n \times n}$ such that
$\bm{Q}^T \bm{X} = \|\bm{X}\|_2\bm{e}_1 = (\|\bm{X}\|_2,0,0,\dotsc,0)^T$. Left-multiplying $\bm{Y}$ by
$\bm{Q}^T$, we get
$\tilde{\bm{Y}} = \bm{Q}^T \bm{Y} = \|\bm{X}\|_2 \bm{e}_1 \bm{\beta}^T
    + \tilde{\bm{Z}} \bm{\Gamma}^T +  \tilde{\bm{E}}$,
where
\begin{equation} \label{eq:Z-tilde}
\tilde{\bm{Z}} = \bm{Q}^T\bm{Z} = \bm{Q}^T (\bm{X \alpha}^T +
\bm{W}) = \|\bm{X}\|_2 \bm{e}_1 \bm{\alpha}^T + \tilde{\bm{W}},
\end{equation}
and $\tilde{\bm{W}} = \bm{Q}^T \bm{W} \overset{d}{=} \bm{W}$,
$\tilde{\bm{E}} = \bm{Q}^T \bm{E} \overset{d}{=} \bm{E}$. As a
consequence, the first and the rest of the rows of $\tilde{\bm{Y}}$ are
\begin{align}
  &\tilde{\bm{Y}}_1 = \|\bm{X}\|_2 \bm{\beta}^T + \tilde{\bm{Z}}_1 \bm{\Gamma}^T +
  \tilde{\bm{E}}_1  \sim \mathrm{N}(\|\bm{X}\|_2 (\bm{\beta} +
  \bm{\Gamma}\bm{\alpha})^T, \bm{\Gamma} \bm{\Gamma}^T + \bm{\Sigma}) , \label{eq:Y-tilde-1} \\
  &\tilde{\bm{Y}}_{-1} = \tilde{\bm{Z}}_{-1} \bm{\Gamma}^T +
  \tilde{\bm{E}}_{-1} \sim \mathrm{MN}(\bm{0},
  \bm{I}_{n-1}, \bm{\Gamma} \bm{\Gamma}^T + \bm{\Sigma}). \label{eq:Y-tilde-m1}
\end{align}
Here $\tilde{\bm{Y}}_1$ is a $1 \times p$ vector,
$\tilde{\bm{Y}}_{-1}$ is a $(n-1) \times p$ matrix, and the
distributions are conditional on $\bm{X}$.

The parameters $\bm{\alpha}$ and
$\bm{\beta}$ only appear in \cref{eq:Y-tilde-1}, so their inference
(step 1 in our procedure) can be completely separated from
the inference of $\bm{\Gamma}$ and $\bm{\Sigma}$ (step 2 in our
procedure). In fact, $\tilde{\bm{Y}}_1 \independent
\tilde{\bm{Y}}_{-1}|\bm{X}$ because $\tilde{\bm{E}}_1 \independent
\tilde{\bm{E}}_{-1}$, so the two steps use mutually independent
information. This in turn greatly simplifies the theoretical analysis.

We intentionally use the symbol $\bm{Q}$ to resemble the QR decomposition of $\bm{X}$. In
\Cref{sec:extens-mult-regr} we show how to use the QR decomposition to
separate the primary effects from confounder and nuisance effects when
$\bm{X}$ has multiple columns. Using the same notation, we discuss
how SVA and RUV decouple the problem in a slightly different manner in \Cref{sec:sva}.

\subsection{Identifiability of \texorpdfstring{$\bm \Gamma$}{TEXT}}
\label{sec:identification-gamma}

Equation \eqref{eq:Y-tilde-m1} is just the exploratory factor analysis
model, thus $\bm{\Gamma}$ can
be easily identified up to some rotation under some mild conditions.
%At this point, it should be clear that under mild conditions, from
 Here we assume a classical sufficient condition for
the identification of $\bm{\Gamma}$ \citep[Theorem 5.1]{anderson1956}.

% \begin{condition}{I}
% \label{condition:identify-gamma-to-rotation}
% If any row of $\Gamma$ is deleted, there remain two disjoint
% submatrices of $\Gamma$ of rank $r$.
% \end{condition}

\begin{lemma}
\label{lemma:identify-gamma}
Let $\bm{\Theta} = \bm{\Theta}_0$ be the parameter space such that
\begin{enumerate}
\item If any row of $\bm{\Gamma}$ is deleted, there remain two
  disjoint submatrices of $\bm{\Gamma}$ of rank $r$, and
\item $\bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}/p$ is
  diagonal and the diagonal elements are distinct, positive, and
  arranged in decreasing order.
\end{enumerate}
Then $\bm{\Gamma}$ and $\bm{\Sigma}$ are identifiable in the model
\cref{eq:linear-model}.
\end{lemma}

  In \Cref{lemma:identify-gamma}, condition (1) requires that $p\geq 2r + 1$.
  Condition (1) identifies $\bm{\Gamma}$ up to a
  rotation which is sufficient to identify $\bm{\beta}$. To
  see this, we can reparameterize $\bm{\Gamma}$ and $\bm{\alpha}$ to
  $\bm{\Gamma}\bm{U}$ and $\bm{U}^T\bm{\alpha}$ using an $r \times r$
  orthogonal matrix $\bm{U}$. This reparameterization does not change
  the distribution of $\tilde{\bm{Y}}_1$ in \cref{eq:Y-tilde-1} if
  $\bm{\beta}$ remains the same. Condition (2) identifies the rotation
  uniquely but is not necessary for our theoretical analysis in later
  sections.
  % Also,
  % if $\bm{\Gamma}$ doesn't satisfy condition (2),
  %  consisting of the
  % eigenvectors of $\bm{\Gamma}^T\bm{\Sigma}^{-1}\bm{\Gamma}$.
  % One can easily check that the
  % representation of our
  % later theorems are not affected by this reparameterization.

\subsection{Identifiability of \texorpdfstring{$\bm \beta$}{TEXT}}
\label{sec:identification-beta}

The parameters $\bm{\beta}$ and $\bm{\alpha}$ cannot be identified from
\eqref{eq:Y-tilde-1} because they have in total $p + r$
parameters while $\tilde{\bm{Y}}_1$ is a length $p$ vector. If we write
$\mathcal{P}_{\bm{\Gamma}}$ and $\mathcal{P}_{\bm{\Gamma}^{\perp}}$ as
the projection onto the column space and orthogonal space of $\bm{\Gamma}$
so that $\bm{\beta} = \mathcal{P}_{\bm{\Gamma}} \bm{\beta} +
\mathcal{P}_{\bm{\Gamma}^{\perp}} \bm{\beta}$, it is impossible to
identify $\mathcal{P}_{\bm{\Gamma}} \bm{\beta}$ from \cref{eq:Y-tilde-1}.
%though $\mathcal{P}_{\bm{\Gamma}^{\perp}} \bm{\beta}$ is identifiable.

This suggests that we should further restrict the
parameter space $\bm{\Theta}$.
We will reduce the degrees of freedom by restricting at least $r$ entries of
$\bm{\beta}$ to equal $0$. We consider two different sufficient conditions to identify $\bm{\beta}$:

\begin{description}
\item[Negative control] $\bm{\Theta}_1 = \{ (\bm{\alpha},
    \bm{\beta}, \bm{\Gamma}, \bm{\Sigma}): \bm{\beta}_{\mathcal{C}} =
\bm{0},~\mathrm{rank}(\bm{\Gamma}_{\mathcal{C}}) = r\}$ for a known
negative control set $|\mathcal{C}| \ge
r$.
\item[Sparsity] $\bm{\Theta}_2(s) = \{ (\bm{\alpha},
    \bm{\beta}, \bm{\Gamma}, \bm{\Sigma}): \|\bm{\beta}\|_0 \le \lfloor (p-s)/2
  \rfloor,~\mathrm{rank}(\bm{\Gamma}_{\mathcal{C}}) = r,~\forall \mathcal{C} \subset
  \{1,\dotsc,p\},~|\mathcal{C}| = s \}$ for some $r \le s \le p$.
\end{description}

\begin{proposition} \label{prop:identifiable}
  If $\bm{\Theta} = \bm{\Theta}_0 \cap \bm{\Theta}_1$ or $\bm{\Theta}
  = \bm{\Theta}_0 \cap \bm{\Theta}_2(s)$ for some $r \le s \le p$, the parameters $\bm{\theta} =
  (\bm{\alpha}, \bm{\beta}, \bm{\Gamma}, \bm{\Sigma})$ in the model
  \cref{eq:linear-model}
  are identifiable.
\end{proposition}
\begin{proof}
  Since $\bm{\Theta} \subset \bm{\Theta}_0$, we know from \Cref{lemma:identify-gamma} that $\bm{\Gamma}$ and $\bm{\Sigma}$ are
  identifiable. Now consider two combinations of parameters
  $\bm{\theta}^{(1)} = (\bm{\alpha}^{(1)}, \bm{\beta}^{(1)}, \bm{\Gamma}, \bm{\Sigma})$ and
  $\bm{\theta}^{(2)} = (\bm{\alpha}^{(2)}, \bm{\beta}^{(2)}, \bm{\Gamma},
  \bm{\Sigma})$ both in the space $\bm{\Theta}$ and inducing the same
  distribution in the model \cref{eq:linear-model}, i.e.\
  $\bm{\beta}^{(1)} + \bm{\Gamma} \bm{\alpha}^{(1)} =  \bm{\beta}^{(2)} + \bm{\Gamma} \bm{\alpha}^{(2)}$.

  Let $\mathcal{C}$ be the set of indices such that $\bm{\beta}^{(1)}_{\mathcal{C}} =
  \bm{\beta}^{(2)}_{\mathcal{C}} = \bm{0}$. If $\bm{\Theta} = \bm{\Theta}_0 \cap
  \bm{\Theta}_1$, we already know $|\mathcal{C}| \ge r$. If $\bm{\Theta} =
  \bm{\Theta}_0 \cap \bm{\Theta}_2(s)$, it is easy to show that $|\mathcal{C}| \ge
  s$ is also true because both $\bm{\beta}^{(1)}$ and
  $\bm{\beta}^{(2)}$ have at most $\lfloor (p-s)/2
  \rfloor$ nonzero entries. Along with the rank constraint on
  $\bm{\Gamma}_\mathcal{C}$, this implies that $\bm{\Gamma}_{\mathcal{C}}
  \bm{\alpha}^{(1)} = \bm{\Gamma}_{\mathcal{C}} \bm{\alpha}^{(2)}$. However, the
  conditions in $\bm{\Theta}_1$ and $\bm{\Theta}_2$ ensure that
  $\bm{\Gamma}_{\mathcal{C}}$ has full rank, so $\bm{\alpha}^{(1)} =
  \bm{\alpha}^{(2)}$ and hence $\bm{\beta}^{(1)} =
  \bm{\beta}^{(2)}$.
\end{proof}

% We make four remarks regarding the identification conditions in
%  \Cref{prop:identifiable}:

\begin{remark}
   The condition (2) in \Cref{lemma:identify-gamma} that uniquely
   identifies $\bm{\Gamma}$ is not necessary for the identification of
   $\bm{\beta}$. This is because for any set $|\mathrm{C}| \ge r$ and any
   orthogonal matrix $\bm{U} \in \mathbb{R}^{r \times r}$, we always
   have $\mathrm{rank}(\bm{\Gamma}_{\mathcal{C}}) =
   \mathrm{rank}(\bm{\Gamma}_{\mathcal{C}}) \bm{U}$. Therefore
   $\bm{\Gamma}$ only needs to be identified up to a rotation.
\end{remark}

\begin{remark}
Almost all dense matrices of $\bm{\Gamma} \in \mathbb{R}^{p \times r}$
satisfy the conditions. However, for $\bm{\Theta}_2(s)$ the sparsity of $\bm{\Gamma}$ allowed
depends on the sparsity of $\bm{\beta}$. The condition $\bm{\Theta}_2(s)$ rules
out some too sparse
$\bm{\Gamma}$. In this case, one may consider
using confirmatory factor analysis instead of exploratory factor
analysis to model the relationship between confounders and
outcomes. For some recent identification results in confirmatory
factor analysis, see \citet{grzebyk2004,kuroki2014}.
\end{remark}

\begin{remark}
The maximum allowed $\|\bm{\beta}\|_0$ in $\bm{\Theta}_2$, $\lfloor
(p-r)/2 \rfloor$, is exactly the maximum breakdown point of a robust
regression with $p$ observations and $r$ predictors
\citep{maronna2006}. Indeed we use a standard robust
regression method to estimate $\bm{\beta}$ in this case in \Cref{sec:unkn-zero-indic}.
\end{remark}

\begin{remark}
To the best of our
knowledge, the only existing literature that explicitly addresses the
identifiability issue is \citet[Chapter 4.2]{sun2011}, where
the author gives sufficient conditions
for \emph{local} identifiability of
$\bm{\beta}$ by viewing \cref{eq:linear-model-y} as a ``sparse plus low
rank'' matrix decomposition problem. See \citet[Section
3.3]{chandrasekaran2012} for a more general discussion of the local
and global identifiability for this problem. Local
identifiability refers to identifiability of the parameters
in a neighborhood of the true values.
In contrast, the conditions in \Cref{prop:identifiable} ensure that
$\bm{\beta}$ is \emph{globally} identifiable in the restricted
parameter space.
%To be more specific, \citet{sun2011} gives conditions
%such that $\bm{\beta}$ is not confused with any
%$\tilde{\bm{\beta}}$ such that $\mathrm{supp}(\tilde{\bm{\beta}})
%%\subset \mathrm{supp}(\bm{\beta})$. In contrast, our sparsity identification
%condition considers when $\bm{\beta}$ is not
%confused with any $\tilde{\bm{\beta}}$ sparser than $\bm{\beta}$,
%i.e.\ $\|\tilde{\bm{\beta}}\|_0 \le \|\bm{\beta}\|_0$.
\end{remark}


==> revision 2/multiple.tex <==
%  JS is editing

In \Cref{sec:model,sec:stat-infer} we assume that there is only one primary variable $\bm{X}$
and all the random variables $\bm{X}$, $\bm{Y}$ and $\bm{Z}$ have mean
$\bm{0}$. In practice, there may
be several predictors, or we may want to include an intercept term
in the regression model.
Here we  develop a multiple regression extension to the
original model \cref{eq:linear-model}.

Suppose we observe in total $d = d_0 + d_1$ random predictors
that can be separated into two groups:
\begin{enumerate}
  \item $\bm{X}_0$: $n \times d_0$ nuisance covariates that we would like
    to include in the regression model, and
  \item $\bm{X}_1$: $n \times d_1$ primary variables whose
    effects we want to study.
\end{enumerate}
For example, the intercept term can be included in $\bm{X}_0$ as a $n
\times 1$ vector of $1$ (i.e. a random variable with mean $1$ and
variance $0$).

\citet{leek2008} consider the case $d_0 = 0$ and $d_1
\ge 1$ for SVA and \citet{sun2012} consider the case $d_0
\ge 0$ and $d_1 = 1$ for LEAPP. Here we study the confounder adjusted
multiple regression in full generality, for any $d_0\ge0$ and $d_1\ge1$.
Our model is
\begin{subequations}\label{eq:linear-model-ext}
\begin{align}
  &
  {\bm{Y}}={\bm{X}_0}{\bm{\Beta}}^T_0
  +{\bm{X}_1}{\bm{\Beta}}^T_1
  +{\bm{Z}}{\bm{\Gamma}}^T
  +{\bm{E}},\\
  &  \begin{pmatrix}
    {\bm{X}}_{0i}\\
    {\bm{X}}_{1i} \\
  \end{pmatrix} \text{ are } \mathrm{i.i.d.}
  \text{ with }  \mathrm{E} \left[
  \begin{pmatrix}
    {\bm{X}}_{0i}\\
    {\bm{X}}_{1i}
  \end{pmatrix}
  \begin{pmatrix}
    {\bm{X}}_{0i}\\
    {\bm{X}}_{1i}
  \end{pmatrix}^T
  \right] ={\bm{\Sigma}}_{\bm{X}},\\
  &  {\bm{Z}} \mid ({\bm{X}}_0,
  {\bm{X}}_1) \sim \mathrm{MN}
  ({\bm{X}}_0{\bm{\Alpha}}_0^T
  +{\bm{X}}_1{\bm{\Alpha}}_1^T,
  {\bm{I}}_n, {\bm{I}}_r),\quad\text{and}\\
  &  {\bm{E}} \independent ({\bm{X}}_0,
  {\bm{X}}_1, {\bm{Z}}) ,~
  {\bm{E}} \sim \mathrm{MN} ({\bm{0}},
  {\bm{I}}_n, {\bm{\Sigma}}).
\end{align}
\end{subequations}
The model does not specify means for ${\bm{X}_{0i}}$
and ${\bm{X}_{1i}}$; we do not need them.
%%%%  Please make sure this is what we intend.  It is what I understand from a discussion.
The parameters in this model are, for $i =0$ or $1$, ${\bm{\Beta}}_i \in \mathbb{R}^{p \times
d_i}$, ${\bm{\Gamma}} \in \mathbb{R}^{p \times r}$,
${\bm{\Sigma}}_{\bm{X}} \in \mathbb{R}^{d \times d}$, and
${\bm{\Alpha}}_i \in \mathbb{R}^{r \times d_i}$. The parameters
$\bm{\Alpha}$ and $\bm{\Beta}$ are the matrix versions of
$\bm{\alpha}$ and $\bm{\beta}$ in model
\cref{eq:linear-model}. Additionally, we assume
${\bm{\Sigma}}_{\bm{X}}$ is invertible. % and let $\bm{\Omega} = {\bm{\Sigma}}_{\bm{X}}^{-1}$.
 To clarify our purpose, we are
primarily interested in estimating and testing for the significance of
$\bm{\Beta}_1$.

For the multiple regression model (\ref{eq:linear-model-ext}), we
again consider the rotation matrix $\bm{Q}^T$ that is given by
the QR decomposition
$
\begin{pmatrix}
  \bm{X}_0 & \bm{X}_1
\end{pmatrix}
={\bm{Q}}{\bm{U}}$ where
${\bm{Q}} \in \mathbb{R}^{n \times n}$ is an orthogonal matrix and
${\bm{U}}$ is an upper triangular matrix of size $n \times
d$. Therefore we have
\[
{\bm{Q}}^T
\begin{pmatrix}
  \bm{X}_0 & \bm{X}_1
\end{pmatrix}
={\bm{U}}=
\begin{pmatrix}
  \bm{U}_{00} & \bm{U}_{01} \\
  \bm{0} & \bm{U}_{11} \\
  \bm{0} & \bm{0} \\
\end{pmatrix}
\]
where $\bm{U}_{00}$ is a $d_0 \times d_0$ upper triangular matrix and
$\bm{U}_{11}$ is a $d_1 \times d_1$ upper triangular matrix. Now let the
rotated $\bm{Y}$ be
\begin{equation} \label{eq:Y-tilde-ext}
  \tilde{\bm{Y}}
  ={\bm{Q}}^T{\bm{Y}}=
  \begin{pmatrix}
    \tilde{\bm{Y}}_0 \\
    \tilde{\bm{Y}}_1 \\
    \tilde{\bm{Y}}_{-1}
  \end{pmatrix}
\end{equation}
where $\tilde{{\bm{Y}}}_0$ is $d_0 \times p$, $\tilde{{\bm{Y}}}_1$ is $d_1 \times p$ and
$\tilde{{\bm{Y}}}_{- 1}$ is $(n - d) \times p$, then we can
partition the model into three parts: conditional on both
${\bm{X}}_0$ and ${\bm{X}}_1$ (hence $\bm{U}$),
\begin{align}
  &\tilde{{\bm{Y}}}_0
  = \bm{U}_{00} \bm{\Beta}_0^T + \bm{U}_{01} \bm{\Beta}_1^T + \tilde{{\bm{Z}}}_0
  {\bm{\Gamma}}^T +
  \tilde{{\bm{E}}}_0, \label{eq:Y-tilde-0-ext}\\
  &\tilde{{\bm{Y}}}_1
  =\bm{U}_{11}
  {\bm{\Beta}}_1^T + \tilde{{\bm{Z}}}_1
  {\bm{\Gamma}}^T + \tilde{{\bm{E}}}_1
  \sim \mathrm{MN}
  ({\bm{U}}_{11}
  ({\bm{\Beta}_1}+{\bm{\Gamma}}{\bm{\Alpha}}_1)^T,
  {\bm{I}}_{d_1},
  {\bm{\Gamma}}{\bm{\Gamma}}^T
  +{\bm{\Sigma}})   \label{eq:Y-tilde-1-ext}\\
  &\tilde{{\bm{Y}}}_{- 1} =
  \tilde{{\bm{Z}}}_{- 1} {\bm{\Gamma}}^T
  + \tilde{{\bm{E}}}_{- 1} \sim \mathrm{\mathrm{MN}}
  ({\bm{0}}, {\bm{I}}_{n - d},
  {\bm{\Gamma}}{\bm{\Gamma}}^T
  +{\bm{\Sigma}}) \label{eq:Y-tilde-m1-ext}
\end{align}
where $\tilde{\bm{Z}} = \bm{Q}^T \bm{Z}$ and $\tilde{\bm{E}} =
\bm{Q}^T \bm{E}
\overset{d}{=} \bm{E}$. Equation \cref{eq:Y-tilde-0-ext} corresponds to the
nuisance parameters $\bm{\Beta}_0$ and is discarded according to the
ancillary principle. Equation \cref{eq:Y-tilde-1-ext} is the multivariate
extension to \cref{eq:Y-tilde-1} that is used to estimate
$\bm{\Beta}_1$ and equation \cref{eq:Y-tilde-m1-ext} plays the same role as
\cref{eq:Y-tilde-m1} to estimate $\bm{\Gamma}$ and $\bm{\Sigma}$.

We consider the asymptotics when $n,p \to \infty$
and $d,r$ are fixed and known. Since $d$ is fixed, the estimation of $\bm{\Gamma}$ is not different
from the simple regression case and we can use the maximum likelihood
factor analysis described in \Cref{sec:inference-gamma-sigma}.
Under
\Cref{assumption:error,assumption:bounded,assumption:large-factor},
the precision results of $\hat{\bm{\Gamma}}$ and $\hat{\bm{\Sigma}}$ (\Cref{lem:gamma-ml})
still hold.

%Since we are only interested in
%${\bm{\Beta}_1}$, we can simply use $\tilde{\bm{Y}}_1$ to estimate
%$\bm{\Beta}_1$ as \eqref{eq:Y-tilde-1-ext} doesn't involve the
%nuisance parameters ${\bm{\Beta}_0}$.
Let
${\bm{\Sigma}}_{\bm{X}}^{- 1} = \bm{\Omega} =
%\left(\begin{array}{cc}
%  {\bm{\Omega}}_{00} &
%  {\bm{\Omega}}_{01}\\
%  {\bm{\Omega}}_{10} &
%  {\bm{\Omega}}_{11}
%\end{array}\right)$.
\bigl(\begin{smallmatrix}
  {\bm{\Omega}}_{00} &  {\bm{\Omega}}_{01}\\
  {\bm{\Omega}}_{10} &  {\bm{\Omega}}_{11}
\end{smallmatrix}\bigr)$.
In the proof of
\Cref{thm:asymptotics-nc,thm:asymptotics-rr}, we consider a fixed
sequence of $\bm{X}$ such that ${\|\bm{X}\|_2}/{\sqrt{n}} \to 1$.
Similarly, we have the following lemma in the multiple regression scenario:
\begin{lemma}\label{lem:part-asym}
  As $n \to \infty$, $\frac{1}{n} \bm{U}_{11}^T
  \bm{U}_{11}
  \overset{a.s.}{\to}
  {\bm{\Omega}}_{11}^{-1}$.
\end{lemma}


Similar to \eqref{eq:y-tilde-1}, we can rewrite \eqref{eq:Y-tilde-1-ext} as
\begin{equation*} %\label{eq:y-tilde-1-ext-new}
  \tilde{\bm{Y}}_1^T \bm{U}_{11}^{-T} = \bm{\Beta}_1 + \bm{\Gamma}
  (\bm{\Alpha}_1 + \tilde{\bm{W}}_1\bm{U}_{11}^{-T}) + \tilde{\bm{E}}_{1}\bm{U}_{11}^{-T}
\end{equation*}
where $\tilde{\bm{W}}_1\sim \mathrm{MN}(\bm{0}, \bm{I}_{d_1}, \bm{I}_p)$ is independent
from $\tilde{\bm{E}}_1$. As in \Cref{sec:inference-beta-alpha}, we derive statistical
properties of the estimate of
$\bm \Beta_1$ for a fixed sequence of $\bm X$, $\tilde{\bm{W}}_1$ and $\bm Z$,
which also hold unconditionally.
%For simplicity, we assume that the negative controls are the known
For simplicity, we assume that the negative controls are a known
%%%% the difference here is that I think we just want to assume that all
%%%% the negative controls have beta = 0 but not that all the beta = 0 are included
%%%% in our list of negative controls
set of variables $\mathcal{C}$ with
$\bm{\Beta}_{1,\mathcal{C}} = \bm{0}$.
We can then estimate each column of ${\bm{\Alpha}}_1$ by applying the
negative control (NC) or robust regression (RR) we discussed in
\Cref{sec:unkn-zero-indic,sec:known-zero-indices} to the corresponding row of $\tilde{\bm{Y}}_1\bm{U}_{11}^{-T}$, and then
estimate ${\bm{\Beta}_1}$ by
\[ \hat{{\bm{\Beta}}}_1
   =   \tilde{{\bm{Y}}}_1^T \bm{U}_{11}^{- T}-
   \hat{{\bm{\Gamma}}}
   \hat{{\bm{\Alpha}}}_1.
\]
Notice that $\tilde{\bm{E}}_1\bm{U}_{11}^{-T}\sim
\mathrm{MN}\big(\bm{0}, \bm{\Sigma}, \bm{U}_{11}^{-1}\bm{U}_{11}^{-T}\big)$. Thus the
``samples'' in the robust regression,
which are actually the $p$ variables in the original problem are still
independent within each column. Though the estimates of each column of $\bm{\Alpha}_1$
may be correlated, we will show that the correlation won't affect inference on
$\bm{\Beta}_1$. As a result,  we still get
asymptotic results similar to
\Cref{thm:asymptotics-rr} for the multiple regression model \eqref{eq:linear-model-ext}:

\begin{theorem} \label{thm:multiple-rr}
  Under \Cref{assumption:error,assumption:bounded,assumption:large-factor,assumption:nc-factor,assumption:rho,% assumption:uniqueness,
    assumption:psi-2nd-derivative}, if $n, p
    \to \infty$, with $p/n^k \to 0$ for some $k > 0$,
    and $\|\mathrm{vec}(\bm{\Beta}_1)\|_1 \sqrt{n} / p
  \to 0$, then for any fixed index set $\mathcal{S}$ with finite cardinality $|\mathcal{S}|$,
  \begin{align}
    \label{eq:nc-asym-ext}
\sqrt{n}
     (\hat{{\bm{\Beta}}}_{1, \mathcal{S}}^{\mathrm{NC}}
     -{\bm{\Beta}_{1, S}}) &\overset{d}{\to} \mathrm{MN}
     ({\bm{0}}_{|\mathcal{S}| \times k_1},
     {\bm{\Sigma}_\mathcal{S}} + \bm{\Delta}_{\mathcal{S}},
     {\bm{\Omega}}_{11}
     +{\bm{\Alpha}}_1^T
     {\bm{\Alpha}}_1),\quad\text{and}\\
\label{eq:rr-asym-ext}
\sqrt{n}
     (\hat{{\bm{\Beta}}}_{1, \mathcal{S}}^{\mathrm{RR}}
     -{\bm{\Beta}_{1, S}}) &\overset{d}{\to} \mathrm{MN}
     ({\bm{0}}_{|\mathcal{S}| \times k_1},
     {\bm{\Sigma}_\mathcal{S}},
     {\bm{\Omega}}_{11}
     +{\bm{\Alpha}}_1^T
     {\bm{\Alpha}}_1)
  \end{align}
where $\bm \Delta_\mathcal{S}$ is defined in \Cref{thm:asymptotics-nc}.
\end{theorem}


As for the asymptotic efficiency of this estimator, we again compare
it to the oracle OLS estimator of $\bm{\Beta}_1$ which observes
confounding variables ${\bm{Z}}$ in \eqref{eq:linear-model-ext}.
In the multiple regression model, we claim that
$\hat{{\bm{\Beta}}}_1^{\mathrm{RR}}$ still
reaches the oracle asymptotic efficiency. In fact, let $\bm{\Beta}= \begin{pmatrix}
  \bm{\Beta}_0 & \bm{\Beta}_1 & \bm{\Gamma}
\end{pmatrix}$. The
oracle OLS estimator of $\bm{\Beta}$,
$\hat{{\bm{\Beta}}}^{\mathrm{OLS}}$, is unbiased and its vectorization
has variance
$\bm{V}^{-1} \otimes \bm{\Sigma}/n$ where
\[
  \bm{V} =
  \begin{pmatrix}
  \bm{\Sigma}_{\bm{X}} & \bm{\Sigma}_{\bm{X}} \bm{\Alpha}^T\\
  \bm{\Alpha}\bm{\Sigma}_{\bm{X}} & \bm{I}_r
  +\bm{\Alpha}\bm{\Sigma}_{\bm{X}} \bm{\Alpha}^T
  \end{pmatrix},~ \mathrm{for}~
  \bm{\Alpha} =
  \begin{pmatrix}
    \bm{\Alpha}_0 & \bm{\Alpha}_1
  \end{pmatrix}.
\]
By the block-wise matrix inversion formula, the top left $d \times d$
block of $\bm{V}^{-1}$ is $\bm{\Sigma}_{\bm{X}}^{-1} +\bm{\Alpha}^T
\bm{\Alpha}$. The variance of $\hat{\bm{\Beta}}_1^{\mathrm{OLS}}$
only depends on the bottom right $d_1 \times d_1$ sub-block of this $d
\times d$ block, which is simply $\bm{\Omega}_{11} +\bm{\Alpha}_1^T
\bm{\Alpha}_1$. Therefore %we conclude that
$\hat{{\bm{\Beta}}}_1^{\mathrm{OLS}}$ is unbiased and its
vectorization has variance $ ({\bm{\Omega}}_{11}
     +{\bm{\Alpha}}_1^T
     {\bm{\Alpha}}_1) \otimes {\bm{\Sigma}}/n$, matching the asymptotic variance
     of $\hat{\bm{\Beta}}^{\mathrm{RR}}_1$ in \Cref{thm:multiple-rr}.


==> revision 2/sensitivity.tex <==
The condition $\|\bm{\beta}\|_0 \sqrt{n} / p \to 0$ in
\ref{thm:asymptotics-rr} allows us to prove
$\hat{\bm{\beta}}^{\mathrm{RR}}$ is consistent. In general, one might
be interested in bounding the maximum bias of
$\hat{\bm{\beta}}^{\mathrm{RR}}$ in the situation of $\|\bm{\beta}\|_0
= \epsilon p$. We call this quantity $b(\epsilon,p)$ and are most
interested in $\lim_{p \to \infty} b(\epsilon,p)$, which allows us to
better understand how sensitive our estimator is to the assumption
that $\|\bm{\beta}\|_0 \sqrt{n} / p \to 0$.

In the proof of \cref{prop:identifiable} we show that without any
further restrictions, $\bm{\beta}$ is identifiable only if
$\|\bm{\beta}\|_0 \le \lfloor (p-r)/2 \rfloor$. Thus if $\epsilon >
\frac{1}{2}$, it is obvious that $b(\epsilon,p) = \infty$.


==> revision 2/stat_infer.tex <==
As mentioned earlier in \Cref{sec:introduction}, the statistical inference consists of two steps:
the factor analysis (\Cref{sec:inference-gamma-sigma}) and the linear
regression (\Cref{sec:inference-beta-alpha}).


==> revision 2/test.tex <==
In this section, we construct significance tests for $\bm{\beta}$ and
$\bm{\alpha}$ based on the asymptotic normal distributions in the previous section.

\subsubsection{Test of the primary effects}
\label{sec:test-primary}

We consider the asymptotic test for $H_{0j}:\beta_j =
0,~j=1,\dotsc,p$ resulting from the asymptotic distributions of
$\hat{\beta}_j$ derived in \Cref{thm:asymptotics-nc,thm:asymptotics-rr}. % in
% % \Cref{sec:known-zero-indices}
% and RR estimator% in
% % \Cref{sec:unkn-zero-indic}
% , the asymptotic test statistic is
\begin{equation}
  \label{eq:test-statistic}
  t_j = \frac{\|\bm{X}\|_2\hat{\beta}_j}{\hat{\sigma}_j \sqrt{1 +
      \|\hat{\bm{\alpha}}\|^2}},\quad j = 1,\dotsc,p
\end{equation}
Here we require $|\mathcal{C}| \to \infty$ for the NC estimator.
The null hypothesis $H_{0j}$ is rejected at level-$\alpha$ if $|t_j| > z_{\alpha/2} =
\mathrm{\Phi}^{-1}(1-\alpha/2)$ as usual, where $\mathrm{\Phi}$ is the cumulative
distribution function of the standard normal. Note that here we slightly
abuse the notation $\alpha$ to represent the significance level and
this should not be confused with the model parameter $\bm{\alpha}$.

The next theorem shows that the overall type-I error and the family-wise error rate
(FWER) can be asymptotically controlled by using the test statistics $t_j,j=1,\dotsc,p$.

\begin{theorem} \label{cor:type-I}
Let $\mathcal{N}_p = \{j| \beta_j = 0, j = 1,\dotsc,p\}$ be all the
true null hypotheses.  Under the assumptions of \Cref{thm:asymptotics-nc} or
  \Cref{thm:asymptotics-rr}, $|\mathcal{C}| \to \infty$ for the NC
  scenario, as $n,p,|\mathcal{N}_p| \to \infty$
\begin{equation} \label{eq:type-I}
\frac{1}{|\mathcal{N}_p|} \sum_{j \in \mathcal{N}_p} I(|t_j| >
z_{\alpha/2}) \overset{p}{\to} \alpha, ~\mathrm{and}
\end{equation}
\begin{equation}
  \label{eq:fwer}
  \lim\sup \, \mathrm{P}\Big(\sum_{j \in \mathcal{N}_p} I(|t_j| > z_{\alpha/(2p)}) \ge
  1\Big) \le \alpha.
\end{equation}
\end{theorem}

Although the individual
test is asymptotically valid as % $\mathrm{P}(|t_j| >
% \varPhi^{-1}(1-\alpha/2)) \to \alpha$ for any fixed $j$ due to
$t_j \overset{d}{\to} \mathrm{N}(0,1)$, %the conclusion in
\Cref{cor:type-I} is not a trivial corollary of the asymptotic normal
distribution in \Cref{thm:asymptotics-nc,thm:asymptotics-rr}. This is because $t_j,j=1,\dotsc,p$
are not independent for finite samples. The proof of \Cref{cor:type-I}
investigates how the dependence of the test statistics diminishes when
$n, p \to \infty$. The proof of
\Cref{cor:type-I} already requires a careful investigation of the convergence
of $\hat{\bm{\beta}}$ in \Cref{thm:asymptotics-rr}. It is more
cumbersome to prove FDR control using our test statistics. % To see
% this, \citet{storey2004} show the key condition in proving FDR control
% is the almost sure convergence of \eqref{eq:type-I}, but we are only able
% to prove the convergence in probability \eqref{eq:type-I}. %as in \Cref{cor:type-I}.
% Although both of them mean the
% dependence of $t_j$ is weak, the higher order terms in $t_j$ are difficult to analyze.
In
\Cref{sec:numerical-experiments} we show that FDR is
usually well controlled in simulations for the
Benjamini-Hochberg procedure when the sample size is large enough.

\begin{remark} \label{rmk:calibration}
We find a calibration technique in \citet{sun2012} very useful
to improve the type I error and FDR control for finite sample size.
%%%% This idea is also called the ``empirical null'' in \citet{efron2010}.
%%% I think they're different things.  Empirical null is a sample histogram
%%% but the calibration is via a sample standard deviation
Because the asymptotic variance used in
\cref{eq:test-statistic} is the variance of an oracle OLS
estimator, when the sample size is not sufficiently large, the
variance of $\hat{\beta}^{\mathrm{RR}}$ should be slightly larger than
this oracle variance. To correct for this inflation, one can use median
absolute deviation (MAD) with customary scaling
to match the standard deviation for a Gaussian distribution to estimate the empirical standard error of
$t_j,j=1,\dotsc,p$ and divide $t_j$ by the estimated standard
error. The performance of this empirical calibration is studied in the simulations in \Cref{sec:simulations}.
\end{remark}


% The weak dependence can be also used to prove FDR control. More
% specifically, we consider the approach in \citep{storey2004} which is
% based on an estimator $\widehat{\mathrm{FDR}}_{\lambda}(t)$ of the FDR
% when the tests are rejected if $|t_j| > t$. Here $\lambda$ is some
% tuning parameter in $[0,1)$. To control the FDR at level $\alpha$, the
% maximum $t$ such that $\widehat{\mathrm{FDR}}_{\lambda}(t) \le \alpha$
% is used.

% The convergence result $\|\hat{\bm{\Gamma}}_j - \bm{\Gamma}_j\|_2 =
% O_p(1/\sqrt{n})$ of factor analysis in \cref{lem:gamma-ml} is slighly
% weaker than what we need to prove the weak dependence conditions in
% \citep{storey2004}. We assume the following technical assumption:
% \begin{assumption} \label{assumption:expectation}
%   For some $\epsilon > 0$, a large constant $D$ and large enough $p$,
%   $\mathrm{E}[p^{\epsilon} \cdot \|\hat{\bm{\Gamma}}_j -
%   \bm{\Gamma}_j\|_2] < D$, $\forall j = 1,\dotsc,p$.
% \end{assumption}

% \begin{theorem}
%   Given the assumptions in \cref{thm:asymptotics-rr}, and further more the technical assumption
%   \cref{assumption:expectation}, when $n,p\to \infty$, $n/p \to \gamma
%   \in (0, \infty)$, $\|\bm{\beta}\|_0 / p \to \pi_0 \in [0, 1/2)$ and
%   $\|\bm{\beta}\|_1 \sqrt{n}/p \to 0$, the procedure
%   in \citep{storey2004} applied to the statistics $t_j, j=1,\dotsc,p$
%   obtained by the robust regression estimator
%   in \eqref{eq:test-statistic} controls the false discovery rate at
%   the nominal level $\alpha$.
% \end{theorem}
% \begin{proof}
%   We verify the conditions in theorem 4 of \citep{storey2004}. The
%   only one nontrivial to prove is its equation (7),
% \[
% \frac{1}{|\mathcal{N}_p|} \sum_{j \in
%   \mathcal{N}_p} I(|t_j| > t) \overset{a.s.}{\to} 2 (1 - \varPhi(t)).
% \]
% This is called the weak dependence condition in \citep{storey2004}. In
% \cref{cor:type-I} we have already proved the weaker in probability
% convergence. To prove the almost surely convergence, we use the
% following sufficient condition of strong law of large numbers for bounded random variables
% \begin{equation} \label{eq:slln-series}
% \sum_{p=1}^{\infty} \frac{1}{p} \mathrm{E} \left[ \frac{1}{|\mathcal{N}_p|} \sum_{j \in
%   \mathcal{N}_p} I(|t_j| > t) - 2 (1 - \varPhi(t)) \right]^2 < \infty
% \end{equation}
% In the proof of \cref{cor:type-I} we show
% \[
% \mathrm{E} \left[ \frac{1}{|\mathcal{N}_p|} \sum_{j \in
%   \mathcal{N}_p} I(|t_j| > t) - 2 (1 - \varPhi(t)) \right]^2 \le
% \frac{c}{|\mathcal{N}_p|} + \frac{c}{|\mathcal{N}_p|} \sum_{j \in
%   \mathcal{N}_p} \mathrm{P}(|v_j| > \epsilon)
% \]
% The expansion \eqref{eq:beta-expand} and \cref{assumption:expectation}
% imply that $\mathrm{E}[p^{\epsilon} \cdot |v_j|] \le D'$ for some
% constant $D'$. By using
% Markov's inequality and $|\mathcal{N}_p| = O(p)$, one can show the
% above expression is of order $O(p^{-\epsilon})$, so the series in
% \eqref{eq:slln-series} is summable.
% \end{proof}

\subsubsection{Test of confounding}
\label{sec:test-confound}
We also consider a significance test for $H_{0, \bm \alpha}: \bm \alpha
= \bm 0$, under which the latent factors are not confounding.

\begin{theorem} \label{thm:alpha-test}
  Let the assumptions of \Cref{thm:asymptotics-nc} or
  \Cref{thm:asymptotics-rr} and  $|\mathcal{C}| \to \infty$ for the NC
  scenario be given. Under the null hypothesis that $\bm \alpha = \bm
  0$, for $\hat{\bm \alpha} = \hat{\bm \alpha}^{\mathrm{NC}}$ in
\eqref{eq:alpha-nc} or $\hat{\bm \alpha} = \hat{\bm
  \alpha}^{\mathrm{RR}}$ in \eqref{eq:alpha-rr}, we have
  $$n \cdot \hat {\bm \alpha}^T \hat{\bm{\alpha}} \overset{d}{\to} \chi_r^2$$
  where $\chi_r^2$ is the chi-square distribution with $r$ degree of freedom.
\end{theorem}

Therefore, the null hypothesis $H_{0, \bm \alpha}: \bm \alpha
= \bm 0$ is rejected if $n\cdot \hat {\bm \alpha}^T
\hat{\bm{\alpha}} > \chi_{r, \alpha}^2$ where $\chi_{r, \alpha}^2$ is
the upper-$\alpha$ quantile of $\chi_r^2$. This test, combined with
exploratory factor analysis, can be used as a
diagnosis tool for practitioners to check whether the data gathering
process has any confounding factors that can bias the multiple
hypothesis testing.


==> revision 2/test_alpha.tex <==



==> revision 2/weak.tex <==
%\marginpar{We probably discussed this before. I think the section
%  title ``weaker factors'' is a little confusing to the reader. I
%  prefer ``weak'' than ``weaker'' because the reader might not
%  understand what you are comparing to when she skims through the
%  paper. How about something like ``Presence of weak
%  factors'' or ``Robustness in presence of weak factors''?}

A key assumption of our analysis is that $\lim_{p \to \infty} \frac{1}{p}
\bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ is positive
definite. This means that
all the confounding factors will have the same order of strength
as the noise entrywise in $\bm Y$, which
are strong enough to be
consistently estimated and the estimating errors have asymptotic normality using
MLE or PCA.
%maximum likelihood or principal component analysis (PCA).
In practice, the researcher may suspect that some of the
confounding factors in her experiment are not strong enough or play a diminishing role as $p \to \infty$. In this section we make use of recent results in random matrix theory,
consider the general setting that 
there is combination of strong and weak factors in our model 
%some of the factors in our model are
%weaker than in \Cref{assumption:large-factor} 
and discuss the properties of $\bm \beta^{\mathrm{RR}}$.

%\marginpar{I'm not sure using all capital letters in Random Matrix
%  Theory is that common. I propose to change it lower case letters and
%avoid using RMT. It only appears a few times in the paper and we don't
%really need the reader to remember this acronym.}

For simplicity, we
assume that the noise variables have equal variances: $\bm{\Sigma} = \sigma^2
\bm{I}_p$, so the statistical properties of PCA are well studied in
random matrix theory. For identification purposes, we assume
$\bm{\Gamma}^T\bm{\Gamma} = \mathrm{diag}(d_1^2,d_2^2, \cdots,
d_r^2)$, where $d_k$ is the ``strength'' of the $k$-th factor. A strong factor in 
\Cref{assumption:large-factor} will have strength $d_i = O(\sqrt p)$. 
Let $d_1 \geq d_2 \geq \cdots \geq d_s = O(\sqrt p)$ be strength of the $s$ strong factors. 
The rest $r - s$ are weak factors for which we adopt the standard random matrix theory assumption to assume that 
$d_k = O(1)$. More specifically, we consider the asymptotics setting that $n ,p \to \infty$ 
and $n/p \to \gamma > 0$, Assume that for the strong factors, 
$(d_1^2, d_2^2, \cdots, d_s^2)/p \to (u_1, u_2, \cdots, u_s)$ and for the weak factors, 
$(d_{s+1}^2, \cdots, d_r^2) \to (u_{s+1}, \cdots, u_r)$. The following assumption requires that 
the latent factors affect the outcome variables evenly:
%We combine the Instead
%of \Cref{assumption:large-factor}, we now allow weak factors in the model:

\begin{assumption}\label{assumption:weak-factor}
%Let $s$ be the number of strong factors and $r - s$ be the number
%of weak factors. Precisely, as $p \to \infty$
%\[
%\frac{d_k^2}{p} \to
%\begin{cases}
%  \tilde{d}_k^2> 0 & \mathrm{if~} k = 1,\dotsc,s \\
%  0 & \mathrm{if~} k = s+1,\dotsc,r
%\end{cases}
%\]
%and $(d_1^2, d_2^2,\cdots, d_r^2) \to (\mu_1, \mu_2, \cdots, \mu_r)$ where
%$\mu_k$ are either $\infty$ or distinct positive constants.
%Also,  as in \Cref{assumption:large-factor}, the confounding
%factors affect the outcome variables evenly: 
For the strong factors there exists a positive constant $D$ such that
%for every $\bm{\Gamma} \in \mathbb{R}^{p \times r}$,
$ |\Gamma_{jk}| \le D$
 for all $j \in \{1, 2, \cdots, p\}$ and $k \in\{1, 2, \cdots, s\}$. 
 For the weak factors there exists some positive $\epsilon \to 0$ such that 
$ |\Gamma_{jk}| \le \epsilon$ 
 for all $j \in \{1, 2, \cdots, p\}$ and $k \in\{s, s+1, \cdots, r\}$. 
%for all $j$; for the weak factors, $\max_{s+1 \le k \le r} |\Gamma_{jk}| =
%o(1)$ for all $j$.
\end{assumption}

The loadings of weak factors are notoriously difficult to estimate as
shown by random matrix theory. In fact if $d_k$ doesn't converge to
$\infty$, there is always a positive angle between the estimated and
true principal component \citep{johnstone2009}. This means
$\bm{\Gamma}$ cannot be $\sqrt{n}$-consistently estimated, which implies
$\bm{\beta}$ in our model cannot be $\sqrt{n}$-consistently
estimated as well. In this section we show that under \Cref{assumption:weak-factor} %some mild conditions
$\bm{\beta}$ may still be recoverable (with unknown efficiency).

The first difficulty is that the number of factors $r$ 
%(or the number of strong factors $s$)
may not be consistently estimated in presence of
weak factors. For example, a standard random matrix theory result is
that when $p/n \to \gamma > 0$, PCA is unable to detect factors with
 $\mu_k \le \sigma^2\sqrt{\gamma}$. \citet{donoho2013} recently show that by using a hard thresholding
rule the factor number estimate $\hat r \overset{a.s.}{\to}
r_0 \in[s, r]$ and the noise estimate $\hat \sigma^2
\overset{a.s.}{\to} \sigma^2$ if $n, p \to \infty$ and $p/n
\to \gamma>0$ where $r_0$ only depends on $\sigma$ and $\gamma$. Another data-driven and robust estimator of $r$ can be
found in \citet{perry2009}, which is later generalized to the
heteroscedastic noise setting by \citet{owen2015}. Due to these reasons, we assume that the
estimated number of factors $\hat{r}$ is always between $s$ and $|\{k: \mu_k^2 > \sigma^2\sqrt{p/n}\}|$ 
for the rest of this section.

% Here we make a note about obtaining a good $\hat r$ in real data. one can also use the bi-cross-validation procedure
%   in \citep{perry2009} which took consideration of finite $n$ and $p$ in real dataset. For
%   heteroscedastic noises cases where $\bm{\Sigma}$ has unequal diagonal entries,
%   it's hard to derive theoretical guarantees, but
%   one can use the ESA-BCV procedure in \citep{owen2015} which empirically works well
%   in getting optimal $\hat r$ and estimating
%   $\bm{\Gamma}$ and $\bm{\Sigma}$.

The next lemma
%suggests that by using PCA, the strong factors can
%still be consistently estimated and the weak factors have little
%influence on the estimation of $\bm{\beta}$.
characterizes some properties of the PCA estimation of the latent factors
that we need for our analysis.

\begin{lemma}\label{lem:weak-gamma}
  Let $\hat{\bm{\Gamma}} \in \mathbb{R}^{p\times \hat{r}}$ be the estimate of $\bm{\Gamma}$
  using PCA on $\tilde{\bm Y}_{-1}$. Then
  under \Cref{assumption:error,assumption:weak-factor}, when
  $n, p \to \infty$ and $p/n \to \gamma>0$, 
  
  \begin{equation}\label{eq:pca}
  \max_{j = 1, 2, \cdots, p}|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%,~
%  \frac{1}{p}\sum_{j = 1}^p
%    |\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%,~k=1,\dotsc,\hat r
  \end{equation}
%Also,
%  \begin{equation}\label{eq:avg-pca}
%  \hat{{\Gamma}}_{jk} = o_p(1),
%    ~  \frac{1}{p}\sum_{j = 1}^p|\hat{{\Gamma}}_{jk}| = o_p(1),~k=s+1,\dotsc,\hat{r}.
%\frac{1}{p}\sum_{j = 1}^p
%   |\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%  \end{equation}
%\begin{equation}\label{eq:angle-pca}
%  \lim_{p \to \infty}\mathrm{corr}(\hat{\bm{\Gamma}}_{\cdot k_1},
%  {\bm{\Gamma}}_{\cdot, k_2}) = 0 \text{ if } k_1 \neq k_2 ,~
%  \lim_{p \to \infty}\mathrm{corr}(\hat{\bm{\Gamma}}_{\cdot k},
%  {\bm{\Gamma}}_{\cdot, k}) < 1 \text{ if } \mu_k < \infty
%\end{equation}
\end{lemma}

% \begin{proof}
% See \Cref{app:lem-weak}.
% \end{proof}

The second difficulty brought up by weak factors is that we cannot get a consistent estimator of
$(\alpha_{s+1},\dotsc,\alpha_r)$ using robust regression. One obvious reason for this is $r$
itself cannot be consistently estimated as discussed above. To
control the bias introduced by estimating
$(\alpha_{s+1},\dotsc,\alpha_r)$, we make the following assumption
\begin{assumption}\label{assumption:bound-alpha}
  $\hat{\bm{\alpha}}^{\mathrm{RR}}$ is estimated inside
  $\{\bm{\alpha} \in \mathbb{R}^{\hat{r}}:
  \|\bm{\alpha}\|_2 < D'\}$ for some positive constant $D'$. Also,
  the true parameter $\bm \alpha \in \mathbb{R}^r$ satisfies $\|\bm{\alpha}\|_2 < D'$.
\end{assumption}

\begin{remark}\label{rmk:bound-alpha}
  \Cref{assumption:bound-alpha} is more reasonable than it first
  appears. Note that
  %$\|\bm{\alpha}\|_2^2/(1 + \|\bm{\alpha}\|_2^2) = \|\bm\rho\|_2^2 <
  %1$, where $\bm{\rho}$ is the correlation of $\bm{X}$ and
  %$\bm{Z}$.
  $\max_{\bm \rho}~\mathrm{corr}(\bm{\rho}^T\bm{Z}_i, X_i) =
  \|\bm{\alpha}\|_2^2/(1 + \|\bm{\alpha}\|_2^2)$.
  Practically,
  %$\|\bm{\rho}\|_2^2$
   the variance of $\bm{X}$
  explained by the latent factors, is almost always bounded
  away from $1$. If we expect $\max_{\bm \rho}
  \mathrm{corr}(\bm{\rho}^T\bm{Z}_i, X_i) < 0.99$ for a
  particular data set, the constant $D'$ in
  \Cref{assumption:bound-alpha} can be set to $10$ accordingly.%  If, for example, we set
  % $C = 10$, then a violation of \Cref{assumption:bound-alpha} indicates that
  % $\|\bm\rho\|_2^2 > 0.99 $, which means that more than $99\%$ of the variance
  % in $X$ can be explained by the latent factors $\bm{Z}$. This won't happen for almost
  % all real data we are interested in.
\end{remark}

%To avoid confusion, we use
%$\bm{\alpha}^* = (\bm{\alpha}_{(S)}^*, \bm{\alpha}_{(W)}^*)$ to represent the true
%$\bm{\alpha}$ and use $\bm{\alpha}$

% Now, we consider the following estimator of $\bm{\alpha}$:
% \begin{equation} \label{eq:alpha-rr-equal}
%   \hat{\bm{\alpha}}^{\mathrm{RR}} = \arg \min_{\bm{\alpha}_0 \in \Omega} \sum_{j=1}^p
%   \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\right)
% \end{equation}
% and $\bm{\beta}$ is still estimated by $\hat{\bm{\beta}}^{\mathrm{RR}}$
% using \eqref{eq:beta-rr}.

We consider the same robust regression estimator of $\bm{\alpha}$ and
$\bm{\beta}$ as in \eqref{eq:alpha-rr} and \eqref{eq:beta-rr} with the additional
constraint in \Cref{assumption:bound-alpha}. The next
theorem shows that even in presence of weaker factors, we can still
consistently estimate $\bm{\beta}$ under the same condition on $\| \bm{\beta}\|_1$.

%Here we consider the inference of $\bm{\beta}$ when we have weaker
%factors. It is well known that the weak factors are intrinsically hard
%to estimate, in fact the correlation of $\hat{\bm{\Gamma}}_j$ and
%$\bm{\Gamma}_j$ is bounded away fromzero  (see e.g.\ \citep{johnstone2009}).

% For simplicity we assume all $\bm{\Gamma}_j,~j=1,2,\dotsc,p$ have
% approximately the same size, so $\lim_{p \to \infty} \frac{1}{p}
% \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma} \succ \bm{0}$ implies
% $\bm{\Gamma}_j = O(1)$.
% % is essentially a nonzero constant.
% As noted in
% \Cref{sec:model}, the existence of confounding factors changes the mean of $\tilde{\bm{Y}}_1^T/\|\bm{X}\|_2$
% from $\bm{\beta}$ to $\bm{\beta} + \bm{\Gamma} \bm{\alpha}$. This
% not only brings up model identification problems
% (\Cref{sec:identification}), but may also bias the estimate of
% ${\bm{\beta}}$. However, in \Cref{lem:gamma-ml} we see that
% $\bm{\Gamma}$ can be $\sqrt{n}$-consistently estimated by maximum
% likelihood and in \Cref{thm:asymptotics-nc,thm:asymptotics-rr} we show
% this leads to $\sqrt{n}$-consistent and efficient estimator of $\bm{\beta}$.

% In the case where there exist weak factors, let $\bm{D} = \frac{1}{p}
% \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ be diagonal and we consider the
% situation that $\bm{D}_{ll}$ are constants for $l=1,\dotsc,r_0$ and
% are converging to $0$ as $p \to \infty$ for $l=r_0+1,\dotsc,r$. Thus
% $\bm{\Gamma}$ can be written as $\tilde{\bm{\Gamma}} \bm{D}$ and
% $\tilde{\bm{\Gamma}}$ is a constant matrix (entries don't converge to
% $0$ as $p \to \infty$). When $n/p \to c \in (0, \infty)$, \citet{johnstone2009} shows that only the
% first $r_0$ columns of $\tilde{\bm{\Gamma}}$ can be consistently estimated. Although not
% proven, we expect the same result holds for the maximum likelihood estimator
% considered in \Cref{sec:inference-gamma-sigma} because this
% inconsistency is intrinsic to the problem. Since the
% mean of $\tilde{Y}_{1j}^T/\|\bm{X}\|_2$ is ${\beta}_j + \bm{\Gamma}_j^T
% \bm{\alpha} = {\beta}_j + \bm{D} \tilde{\bm{\Gamma}}_j^T \bm{\alpha}$,
% this means $\beta_j$ can still be consistently estimated. Here is a
% precise version of this statement (proof of this theorem can be found
% in \Cref{app:thm-rr}):

\begin{theorem} \label{thm:consistency-weak}
  Under \Cref{assumption:error,assumption:weak-factor,assumption:rho%, assumption:uniqueness
    ,assumption:psi-2nd-derivative,assumption:bound-alpha}, if $n,p \to \infty$,
  $p/n \to \gamma > 0$ and $\|
  \bm{\beta} \|_1 /p \to 0$, then $\hat{\alpha}_k^{\mathrm{RR}}
  \overset{p}{\to} \alpha_k,~k=1,2,\dotsc,s$. Moreover, for any $j$, $\hat{{\beta}}_j^{\mathrm{RR}} \overset{p}{\to} {\beta}_j$.
\end{theorem}
% \begin{proof}
%   See \Cref{app:thm-weak}.
% \end{proof}

Therefore, the procedure described in \Cref{sec:stat-infer}
can still successfully correct the intrinsic bias brought by strong
factors. A practical consequence is that we can rely on the ranking of
$\hat\beta_j,j=1,\dotsc,p$ to select some potentially interesting
variables for further validation. Moreover, a slight
modification of \Cref{lem:weak-gamma} and the proof of
\Cref{thm:consistency-weak} show that over-estimating the number of
factors has little impact on the consistency of $\hat \beta_j$, as long as $\hat r \ll \min(n,p)$.
This phenomenon is empirically discovered by \citet{gagnon2013} for
the negative control estimator.
%In the numerical experiments in \Cref{sec:numerical-experiments}, we demonstrate the robust
%regression estimator is also insensitive to using a $\hat{r}$ that is
%slightly larger than $r$.
%by comparing the ranking of $\beta_j$ given by our estimator and the
%naive linear regression estimator.

Finally, we want to emphasize that the
asymptotic normality of $\sqrt{n} (\hat{\beta}_j - \beta_j)$ in
\Cref{thm:asymptotics-nc,thm:asymptotics-rr} may not be true when there are weak factors in the model. For example, if $\hat r < r$, then the missed latent factors will have
a contribution of $\sqrt n \bm{\Gamma}_{k \cdot} \alpha_k = \bm{O}(1)$ (for $k > \hat r$) to the bias of
 $\sqrt{n} (\hat{\bm{\beta}} - \bm{\beta})$. Even when $\hat r = r$, for the weak factors with
 $\mu_k < \infty$, because of \eqref{eq:angle-pca},
 $\sqrt n \big(\mathrm{E}(\hat{\bm{\Gamma}}_{k \cdot} \hat{\alpha}_k) -
 {\bm{\Gamma}}_{\cdot k} {\alpha}_k\big)$ is also likely to contribute an $\bm{O}(1)$ bias to
$\sqrt{n} (\hat{\bm{\beta}} - \bm{\beta})$.
 Consequently,
the p-values derived based on an asymptotic $z$-test are in general biased and correlated.
In \Cref{sec:numerical-experiments}, we also demonstrate how the
 p-values and FDR are affected by weak factors in simulated data.
Developing a valid and efficient testing procedure in
presence of weak factors is an interesting and important problem for
future research.



% \qz{Here we might want to say we will use simulations to demonstrates
%   the impacts of these weak factors. The marginal distribution of all
%   the z-values may just look inflated like what \citet{efron2010} observed, but
%   the truth is the individual z-values are quite biased. The hope is
%   that nonzero $\beta_j$ is large enough so this bias doesn't mask it,
%   but even so there is no $\sqrt{n}$-power anymore.}

% \qz{This is only what I thought and I expect you to make a lot of
%   changes. If we can't show any good results for weak factors, we might
%   not want to say too much to diminish our good results for strong
%   factors. So I didn't talk much about the random matrix stuff (also
%   because I don't know much about it). What do you think?}

% \qz{Another comment: not sure how valuable this is, but with very
%   little extra effort I think we can rigorously prove our
%   $\hat{\beta}_j$ is consistent and make it a theorem. Let's do that!
%   I am convinced that we just need to restate (well I guess it's more
%   than just restate...) the Johnstone and Lu
%   result because the estimation of $\bm{\Sigma}$ doesn't matter for just consistency.}


==> sensitivity.tex <==
The condition $\|\bm{\beta}\|_0 \sqrt{n} / p \to 0$ in
\ref{thm:asymptotics-rr} allows us to prove
$\hat{\bm{\beta}}^{\mathrm{RR}}$ is consistent. In general, one might
be interested in bounding the maximum bias of
$\hat{\bm{\beta}}^{\mathrm{RR}}$ in the situation of $\|\bm{\beta}\|_0
= \epsilon p$. We call this quantity $b(\epsilon,p)$ and are most
interested in $\lim_{p \to \infty} b(\epsilon,p)$, which allows us to
better understand how sensitive our estimator is to the assumption
that $\|\bm{\beta}\|_0 \sqrt{n} / p \to 0$.

In the proof of \cref{prop:identifiable} we show that without any
further restrictions, $\bm{\beta}$ is identifiable only if
$\|\bm{\beta}\|_0 \le \lfloor (p-r)/2 \rfloor$. Thus if $\epsilon >
\frac{1}{2}$, it is obvious that $b(\epsilon,p) = \infty$.


==> test_alpha.tex <==



==> weak.tex <==
%\marginpar{We probably discussed this before. I think the section
%  title ``weaker factors'' is a little confusing to the reader. I
%  prefer ``weak'' than ``weaker'' because the reader might not
%  understand what you are comparing to when she skims through the
%  paper. How about something like ``Presence of weak
%  factors'' or ``Robustness in presence of weak factors''?}

A key assumption of our analysis is that $\lim_{p \to \infty} \frac{1}{p}
\bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ is positive
definite. This means that
all the confounding factors will have the same order of strength
as the noise entrywise in $\bm Y$, which
are strong enough to be
consistently estimated and the estimating errors have asymptotic normality using
MLE or PCA.
%maximum likelihood or principal component analysis (PCA).
In practice, the researcher may suspect that some of the
confounding factors in her experiment are not strong enough or play a diminishing role as $p \to \infty$. In this section we make use of recent results in random matrix theory,
consider the general setting that 
there is combination of strong and weak factors in our model 
%some of the factors in our model are
%weaker than in \Cref{assumption:large-factor} 
and discuss the properties of $\bm \beta^{\mathrm{RR}}$.

%\marginpar{I'm not sure using all capital letters in Random Matrix
%  Theory is that common. I propose to change it lower case letters and
%avoid using RMT. It only appears a few times in the paper and we don't
%really need the reader to remember this acronym.}

For simplicity, we
assume that the noise variables have equal variances: $\bm{\Sigma} = \sigma^2
\bm{I}_p$, so the statistical properties of PCA are well studied in
random matrix theory. For identification purposes, we assume
$\bm{\Gamma}^T\bm{\Gamma} = \mathrm{diag}(d_1^2,d_2^2, \cdots,
d_r^2)$, where $d_k$ is the ``strength'' of the $k$-th factor. A strong factor in 
\Cref{assumption:large-factor} will have strength $d_i = O(\sqrt p)$. 
Let $d_1 \geq d_2 \geq \cdots \geq d_s = O(\sqrt p)$ be strength of the $s$ strong factors. 
The rest $r - s$ are weak factors for which we adopt the standard random matrix theory assumption to assume that 
$d_k = O(1)$. More specifically, we consider the asymptotics setting that $n ,p \to \infty$ 
and $n/p \to \gamma > 0$, Assume that for the strong factors, 
$(d_1^2, d_2^2, \cdots, d_s^2)/p \to (u_1, u_2, \cdots, u_s)$ and for the weak factors, 
$(d_{s+1}^2, \cdots, d_r^2) \to (u_{s+1}, \cdots, u_r)$. The following assumption requires that 
the latent factors affect the outcome variables evenly:
%We combine the Instead
%of \Cref{assumption:large-factor}, we now allow weak factors in the model:

\begin{assumption}\label{assumption:weak-factor}
%Let $s$ be the number of strong factors and $r - s$ be the number
%of weak factors. Precisely, as $p \to \infty$
%\[
%\frac{d_k^2}{p} \to
%\begin{cases}
%  \tilde{d}_k^2> 0 & \mathrm{if~} k = 1,\dotsc,s \\
%  0 & \mathrm{if~} k = s+1,\dotsc,r
%\end{cases}
%\]
%and $(d_1^2, d_2^2,\cdots, d_r^2) \to (\mu_1, \mu_2, \cdots, \mu_r)$ where
%$\mu_k$ are either $\infty$ or distinct positive constants.
%Also,  as in \Cref{assumption:large-factor}, the confounding
%factors affect the outcome variables evenly: 
For the strong factors there exists a positive constant $D$ such that
%for every $\bm{\Gamma} \in \mathbb{R}^{p \times r}$,
$ |\Gamma_{jk}| \le D$
 for all $j \in \{1, 2, \cdots, p\}$ and $k \in\{1, 2, \cdots, s\}$. 
 For the weak factors there exists some positive $\epsilon \to 0$ such that 
$ |\Gamma_{jk}| \le \epsilon$ 
 for all $j \in \{1, 2, \cdots, p\}$ and $k \in\{s, s+1, \cdots, r\}$. 
%for all $j$; for the weak factors, $\max_{s+1 \le k \le r} |\Gamma_{jk}| =
%o(1)$ for all $j$.
\end{assumption}

The loadings of weak factors are notoriously difficult to estimate as
shown by random matrix theory. In fact if $d_k$ doesn't converge to
$\infty$, there is always a positive angle between the estimated and
true principal component \citep{johnstone2009}. This means
$\bm{\Gamma}$ cannot be $\sqrt{n}$-consistently estimated, which implies
$\bm{\beta}$ in our model cannot be $\sqrt{n}$-consistently
estimated as well. In this section we show that under \Cref{assumption:weak-factor} %some mild conditions
$\bm{\beta}$ may still be recoverable (with unknown efficiency).

The first difficulty is that the number of factors $r$ 
%(or the number of strong factors $s$)
may not be consistently estimated in presence of
weak factors. For example, a standard random matrix theory result is
that when $p/n \to \gamma > 0$, PCA is unable to detect factors with
 $\mu_k \le \sigma^2\sqrt{\gamma}$. \citet{donoho2013} recently show that by using a hard thresholding
rule the factor number estimate $\hat r \overset{a.s.}{\to}
r_0 \in[s, r]$ and the noise estimate $\hat \sigma^2
\overset{a.s.}{\to} \sigma^2$ if $n, p \to \infty$ and $p/n
\to \gamma>0$ where $r_0$ only depends on $\sigma$ and $\gamma$. Another data-driven and robust estimator of $r$ can be
found in \citet{perry2009}, which is later generalized to the
heteroscedastic noise setting by \citet{owen2015}. Due to these reasons, we assume that the
estimated number of factors $\hat{r}$ is always between $s$ and $|\{k: \mu_k^2 > \sigma^2\sqrt{p/n}\}|$ 
for the rest of this section.

% Here we make a note about obtaining a good $\hat r$ in real data. one can also use the bi-cross-validation procedure
%   in \citep{perry2009} which took consideration of finite $n$ and $p$ in real dataset. For
%   heteroscedastic noises cases where $\bm{\Sigma}$ has unequal diagonal entries,
%   it's hard to derive theoretical guarantees, but
%   one can use the ESA-BCV procedure in \citep{owen2015} which empirically works well
%   in getting optimal $\hat r$ and estimating
%   $\bm{\Gamma}$ and $\bm{\Sigma}$.

The next lemma
%suggests that by using PCA, the strong factors can
%still be consistently estimated and the weak factors have little
%influence on the estimation of $\bm{\beta}$.
characterizes some properties of the PCA estimation of the latent factors
that we need for our analysis.

\begin{lemma}\label{lem:weak-gamma}
  Let $\hat{\bm{\Gamma}} \in \mathbb{R}^{p\times \hat{r}}$ be the estimate of $\bm{\Gamma}$
  using PCA on $\tilde{\bm Y}_{-1}$. Then
  under \Cref{assumption:error,assumption:weak-factor}, when
  $n, p \to \infty$ and $p/n \to \gamma>0$, 
  
  \begin{equation}\label{eq:pca}
  \max_{j = 1, 2, \cdots, p}|\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%,~
%  \frac{1}{p}\sum_{j = 1}^p
%    |\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%,~k=1,\dotsc,\hat r
  \end{equation}
%Also,
%  \begin{equation}\label{eq:avg-pca}
%  \hat{{\Gamma}}_{jk} = o_p(1),
%    ~  \frac{1}{p}\sum_{j = 1}^p|\hat{{\Gamma}}_{jk}| = o_p(1),~k=s+1,\dotsc,\hat{r}.
%\frac{1}{p}\sum_{j = 1}^p
%   |\hat{{\Gamma}}_{jk} - {\Gamma}_{jk}| = o_p(1)
%  \end{equation}
%\begin{equation}\label{eq:angle-pca}
%  \lim_{p \to \infty}\mathrm{corr}(\hat{\bm{\Gamma}}_{\cdot k_1},
%  {\bm{\Gamma}}_{\cdot, k_2}) = 0 \text{ if } k_1 \neq k_2 ,~
%  \lim_{p \to \infty}\mathrm{corr}(\hat{\bm{\Gamma}}_{\cdot k},
%  {\bm{\Gamma}}_{\cdot, k}) < 1 \text{ if } \mu_k < \infty
%\end{equation}
\end{lemma}

% \begin{proof}
% See \Cref{app:lem-weak}.
% \end{proof}

The second difficulty brought up by weak factors is that we cannot get a consistent estimator of
$(\alpha_{s+1},\dotsc,\alpha_r)$ using robust regression. One obvious reason for this is $r$
itself cannot be consistently estimated as discussed above. To
control the bias introduced by estimating
$(\alpha_{s+1},\dotsc,\alpha_r)$, we make the following assumption
\begin{assumption}\label{assumption:bound-alpha}
  $\hat{\bm{\alpha}}^{\mathrm{RR}}$ is estimated inside
  $\{\bm{\alpha} \in \mathbb{R}^{\hat{r}}:
  \|\bm{\alpha}\|_2 < D'\}$ for some positive constant $D'$. Also,
  the true parameter $\bm \alpha \in \mathbb{R}^r$ satisfies $\|\bm{\alpha}\|_2 < D'$.
\end{assumption}

\begin{remark}\label{rmk:bound-alpha}
  \Cref{assumption:bound-alpha} is more reasonable than it first
  appears. Note that
  %$\|\bm{\alpha}\|_2^2/(1 + \|\bm{\alpha}\|_2^2) = \|\bm\rho\|_2^2 <
  %1$, where $\bm{\rho}$ is the correlation of $\bm{X}$ and
  %$\bm{Z}$.
  $\max_{\bm \rho}~\mathrm{corr}(\bm{\rho}^T\bm{Z}_i, X_i) =
  \|\bm{\alpha}\|_2^2/(1 + \|\bm{\alpha}\|_2^2)$.
  Practically,
  %$\|\bm{\rho}\|_2^2$
   the variance of $\bm{X}$
  explained by the latent factors, is almost always bounded
  away from $1$. If we expect $\max_{\bm \rho}
  \mathrm{corr}(\bm{\rho}^T\bm{Z}_i, X_i) < 0.99$ for a
  particular data set, the constant $D'$ in
  \Cref{assumption:bound-alpha} can be set to $10$ accordingly.%  If, for example, we set
  % $C = 10$, then a violation of \Cref{assumption:bound-alpha} indicates that
  % $\|\bm\rho\|_2^2 > 0.99 $, which means that more than $99\%$ of the variance
  % in $X$ can be explained by the latent factors $\bm{Z}$. This won't happen for almost
  % all real data we are interested in.
\end{remark}

%To avoid confusion, we use
%$\bm{\alpha}^* = (\bm{\alpha}_{(S)}^*, \bm{\alpha}_{(W)}^*)$ to represent the true
%$\bm{\alpha}$ and use $\bm{\alpha}$

% Now, we consider the following estimator of $\bm{\alpha}$:
% \begin{equation} \label{eq:alpha-rr-equal}
%   \hat{\bm{\alpha}}^{\mathrm{RR}} = \arg \min_{\bm{\alpha}_0 \in \Omega} \sum_{j=1}^p
%   \rho \left( \frac{\tilde{Y}_{1j} / \|\bm{X}\|_2 - \hat{\bm{\Gamma}}_j^T \bm{\alpha}_0}{\hat{\sigma}}\right)
% \end{equation}
% and $\bm{\beta}$ is still estimated by $\hat{\bm{\beta}}^{\mathrm{RR}}$
% using \eqref{eq:beta-rr}.

We consider the same robust regression estimator of $\bm{\alpha}$ and
$\bm{\beta}$ as in \eqref{eq:alpha-rr} and \eqref{eq:beta-rr} with the additional
constraint in \Cref{assumption:bound-alpha}. The next
theorem shows that even in presence of weaker factors, we can still
consistently estimate $\bm{\beta}$ under the same condition on $\| \bm{\beta}\|_1$.

%Here we consider the inference of $\bm{\beta}$ when we have weaker
%factors. It is well known that the weak factors are intrinsically hard
%to estimate, in fact the correlation of $\hat{\bm{\Gamma}}_j$ and
%$\bm{\Gamma}_j$ is bounded away fromzero  (see e.g.\ \citep{johnstone2009}).

% For simplicity we assume all $\bm{\Gamma}_j,~j=1,2,\dotsc,p$ have
% approximately the same size, so $\lim_{p \to \infty} \frac{1}{p}
% \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma} \succ \bm{0}$ implies
% $\bm{\Gamma}_j = O(1)$.
% % is essentially a nonzero constant.
% As noted in
% \Cref{sec:model}, the existence of confounding factors changes the mean of $\tilde{\bm{Y}}_1^T/\|\bm{X}\|_2$
% from $\bm{\beta}$ to $\bm{\beta} + \bm{\Gamma} \bm{\alpha}$. This
% not only brings up model identification problems
% (\Cref{sec:identification}), but may also bias the estimate of
% ${\bm{\beta}}$. However, in \Cref{lem:gamma-ml} we see that
% $\bm{\Gamma}$ can be $\sqrt{n}$-consistently estimated by maximum
% likelihood and in \Cref{thm:asymptotics-nc,thm:asymptotics-rr} we show
% this leads to $\sqrt{n}$-consistent and efficient estimator of $\bm{\beta}$.

% In the case where there exist weak factors, let $\bm{D} = \frac{1}{p}
% \bm{\Gamma}^T \bm{\Sigma}^{-1} \bm{\Gamma}$ be diagonal and we consider the
% situation that $\bm{D}_{ll}$ are constants for $l=1,\dotsc,r_0$ and
% are converging to $0$ as $p \to \infty$ for $l=r_0+1,\dotsc,r$. Thus
% $\bm{\Gamma}$ can be written as $\tilde{\bm{\Gamma}} \bm{D}$ and
% $\tilde{\bm{\Gamma}}$ is a constant matrix (entries don't converge to
% $0$ as $p \to \infty$). When $n/p \to c \in (0, \infty)$, \citet{johnstone2009} shows that only the
% first $r_0$ columns of $\tilde{\bm{\Gamma}}$ can be consistently estimated. Although not
% proven, we expect the same result holds for the maximum likelihood estimator
% considered in \Cref{sec:inference-gamma-sigma} because this
% inconsistency is intrinsic to the problem. Since the
% mean of $\tilde{Y}_{1j}^T/\|\bm{X}\|_2$ is ${\beta}_j + \bm{\Gamma}_j^T
% \bm{\alpha} = {\beta}_j + \bm{D} \tilde{\bm{\Gamma}}_j^T \bm{\alpha}$,
% this means $\beta_j$ can still be consistently estimated. Here is a
% precise version of this statement (proof of this theorem can be found
% in \Cref{app:thm-rr}):

\begin{theorem} \label{thm:consistency-weak}
  Under \Cref{assumption:error,assumption:weak-factor,assumption:rho%, assumption:uniqueness
    ,assumption:psi-2nd-derivative,assumption:bound-alpha}, if $n,p \to \infty$,
  $p/n \to \gamma > 0$ and $\|
  \bm{\beta} \|_1 /p \to 0$, then $\hat{\alpha}_k^{\mathrm{RR}}
  \overset{p}{\to} \alpha_k,~k=1,2,\dotsc,s$. Moreover, for any $j$, $\hat{{\beta}}_j^{\mathrm{RR}} \overset{p}{\to} {\beta}_j$.
\end{theorem}
% \begin{proof}
%   See \Cref{app:thm-weak}.
% \end{proof}

Therefore, the procedure described in \Cref{sec:stat-infer}
can still successfully correct the intrinsic bias brought by strong
factors. A practical consequence is that we can rely on the ranking of
$\hat\beta_j,j=1,\dotsc,p$ to select some potentially interesting
variables for further validation. Moreover, a slight
modification of \Cref{lem:weak-gamma} and the proof of
\Cref{thm:consistency-weak} show that over-estimating the number of
factors has little impact on the consistency of $\hat \beta_j$, as long as $\hat r \ll \min(n,p)$.
This phenomenon is empirically discovered by \citet{gagnon2013} for
the negative control estimator.
%In the numerical experiments in \Cref{sec:numerical-experiments}, we demonstrate the robust
%regression estimator is also insensitive to using a $\hat{r}$ that is
%slightly larger than $r$.
%by comparing the ranking of $\beta_j$ given by our estimator and the
%naive linear regression estimator.

Finally, we want to emphasize that the
asymptotic normality of $\sqrt{n} (\hat{\beta}_j - \beta_j)$ in
\Cref{thm:asymptotics-nc,thm:asymptotics-rr} may not be true when there are weak factors in the model. For example, if $\hat r < r$, then the missed latent factors will have
a contribution of $\sqrt n \bm{\Gamma}_{k \cdot} \alpha_k = \bm{O}(1)$ (for $k > \hat r$) to the bias of
 $\sqrt{n} (\hat{\bm{\beta}} - \bm{\beta})$. Even when $\hat r = r$, for the weak factors with
 $\mu_k < \infty$, because of \eqref{eq:angle-pca},
 $\sqrt n \big(\mathrm{E}(\hat{\bm{\Gamma}}_{k \cdot} \hat{\alpha}_k) -
 {\bm{\Gamma}}_{\cdot k} {\alpha}_k\big)$ is also likely to contribute an $\bm{O}(1)$ bias to
$\sqrt{n} (\hat{\bm{\beta}} - \bm{\beta})$.
 Consequently,
the p-values derived based on an asymptotic $z$-test are in general biased and correlated.
In \Cref{sec:numerical-experiments}, we also demonstrate how the
 p-values and FDR are affected by weak factors in simulated data.
Developing a valid and efficient testing procedure in
presence of weak factors is an interesting and important problem for
future research.



% \qz{Here we might want to say we will use simulations to demonstrates
%   the impacts of these weak factors. The marginal distribution of all
%   the z-values may just look inflated like what \citet{efron2010} observed, but
%   the truth is the individual z-values are quite biased. The hope is
%   that nonzero $\beta_j$ is large enough so this bias doesn't mask it,
%   but even so there is no $\sqrt{n}$-power anymore.}

% \qz{This is only what I thought and I expect you to make a lot of
%   changes. If we can't show any good results for weak factors, we might
%   not want to say too much to diminish our good results for strong
%   factors. So I didn't talk much about the random matrix stuff (also
%   because I don't know much about it). What do you think?}

% \qz{Another comment: not sure how valuable this is, but with very
%   little extra effort I think we can rigorously prove our
%   $\hat{\beta}_j$ is consistent and make it a theorem. Let's do that!
%   I am convinced that we just need to restate (well I guess it's more
%   than just restate...) the Johnstone and Lu
%   result because the estimation of $\bm{\Sigma}$ doesn't matter for just consistency.}

